Data Smashing

Investigation of the underlying physics or biology from empirical data requires a quantifiable notion of similarity - when do two observed data sets indicate nearly identical generating processes, and when they do not. The discriminating characteristics to look for in data is often determined by heuristics designed by experts, $e.g.$, distinct shapes of "folded" lightcurves may be used as "features" to classify variable stars, while determination of pathological brain states might require a Fourier analysis of brainwave activity. Finding good features is non-trivial. Here, we propose a universal solution to this problem: we delineate a principle for quantifying similarity between sources of arbitrary data streams, without a priori knowledge, features or training. We uncover an algebraic structure on a space of symbolic models for quantized data, and show that such stochastic generators may be added and uniquely inverted; and that a model and its inverse always sum to the generator of flat white noise. Therefore, every data stream has an anti-stream: data generated by the inverse model. Similarity between two streams, then, is the degree to which one, when summed to the other's anti-stream, mutually annihilates all statistical structure to noise. We call this data smashing. We present diverse applications, including disambiguation of brainwaves pertaining to epileptic seizures, detection of anomalous cardiac rhythms, and classification of astronomical objects from raw photometry. In our examples, the data smashing principle, without access to any domain knowledge, meets or exceeds the performance of specialized algorithms tuned by domain experts.

==> Figures/TSp.tex <==
\addplot[semithick,gray] plot coordinates {
(0.00576, 11.00000)
(0.01152, 5.00000)
(0.01729, 5.00000)
(0.02305, -11.00000)
(0.02881, -11.00000)
(0.03457, -15.00000)
(0.04033, 5.00000)
(0.04609, 20.00000)
(0.05186, 4.00000)
(0.05762, -2.00000)
(0.06338, 1.00000)
(0.06914, -3.00000)
(0.07490, 5.00000)
(0.08066, 30.00000)
(0.08643, 0.00000)
(0.09219, -11.00000)
(0.09795, -21.00000)
(0.10371, -13.00000)
(0.10947, 1.00000)
(0.11523, -1.00000)
(0.12100, -8.00000)
(0.12676, -10.00000)
(0.13252, -17.00000)
(0.13828, 13.00000)
(0.14404, 31.00000)
(0.14980, -3.00000)
(0.15557, -18.00000)
(0.16133, -32.00000)
(0.16709, -13.00000)
(0.17285, 11.00000)
(0.17861, 12.00000)
(0.18438, 9.00000)
(0.19014, -3.00000)
(0.19590, 15.00000)
(0.20166, 8.00000)
(0.20742, -4.00000)
(0.21318, -7.00000)
(0.21895, -3.00000)
(0.22471, 19.00000)
(0.23047, 21.00000)
(0.23623, -1.00000)
(0.24199, -12.00000)
(0.24775, -49.00000)
(0.25352, -15.00000)
(0.25928, -3.00000)
(0.26504, 13.00000)
(0.27080, -10.00000)
(0.27656, -9.00000)
(0.28232, 5.00000)
(0.28809, 30.00000)
(0.29385, 28.00000)
(0.29961, 15.00000)
(0.30537, -1.00000)
(0.31113, 2.00000)
(0.31689, 29.00000)
(0.32266, 2.00000)
(0.32842, -10.00000)
(0.33418, -26.00000)
(0.33994, -20.00000)
(0.34570, -14.00000)
(0.35146, -5.00000)
(0.35723, -2.00000)
(0.36299, 20.00000)
(0.36875, 6.00000)
(0.37451, 13.00000)
(0.38027, 9.00000)
(0.38604, -22.00000)
(0.39180, -25.00000)
(0.39756, -24.00000)
(0.40332, 5.00000)
(0.40908, 12.00000)
(0.41484, -2.00000)
(0.42061, 2.00000)
(0.42637, 9.00000)
(0.43213, 15.00000)
(0.43789, 29.00000)
(0.44365, -7.00000)
(0.44941, -33.00000)
(0.45518, -47.00000)
(0.46094, -26.00000)
(0.46670, 5.00000)
(0.47246, 20.00000)
(0.47822, 28.00000)
(0.48398, 25.00000)
(0.48975, 30.00000)
(0.49551, -15.00000)
(0.50127, 18.00000)
(0.50703, -12.00000)
(0.51279, 4.00000)
(0.51855, 18.00000)
(0.52432, -10.00000)
(0.53008, -22.00000)
(0.53584, -17.00000)
(0.54160, -15.00000)
(0.54736, -10.00000)
(0.55313, -10.00000)
(0.55889, 10.00000)
(0.56465, -2.00000)
(0.57041, 5.00000)
(0.57617, 6.00000)
(0.58193, 19.00000)
(0.58770, 27.00000)
(0.59346, 3.00000)
(0.59922, 7.00000)
(0.60498, -5.00000)
(0.61074, -5.00000)
(0.61650, -8.00000)
(0.62227, 12.00000)
(0.62803, 9.00000)
(0.63379, -4.00000)
(0.63955, -7.00000)
(0.64531, -24.00000)
(0.65107, -6.00000)
(0.65684, 6.00000)
(0.66260, 10.00000)
(0.66836, 11.00000)
(0.67412, 18.00000)
(0.67988, 21.00000)
(0.68564, 23.00000)
(0.69141, 11.00000)
(0.69717, -9.00000)
(0.70293, -10.00000)
(0.70869, -38.00000)
(0.71445, -30.00000)
(0.72021, -11.00000)
(0.72598, -25.00000)
(0.73174, -30.00000)
(0.73750, -23.00000)
(0.74326, 4.00000)
(0.74902, 18.00000)
(0.75479, 38.00000)
(0.76055, 18.00000)
(0.76631, 4.00000)
(0.77207, 0.00000)
(0.77783, -32.00000)
(0.78359, 7.00000)
(0.78936, 11.00000)
(0.79512, 19.00000)
(0.80088, 8.00000)
(0.80664, -2.00000)
(0.81240, -13.00000)
(0.81816, -32.00000)
(0.82393, -29.00000)
(0.82969, -7.00000)
(0.83545, -12.00000)
(0.84121, 11.00000)
(0.84697, 5.00000)
(0.85273, 14.00000)
(0.85850, 24.00000)
(0.86426, 28.00000)
(0.87002, 8.00000)
(0.87578, 18.00000)
(0.88154, 10.00000)
(0.88730, 28.00000)
(0.89307, 24.00000)
(0.89883, -33.00000)
(0.90459, -30.00000)
(0.91035, -58.00000)
(0.91611, -47.00000)
(0.92188, -20.00000)
(0.92764, -4.00000)
(0.93340, -8.00000)
(0.93916, 32.00000)
(0.94492, 18.00000)
(0.95068, 35.00000)
(0.95645, 17.00000)
(0.96221, 0.00000)
(0.96797, 48.00000)
(0.97373, 33.00000)
(0.97949, 18.00000)
(0.98525, -9.00000)
(0.99102, -17.00000)
(0.99678, -45.00000)
(1.00254, -47.00000)
(1.00830, -48.00000)
(1.01406, -28.00000)
(1.01982, 18.00000)
(1.02559, 38.00000)
(1.03135, 31.00000)
(1.03711, 25.00000)
(1.04287, 32.00000)
(1.04863, 12.00000)
(1.05439, -8.00000)
(1.06016, -28.00000)
(1.06592, -30.00000)
(1.07168, -9.00000)
(1.07744, -8.00000)
(1.08320, -18.00000)
(1.08896, -8.00000)
(1.09473, -30.00000)
(1.10049, -11.00000)
(1.10625, 6.00000)
(1.11201, 16.00000)
(1.11777, 37.00000)
(1.12354, 44.00000)
(1.12930, 40.00000)
(1.13506, 14.00000)
(1.14082, 4.00000)
(1.14658, 7.00000)
(1.15234, 6.00000)
(1.15811, -20.00000)
(1.16387, -33.00000)
(1.16963, -43.00000)
(1.17539, -43.00000)
(1.18115, -32.00000)
(1.18691, -14.00000)
(1.19268, 6.00000)
(1.19844, 20.00000)
(1.20420, 51.00000)
(1.20996, 37.00000)
(1.21572, 25.00000)
(1.22148, 27.00000)
(1.22725, 51.00000)
(1.23301, 22.00000)
(1.23877, 14.00000)
(1.24453, -6.00000)
(1.25029, -29.00000)
(1.25605, -38.00000)
(1.26182, -54.00000)
(1.26758, -45.00000)
(1.27334, -32.00000)
(1.27910, -20.00000)
(1.28486, 0.00000)
(1.29063, 13.00000)
(1.29639, 21.00000)
(1.30215, 24.00000)
(1.30791, 37.00000)
(1.31367, 22.00000)
(1.31943, 5.00000)
(1.32520, 4.00000)
(1.33096, -29.00000)
(1.33672, -32.00000)
(1.34248, -37.00000)
(1.34824, -20.00000)
(1.35400, -39.00000)
(1.35977, -13.00000)
(1.36553, 12.00000)
(1.37129, 36.00000)
(1.37705, 53.00000)
(1.38281, 25.00000)
(1.38857, 9.00000)
(1.39434, -6.00000)
(1.40010, 11.00000)
(1.40586, 33.00000)
(1.41162, 26.00000)
(1.41738, 7.00000)
(1.42314, -14.00000)
(1.42891, -28.00000)
(1.43467, -43.00000)
(1.44043, -28.00000)
(1.44619, -24.00000)
(1.45195, 15.00000)
(1.45771, 7.00000)
(1.46348, 31.00000)
(1.46924, 42.00000)
(1.47500, 15.00000)
(1.48076, 12.00000)
(1.48652, -3.00000)
(1.49229, -11.00000)
(1.49805, -14.00000)
(1.50381, 7.00000)
(1.50957, -10.00000)
(1.51533, -18.00000)
(1.52109, -24.00000)
(1.52686, -5.00000)
(1.53262, 12.00000)
(1.53838, 10.00000)
(1.54414, 11.00000)
(1.54990, 12.00000)
(1.55566, 7.00000)
(1.56143, 14.00000)
(1.56719, 6.00000)
(1.57295, 18.00000)
(1.57871, 8.00000)
(1.58447, -5.00000)
(1.59023, -21.00000)
(1.59600, -44.00000)
(1.60176, -28.00000)
(1.60752, -5.00000)
(1.61328, -4.00000)
(1.61904, -25.00000)
(1.62480, 16.00000)
(1.63057, 3.00000)
(1.63633, 11.00000)
(1.64209, 38.00000)
(1.64785, 33.00000)
(1.65361, 53.00000)
(1.65938, 40.00000)
(1.66514, 32.00000)
(1.67090, -14.00000)
(1.67666, -30.00000)
(1.68242, -57.00000)
(1.68818, -52.00000)
(1.69395, -41.00000)
(1.69971, -38.00000)
(1.70547, -22.00000)
(1.71123, -1.00000)
(1.71699, 2.00000)
(1.72275, 15.00000)
(1.72852, 28.00000)
(1.73428, 50.00000)
(1.74004, 88.00000)
(1.74580, 97.00000)
(1.75156, 53.00000)
(1.75732, 4.00000)
(1.76309, -50.00000)
(1.76885, -58.00000)
(1.77461, -69.00000)
(1.78037, -62.00000)
(1.78613, -53.00000)
(1.79189, -33.00000)
(1.79766, -15.00000)
(1.80342, 5.00000)
(1.80918, 27.00000)
(1.81494, 0.00000)
(1.82070, 30.00000)
(1.82646, 31.00000)
(1.83223, 50.00000)
(1.83799, 25.00000)
(1.84375, 25.00000)
(1.84951, 0.00000)
(1.85527, -15.00000)
(1.86104, -17.00000)
(1.86680, -22.00000)
(1.87256, 13.00000)
(1.87832, -18.00000)
(1.88408, -15.00000)
(1.88984, -49.00000)
(1.89561, -56.00000)
(1.90137, -43.00000)
(1.90713, -26.00000)
(1.91289, -10.00000)
(1.91865, 0.00000)
(1.92441, 29.00000)
(1.93018, 11.00000)
(1.93594, 23.00000)
(1.94170, 14.00000)
(1.94746, 36.00000)
(1.95322, 18.00000)
(1.95898, 10.00000)
(1.96475, 15.00000)
(1.97051, 16.00000)
(1.97627, 21.00000)
(1.98203, -2.00000)
(1.98779, -12.00000)
(1.99355, -16.00000)
(1.99932, -18.00000)
(2.00508, -11.00000)
(2.01084, -7.00000)
(2.01660, -5.00000)
(2.02236, -20.00000)
(2.02813, -21.00000)
(2.03389, -23.00000)
(2.03965, -3.00000)
(2.04541, 19.00000)
(2.05117, 32.00000)
(2.05693, 4.00000)
(2.06270, 6.00000)
(2.06846, -2.00000)
(2.07422, -12.00000)
(2.07998, -1.00000)
(2.08574, 1.00000)
(2.09150, -11.00000)
(2.09727, -21.00000)
(2.10303, -32.00000)
(2.10879, -6.00000)
(2.11455, 4.00000)
(2.12031, 17.00000)
(2.12607, 0.00000)
(2.13184, 27.00000)
(2.13760, 14.00000)
(2.14336, 21.00000)
(2.14912, 7.00000)
(2.15488, -7.00000)
(2.16064, -3.00000)
(2.16641, 19.00000)
(2.17217, 0.00000)
(2.17793, -11.00000)
(2.18369, -23.00000)
(2.18945, -12.00000)
(2.19521, -3.00000)
(2.20098, 16.00000)
(2.20674, 10.00000)
(2.21250, 17.00000)
(2.21826, 2.00000)
(2.22402, 12.00000)
(2.22979, 14.00000)
(2.23555, -3.00000)
(2.24131, -20.00000)
(2.24707, -12.00000)
(2.25283, -12.00000)
(2.25859, 4.00000)
(2.26436, 18.00000)
(2.27012, 6.00000)
(2.27588, -20.00000)
(2.28164, 5.00000)
(2.28740, 10.00000)
(2.29316, 23.00000)
(2.29893, 13.00000)
(2.30469, 12.00000)
(2.31045, 7.00000)
(2.31621, -15.00000)
(2.32197, 14.00000)
(2.32773, -32.00000)
(2.33350, -7.00000)
(2.33926, -31.00000)
(2.34502, -2.00000)
(2.35078, 2.00000)
(2.35654, -6.00000)
(2.36230, -13.00000)
(2.36807, -5.00000)
(2.37383, 10.00000)
(2.37959, 19.00000)
(2.38535, 24.00000)
(2.39111, 5.00000)
(2.39688, -3.00000)
(2.40264, -16.00000)
(2.40840, -28.00000)
(2.41416, -37.00000)
(2.41992, -40.00000)
(2.42568, -6.00000)
(2.43145, 7.00000)
(2.43721, 1.00000)
(2.44297, -10.00000)
(2.44873, 11.00000)
(2.45449, 5.00000)
(2.46025, 20.00000)
(2.46602, -12.00000)
(2.47178, 34.00000)
(2.47754, 15.00000)
(2.48330, 14.00000)
(2.48906, -9.00000)
(2.49482, -31.00000)
(2.50059, -13.00000)
(2.50635, 2.00000)
(2.51211, 6.00000)
(2.51787, 13.00000)
(2.52363, 26.00000)
(2.52939, 16.00000)
(2.53516, 2.00000)
(2.54092, -17.00000)
(2.54668, -23.00000)
(2.55244, -31.00000)
(2.55820, 16.00000)
(2.56396, 10.00000)
(2.56973, 26.00000)
(2.57549, -10.00000)
(2.58125, 0.00000)
(2.58701, 22.00000)
(2.59277, 4.00000)
(2.59854, 8.00000)
(2.60430, 5.00000)
(2.61006, -1.00000)
(2.61582, -12.00000)
(2.62158, -30.00000)
(2.62734, -2.00000)
(2.63311, 16.00000)
(2.63887, 6.00000)
(2.64463, 8.00000)
(2.65039, -6.00000)
(2.65615, 9.00000)
(2.66191, 25.00000)
(2.66768, 30.00000)
(2.67344, -12.00000)
(2.67920, -20.00000)
(2.68496, -4.00000)
(2.69072, -5.00000)
(2.69648, -3.00000)
(2.70225, -2.00000)
(2.70801, -2.00000)
(2.71377, -3.00000)
(2.71953, 12.00000)
(2.72529, 2.00000)
(2.73105, -1.00000)
(2.73682, -7.00000)
(2.74258, -7.00000)
(2.74834, 20.00000)
(2.75410, -3.00000)
(2.75986, -5.00000)
(2.76562, -6.00000)
(2.77139, -7.00000)
(2.77715, 8.00000)
(2.78291, -13.00000)
(2.78867, -4.00000)
(2.79443, -16.00000)
(2.80020, -11.00000)
(2.80596, -8.00000)
(2.81172, -15.00000)
(2.81748, 5.00000)
(2.82324, 19.00000)
(2.82900, 32.00000)
(2.83477, 15.00000)
(2.84053, 22.00000)
(2.84629, 16.00000)
(2.85205, 16.00000)
(2.85781, 2.00000)
(2.86357, -27.00000)
(2.86934, 3.00000)
(2.87510, -10.00000)
(2.88086, 17.00000)
(2.88662, 33.00000)
(2.89238, -18.00000)
(2.89814, -37.00000)
(2.90391, -47.00000)
(2.90967, -24.00000)
(2.91543, 17.00000)
(2.92119, 25.00000)
(2.92695, 21.00000)
(2.93271, 6.00000)
(2.93848, -7.00000)
(2.94424, -2.00000)
(2.95000, -11.00000)
(2.95576, 6.00000)
(2.96152, 5.00000)
(2.96729, -15.00000)
(2.97305, -25.00000)
(2.97881, -42.00000)
(2.98457, -24.00000)
(2.99033, -5.00000)
(2.99609, 2.00000)
(3.00186, 18.00000)
(3.00762, 31.00000)
(3.01338, 11.00000)
(3.01914, 13.00000)
(3.02490, 23.00000)
(3.03066, 31.00000)
(3.03643, -6.00000)
(3.04219, -16.00000)
(3.04795, -35.00000)
(3.05371, -32.00000)
(3.05947, -4.00000)
(3.06523, 15.00000)
(3.07100, 18.00000)
(3.07676, 5.00000)
(3.08252, -1.00000)
(3.08828, 13.00000)
(3.09404, 21.00000)
(3.09980, 23.00000)
(3.10557, 39.00000)
(3.11133, 5.00000)
(3.11709, -2.00000)
(3.12285, -23.00000)
(3.12861, -14.00000)
(3.13438, -9.00000)
(3.14014, -1.00000)
(3.14590, -10.00000)
(3.15166, -5.00000)
(3.15742, -10.00000)
(3.16318, -1.00000)
(3.16895, 9.00000)
(3.17471, 7.00000)
(3.18047, 21.00000)
(3.18623, 13.00000)
(3.19199, -9.00000)
(3.19775, -25.00000)
(3.20352, -14.00000)
(3.20928, -1.00000)
(3.21504, -3.00000)
(3.22080, -6.00000)
(3.22656, -13.00000)
(3.23232, -15.00000)
(3.23809, -14.00000)
(3.24385, 0.00000)
(3.24961, 35.00000)
(3.25537, 11.00000)
(3.26113, 5.00000)
(3.26689, -24.00000)
(3.27266, -10.00000)
(3.27842, -8.00000)
(3.28418, 19.00000)
(3.28994, 8.00000)
(3.29570, -4.00000)
(3.30146, 7.00000)
(3.30723, -5.00000)
(3.31299, 1.00000)
(3.31875, -6.00000)
(3.32451, 1.00000)
(3.33027, -3.00000)
(3.33604, -1.00000)
(3.34180, -4.00000)
(3.34756, 14.00000)
(3.35332, 13.00000)
(3.35908, 1.00000)
(3.36484, -2.00000)
(3.37061, -4.00000)
(3.37637, 10.00000)
(3.38213, 13.00000)
(3.38789, -2.00000)
(3.39365, 1.00000)
(3.39941, -7.00000)
(3.40518, 28.00000)
(3.41094, 18.00000)
(3.41670, 11.00000)
(3.42246, 17.00000)
(3.42822, 11.00000)
(3.43398, -14.00000)
(3.43975, -22.00000)
(3.44551, 2.00000)
(3.45127, -14.00000)
(3.45703, -19.00000)
(3.46279, -48.00000)
(3.46855, -22.00000)
(3.47432, -17.00000)
(3.48008, 15.00000)
(3.48584, 29.00000)
(3.49160, 45.00000)
(3.49736, 34.00000)
(3.50313, 24.00000)
(3.50889, 11.00000)
(3.51465, -3.00000)
(3.52041, -17.00000)
(3.52617, -33.00000)
(3.53193, -44.00000)
(3.53770, -28.00000)
(3.54346, -6.00000)
(3.54922, 2.00000)
(3.55498, 1.00000)
(3.56074, 9.00000)
(3.56650, 20.00000)
(3.57227, 28.00000)
(3.57803, 25.00000)
(3.58379, 32.00000)
(3.58955, 6.00000)
(3.59531, -1.00000)
(3.60107, -23.00000)
(3.60684, -17.00000)
(3.61260, -4.00000)
(3.61836, -14.00000)
(3.62412, -6.00000)
(3.62988, -10.00000)
(3.63564, -3.00000)
(3.64141, -10.00000)
(3.64717, 18.00000)
(3.65293, 16.00000)
(3.65869, 56.00000)
(3.66445, 37.00000)
(3.67021, 11.00000)
(3.67598, -15.00000)
(3.68174, -21.00000)
(3.68750, 4.00000)
(3.69326, -10.00000)
(3.69902, -16.00000)
(3.70479, -15.00000)
(3.71055, -27.00000)
(3.71631, -40.00000)
(3.72207, -3.00000)
(3.72783, 6.00000)
(3.73359, 38.00000)
(3.73936, 32.00000)
(3.74512, 20.00000)
(3.75088, -6.00000)
(3.75664, -31.00000)
(3.76240, -26.00000)
(3.76816, -17.00000)
(3.77393, -7.00000)
(3.77969, -2.00000)
(3.78545, 12.00000)
(3.79121, -2.00000)
(3.79697, 6.00000)
(3.80273, -16.00000)
(3.80850, -5.00000)
(3.81426, 24.00000)
(3.82002, 8.00000)
(3.82578, 18.00000)
(3.83154, 1.00000)
(3.83730, -13.00000)
(3.84307, -7.00000)
(3.84883, -6.00000)
(3.85459, -13.00000)
(3.86035, 0.00000)
(3.86611, 6.00000)
(3.87188, -13.00000)
(3.87764, -9.00000)
(3.88340, -9.00000)
(3.88916, 15.00000)
(3.89492, -5.00000)
(3.90068, -13.00000)
(3.90645, -8.00000)
(3.91221, 12.00000)
(3.91797, 23.00000)
(3.92373, 23.00000)
(3.92949, 10.00000)
(3.93525, -8.00000)
(3.94102, -4.00000)
(3.94678, 1.00000)
(3.95254, 23.00000)
(3.95830, -8.00000)
(3.96406, -15.00000)
(3.96982, -26.00000)
(3.97559, -38.00000)
(3.98135, -12.00000)
(3.98711, -23.00000)
(3.99287, 3.00000)
(3.99863, 17.00000)
(4.00439, 44.00000)
(4.01016, 30.00000)
(4.01592, 26.00000)
(4.02168, -10.00000)
(4.02744, -23.00000)
(4.03320, -28.00000)
(4.03896, -16.00000)
(4.04473, 13.00000)
(4.05049, 10.00000)
(4.05625, -16.00000)
(4.06201, -7.00000)
(4.06777, -3.00000)
(4.07354, -6.00000)
(4.07930, -6.00000)
(4.08506, -11.00000)
(4.09082, 12.00000)
(4.09658, -10.00000)
(4.10234, 9.00000)
(4.10811, 13.00000)
(4.11387, 15.00000)
(4.11963, 18.00000)
(4.12539, 6.00000)
(4.13115, -5.00000)
(4.13691, -11.00000)
(4.14268, 2.00000)
(4.14844, 15.00000)
(4.15420, -4.00000)
(4.15996, -3.00000)
(4.16572, -12.00000)
(4.17148, -7.00000)
(4.17725, 4.00000)
(4.18301, 6.00000)
(4.18877, 15.00000)
(4.19453, 22.00000)
(4.20029, 39.00000)
(4.20605, 10.00000)
(4.21182, -16.00000)
(4.21758, -48.00000)
(4.22334, -31.00000)
(4.22910, 5.00000)
(4.23486, 13.00000)
(4.24063, -6.00000)
(4.24639, 18.00000)
(4.25215, 2.00000)
(4.25791, 15.00000)
(4.26367, 11.00000)
(4.26943, -4.00000)
(4.27520, -4.00000)
(4.28096, -7.00000)
(4.28672, 12.00000)
(4.29248, 19.00000)
(4.29824, 7.00000)
(4.30400, -2.00000)
(4.30977, -15.00000)
(4.31553, -13.00000)
(4.32129, -5.00000)
(4.32705, -2.00000)
(4.33281, -14.00000)
(4.33857, -23.00000)
(4.34434, -9.00000)
(4.35010, 1.00000)
(4.35586, 4.00000)
(4.36162, 10.00000)
(4.36738, 18.00000)
(4.37314, 37.00000)
(4.37891, 25.00000)
(4.38467, 11.00000)
(4.39043, -16.00000)
(4.39619, -33.00000)
(4.40195, -16.00000)
(4.40771, 3.00000)
(4.41348, -4.00000)
(4.41924, -11.00000)
(4.42500, 5.00000)
(4.43076, 0.00000)
(4.43652, 15.00000)
(4.44229, 32.00000)
(4.44805, 13.00000)
(4.45381, 13.00000)
(4.45957, -31.00000)
(4.46533, -15.00000)
(4.47109, 2.00000)
(4.47686, 1.00000)
(4.48262, 9.00000)
(4.48838, -16.00000)
(4.49414, -19.00000)
(4.49990, -19.00000)
(4.50566, 11.00000)
(4.51143, -3.00000)
(4.51719, 5.00000)
(4.52295, -13.00000)
(4.52871, 0.00000)
(4.53447, -4.00000)
(4.54023, 5.00000)
(4.54600, 19.00000)
(4.55176, -5.00000)
(4.55752, -11.00000)
(4.56328, 4.00000)
(4.56904, -8.00000)
(4.57480, -12.00000)
(4.58057, -15.00000)
(4.58633, -9.00000)
(4.59209, 21.00000)
(4.59785, 19.00000)
(4.60361, 17.00000)
(4.60938, 19.00000)
(4.61514, -3.00000)
(4.62090, 15.00000)
(4.62666, -29.00000)
(4.63242, -20.00000)
(4.63818, -30.00000)
(4.64395, -11.00000)
(4.64971, 9.00000)
(4.65547, 3.00000)
(4.66123, -8.00000)
(4.66699, 4.00000)
(4.67275, 30.00000)
(4.67852, 31.00000)
(4.68428, 16.00000)
(4.69004, -15.00000)
(4.69580, -38.00000)
(4.70156, -11.00000)
(4.70732, -7.00000)
(4.71309, 25.00000)
(4.71885, 6.00000)
(4.72461, 27.00000)
(4.73037, 5.00000)
(4.73613, -37.00000)
(4.74189, -40.00000)
(4.74766, -29.00000)
(4.75342, -3.00000)
(4.75918, 7.00000)
(4.76494, 16.00000)
(4.77070, 14.00000)
(4.77646, 11.00000)
(4.78223, 8.00000)
(4.78799, 9.00000)
(4.79375, 8.00000)
(4.79951, -11.00000)
(4.80527, 4.00000)
(4.81104, -12.00000)
(4.81680, -5.00000)
(4.82256, -4.00000)
(4.82832, 9.00000)
(4.83408, -3.00000)
(4.83984, 14.00000)
(4.84561, 29.00000)
(4.85137, 24.00000)
(4.85713, 5.00000)
(4.86289, -12.00000)
(4.86865, -13.00000)
(4.87441, -11.00000)
(4.88018, 0.00000)
(4.88594, 0.00000)
(4.89170, -1.00000)
(4.89746, -11.00000)
(4.90322, -1.00000)
(4.90898, -1.00000)
(4.91475, -10.00000)
(4.92051, 2.00000)
(4.92627, 2.00000)
(4.93203, 11.00000)
(4.93779, -8.00000)
(4.94355, -11.00000)
(4.94932, -8.00000)
(4.95508, 1.00000)
(4.96084, 7.00000)
(4.96660, 28.00000)
(4.97236, -8.00000)
(4.97813, -19.00000)
(4.98389, -19.00000)
(4.98965, 6.00000)
(4.99541, -2.00000)
(5.00117, 31.00000)
(5.00693, 5.00000)
(5.01270, 31.00000)
(5.01846, 30.00000)
(5.02422, 8.00000)
(5.02998, 2.00000)
(5.03574, -17.00000)
(5.04150, -18.00000)
(5.04727, -3.00000)
(5.05303, -7.00000)
(5.05879, -9.00000)
(5.06455, -1.00000)
(5.07031, -6.00000)
(5.07607, -2.00000)
(5.08184, 5.00000)
(5.08760, -17.00000)
(5.09336, -39.00000)
(5.09912, -33.00000)
(5.10488, -18.00000)
(5.11064, 16.00000)
(5.11641, 26.00000)
(5.12217, 10.00000)
(5.12793, 21.00000)
(5.13369, 6.00000)
(5.13945, 10.00000)
(5.14521, 22.00000)
(5.15098, -23.00000)
(5.15674, -33.00000)
(5.16250, -57.00000)
(5.16826, -22.00000)
(5.17402, -4.00000)
(5.17979, 16.00000)
(5.18555, 29.00000)
(5.19131, 31.00000)
(5.19707, 51.00000)
(5.20283, 16.00000)
(5.20859, 4.00000)
(5.21436, -12.00000)
(5.22012, -3.00000)
(5.22588, 16.00000)
(5.23164, 1.00000)
(5.23740, -13.00000)
(5.24316, 2.00000)
(5.24893, -1.00000)
(5.25469, -19.00000)
(5.26045, -27.00000)
(5.26621, -24.00000)
(5.27197, -31.00000)
(5.27773, -23.00000)
(5.28350, -14.00000)
(5.28926, 23.00000)
(5.29502, 42.00000)
(5.30078, 48.00000)
(5.30654, 31.00000)
(5.31230, 22.00000)
(5.31807, 8.00000)
(5.32383, 18.00000)
(5.32959, 10.00000)
(5.33535, -12.00000)
(5.34111, -23.00000)
(5.34688, -34.00000)
(5.35264, -37.00000)
(5.35840, -43.00000)
(5.36416, -16.00000)
(5.36992, 4.00000)
(5.37568, 22.00000)
(5.38145, 42.00000)
(5.38721, 51.00000)
(5.39297, 37.00000)
(5.39873, 46.00000)
(5.40449, 17.00000)
(5.41025, -10.00000)
(5.41602, -34.00000)
(5.42178, -43.00000)
(5.42754, -19.00000)
(5.43330, -17.00000)
(5.43906, -31.00000)
(5.44482, -22.00000)
(5.45059, -26.00000)
(5.45635, -3.00000)
(5.46211, 23.00000)
(5.46787, 47.00000)
(5.47363, 23.00000)
(5.47939, -1.00000)
(5.48516, -17.00000)
(5.49092, -6.00000)
(5.49668, 15.00000)
(5.50244, 21.00000)
(5.50820, 21.00000)
(5.51396, -3.00000)
(5.51973, -33.00000)
(5.52549, -36.00000)
(5.53125, -41.00000)
(5.53701, -17.00000)
(5.54277, -1.00000)
(5.54854, 27.00000)
(5.55430, 46.00000)
(5.56006, 53.00000)
(5.56582, 38.00000)
(5.57158, 18.00000)
(5.57734, 5.00000)
(5.58311, -9.00000)
(5.58887, -6.00000)
(5.59463, -24.00000)
(5.60039, -11.00000)
(5.60615, -23.00000)
(5.61191, -26.00000)
(5.61768, -11.00000)
(5.62344, -14.00000)
(5.62920, 7.00000)
(5.63496, -4.00000)
(5.64072, 12.00000)
(5.64648, 21.00000)
(5.65225, 11.00000)
(5.65801, 6.00000)
(5.66377, -5.00000)
(5.66953, -5.00000)
(5.67529, -30.00000)
(5.68105, -26.00000)
(5.68682, -17.00000)
(5.69258, -6.00000)
(5.69834, 6.00000)
(5.70410, 27.00000)
(5.70986, 24.00000)
(5.71563, 6.00000)
(5.72139, 7.00000)
(5.72715, 2.00000)
(5.73291, 17.00000)
(5.73867, 4.00000)
(5.74443, -1.00000)
(5.75020, -9.00000)
(5.75596, -13.00000)
(5.76172, -19.00000)
};


==> Figures/convEEG.tex <==
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,Red1] plot coordinates {
(100.00000, 0.39692)
(110.00000, 0.45390)
(120.00000, 0.38300)
(130.00000, 0.36000)
(140.00000, 0.40014)
(150.00000, 0.37276)
(160.00000, 0.32232)
(170.00000, 0.64903)
(180.00000, 0.34143)
(190.00000, 0.60171)
(200.00000, 0.30456)
(210.00000, 0.33223)
(220.00000, 0.23930)
(230.00000, 0.27002)
(240.00000, 0.18024)
(250.00000, 0.23322)
(260.00000, 0.24117)
(270.00000, 0.22894)
(280.00000, 0.16793)
(290.00000, 0.19975)
(300.00000, 0.19309)
(310.00000, 0.16672)
(320.00000, 0.21462)
(330.00000, 0.19323)
(340.00000, 0.17858)
(350.00000, 0.19933)
(360.00000, 0.17135)
(370.00000, 0.17797)
(380.00000, 0.18909)
(390.00000, 0.19051)
(400.00000, 0.21754)
(410.00000, 0.21452)
(420.00000, 0.18994)
(430.00000, 0.14092)
(440.00000, 0.20386)
(450.00000, 0.16950)
(460.00000, 0.16167)
(470.00000, 0.19604)
(480.00000, 0.18149)
(490.00000, 0.19288)
(500.00000, 0.15999)
(510.00000, 0.15701)
(520.00000, 0.17205)
(530.00000, 0.17428)
(540.00000, 0.14458)
(550.00000, 0.19433)
(560.00000, 0.16041)
(570.00000, 0.15276)
(580.00000, 0.15392)
(590.00000, 0.18241)
(600.00000, 0.14817)
(610.00000, 0.15291)
(620.00000, 0.18774)
(630.00000, 0.19675)
(640.00000, 0.16044)
(650.00000, 0.17372)
(660.00000, 0.14730)
(670.00000, 0.19996)
(680.00000, 0.19487)
(690.00000, 0.18949)
(700.00000, 0.18525)
(710.00000, 0.18632)
(720.00000, 0.17376)
(730.00000, 0.17522)
(740.00000, 0.20157)
(750.00000, 0.17817)
(760.00000, 0.20605)
(770.00000, 0.21122)
(780.00000, 0.18703)
(790.00000, 0.14876)
(800.00000, 0.18944)
(810.00000, 0.18302)
(820.00000, 0.19099)
(830.00000, 0.20199)
(840.00000, 0.19956)
(850.00000, 0.21313)
(860.00000, 0.18944)
(870.00000, 0.21601)
(880.00000, 0.19643)
(890.00000, 0.21536)
(900.00000, 0.20689)
(910.00000, 0.21289)
(920.00000, 0.20717)
(930.00000, 0.21533)
(940.00000, 0.19070)
(950.00000, 0.18663)
(960.00000, 0.18593)
(970.00000, 0.22619)
(980.00000, 0.21909)
(990.00000, 0.23590)
(1000.00000, 0.22368)
(1010.00000, 0.22954)
(1020.00000, 0.27782)
(1030.00000, 0.23424)
(1040.00000, 0.23884)
(1050.00000, 0.22512)
(1060.00000, 0.22597)
(1070.00000, 0.19102)
(1080.00000, 0.22167)
(1090.00000, 0.21799)
(1100.00000, 0.19618)
(1110.00000, 0.20834)
(1120.00000, 0.18185)
(1130.00000, 0.19474)
(1140.00000, 0.20615)
(1150.00000, 0.18631)
(1160.00000, 0.18515)
(1170.00000, 0.19124)
(1180.00000, 0.18694)
(1190.00000, 0.16787)
(1200.00000, 0.16033)
(1210.00000, 0.15845)
(1220.00000, 0.14519)
(1230.00000, 0.15235)
(1240.00000, 0.12214)
(1250.00000, 0.15907)
(1260.00000, 0.16661)
(1270.00000, 0.14713)
(1280.00000, 0.16213)
(1290.00000, 0.13650)
(1300.00000, 0.16279)
(1310.00000, 0.15386)
(1320.00000, 0.13298)
(1330.00000, 0.16088)
(1340.00000, 0.13338)
(1350.00000, 0.15075)
(1360.00000, 0.17449)
(1370.00000, 0.15172)
(1380.00000, 0.17570)
(1390.00000, 0.14712)
(1400.00000, 0.12836)
(1410.00000, 0.15339)
(1420.00000, 0.15865)
(1430.00000, 0.16255)
(1440.00000, 0.14334)
(1450.00000, 0.14744)
(1460.00000, 0.16751)
(1470.00000, 0.14768)
(1480.00000, 0.12298)
(1490.00000, 0.14501)
(1500.00000, 0.13229)
(1510.00000, 0.13968)
(1520.00000, 0.16251)
(1530.00000, 0.13497)
(1540.00000, 0.14590)
(1550.00000, 0.16908)
(1560.00000, 0.15869)
(1570.00000, 0.13657)
(1580.00000, 0.13246)
(1590.00000, 0.14469)
(1600.00000, 0.14677)
(1610.00000, 0.11686)
(1620.00000, 0.10530)
(1630.00000, 0.11679)
(1640.00000, 0.13536)
(1650.00000, 0.12483)
(1660.00000, 0.12627)
(1670.00000, 0.13013)
(1680.00000, 0.10498)
(1690.00000, 0.13363)
(1700.00000, 0.11202)
(1710.00000, 0.10523)
(1720.00000, 0.13253)
(1730.00000, 0.10780)
(1740.00000, 0.12523)
(1750.00000, 0.12948)
(1760.00000, 0.14796)
(1770.00000, 0.12229)
(1780.00000, 0.13860)
(1790.00000, 0.13520)
(1800.00000, 0.12076)
(1810.00000, 0.14166)
(1820.00000, 0.12545)
(1830.00000, 0.14077)
(1840.00000, 0.13298)
(1850.00000, 0.13044)
(1860.00000, 0.15125)
(1870.00000, 0.13801)
(1880.00000, 0.13981)
(1890.00000, 0.15757)
(1900.00000, 0.13915)
(1910.00000, 0.12640)
(1920.00000, 0.15361)
(1930.00000, 0.15015)
(1940.00000, 0.16068)
(1950.00000, 0.17088)
(1960.00000, 0.15868)
(1970.00000, 0.17087)
(1980.00000, 0.16268)
(1990.00000, 0.15652)
(2000.00000, 0.14756)
(2010.00000, 0.15833)
(2020.00000, 0.17847)
(2030.00000, 0.18024)
(2040.00000, 0.15770)
(2050.00000, 0.15709)
(2060.00000, 0.16265)
(2070.00000, 0.15484)
(2080.00000, 0.15629)
(2090.00000, 0.15720)
(2100.00000, 0.16302)
(2110.00000, 0.15347)
(2120.00000, 0.16713)
(2130.00000, 0.16089)
(2140.00000, 0.14961)
(2150.00000, 0.14542)
(2160.00000, 0.16837)
(2170.00000, 0.16626)
(2180.00000, 0.15804)
(2190.00000, 0.13574)
(2200.00000, 0.15012)
(2210.00000, 0.15128)
(2220.00000, 0.16809)
(2230.00000, 0.16097)
(2240.00000, 0.15888)
(2250.00000, 0.15777)
(2260.00000, 0.15733)
(2270.00000, 0.14725)
(2280.00000, 0.14789)
(2290.00000, 0.16925)
(2300.00000, 0.14072)
(2310.00000, 0.15394)
(2320.00000, 0.14589)
(2330.00000, 0.14195)
(2340.00000, 0.15267)
(2350.00000, 0.15501)
(2360.00000, 0.15389)
(2370.00000, 0.14264)
(2380.00000, 0.15531)
(2390.00000, 0.14529)
(2400.00000, 0.15166)
(2410.00000, 0.14853)
(2420.00000, 0.15543)
(2430.00000, 0.14514)
(2440.00000, 0.15479)
(2450.00000, 0.14841)
(2460.00000, 0.14949)
(2470.00000, 0.14799)
(2480.00000, 0.14956)
(2490.00000, 0.12371)
(2500.00000, 0.14008)
(2510.00000, 0.14433)
(2520.00000, 0.14654)
(2530.00000, 0.12844)
(2540.00000, 0.11794)
(2550.00000, 0.13219)
(2560.00000, 0.12386)
(2570.00000, 0.11259)
(2580.00000, 0.11761)
(2590.00000, 0.12067)
(2600.00000, 0.13159)
(2610.00000, 0.09849)
(2620.00000, 0.10681)
(2630.00000, 0.11997)
(2640.00000, 0.10304)
(2650.00000, 0.09800)
(2660.00000, 0.11248)
(2670.00000, 0.10209)
(2680.00000, 0.10757)
(2690.00000, 0.11391)
(2700.00000, 0.09333)
(2710.00000, 0.10470)
(2720.00000, 0.09736)
(2730.00000, 0.09038)
(2740.00000, 0.09623)
(2750.00000, 0.09958)
(2760.00000, 0.09432)
(2770.00000, 0.09628)
(2780.00000, 0.10092)
(2790.00000, 0.08952)
(2800.00000, 0.09255)
(2810.00000, 0.10360)
(2820.00000, 0.08559)
(2830.00000, 0.10112)
(2840.00000, 0.11000)
(2850.00000, 0.10346)
(2860.00000, 0.08510)
(2870.00000, 0.08847)
(2880.00000, 0.09604)
(2890.00000, 0.10253)
(2900.00000, 0.08574)
(2910.00000, 0.08829)
(2920.00000, 0.09844)
(2930.00000, 0.08388)
(2940.00000, 0.09807)
(2950.00000, 0.09995)
(2960.00000, 0.08935)
(2970.00000, 0.09296)
(2980.00000, 0.10155)
(2990.00000, 0.09631)
(3000.00000, 0.09376)
(3010.00000, 0.08442)
(3020.00000, 0.09117)
(3030.00000, 0.08657)
(3040.00000, 0.08185)
(3050.00000, 0.08223)
(3060.00000, 0.11368)
(3070.00000, 0.08746)
(3080.00000, 0.08788)
(3090.00000, 0.09656)
(3100.00000, 0.10104)
(3110.00000, 0.07613)
(3120.00000, 0.07863)
(3130.00000, 0.08247)
(3140.00000, 0.08510)
(3150.00000, 0.09228)
(3160.00000, 0.07352)
(3170.00000, 0.07374)
(3180.00000, 0.07112)
(3190.00000, 0.09194)
(3200.00000, 0.08141)
(3210.00000, 0.07798)
(3220.00000, 0.08296)
(3230.00000, 0.08546)
(3240.00000, 0.08319)
(3250.00000, 0.07270)
(3260.00000, 0.08213)
(3270.00000, 0.08339)
(3280.00000, 0.07347)
(3290.00000, 0.07418)
(3300.00000, 0.07993)
(3310.00000, 0.07766)
(3320.00000, 0.07554)
(3330.00000, 0.07597)
(3340.00000, 0.07092)
(3350.00000, 0.06164)
(3360.00000, 0.06135)
(3370.00000, 0.07455)
(3380.00000, 0.06925)
(3390.00000, 0.06324)
(3400.00000, 0.06348)
(3410.00000, 0.07232)
(3420.00000, 0.06549)
(3430.00000, 0.06860)
(3440.00000, 0.06734)
(3450.00000, 0.06615)
(3460.00000, 0.05835)
(3470.00000, 0.07499)
(3480.00000, 0.06661)
(3490.00000, 0.07684)
(3500.00000, 0.06277)
(3510.00000, 0.08113)
(3520.00000, 0.06745)
(3530.00000, 0.08359)
(3540.00000, 0.06340)
(3550.00000, 0.07365)
(3560.00000, 0.07305)
(3570.00000, 0.07105)
(3580.00000, 0.07231)
(3590.00000, 0.06579)
(3600.00000, 0.06776)
(3610.00000, 0.06292)
(3620.00000, 0.06678)
(3630.00000, 0.07380)
(3640.00000, 0.07153)
(3650.00000, 0.06923)
(3660.00000, 0.07245)
(3670.00000, 0.07250)
(3680.00000, 0.07175)
(3690.00000, 0.07081)
(3700.00000, 0.06695)
(3710.00000, 0.06898)
(3720.00000, 0.05973)
(3730.00000, 0.06756)
(3740.00000, 0.06416)
(3750.00000, 0.07183)
(3760.00000, 0.07167)
(3770.00000, 0.06573)
(3780.00000, 0.06142)
(3790.00000, 0.07586)
(3800.00000, 0.06664)
(3810.00000, 0.06398)
(3820.00000, 0.06732)
(3830.00000, 0.07649)
(3840.00000, 0.06996)
(3850.00000, 0.07478)
(3860.00000, 0.07907)
(3870.00000, 0.06185)
(3880.00000, 0.08372)
(3890.00000, 0.06432)
(3900.00000, 0.06074)
(3910.00000, 0.06710)
(3920.00000, 0.07738)
(3930.00000, 0.07085)
(3940.00000, 0.07061)
(3950.00000, 0.07027)
(3960.00000, 0.07507)
(3970.00000, 0.07579)
(3980.00000, 0.07771)
(3990.00000, 0.07114)
(4000.00000, 0.07828)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,Cyan2] plot coordinates {
(100.00000, 0.57746)
(110.00000, 0.85540)
(120.00000, 0.44508)
(130.00000, 0.36671)
(140.00000, 0.33190)
(150.00000, 0.29503)
(160.00000, 0.32934)
(170.00000, 0.27149)
(180.00000, 0.21958)
(190.00000, 0.19088)
(200.00000, 0.18109)
(210.00000, 0.17477)
(220.00000, 0.20635)
(230.00000, 0.20994)
(240.00000, 0.16855)
(250.00000, 0.18142)
(260.00000, 0.18751)
(270.00000, 0.19145)
(280.00000, 0.17530)
(290.00000, 0.16634)
(300.00000, 0.17196)
(310.00000, 0.16599)
(320.00000, 0.17946)
(330.00000, 0.16365)
(340.00000, 0.17581)
(350.00000, 0.18068)
(360.00000, 0.13385)
(370.00000, 0.16991)
(380.00000, 0.18801)
(390.00000, 0.15400)
(400.00000, 0.14416)
(410.00000, 0.10153)
(420.00000, 0.15510)
(430.00000, 0.12896)
(440.00000, 0.14095)
(450.00000, 0.15033)
(460.00000, 0.13223)
(470.00000, 0.15111)
(480.00000, 0.12290)
(490.00000, 0.11920)
(500.00000, 0.13175)
(510.00000, 0.13389)
(520.00000, 0.15455)
(530.00000, 0.15237)
(540.00000, 0.14608)
(550.00000, 0.15736)
(560.00000, 0.13480)
(570.00000, 0.12946)
(580.00000, 0.13504)
(590.00000, 0.14551)
(600.00000, 0.14346)
(610.00000, 0.13486)
(620.00000, 0.12069)
(630.00000, 0.11225)
(640.00000, 0.11059)
(650.00000, 0.15342)
(660.00000, 0.14781)
(670.00000, 0.12081)
(680.00000, 0.12443)
(690.00000, 0.12513)
(700.00000, 0.11775)
(710.00000, 0.12945)
(720.00000, 0.13250)
(730.00000, 0.11860)
(740.00000, 0.13092)
(750.00000, 0.11805)
(760.00000, 0.12263)
(770.00000, 0.11806)
(780.00000, 0.13506)
(790.00000, 0.09945)
(800.00000, 0.11211)
(810.00000, 0.09649)
(820.00000, 0.11038)
(830.00000, 0.11328)
(840.00000, 0.09499)
(850.00000, 0.10905)
(860.00000, 0.08509)
(870.00000, 0.10808)
(880.00000, 0.09683)
(890.00000, 0.11420)
(900.00000, 0.10276)
(910.00000, 0.11462)
(920.00000, 0.12929)
(930.00000, 0.09310)
(940.00000, 0.09897)
(950.00000, 0.10247)
(960.00000, 0.10719)
(970.00000, 0.10761)
(980.00000, 0.09643)
(990.00000, 0.08596)
(1000.00000, 0.08786)
(1010.00000, 0.07352)
(1020.00000, 0.08994)
(1030.00000, 0.07870)
(1040.00000, 0.09982)
(1050.00000, 0.07454)
(1060.00000, 0.08617)
(1070.00000, 0.08121)
(1080.00000, 0.07228)
(1090.00000, 0.08858)
(1100.00000, 0.08920)
(1110.00000, 0.08853)
(1120.00000, 0.08379)
(1130.00000, 0.08719)
(1140.00000, 0.09226)
(1150.00000, 0.08926)
(1160.00000, 0.09842)
(1170.00000, 0.09820)
(1180.00000, 0.09029)
(1190.00000, 0.08249)
(1200.00000, 0.11057)
(1210.00000, 0.08841)
(1220.00000, 0.08824)
(1230.00000, 0.09521)
(1240.00000, 0.08556)
(1250.00000, 0.08764)
(1260.00000, 0.10373)
(1270.00000, 0.09156)
(1280.00000, 0.10543)
(1290.00000, 0.09893)
(1300.00000, 0.09531)
(1310.00000, 0.10854)
(1320.00000, 0.09577)
(1330.00000, 0.10952)
(1340.00000, 0.10672)
(1350.00000, 0.09423)
(1360.00000, 0.09480)
(1370.00000, 0.10919)
(1380.00000, 0.10631)
(1390.00000, 0.09879)
(1400.00000, 0.10321)
(1410.00000, 0.10398)
(1420.00000, 0.08831)
(1430.00000, 0.10457)
(1440.00000, 0.12418)
(1450.00000, 0.09113)
(1460.00000, 0.09642)
(1470.00000, 0.11507)
(1480.00000, 0.10531)
(1490.00000, 0.09468)
(1500.00000, 0.10449)
(1510.00000, 0.11298)
(1520.00000, 0.11367)
(1530.00000, 0.11477)
(1540.00000, 0.10924)
(1550.00000, 0.11068)
(1560.00000, 0.10120)
(1570.00000, 0.09297)
(1580.00000, 0.11204)
(1590.00000, 0.10540)
(1600.00000, 0.10222)
(1610.00000, 0.08296)
(1620.00000, 0.11248)
(1630.00000, 0.09473)
(1640.00000, 0.08335)
(1650.00000, 0.09819)
(1660.00000, 0.10654)
(1670.00000, 0.08237)
(1680.00000, 0.08525)
(1690.00000, 0.08181)
(1700.00000, 0.09210)
(1710.00000, 0.08612)
(1720.00000, 0.07850)
(1730.00000, 0.11316)
(1740.00000, 0.08054)
(1750.00000, 0.08294)
(1760.00000, 0.07705)
(1770.00000, 0.07658)
(1780.00000, 0.07575)
(1790.00000, 0.07259)
(1800.00000, 0.07713)
(1810.00000, 0.07954)
(1820.00000, 0.08039)
(1830.00000, 0.07987)
(1840.00000, 0.07443)
(1850.00000, 0.08632)
(1860.00000, 0.08352)
(1870.00000, 0.07507)
(1880.00000, 0.07015)
(1890.00000, 0.08408)
(1900.00000, 0.07308)
(1910.00000, 0.06987)
(1920.00000, 0.07715)
(1930.00000, 0.07779)
(1940.00000, 0.07394)
(1950.00000, 0.07716)
(1960.00000, 0.09441)
(1970.00000, 0.08767)
(1980.00000, 0.08455)
(1990.00000, 0.06593)
(2000.00000, 0.07890)
(2010.00000, 0.08410)
(2020.00000, 0.07408)
(2030.00000, 0.07851)
(2040.00000, 0.07886)
(2050.00000, 0.07211)
(2060.00000, 0.07408)
(2070.00000, 0.06953)
(2080.00000, 0.07356)
(2090.00000, 0.07228)
(2100.00000, 0.06690)
(2110.00000, 0.05957)
(2120.00000, 0.06641)
(2130.00000, 0.06334)
(2140.00000, 0.06449)
(2150.00000, 0.06603)
(2160.00000, 0.06535)
(2170.00000, 0.06540)
(2180.00000, 0.05700)
(2190.00000, 0.06625)
(2200.00000, 0.06272)
(2210.00000, 0.05715)
(2220.00000, 0.06476)
(2230.00000, 0.05239)
(2240.00000, 0.05619)
(2250.00000, 0.05813)
(2260.00000, 0.05380)
(2270.00000, 0.05877)
(2280.00000, 0.05460)
(2290.00000, 0.05580)
(2300.00000, 0.05525)
(2310.00000, 0.05634)
(2320.00000, 0.06321)
(2330.00000, 0.06490)
(2340.00000, 0.05568)
(2350.00000, 0.05901)
(2360.00000, 0.05307)
(2370.00000, 0.06469)
(2380.00000, 0.06189)
(2390.00000, 0.04840)
(2400.00000, 0.05788)
(2410.00000, 0.05600)
(2420.00000, 0.05741)
(2430.00000, 0.05249)
(2440.00000, 0.04863)
(2450.00000, 0.04784)
(2460.00000, 0.05040)
(2470.00000, 0.05812)
(2480.00000, 0.05431)
(2490.00000, 0.04951)
(2500.00000, 0.05839)
(2510.00000, 0.05240)
(2520.00000, 0.05619)
(2530.00000, 0.05404)
(2540.00000, 0.04662)
(2550.00000, 0.05604)
(2560.00000, 0.05899)
(2570.00000, 0.05228)
(2580.00000, 0.05563)
(2590.00000, 0.05398)
(2600.00000, 0.05242)
(2610.00000, 0.05184)
(2620.00000, 0.04860)
(2630.00000, 0.04696)
(2640.00000, 0.05425)
(2650.00000, 0.05507)
(2660.00000, 0.05000)
(2670.00000, 0.05274)
(2680.00000, 0.06125)
(2690.00000, 0.05428)
(2700.00000, 0.05161)
(2710.00000, 0.05044)
(2720.00000, 0.04981)
(2730.00000, 0.06134)
(2740.00000, 0.05113)
(2750.00000, 0.05183)
(2760.00000, 0.05905)
(2770.00000, 0.05606)
(2780.00000, 0.05074)
(2790.00000, 0.05356)
(2800.00000, 0.05381)
(2810.00000, 0.06166)
(2820.00000, 0.04842)
(2830.00000, 0.05485)
(2840.00000, 0.05386)
(2850.00000, 0.04832)
(2860.00000, 0.05093)
(2870.00000, 0.05035)
(2880.00000, 0.05409)
(2890.00000, 0.04874)
(2900.00000, 0.05448)
(2910.00000, 0.05388)
(2920.00000, 0.05396)
(2930.00000, 0.05143)
(2940.00000, 0.04769)
(2950.00000, 0.05683)
(2960.00000, 0.04654)
(2970.00000, 0.04821)
(2980.00000, 0.04984)
(2990.00000, 0.06200)
(3000.00000, 0.05319)
(3010.00000, 0.05189)
(3020.00000, 0.05359)
(3030.00000, 0.04643)
(3040.00000, 0.04984)
(3050.00000, 0.05248)
(3060.00000, 0.04144)
(3070.00000, 0.03683)
(3080.00000, 0.04077)
(3090.00000, 0.05032)
(3100.00000, 0.04505)
(3110.00000, 0.04952)
(3120.00000, 0.04776)
(3130.00000, 0.04507)
(3140.00000, 0.04766)
(3150.00000, 0.04312)
(3160.00000, 0.04546)
(3170.00000, 0.04260)
(3180.00000, 0.04949)
(3190.00000, 0.04473)
(3200.00000, 0.04636)
(3210.00000, 0.05039)
(3220.00000, 0.04462)
(3230.00000, 0.04796)
(3240.00000, 0.04879)
(3250.00000, 0.03834)
(3260.00000, 0.05304)
(3270.00000, 0.04239)
(3280.00000, 0.04010)
(3290.00000, 0.04291)
(3300.00000, 0.03720)
(3310.00000, 0.04136)
(3320.00000, 0.05308)
(3330.00000, 0.04598)
(3340.00000, 0.04971)
(3350.00000, 0.05377)
(3360.00000, 0.04483)
(3370.00000, 0.05429)
(3380.00000, 0.04857)
(3390.00000, 0.05100)
(3400.00000, 0.05145)
(3410.00000, 0.04443)
(3420.00000, 0.04782)
(3430.00000, 0.04524)
(3440.00000, 0.05135)
(3450.00000, 0.04537)
(3460.00000, 0.04351)
(3470.00000, 0.05029)
(3480.00000, 0.05475)
(3490.00000, 0.05079)
(3500.00000, 0.04981)
(3510.00000, 0.04515)
(3520.00000, 0.05533)
(3530.00000, 0.04654)
(3540.00000, 0.05418)
(3550.00000, 0.05276)
(3560.00000, 0.05286)
(3570.00000, 0.04007)
(3580.00000, 0.04485)
(3590.00000, 0.04682)
(3600.00000, 0.04993)
(3610.00000, 0.04379)
(3620.00000, 0.05605)
(3630.00000, 0.03905)
(3640.00000, 0.05288)
(3650.00000, 0.04560)
(3660.00000, 0.04649)
(3670.00000, 0.04426)
(3680.00000, 0.04288)
(3690.00000, 0.04666)
(3700.00000, 0.04333)
(3710.00000, 0.04413)
(3720.00000, 0.04843)
(3730.00000, 0.04019)
(3740.00000, 0.04543)
(3750.00000, 0.04837)
(3760.00000, 0.04174)
(3770.00000, 0.05111)
(3780.00000, 0.04728)
(3790.00000, 0.04494)
(3800.00000, 0.05115)
(3810.00000, 0.05075)
(3820.00000, 0.04338)
(3830.00000, 0.04294)
(3840.00000, 0.03808)
(3850.00000, 0.04743)
(3860.00000, 0.04710)
(3870.00000, 0.04185)
(3880.00000, 0.04878)
(3890.00000, 0.04830)
(3900.00000, 0.04224)
(3910.00000, 0.04352)
(3920.00000, 0.03981)
(3930.00000, 0.04931)
(3940.00000, 0.05081)
(3950.00000, 0.05007)
(3960.00000, 0.03923)
(3970.00000, 0.04560)
(3980.00000, 0.05314)
(3990.00000, 0.05001)
(4000.00000, 0.04484)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,Green4] plot coordinates {
(100.00000, 1.93130)
(110.00000, 2.51422)
(120.00000, 2.53722)
(130.00000, 3.11897)
(140.00000, 1.15968)
(150.00000, 0.80870)
(160.00000, 1.10679)
(170.00000, 0.53079)
(180.00000, 0.38234)
(190.00000, 0.41664)
(200.00000, 0.39382)
(210.00000, 0.37101)
(220.00000, 0.36061)
(230.00000, 0.32640)
(240.00000, 0.38106)
(250.00000, 0.33170)
(260.00000, 0.31785)
(270.00000, 0.37256)
(280.00000, 0.32519)
(290.00000, 0.32851)
(300.00000, 0.30709)
(310.00000, 0.29516)
(320.00000, 0.29177)
(330.00000, 0.28628)
(340.00000, 0.25919)
(350.00000, 0.24185)
(360.00000, 0.28175)
(370.00000, 0.29442)
(380.00000, 0.29519)
(390.00000, 0.27775)
(400.00000, 0.26093)
(410.00000, 0.26345)
(420.00000, 0.29159)
(430.00000, 0.22028)
(440.00000, 0.28922)
(450.00000, 0.26468)
(460.00000, 0.21133)
(470.00000, 0.26592)
(480.00000, 0.27635)
(490.00000, 0.26674)
(500.00000, 0.29320)
(510.00000, 0.23602)
(520.00000, 0.22851)
(530.00000, 0.25853)
(540.00000, 0.22214)
(550.00000, 0.23808)
(560.00000, 0.26368)
(570.00000, 0.26286)
(580.00000, 0.31577)
(590.00000, 0.25880)
(600.00000, 0.25524)
(610.00000, 0.23549)
(620.00000, 0.25734)
(630.00000, 0.23626)
(640.00000, 0.27248)
(650.00000, 0.28173)
(660.00000, 0.27531)
(670.00000, 0.24770)
(680.00000, 0.27631)
(690.00000, 0.22440)
(700.00000, 0.18544)
(710.00000, 0.18082)
(720.00000, 0.23732)
(730.00000, 0.19821)
(740.00000, 0.22293)
(750.00000, 0.22021)
(760.00000, 0.20337)
(770.00000, 0.20828)
(780.00000, 0.23156)
(790.00000, 0.19210)
(800.00000, 0.14535)
(810.00000, 0.17916)
(820.00000, 0.18671)
(830.00000, 0.17015)
(840.00000, 0.14695)
(850.00000, 0.15476)
(860.00000, 0.14533)
(870.00000, 0.15015)
(880.00000, 0.13255)
(890.00000, 0.14396)
(900.00000, 0.12955)
(910.00000, 0.15032)
(920.00000, 0.14101)
(930.00000, 0.12412)
(940.00000, 0.10278)
(950.00000, 0.11601)
(960.00000, 0.14041)
(970.00000, 0.10228)
(980.00000, 0.09918)
(990.00000, 0.10842)
(1000.00000, 0.09115)
(1010.00000, 0.11243)
(1020.00000, 0.09427)
(1030.00000, 0.13233)
(1040.00000, 0.11530)
(1050.00000, 0.10526)
(1060.00000, 0.10909)
(1070.00000, 0.10873)
(1080.00000, 0.09481)
(1090.00000, 0.10902)
(1100.00000, 0.10376)
(1110.00000, 0.09925)
(1120.00000, 0.09943)
(1130.00000, 0.09887)
(1140.00000, 0.10939)
(1150.00000, 0.08351)
(1160.00000, 0.11083)
(1170.00000, 0.09798)
(1180.00000, 0.11487)
(1190.00000, 0.10587)
(1200.00000, 0.09412)
(1210.00000, 0.12197)
(1220.00000, 0.10397)
(1230.00000, 0.10558)
(1240.00000, 0.10493)
(1250.00000, 0.08939)
(1260.00000, 0.11577)
(1270.00000, 0.11124)
(1280.00000, 0.10864)
(1290.00000, 0.10797)
(1300.00000, 0.10071)
(1310.00000, 0.09458)
(1320.00000, 0.10226)
(1330.00000, 0.09741)
(1340.00000, 0.11911)
(1350.00000, 0.10448)
(1360.00000, 0.09261)
(1370.00000, 0.08615)
(1380.00000, 0.09826)
(1390.00000, 0.09859)
(1400.00000, 0.09226)
(1410.00000, 0.09578)
(1420.00000, 0.08603)
(1430.00000, 0.09419)
(1440.00000, 0.08929)
(1450.00000, 0.09327)
(1460.00000, 0.08104)
(1470.00000, 0.09096)
(1480.00000, 0.10450)
(1490.00000, 0.08859)
(1500.00000, 0.09938)
(1510.00000, 0.07840)
(1520.00000, 0.07742)
(1530.00000, 0.08843)
(1540.00000, 0.09576)
(1550.00000, 0.08892)
(1560.00000, 0.10319)
(1570.00000, 0.08727)
(1580.00000, 0.08130)
(1590.00000, 0.09392)
(1600.00000, 0.09055)
(1610.00000, 0.08930)
(1620.00000, 0.09054)
(1630.00000, 0.09413)
(1640.00000, 0.09978)
(1650.00000, 0.08684)
(1660.00000, 0.07854)
(1670.00000, 0.08223)
(1680.00000, 0.10877)
(1690.00000, 0.09099)
(1700.00000, 0.06561)
(1710.00000, 0.09292)
(1720.00000, 0.09106)
(1730.00000, 0.08899)
(1740.00000, 0.09200)
(1750.00000, 0.09596)
(1760.00000, 0.09985)
(1770.00000, 0.08197)
(1780.00000, 0.08519)
(1790.00000, 0.10054)
(1800.00000, 0.10725)
(1810.00000, 0.10434)
(1820.00000, 0.08666)
(1830.00000, 0.08654)
(1840.00000, 0.08832)
(1850.00000, 0.07203)
(1860.00000, 0.08126)
(1870.00000, 0.09632)
(1880.00000, 0.09849)
(1890.00000, 0.09152)
(1900.00000, 0.09569)
(1910.00000, 0.08597)
(1920.00000, 0.08774)
(1930.00000, 0.09560)
(1940.00000, 0.09337)
(1950.00000, 0.09099)
(1960.00000, 0.08675)
(1970.00000, 0.08997)
(1980.00000, 0.09004)
(1990.00000, 0.09154)
(2000.00000, 0.08800)
(2010.00000, 0.06345)
(2020.00000, 0.08444)
(2030.00000, 0.06910)
(2040.00000, 0.08726)
(2050.00000, 0.08460)
(2060.00000, 0.07581)
(2070.00000, 0.07807)
(2080.00000, 0.06932)
(2090.00000, 0.07143)
(2100.00000, 0.07613)
(2110.00000, 0.07774)
(2120.00000, 0.07465)
(2130.00000, 0.05830)
(2140.00000, 0.08330)
(2150.00000, 0.07890)
(2160.00000, 0.08323)
(2170.00000, 0.07742)
(2180.00000, 0.06482)
(2190.00000, 0.08186)
(2200.00000, 0.07325)
(2210.00000, 0.06814)
(2220.00000, 0.08067)
(2230.00000, 0.06173)
(2240.00000, 0.07096)
(2250.00000, 0.05540)
(2260.00000, 0.07629)
(2270.00000, 0.04955)
(2280.00000, 0.05248)
(2290.00000, 0.05871)
(2300.00000, 0.06319)
(2310.00000, 0.06673)
(2320.00000, 0.06137)
(2330.00000, 0.06711)
(2340.00000, 0.06690)
(2350.00000, 0.07411)
(2360.00000, 0.05498)
(2370.00000, 0.07021)
(2380.00000, 0.05708)
(2390.00000, 0.05228)
(2400.00000, 0.06656)
(2410.00000, 0.06241)
(2420.00000, 0.06052)
(2430.00000, 0.06559)
(2440.00000, 0.06609)
(2450.00000, 0.05029)
(2460.00000, 0.06313)
(2470.00000, 0.06171)
(2480.00000, 0.06042)
(2490.00000, 0.06472)
(2500.00000, 0.06569)
(2510.00000, 0.07609)
(2520.00000, 0.06796)
(2530.00000, 0.06182)
(2540.00000, 0.06080)
(2550.00000, 0.06658)
(2560.00000, 0.05694)
(2570.00000, 0.05022)
(2580.00000, 0.07448)
(2590.00000, 0.06868)
(2600.00000, 0.05414)
(2610.00000, 0.06560)
(2620.00000, 0.05375)
(2630.00000, 0.07070)
(2640.00000, 0.06873)
(2650.00000, 0.06081)
(2660.00000, 0.05569)
(2670.00000, 0.06721)
(2680.00000, 0.05691)
(2690.00000, 0.06952)
(2700.00000, 0.06788)
(2710.00000, 0.06425)
(2720.00000, 0.05796)
(2730.00000, 0.05765)
(2740.00000, 0.05987)
(2750.00000, 0.05455)
(2760.00000, 0.05874)
(2770.00000, 0.05353)
(2780.00000, 0.05676)
(2790.00000, 0.05604)
(2800.00000, 0.06579)
(2810.00000, 0.07029)
(2820.00000, 0.05105)
(2830.00000, 0.05255)
(2840.00000, 0.05688)
(2850.00000, 0.06670)
(2860.00000, 0.05375)
(2870.00000, 0.06023)
(2880.00000, 0.05740)
(2890.00000, 0.05345)
(2900.00000, 0.05773)
(2910.00000, 0.06246)
(2920.00000, 0.06718)
(2930.00000, 0.05970)
(2940.00000, 0.06010)
(2950.00000, 0.05973)
(2960.00000, 0.06407)
(2970.00000, 0.05747)
(2980.00000, 0.05765)
(2990.00000, 0.06557)
(3000.00000, 0.07270)
(3010.00000, 0.06125)
(3020.00000, 0.06675)
(3030.00000, 0.06996)
(3040.00000, 0.05755)
(3050.00000, 0.06701)
(3060.00000, 0.05911)
(3070.00000, 0.07065)
(3080.00000, 0.06888)
(3090.00000, 0.06272)
(3100.00000, 0.06473)
(3110.00000, 0.07080)
(3120.00000, 0.06575)
(3130.00000, 0.06238)
(3140.00000, 0.05461)
(3150.00000, 0.06004)
(3160.00000, 0.06494)
(3170.00000, 0.06515)
(3180.00000, 0.06868)
(3190.00000, 0.06519)
(3200.00000, 0.06449)
(3210.00000, 0.06901)
(3220.00000, 0.05538)
(3230.00000, 0.07183)
(3240.00000, 0.07026)
(3250.00000, 0.06748)
(3260.00000, 0.05440)
(3270.00000, 0.06312)
(3280.00000, 0.07462)
(3290.00000, 0.06710)
(3300.00000, 0.06776)
(3310.00000, 0.06411)
(3320.00000, 0.06604)
(3330.00000, 0.06787)
(3340.00000, 0.05134)
(3350.00000, 0.05842)
(3360.00000, 0.06458)
(3370.00000, 0.04704)
(3380.00000, 0.06209)
(3390.00000, 0.05651)
(3400.00000, 0.04965)
(3410.00000, 0.06653)
(3420.00000, 0.05235)
(3430.00000, 0.05332)
(3440.00000, 0.06642)
(3450.00000, 0.05914)
(3460.00000, 0.05645)
(3470.00000, 0.05162)
(3480.00000, 0.06306)
(3490.00000, 0.06299)
(3500.00000, 0.06535)
(3510.00000, 0.06108)
(3520.00000, 0.06335)
(3530.00000, 0.06431)
(3540.00000, 0.05793)
(3550.00000, 0.05228)
(3560.00000, 0.04924)
(3570.00000, 0.06272)
(3580.00000, 0.04902)
(3590.00000, 0.07006)
(3600.00000, 0.06135)
(3610.00000, 0.05119)
(3620.00000, 0.06059)
(3630.00000, 0.05421)
(3640.00000, 0.05197)
(3650.00000, 0.06184)
(3660.00000, 0.06050)
(3670.00000, 0.06322)
(3680.00000, 0.06696)
(3690.00000, 0.05976)
(3700.00000, 0.06126)
(3710.00000, 0.06252)
(3720.00000, 0.05939)
(3730.00000, 0.05497)
(3740.00000, 0.06506)
(3750.00000, 0.06006)
(3760.00000, 0.06047)
(3770.00000, 0.05987)
(3780.00000, 0.04987)
(3790.00000, 0.06240)
(3800.00000, 0.06069)
(3810.00000, 0.05823)
(3820.00000, 0.05497)
(3830.00000, 0.06456)
(3840.00000, 0.06333)
(3850.00000, 0.06614)
(3860.00000, 0.05549)
(3870.00000, 0.05600)
(3880.00000, 0.06448)
(3890.00000, 0.06058)
(3900.00000, 0.06476)
(3910.00000, 0.05782)
(3920.00000, 0.06638)
(3930.00000, 0.06730)
(3940.00000, 0.06378)
(3950.00000, 0.05501)
(3960.00000, 0.05229)
(3970.00000, 0.06493)
(3980.00000, 0.05536)
(3990.00000, 0.06304)
(4000.00000, 0.07137)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,blue] plot coordinates {
(100.00000, 0.57040)
(110.00000, 0.86924)
(120.00000, 0.49369)
(130.00000, 0.43132)
(140.00000, 0.36865)
(150.00000, 0.31633)
(160.00000, 0.33049)
(170.00000, 0.26016)
(180.00000, 0.27548)
(190.00000, 0.23877)
(200.00000, 0.20294)
(210.00000, 0.23448)
(220.00000, 0.17620)
(230.00000, 0.17278)
(240.00000, 0.19360)
(250.00000, 0.19385)
(260.00000, 0.20209)
(270.00000, 0.15610)
(280.00000, 0.16911)
(290.00000, 0.13839)
(300.00000, 0.16130)
(310.00000, 0.15519)
(320.00000, 0.15457)
(330.00000, 0.16784)
(340.00000, 0.16300)
(350.00000, 0.18415)
(360.00000, 0.16828)
(370.00000, 0.14202)
(380.00000, 0.14919)
(390.00000, 0.12617)
(400.00000, 0.13468)
(410.00000, 0.15536)
(420.00000, 0.13551)
(430.00000, 0.13929)
(440.00000, 0.12016)
(450.00000, 0.13917)
(460.00000, 0.11392)
(470.00000, 0.11576)
(480.00000, 0.12882)
(490.00000, 0.12448)
(500.00000, 0.11983)
(510.00000, 0.11190)
(520.00000, 0.10990)
(530.00000, 0.10709)
(540.00000, 0.11937)
(550.00000, 0.10178)
(560.00000, 0.11315)
(570.00000, 0.09624)
(580.00000, 0.09979)
(590.00000, 0.10527)
(600.00000, 0.09123)
(610.00000, 0.10495)
(620.00000, 0.08890)
(630.00000, 0.09868)
(640.00000, 0.10567)
(650.00000, 0.10215)
(660.00000, 0.10037)
(670.00000, 0.10085)
(680.00000, 0.12031)
(690.00000, 0.11323)
(700.00000, 0.09612)
(710.00000, 0.07852)
(720.00000, 0.10001)
(730.00000, 0.09228)
(740.00000, 0.10169)
(750.00000, 0.09899)
(760.00000, 0.09608)
(770.00000, 0.11452)
(780.00000, 0.09322)
(790.00000, 0.10603)
(800.00000, 0.10473)
(810.00000, 0.10460)
(820.00000, 0.11337)
(830.00000, 0.11788)
(840.00000, 0.10416)
(850.00000, 0.10222)
(860.00000, 0.11254)
(870.00000, 0.10730)
(880.00000, 0.12945)
(890.00000, 0.11640)
(900.00000, 0.13390)
(910.00000, 0.10538)
(920.00000, 0.11811)
(930.00000, 0.13475)
(940.00000, 0.11737)
(950.00000, 0.12068)
(960.00000, 0.10984)
(970.00000, 0.14876)
(980.00000, 0.11128)
(990.00000, 0.14723)
(1000.00000, 0.12140)
(1010.00000, 0.12727)
(1020.00000, 0.12394)
(1030.00000, 0.12226)
(1040.00000, 0.12163)
(1050.00000, 0.12196)
(1060.00000, 0.12162)
(1070.00000, 0.10298)
(1080.00000, 0.10332)
(1090.00000, 0.09513)
(1100.00000, 0.09953)
(1110.00000, 0.11059)
(1120.00000, 0.12582)
(1130.00000, 0.08747)
(1140.00000, 0.10506)
(1150.00000, 0.09125)
(1160.00000, 0.10765)
(1170.00000, 0.08351)
(1180.00000, 0.09660)
(1190.00000, 0.08919)
(1200.00000, 0.09904)
(1210.00000, 0.08712)
(1220.00000, 0.08711)
(1230.00000, 0.07910)
(1240.00000, 0.08820)
(1250.00000, 0.08904)
(1260.00000, 0.08986)
(1270.00000, 0.08547)
(1280.00000, 0.08819)
(1290.00000, 0.09562)
(1300.00000, 0.09644)
(1310.00000, 0.08334)
(1320.00000, 0.08292)
(1330.00000, 0.09836)
(1340.00000, 0.07459)
(1350.00000, 0.08826)
(1360.00000, 0.08332)
(1370.00000, 0.08987)
(1380.00000, 0.08106)
(1390.00000, 0.09291)
(1400.00000, 0.07876)
(1410.00000, 0.07266)
(1420.00000, 0.07987)
(1430.00000, 0.07706)
(1440.00000, 0.07613)
(1450.00000, 0.08022)
(1460.00000, 0.07784)
(1470.00000, 0.08077)
(1480.00000, 0.07440)
(1490.00000, 0.08924)
(1500.00000, 0.08018)
(1510.00000, 0.07339)
(1520.00000, 0.06754)
(1530.00000, 0.07093)
(1540.00000, 0.07531)
(1550.00000, 0.07411)
(1560.00000, 0.06510)
(1570.00000, 0.07422)
(1580.00000, 0.07317)
(1590.00000, 0.07440)
(1600.00000, 0.06233)
(1610.00000, 0.07097)
(1620.00000, 0.06448)
(1630.00000, 0.07932)
(1640.00000, 0.06407)
(1650.00000, 0.06364)
(1660.00000, 0.07081)
(1670.00000, 0.06725)
(1680.00000, 0.06568)
(1690.00000, 0.06135)
(1700.00000, 0.06214)
(1710.00000, 0.06016)
(1720.00000, 0.06436)
(1730.00000, 0.07393)
(1740.00000, 0.05777)
(1750.00000, 0.07418)
(1760.00000, 0.06404)
(1770.00000, 0.06359)
(1780.00000, 0.04992)
(1790.00000, 0.06175)
(1800.00000, 0.06095)
(1810.00000, 0.05886)
(1820.00000, 0.05109)
(1830.00000, 0.05389)
(1840.00000, 0.06440)
(1850.00000, 0.06434)
(1860.00000, 0.05455)
(1870.00000, 0.06412)
(1880.00000, 0.05837)
(1890.00000, 0.05781)
(1900.00000, 0.05492)
(1910.00000, 0.05234)
(1920.00000, 0.06220)
(1930.00000, 0.05804)
(1940.00000, 0.05065)
(1950.00000, 0.05206)
(1960.00000, 0.05221)
(1970.00000, 0.05147)
(1980.00000, 0.06174)
(1990.00000, 0.04445)
(2000.00000, 0.05801)
(2010.00000, 0.04999)
(2020.00000, 0.05979)
(2030.00000, 0.05519)
(2040.00000, 0.05817)
(2050.00000, 0.05320)
(2060.00000, 0.05171)
(2070.00000, 0.05314)
(2080.00000, 0.05890)
(2090.00000, 0.04801)
(2100.00000, 0.05561)
(2110.00000, 0.04697)
(2120.00000, 0.05249)
(2130.00000, 0.05588)
(2140.00000, 0.05310)
(2150.00000, 0.05258)
(2160.00000, 0.06003)
(2170.00000, 0.06101)
(2180.00000, 0.04495)
(2190.00000, 0.05660)
(2200.00000, 0.05917)
(2210.00000, 0.04437)
(2220.00000, 0.05926)
(2230.00000, 0.04878)
(2240.00000, 0.05448)
(2250.00000, 0.04636)
(2260.00000, 0.05795)
(2270.00000, 0.05564)
(2280.00000, 0.04652)
(2290.00000, 0.04622)
(2300.00000, 0.04762)
(2310.00000, 0.05542)
(2320.00000, 0.04944)
(2330.00000, 0.04567)
(2340.00000, 0.04649)
(2350.00000, 0.04643)
(2360.00000, 0.05188)
(2370.00000, 0.05971)
(2380.00000, 0.05060)
(2390.00000, 0.04505)
(2400.00000, 0.05475)
(2410.00000, 0.03963)
(2420.00000, 0.05505)
(2430.00000, 0.05713)
(2440.00000, 0.04270)
(2450.00000, 0.05170)
(2460.00000, 0.05176)
(2470.00000, 0.04275)
(2480.00000, 0.04869)
(2490.00000, 0.04384)
(2500.00000, 0.05298)
(2510.00000, 0.05308)
(2520.00000, 0.04799)
(2530.00000, 0.04252)
(2540.00000, 0.05419)
(2550.00000, 0.05096)
(2560.00000, 0.04680)
(2570.00000, 0.04978)
(2580.00000, 0.05636)
(2590.00000, 0.05107)
(2600.00000, 0.05364)
(2610.00000, 0.05526)
(2620.00000, 0.04984)
(2630.00000, 0.04902)
(2640.00000, 0.05306)
(2650.00000, 0.04398)
(2660.00000, 0.05399)
(2670.00000, 0.04526)
(2680.00000, 0.04841)
(2690.00000, 0.04800)
(2700.00000, 0.05163)
(2710.00000, 0.04444)
(2720.00000, 0.05635)
(2730.00000, 0.04897)
(2740.00000, 0.04938)
(2750.00000, 0.04579)
(2760.00000, 0.05281)
(2770.00000, 0.04288)
(2780.00000, 0.05858)
(2790.00000, 0.04806)
(2800.00000, 0.04067)
(2810.00000, 0.04822)
(2820.00000, 0.05024)
(2830.00000, 0.04730)
(2840.00000, 0.04852)
(2850.00000, 0.04669)
(2860.00000, 0.04696)
(2870.00000, 0.04158)
(2880.00000, 0.04715)
(2890.00000, 0.04123)
(2900.00000, 0.05045)
(2910.00000, 0.04616)
(2920.00000, 0.04918)
(2930.00000, 0.04462)
(2940.00000, 0.04535)
(2950.00000, 0.03988)
(2960.00000, 0.04264)
(2970.00000, 0.04865)
(2980.00000, 0.04347)
(2990.00000, 0.04092)
(3000.00000, 0.04701)
(3010.00000, 0.04423)
(3020.00000, 0.05016)
(3030.00000, 0.04066)
(3040.00000, 0.03371)
(3050.00000, 0.04603)
(3060.00000, 0.05250)
(3070.00000, 0.04706)
(3080.00000, 0.04116)
(3090.00000, 0.04017)
(3100.00000, 0.04544)
(3110.00000, 0.04743)
(3120.00000, 0.04604)
(3130.00000, 0.04310)
(3140.00000, 0.04145)
(3150.00000, 0.04460)
(3160.00000, 0.04714)
(3170.00000, 0.03966)
(3180.00000, 0.03707)
(3190.00000, 0.03966)
(3200.00000, 0.04016)
(3210.00000, 0.03952)
(3220.00000, 0.04502)
(3230.00000, 0.04030)
(3240.00000, 0.03762)
(3250.00000, 0.04539)
(3260.00000, 0.04728)
(3270.00000, 0.03995)
(3280.00000, 0.04902)
(3290.00000, 0.03795)
(3300.00000, 0.04511)
(3310.00000, 0.04829)
(3320.00000, 0.04799)
(3330.00000, 0.04278)
(3340.00000, 0.04473)
(3350.00000, 0.04094)
(3360.00000, 0.04119)
(3370.00000, 0.04564)
(3380.00000, 0.04382)
(3390.00000, 0.03606)
(3400.00000, 0.03869)
(3410.00000, 0.04386)
(3420.00000, 0.04528)
(3430.00000, 0.03947)
(3440.00000, 0.03384)
(3450.00000, 0.04053)
(3460.00000, 0.04021)
(3470.00000, 0.04530)
(3480.00000, 0.04645)
(3490.00000, 0.04813)
(3500.00000, 0.04510)
(3510.00000, 0.04079)
(3520.00000, 0.04242)
(3530.00000, 0.04140)
(3540.00000, 0.04286)
(3550.00000, 0.04626)
(3560.00000, 0.04351)
(3570.00000, 0.03705)
(3580.00000, 0.03866)
(3590.00000, 0.04617)
(3600.00000, 0.04334)
(3610.00000, 0.03711)
(3620.00000, 0.03666)
(3630.00000, 0.04092)
(3640.00000, 0.04271)
(3650.00000, 0.04418)
(3660.00000, 0.04472)
(3670.00000, 0.04145)
(3680.00000, 0.03376)
(3690.00000, 0.03901)
(3700.00000, 0.04149)
(3710.00000, 0.03679)
(3720.00000, 0.04993)
(3730.00000, 0.03779)
(3740.00000, 0.04201)
(3750.00000, 0.04074)
(3760.00000, 0.03273)
(3770.00000, 0.04082)
(3780.00000, 0.03332)
(3790.00000, 0.03986)
(3800.00000, 0.04013)
(3810.00000, 0.03318)
(3820.00000, 0.04012)
(3830.00000, 0.03897)
(3840.00000, 0.03715)
(3850.00000, 0.04369)
(3860.00000, 0.04226)
(3870.00000, 0.04365)
(3880.00000, 0.04045)
(3890.00000, 0.03808)
(3900.00000, 0.03620)
(3910.00000, 0.04428)
(3920.00000, 0.03724)
(3930.00000, 0.03517)
(3940.00000, 0.04337)
(3950.00000, 0.04189)
(3960.00000, 0.03538)
(3970.00000, 0.03997)
(3980.00000, 0.03879)
(3990.00000, 0.04190)
(4000.00000, 0.03701)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,Green3] plot coordinates {
(100.00000, 8.16330)
(110.00000, 8.45581)
(120.00000, 5.99327)
(130.00000, 4.74158)
(140.00000, 4.15656)
(150.00000, 5.35592)
(160.00000, 3.54644)
(170.00000, 4.09484)
(180.00000, 2.85484)
(190.00000, 3.21100)
(200.00000, 2.84395)
(210.00000, 2.22882)
(220.00000, 1.95413)
(230.00000, 3.44407)
(240.00000, 2.51632)
(250.00000, 1.55666)
(260.00000, 2.51132)
(270.00000, 0.60463)
(280.00000, 2.84447)
(290.00000, 0.82442)
(300.00000, 1.15162)
(310.00000, 0.49373)
(320.00000, 0.55020)
(330.00000, 0.44582)
(340.00000, 0.49862)
(350.00000, 0.46660)
(360.00000, 0.35910)
(370.00000, 0.34983)
(380.00000, 0.37622)
(390.00000, 0.37002)
(400.00000, 0.44378)
(410.00000, 0.37237)
(420.00000, 0.43650)
(430.00000, 0.43320)
(440.00000, 0.36044)
(450.00000, 0.38753)
(460.00000, 0.43730)
(470.00000, 0.36123)
(480.00000, 0.43381)
(490.00000, 0.41938)
(500.00000, 0.41403)
(510.00000, 0.39169)
(520.00000, 0.40293)
(530.00000, 0.38161)
(540.00000, 0.31224)
(550.00000, 0.39748)
(560.00000, 0.40062)
(570.00000, 0.39828)
(580.00000, 0.39048)
(590.00000, 0.38771)
(600.00000, 0.43821)
(610.00000, 0.39122)
(620.00000, 0.41605)
(630.00000, 0.42344)
(640.00000, 0.39422)
(650.00000, 0.39191)
(660.00000, 0.39038)
(670.00000, 0.47236)
(680.00000, 0.41492)
(690.00000, 0.38077)
(700.00000, 0.40175)
(710.00000, 0.38616)
(720.00000, 0.39283)
(730.00000, 0.36020)
(740.00000, 0.38003)
(750.00000, 0.35083)
(760.00000, 0.34170)
(770.00000, 0.35828)
(780.00000, 0.31185)
(790.00000, 0.29938)
(800.00000, 0.32923)
(810.00000, 0.32147)
(820.00000, 0.30131)
(830.00000, 0.35185)
(840.00000, 0.31771)
(850.00000, 0.28855)
(860.00000, 0.31744)
(870.00000, 0.27779)
(880.00000, 0.28952)
(890.00000, 0.29953)
(900.00000, 0.27156)
(910.00000, 0.27031)
(920.00000, 0.25650)
(930.00000, 0.26954)
(940.00000, 0.28434)
(950.00000, 0.26817)
(960.00000, 0.28019)
(970.00000, 0.26446)
(980.00000, 0.28203)
(990.00000, 0.26896)
(1000.00000, 0.25516)
(1010.00000, 0.28302)
(1020.00000, 0.23791)
(1030.00000, 0.25407)
(1040.00000, 0.25907)
(1050.00000, 0.28426)
(1060.00000, 0.25229)
(1070.00000, 0.22471)
(1080.00000, 0.27186)
(1090.00000, 0.21838)
(1100.00000, 0.26128)
(1110.00000, 0.26678)
(1120.00000, 0.24804)
(1130.00000, 0.24894)
(1140.00000, 0.22203)
(1150.00000, 0.22022)
(1160.00000, 0.25007)
(1170.00000, 0.25122)
(1180.00000, 0.19574)
(1190.00000, 0.25867)
(1200.00000, 0.24225)
(1210.00000, 0.22320)
(1220.00000, 0.18985)
(1230.00000, 0.21247)
(1240.00000, 0.24139)
(1250.00000, 0.22363)
(1260.00000, 0.22298)
(1270.00000, 0.22593)
(1280.00000, 0.26103)
(1290.00000, 0.19430)
(1300.00000, 0.20231)
(1310.00000, 0.17796)
(1320.00000, 0.22915)
(1330.00000, 0.18743)
(1340.00000, 0.24331)
(1350.00000, 0.22591)
(1360.00000, 0.23683)
(1370.00000, 0.21700)
(1380.00000, 0.22206)
(1390.00000, 0.21580)
(1400.00000, 0.19593)
(1410.00000, 0.18599)
(1420.00000, 0.20539)
(1430.00000, 0.23288)
(1440.00000, 0.22409)
(1450.00000, 0.17430)
(1460.00000, 0.18387)
(1470.00000, 0.20331)
(1480.00000, 0.18705)
(1490.00000, 0.20255)
(1500.00000, 0.18009)
(1510.00000, 0.18517)
(1520.00000, 0.17583)
(1530.00000, 0.18902)
(1540.00000, 0.21844)
(1550.00000, 0.17094)
(1560.00000, 0.18959)
(1570.00000, 0.21434)
(1580.00000, 0.17291)
(1590.00000, 0.17486)
(1600.00000, 0.18353)
(1610.00000, 0.17666)
(1620.00000, 0.20020)
(1630.00000, 0.19640)
(1640.00000, 0.18588)
(1650.00000, 0.17214)
(1660.00000, 0.19715)
(1670.00000, 0.20344)
(1680.00000, 0.19920)
(1690.00000, 0.24061)
(1700.00000, 0.19507)
(1710.00000, 0.17854)
(1720.00000, 0.18236)
(1730.00000, 0.19907)
(1740.00000, 0.20949)
(1750.00000, 0.17445)
(1760.00000, 0.20296)
(1770.00000, 0.18105)
(1780.00000, 0.20265)
(1790.00000, 0.19052)
(1800.00000, 0.19662)
(1810.00000, 0.20601)
(1820.00000, 0.18145)
(1830.00000, 0.18371)
(1840.00000, 0.22824)
(1850.00000, 0.17847)
(1860.00000, 0.20181)
(1870.00000, 0.16728)
(1880.00000, 0.20035)
(1890.00000, 0.19780)
(1900.00000, 0.18345)
(1910.00000, 0.19176)
(1920.00000, 0.17925)
(1930.00000, 0.19615)
(1940.00000, 0.19368)
(1950.00000, 0.18345)
(1960.00000, 0.19098)
(1970.00000, 0.19345)
(1980.00000, 0.17467)
(1990.00000, 0.20443)
(2000.00000, 0.17861)
(2010.00000, 0.15651)
(2020.00000, 0.17266)
(2030.00000, 0.14952)
(2040.00000, 0.15058)
(2050.00000, 0.17447)
(2060.00000, 0.17077)
(2070.00000, 0.19209)
(2080.00000, 0.15270)
(2090.00000, 0.17332)
(2100.00000, 0.15875)
(2110.00000, 0.16831)
(2120.00000, 0.14733)
(2130.00000, 0.15975)
(2140.00000, 0.17157)
(2150.00000, 0.17042)
(2160.00000, 0.12268)
(2170.00000, 0.16607)
(2180.00000, 0.15532)
(2190.00000, 0.14323)
(2200.00000, 0.15581)
(2210.00000, 0.15925)
(2220.00000, 0.13673)
(2230.00000, 0.15433)
(2240.00000, 0.15419)
(2250.00000, 0.14634)
(2260.00000, 0.16592)
(2270.00000, 0.15272)
(2280.00000, 0.15626)
(2290.00000, 0.14691)
(2300.00000, 0.13501)
(2310.00000, 0.12680)
(2320.00000, 0.12298)
(2330.00000, 0.14569)
(2340.00000, 0.16292)
(2350.00000, 0.14155)
(2360.00000, 0.14446)
(2370.00000, 0.13343)
(2380.00000, 0.13066)
(2390.00000, 0.15296)
(2400.00000, 0.13618)
(2410.00000, 0.16385)
(2420.00000, 0.15190)
(2430.00000, 0.14467)
(2440.00000, 0.13468)
(2450.00000, 0.15014)
(2460.00000, 0.15218)
(2470.00000, 0.14476)
(2480.00000, 0.13360)
(2490.00000, 0.11723)
(2500.00000, 0.12968)
(2510.00000, 0.13358)
(2520.00000, 0.14281)
(2530.00000, 0.12215)
(2540.00000, 0.11357)
(2550.00000, 0.15130)
(2560.00000, 0.14207)
(2570.00000, 0.13771)
(2580.00000, 0.13335)
(2590.00000, 0.13362)
(2600.00000, 0.12200)
(2610.00000, 0.12710)
(2620.00000, 0.10727)
(2630.00000, 0.13026)
(2640.00000, 0.11769)
(2650.00000, 0.10131)
(2660.00000, 0.12193)
(2670.00000, 0.11372)
(2680.00000, 0.12164)
(2690.00000, 0.12302)
(2700.00000, 0.12873)
(2710.00000, 0.11960)
(2720.00000, 0.10167)
(2730.00000, 0.11674)
(2740.00000, 0.14005)
(2750.00000, 0.11434)
(2760.00000, 0.10742)
(2770.00000, 0.11339)
(2780.00000, 0.10162)
(2790.00000, 0.10438)
(2800.00000, 0.13287)
(2810.00000, 0.12908)
(2820.00000, 0.10950)
(2830.00000, 0.10952)
(2840.00000, 0.10473)
(2850.00000, 0.10918)
(2860.00000, 0.09766)
(2870.00000, 0.10230)
(2880.00000, 0.08293)
(2890.00000, 0.10158)
(2900.00000, 0.09158)
(2910.00000, 0.09860)
(2920.00000, 0.12009)
(2930.00000, 0.08122)
(2940.00000, 0.10243)
(2950.00000, 0.10224)
(2960.00000, 0.10423)
(2970.00000, 0.11009)
(2980.00000, 0.08738)
(2990.00000, 0.09045)
(3000.00000, 0.08324)
(3010.00000, 0.08992)
(3020.00000, 0.06273)
(3030.00000, 0.08742)
(3040.00000, 0.09295)
(3050.00000, 0.08460)
(3060.00000, 0.08508)
(3070.00000, 0.08468)
(3080.00000, 0.08399)
(3090.00000, 0.08614)
(3100.00000, 0.08536)
(3110.00000, 0.08809)
(3120.00000, 0.08887)
(3130.00000, 0.09731)
(3140.00000, 0.09048)
(3150.00000, 0.09376)
(3160.00000, 0.08973)
(3170.00000, 0.06935)
(3180.00000, 0.09113)
(3190.00000, 0.08831)
(3200.00000, 0.08606)
(3210.00000, 0.08099)
(3220.00000, 0.08737)
(3230.00000, 0.09733)
(3240.00000, 0.09139)
(3250.00000, 0.08022)
(3260.00000, 0.07779)
(3270.00000, 0.08953)
(3280.00000, 0.10577)
(3290.00000, 0.07587)
(3300.00000, 0.07804)
(3310.00000, 0.09017)
(3320.00000, 0.08473)
(3330.00000, 0.10957)
(3340.00000, 0.09592)
(3350.00000, 0.08137)
(3360.00000, 0.10118)
(3370.00000, 0.08909)
(3380.00000, 0.08675)
(3390.00000, 0.07542)
(3400.00000, 0.08051)
(3410.00000, 0.08374)
(3420.00000, 0.07417)
(3430.00000, 0.07891)
(3440.00000, 0.08780)
(3450.00000, 0.09543)
(3460.00000, 0.09673)
(3470.00000, 0.06779)
(3480.00000, 0.09625)
(3490.00000, 0.08456)
(3500.00000, 0.09692)
(3510.00000, 0.08634)
(3520.00000, 0.09251)
(3530.00000, 0.07999)
(3540.00000, 0.08413)
(3550.00000, 0.07824)
(3560.00000, 0.09597)
(3570.00000, 0.09690)
(3580.00000, 0.08536)
(3590.00000, 0.10562)
(3600.00000, 0.10104)
(3610.00000, 0.09336)
(3620.00000, 0.08930)
(3630.00000, 0.08782)
(3640.00000, 0.08253)
(3650.00000, 0.09772)
(3660.00000, 0.10401)
(3670.00000, 0.09727)
(3680.00000, 0.09256)
(3690.00000, 0.09046)
(3700.00000, 0.09438)
(3710.00000, 0.08785)
(3720.00000, 0.08092)
(3730.00000, 0.10601)
(3740.00000, 0.09223)
(3750.00000, 0.06287)
(3760.00000, 0.07710)
(3770.00000, 0.10406)
(3780.00000, 0.08140)
(3790.00000, 0.10308)
(3800.00000, 0.10743)
(3810.00000, 0.09338)
(3820.00000, 0.10729)
(3830.00000, 0.08443)
(3840.00000, 0.08810)
(3850.00000, 0.10670)
(3860.00000, 0.09082)
(3870.00000, 0.10578)
(3880.00000, 0.10057)
(3890.00000, 0.09561)
(3900.00000, 0.09959)
(3910.00000, 0.10270)
(3920.00000, 0.09420)
(3930.00000, 0.10325)
(3940.00000, 0.09602)
(3950.00000, 0.09918)
(3960.00000, 0.10632)
(3970.00000, 0.11341)
(3980.00000, 0.10440)
(3990.00000, 0.09082)
(4000.00000, 0.10542)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,Yellow3] plot coordinates {
(100.00000, 0.31171)
(110.00000, 0.29753)
(120.00000, 0.25759)
(130.00000, 0.29028)
(140.00000, 0.27011)
(150.00000, 0.23053)
(160.00000, 0.18667)
(170.00000, 0.21784)
(180.00000, 0.23242)
(190.00000, 0.18902)
(200.00000, 0.20530)
(210.00000, 0.19137)
(220.00000, 0.19857)
(230.00000, 0.17085)
(240.00000, 0.20149)
(250.00000, 0.16919)
(260.00000, 0.18032)
(270.00000, 0.17878)
(280.00000, 0.18190)
(290.00000, 0.15294)
(300.00000, 0.16829)
(310.00000, 0.13770)
(320.00000, 0.14464)
(330.00000, 0.14390)
(340.00000, 0.16293)
(350.00000, 0.12642)
(360.00000, 0.12632)
(370.00000, 0.14149)
(380.00000, 0.15740)
(390.00000, 0.17348)
(400.00000, 0.13187)
(410.00000, 0.13689)
(420.00000, 0.15099)
(430.00000, 0.15081)
(440.00000, 0.09702)
(450.00000, 0.12822)
(460.00000, 0.12789)
(470.00000, 0.13411)
(480.00000, 0.15216)
(490.00000, 0.11648)
(500.00000, 0.11799)
(510.00000, 0.11377)
(520.00000, 0.12346)
(530.00000, 0.08807)
(540.00000, 0.10557)
(550.00000, 0.10275)
(560.00000, 0.11383)
(570.00000, 0.09736)
(580.00000, 0.10136)
(590.00000, 0.10481)
(600.00000, 0.11294)
(610.00000, 0.11654)
(620.00000, 0.10375)
(630.00000, 0.10777)
(640.00000, 0.08946)
(650.00000, 0.10982)
(660.00000, 0.10302)
(670.00000, 0.11427)
(680.00000, 0.08173)
(690.00000, 0.11935)
(700.00000, 0.09779)
(710.00000, 0.07983)
(720.00000, 0.10539)
(730.00000, 0.10783)
(740.00000, 0.07932)
(750.00000, 0.08487)
(760.00000, 0.08336)
(770.00000, 0.08523)
(780.00000, 0.09998)
(790.00000, 0.08594)
(800.00000, 0.08486)
(810.00000, 0.09033)
(820.00000, 0.09826)
(830.00000, 0.10260)
(840.00000, 0.07277)
(850.00000, 0.07928)
(860.00000, 0.07724)
(870.00000, 0.08952)
(880.00000, 0.08208)
(890.00000, 0.07909)
(900.00000, 0.08871)
(910.00000, 0.08611)
(920.00000, 0.08131)
(930.00000, 0.08308)
(940.00000, 0.07877)
(950.00000, 0.08666)
(960.00000, 0.08126)
(970.00000, 0.08320)
(980.00000, 0.07416)
(990.00000, 0.06943)
(1000.00000, 0.08234)
(1010.00000, 0.09094)
(1020.00000, 0.07196)
(1030.00000, 0.08463)
(1040.00000, 0.07664)
(1050.00000, 0.07574)
(1060.00000, 0.07810)
(1070.00000, 0.07916)
(1080.00000, 0.07746)
(1090.00000, 0.06855)
(1100.00000, 0.06432)
(1110.00000, 0.06863)
(1120.00000, 0.08799)
(1130.00000, 0.06129)
(1140.00000, 0.06660)
(1150.00000, 0.07530)
(1160.00000, 0.08230)
(1170.00000, 0.06984)
(1180.00000, 0.07878)
(1190.00000, 0.08513)
(1200.00000, 0.07435)
(1210.00000, 0.07511)
(1220.00000, 0.07845)
(1230.00000, 0.08243)
(1240.00000, 0.07639)
(1250.00000, 0.07808)
(1260.00000, 0.07398)
(1270.00000, 0.08331)
(1280.00000, 0.06909)
(1290.00000, 0.07074)
(1300.00000, 0.07385)
(1310.00000, 0.06524)
(1320.00000, 0.06959)
(1330.00000, 0.07984)
(1340.00000, 0.07188)
(1350.00000, 0.07176)
(1360.00000, 0.07029)
(1370.00000, 0.06549)
(1380.00000, 0.07523)
(1390.00000, 0.06864)
(1400.00000, 0.07582)
(1410.00000, 0.06864)
(1420.00000, 0.06829)
(1430.00000, 0.07294)
(1440.00000, 0.06742)
(1450.00000, 0.06398)
(1460.00000, 0.06577)
(1470.00000, 0.06334)
(1480.00000, 0.05664)
(1490.00000, 0.06343)
(1500.00000, 0.07026)
(1510.00000, 0.06556)
(1520.00000, 0.05627)
(1530.00000, 0.06026)
(1540.00000, 0.07428)
(1550.00000, 0.07151)
(1560.00000, 0.07169)
(1570.00000, 0.07622)
(1580.00000, 0.06200)
(1590.00000, 0.06473)
(1600.00000, 0.07450)
(1610.00000, 0.06925)
(1620.00000, 0.06846)
(1630.00000, 0.07000)
(1640.00000, 0.06896)
(1650.00000, 0.08288)
(1660.00000, 0.07436)
(1670.00000, 0.07428)
(1680.00000, 0.07254)
(1690.00000, 0.08130)
(1700.00000, 0.06824)
(1710.00000, 0.07268)
(1720.00000, 0.06726)
(1730.00000, 0.06307)
(1740.00000, 0.06926)
(1750.00000, 0.06305)
(1760.00000, 0.06878)
(1770.00000, 0.08283)
(1780.00000, 0.07769)
(1790.00000, 0.07073)
(1800.00000, 0.06769)
(1810.00000, 0.06662)
(1820.00000, 0.07678)
(1830.00000, 0.06990)
(1840.00000, 0.08089)
(1850.00000, 0.07229)
(1860.00000, 0.07067)
(1870.00000, 0.07669)
(1880.00000, 0.06930)
(1890.00000, 0.08175)
(1900.00000, 0.07623)
(1910.00000, 0.06991)
(1920.00000, 0.07328)
(1930.00000, 0.07105)
(1940.00000, 0.06174)
(1950.00000, 0.07003)
(1960.00000, 0.07578)
(1970.00000, 0.07214)
(1980.00000, 0.06738)
(1990.00000, 0.07778)
(2000.00000, 0.07220)
(2010.00000, 0.07457)
(2020.00000, 0.06338)
(2030.00000, 0.07348)
(2040.00000, 0.08512)
(2050.00000, 0.07700)
(2060.00000, 0.08466)
(2070.00000, 0.07120)
(2080.00000, 0.07438)
(2090.00000, 0.07966)
(2100.00000, 0.07156)
(2110.00000, 0.07094)
(2120.00000, 0.05914)
(2130.00000, 0.07214)
(2140.00000, 0.07460)
(2150.00000, 0.07752)
(2160.00000, 0.08833)
(2170.00000, 0.08390)
(2180.00000, 0.08530)
(2190.00000, 0.08296)
(2200.00000, 0.08139)
(2210.00000, 0.07197)
(2220.00000, 0.08852)
(2230.00000, 0.09798)
(2240.00000, 0.09433)
(2250.00000, 0.09040)
(2260.00000, 0.07935)
(2270.00000, 0.08712)
(2280.00000, 0.08982)
(2290.00000, 0.08055)
(2300.00000, 0.08658)
(2310.00000, 0.07924)
(2320.00000, 0.08318)
(2330.00000, 0.09562)
(2340.00000, 0.08217)
(2350.00000, 0.08760)
(2360.00000, 0.09099)
(2370.00000, 0.09295)
(2380.00000, 0.08507)
(2390.00000, 0.08089)
(2400.00000, 0.07718)
(2410.00000, 0.08858)
(2420.00000, 0.10325)
(2430.00000, 0.07627)
(2440.00000, 0.08387)
(2450.00000, 0.08645)
(2460.00000, 0.09102)
(2470.00000, 0.09053)
(2480.00000, 0.08417)
(2490.00000, 0.09143)
(2500.00000, 0.08225)
(2510.00000, 0.09174)
(2520.00000, 0.08889)
(2530.00000, 0.09284)
(2540.00000, 0.09283)
(2550.00000, 0.08503)
(2560.00000, 0.08271)
(2570.00000, 0.09515)
(2580.00000, 0.07736)
(2590.00000, 0.08617)
(2600.00000, 0.08402)
(2610.00000, 0.07322)
(2620.00000, 0.09169)
(2630.00000, 0.07877)
(2640.00000, 0.08374)
(2650.00000, 0.08308)
(2660.00000, 0.09338)
(2670.00000, 0.07673)
(2680.00000, 0.09719)
(2690.00000, 0.09745)
(2700.00000, 0.09536)
(2710.00000, 0.09041)
(2720.00000, 0.10106)
(2730.00000, 0.10157)
(2740.00000, 0.08280)
(2750.00000, 0.08948)
(2760.00000, 0.09013)
(2770.00000, 0.10110)
(2780.00000, 0.09089)
(2790.00000, 0.08812)
(2800.00000, 0.08808)
(2810.00000, 0.08685)
(2820.00000, 0.10006)
(2830.00000, 0.07908)
(2840.00000, 0.07717)
(2850.00000, 0.08412)
(2860.00000, 0.08722)
(2870.00000, 0.08621)
(2880.00000, 0.07996)
(2890.00000, 0.08763)
(2900.00000, 0.08795)
(2910.00000, 0.08048)
(2920.00000, 0.08294)
(2930.00000, 0.08486)
(2940.00000, 0.08184)
(2950.00000, 0.08920)
(2960.00000, 0.08470)
(2970.00000, 0.08314)
(2980.00000, 0.08584)
(2990.00000, 0.08207)
(3000.00000, 0.07353)
(3010.00000, 0.07897)
(3020.00000, 0.08215)
(3030.00000, 0.08317)
(3040.00000, 0.09176)
(3050.00000, 0.09235)
(3060.00000, 0.09191)
(3070.00000, 0.06989)
(3080.00000, 0.08128)
(3090.00000, 0.08713)
(3100.00000, 0.07516)
(3110.00000, 0.07413)
(3120.00000, 0.08308)
(3130.00000, 0.08058)
(3140.00000, 0.08195)
(3150.00000, 0.07724)
(3160.00000, 0.07297)
(3170.00000, 0.07557)
(3180.00000, 0.08285)
(3190.00000, 0.06768)
(3200.00000, 0.07389)
(3210.00000, 0.07531)
(3220.00000, 0.08626)
(3230.00000, 0.07355)
(3240.00000, 0.07864)
(3250.00000, 0.08084)
(3260.00000, 0.08090)
(3270.00000, 0.07738)
(3280.00000, 0.07225)
(3290.00000, 0.09407)
(3300.00000, 0.07712)
(3310.00000, 0.08195)
(3320.00000, 0.07225)
(3330.00000, 0.07378)
(3340.00000, 0.07113)
(3350.00000, 0.08640)
(3360.00000, 0.06951)
(3370.00000, 0.06782)
(3380.00000, 0.08052)
(3390.00000, 0.07305)
(3400.00000, 0.07465)
(3410.00000, 0.07315)
(3420.00000, 0.07950)
(3430.00000, 0.07792)
(3440.00000, 0.07507)
(3450.00000, 0.07584)
(3460.00000, 0.06771)
(3470.00000, 0.07042)
(3480.00000, 0.07170)
(3490.00000, 0.07396)
(3500.00000, 0.07749)
(3510.00000, 0.07773)
(3520.00000, 0.07057)
(3530.00000, 0.06654)
(3540.00000, 0.07297)
(3550.00000, 0.07380)
(3560.00000, 0.07260)
(3570.00000, 0.07143)
(3580.00000, 0.07637)
(3590.00000, 0.07147)
(3600.00000, 0.06620)
(3610.00000, 0.07378)
(3620.00000, 0.06845)
(3630.00000, 0.07784)
(3640.00000, 0.06921)
(3650.00000, 0.07551)
(3660.00000, 0.07171)
(3670.00000, 0.06642)
(3680.00000, 0.07072)
(3690.00000, 0.06753)
(3700.00000, 0.06715)
(3710.00000, 0.06337)
(3720.00000, 0.06627)
(3730.00000, 0.06724)
(3740.00000, 0.06876)
(3750.00000, 0.07489)
(3760.00000, 0.05926)
(3770.00000, 0.07515)
(3780.00000, 0.07230)
(3790.00000, 0.06095)
(3800.00000, 0.07167)
(3810.00000, 0.06489)
(3820.00000, 0.07233)
(3830.00000, 0.07565)
(3840.00000, 0.06692)
(3850.00000, 0.06097)
(3860.00000, 0.07793)
(3870.00000, 0.07576)
(3880.00000, 0.06799)
(3890.00000, 0.06507)
(3900.00000, 0.06446)
(3910.00000, 0.06794)
(3920.00000, 0.06664)
(3930.00000, 0.06953)
(3940.00000, 0.06772)
(3950.00000, 0.07723)
(3960.00000, 0.07083)
(3970.00000, 0.07349)
(3980.00000, 0.06486)
(3990.00000, 0.07093)
(4000.00000, 0.07487)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,IndianRed2] plot coordinates {
(100.00000, 1.83952)
(110.00000, 0.85950)
(120.00000, 0.38117)
(130.00000, 0.28277)
(140.00000, 0.26958)
(150.00000, 0.30398)
(160.00000, 0.23611)
(170.00000, 0.27987)
(180.00000, 0.23362)
(190.00000, 0.63116)
(200.00000, 0.27685)
(210.00000, 0.25146)
(220.00000, 0.25326)
(230.00000, 0.25429)
(240.00000, 0.24798)
(250.00000, 0.25466)
(260.00000, 0.25638)
(270.00000, 0.25579)
(280.00000, 0.28360)
(290.00000, 0.27219)
(300.00000, 0.19699)
(310.00000, 0.28148)
(320.00000, 0.18901)
(330.00000, 0.26763)
(340.00000, 0.23023)
(350.00000, 0.21163)
(360.00000, 0.19928)
(370.00000, 0.26154)
(380.00000, 0.18373)
(390.00000, 0.20279)
(400.00000, 0.22402)
(410.00000, 0.18522)
(420.00000, 0.19839)
(430.00000, 0.25737)
(440.00000, 0.19565)
(450.00000, 0.19271)
(460.00000, 0.21222)
(470.00000, 0.20890)
(480.00000, 0.20556)
(490.00000, 0.18389)
(500.00000, 0.19480)
(510.00000, 0.15852)
(520.00000, 0.21268)
(530.00000, 0.19186)
(540.00000, 0.18321)
(550.00000, 0.21717)
(560.00000, 0.20290)
(570.00000, 0.21220)
(580.00000, 0.20356)
(590.00000, 0.19201)
(600.00000, 0.21977)
(610.00000, 0.22379)
(620.00000, 0.16153)
(630.00000, 0.15769)
(640.00000, 0.18058)
(650.00000, 0.16200)
(660.00000, 0.18427)
(670.00000, 0.15852)
(680.00000, 0.14586)
(690.00000, 0.12859)
(700.00000, 0.17919)
(710.00000, 0.14067)
(720.00000, 0.18427)
(730.00000, 0.16988)
(740.00000, 0.17157)
(750.00000, 0.13742)
(760.00000, 0.15773)
(770.00000, 0.17533)
(780.00000, 0.12857)
(790.00000, 0.15745)
(800.00000, 0.15909)
(810.00000, 0.14781)
(820.00000, 0.16284)
(830.00000, 0.17511)
(840.00000, 0.17628)
(850.00000, 0.19209)
(860.00000, 0.17154)
(870.00000, 0.17662)
(880.00000, 0.22630)
(890.00000, 0.21238)
(900.00000, 0.20012)
(910.00000, 0.21850)
(920.00000, 0.24747)
(930.00000, 0.25860)
(940.00000, 0.23170)
(950.00000, 0.24634)
(960.00000, 0.25669)
(970.00000, 0.25739)
(980.00000, 0.20755)
(990.00000, 0.23046)
(1000.00000, 0.25103)
(1010.00000, 0.27581)
(1020.00000, 0.27389)
(1030.00000, 0.23355)
(1040.00000, 0.27879)
(1050.00000, 0.27095)
(1060.00000, 0.26362)
(1070.00000, 0.30072)
(1080.00000, 0.27353)
(1090.00000, 0.27880)
(1100.00000, 0.28478)
(1110.00000, 0.27117)
(1120.00000, 0.27834)
(1130.00000, 0.27279)
(1140.00000, 0.27719)
(1150.00000, 0.25099)
(1160.00000, 0.24748)
(1170.00000, 0.24396)
(1180.00000, 0.23312)
(1190.00000, 0.20030)
(1200.00000, 0.25129)
(1210.00000, 0.21685)
(1220.00000, 0.21128)
(1230.00000, 0.21501)
(1240.00000, 0.22511)
(1250.00000, 0.22397)
(1260.00000, 0.19653)
(1270.00000, 0.20049)
(1280.00000, 0.19283)
(1290.00000, 0.21327)
(1300.00000, 0.20081)
(1310.00000, 0.19261)
(1320.00000, 0.18793)
(1330.00000, 0.20235)
(1340.00000, 0.17345)
(1350.00000, 0.17402)
(1360.00000, 0.20347)
(1370.00000, 0.17990)
(1380.00000, 0.18606)
(1390.00000, 0.17041)
(1400.00000, 0.16172)
(1410.00000, 0.16034)
(1420.00000, 0.16650)
(1430.00000, 0.16586)
(1440.00000, 0.16799)
(1450.00000, 0.16861)
(1460.00000, 0.15209)
(1470.00000, 0.16686)
(1480.00000, 0.17317)
(1490.00000, 0.16881)
(1500.00000, 0.15691)
(1510.00000, 0.16424)
(1520.00000, 0.17169)
(1530.00000, 0.16007)
(1540.00000, 0.18924)
(1550.00000, 0.16879)
(1560.00000, 0.16595)
(1570.00000, 0.17518)
(1580.00000, 0.18052)
(1590.00000, 0.13678)
(1600.00000, 0.15676)
(1610.00000, 0.15293)
(1620.00000, 0.17189)
(1630.00000, 0.17063)
(1640.00000, 0.16923)
(1650.00000, 0.17822)
(1660.00000, 0.17079)
(1670.00000, 0.15496)
(1680.00000, 0.15553)
(1690.00000, 0.15507)
(1700.00000, 0.14741)
(1710.00000, 0.16256)
(1720.00000, 0.15205)
(1730.00000, 0.17760)
(1740.00000, 0.14931)
(1750.00000, 0.15769)
(1760.00000, 0.13770)
(1770.00000, 0.14034)
(1780.00000, 0.13416)
(1790.00000, 0.15717)
(1800.00000, 0.15735)
(1810.00000, 0.15428)
(1820.00000, 0.14614)
(1830.00000, 0.12598)
(1840.00000, 0.13883)
(1850.00000, 0.12128)
(1860.00000, 0.13234)
(1870.00000, 0.13295)
(1880.00000, 0.12677)
(1890.00000, 0.13262)
(1900.00000, 0.14460)
(1910.00000, 0.13547)
(1920.00000, 0.14138)
(1930.00000, 0.12996)
(1940.00000, 0.12837)
(1950.00000, 0.12634)
(1960.00000, 0.13660)
(1970.00000, 0.13530)
(1980.00000, 0.13412)
(1990.00000, 0.11747)
(2000.00000, 0.11417)
(2010.00000, 0.11672)
(2020.00000, 0.11264)
(2030.00000, 0.11436)
(2040.00000, 0.11478)
(2050.00000, 0.09844)
(2060.00000, 0.11173)
(2070.00000, 0.11365)
(2080.00000, 0.11314)
(2090.00000, 0.10711)
(2100.00000, 0.09186)
(2110.00000, 0.13311)
(2120.00000, 0.10476)
(2130.00000, 0.10989)
(2140.00000, 0.09210)
(2150.00000, 0.11148)
(2160.00000, 0.10828)
(2170.00000, 0.09625)
(2180.00000, 0.09349)
(2190.00000, 0.10975)
(2200.00000, 0.10707)
(2210.00000, 0.10085)
(2220.00000, 0.11544)
(2230.00000, 0.10724)
(2240.00000, 0.10737)
(2250.00000, 0.10160)
(2260.00000, 0.11869)
(2270.00000, 0.10689)
(2280.00000, 0.11439)
(2290.00000, 0.13060)
(2300.00000, 0.08902)
(2310.00000, 0.10049)
(2320.00000, 0.10938)
(2330.00000, 0.09309)
(2340.00000, 0.08721)
(2350.00000, 0.10004)
(2360.00000, 0.11409)
(2370.00000, 0.11351)
(2380.00000, 0.09622)
(2390.00000, 0.10155)
(2400.00000, 0.10012)
(2410.00000, 0.09354)
(2420.00000, 0.08825)
(2430.00000, 0.09530)
(2440.00000, 0.10667)
(2450.00000, 0.09158)
(2460.00000, 0.10965)
(2470.00000, 0.08097)
(2480.00000, 0.10631)
(2490.00000, 0.09674)
(2500.00000, 0.09312)
(2510.00000, 0.10348)
(2520.00000, 0.09539)
(2530.00000, 0.08444)
(2540.00000, 0.09361)
(2550.00000, 0.08106)
(2560.00000, 0.09056)
(2570.00000, 0.09610)
(2580.00000, 0.11044)
(2590.00000, 0.09777)
(2600.00000, 0.10152)
(2610.00000, 0.09142)
(2620.00000, 0.09822)
(2630.00000, 0.09428)
(2640.00000, 0.08565)
(2650.00000, 0.08190)
(2660.00000, 0.10424)
(2670.00000, 0.09694)
(2680.00000, 0.08802)
(2690.00000, 0.11417)
(2700.00000, 0.08033)
(2710.00000, 0.10259)
(2720.00000, 0.09839)
(2730.00000, 0.10531)
(2740.00000, 0.10080)
(2750.00000, 0.08414)
(2760.00000, 0.09400)
(2770.00000, 0.08277)
(2780.00000, 0.08380)
(2790.00000, 0.08033)
(2800.00000, 0.08991)
(2810.00000, 0.08886)
(2820.00000, 0.07232)
(2830.00000, 0.08228)
(2840.00000, 0.09137)
(2850.00000, 0.08622)
(2860.00000, 0.08261)
(2870.00000, 0.09670)
(2880.00000, 0.07921)
(2890.00000, 0.09501)
(2900.00000, 0.09448)
(2910.00000, 0.07570)
(2920.00000, 0.09424)
(2930.00000, 0.07065)
(2940.00000, 0.07861)
(2950.00000, 0.08210)
(2960.00000, 0.06898)
(2970.00000, 0.07132)
(2980.00000, 0.09488)
(2990.00000, 0.07882)
(3000.00000, 0.07948)
(3010.00000, 0.07357)
(3020.00000, 0.08104)
(3030.00000, 0.07916)
(3040.00000, 0.09490)
(3050.00000, 0.07569)
(3060.00000, 0.08153)
(3070.00000, 0.07456)
(3080.00000, 0.06830)
(3090.00000, 0.08824)
(3100.00000, 0.07735)
(3110.00000, 0.09437)
(3120.00000, 0.06715)
(3130.00000, 0.07903)
(3140.00000, 0.08048)
(3150.00000, 0.07557)
(3160.00000, 0.08415)
(3170.00000, 0.07420)
(3180.00000, 0.06656)
(3190.00000, 0.07113)
(3200.00000, 0.08010)
(3210.00000, 0.07903)
(3220.00000, 0.07579)
(3230.00000, 0.09282)
(3240.00000, 0.07386)
(3250.00000, 0.07456)
(3260.00000, 0.08014)
(3270.00000, 0.07125)
(3280.00000, 0.07099)
(3290.00000, 0.07127)
(3300.00000, 0.06838)
(3310.00000, 0.07713)
(3320.00000, 0.06078)
(3330.00000, 0.07775)
(3340.00000, 0.06476)
(3350.00000, 0.06473)
(3360.00000, 0.07199)
(3370.00000, 0.06089)
(3380.00000, 0.06804)
(3390.00000, 0.06511)
(3400.00000, 0.06110)
(3410.00000, 0.07595)
(3420.00000, 0.07601)
(3430.00000, 0.06856)
(3440.00000, 0.07810)
(3450.00000, 0.07146)
(3460.00000, 0.07241)
(3470.00000, 0.07662)
(3480.00000, 0.07688)
(3490.00000, 0.06897)
(3500.00000, 0.06201)
(3510.00000, 0.07132)
(3520.00000, 0.07521)
(3530.00000, 0.06884)
(3540.00000, 0.07152)
(3550.00000, 0.06869)
(3560.00000, 0.06274)
(3570.00000, 0.06666)
(3580.00000, 0.06332)
(3590.00000, 0.07872)
(3600.00000, 0.07823)
(3610.00000, 0.07308)
(3620.00000, 0.06752)
(3630.00000, 0.06147)
(3640.00000, 0.06558)
(3650.00000, 0.06955)
(3660.00000, 0.06481)
(3670.00000, 0.06375)
(3680.00000, 0.06874)
(3690.00000, 0.06523)
(3700.00000, 0.06349)
(3710.00000, 0.06894)
(3720.00000, 0.06615)
(3730.00000, 0.06959)
(3740.00000, 0.06118)
(3750.00000, 0.05900)
(3760.00000, 0.05618)
(3770.00000, 0.06354)
(3780.00000, 0.05929)
(3790.00000, 0.05944)
(3800.00000, 0.05908)
(3810.00000, 0.05278)
(3820.00000, 0.05733)
(3830.00000, 0.05471)
(3840.00000, 0.06478)
(3850.00000, 0.06272)
(3860.00000, 0.06683)
(3870.00000, 0.06488)
(3880.00000, 0.05665)
(3890.00000, 0.07021)
(3900.00000, 0.05796)
(3910.00000, 0.06044)
(3920.00000, 0.04950)
(3930.00000, 0.06369)
(3940.00000, 0.05863)
(3950.00000, 0.06205)
(3960.00000, 0.05572)
(3970.00000, 0.06085)
(3980.00000, 0.06414)
(3990.00000, 0.05623)
(4000.00000, 0.07349)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,gray] plot coordinates {
(100.00000, 1.55590)
(110.00000, 0.52752)
(120.00000, 0.59973)
(130.00000, 0.49296)
(140.00000, 0.38953)
(150.00000, 0.39505)
(160.00000, 0.35297)
(170.00000, 0.29886)
(180.00000, 0.29576)
(190.00000, 0.60458)
(200.00000, 0.25653)
(210.00000, 0.22853)
(220.00000, 0.25100)
(230.00000, 0.25817)
(240.00000, 0.23674)
(250.00000, 0.28174)
(260.00000, 0.28638)
(270.00000, 0.30444)
(280.00000, 0.19233)
(290.00000, 0.25830)
(300.00000, 0.24727)
(310.00000, 0.22726)
(320.00000, 0.21600)
(330.00000, 0.22909)
(340.00000, 0.20218)
(350.00000, 0.20193)
(360.00000, 0.21781)
(370.00000, 0.20906)
(380.00000, 0.20821)
(390.00000, 0.20784)
(400.00000, 0.22106)
(410.00000, 0.23429)
(420.00000, 0.21464)
(430.00000, 0.22073)
(440.00000, 0.21802)
(450.00000, 0.22634)
(460.00000, 0.22852)
(470.00000, 0.21805)
(480.00000, 0.20279)
(490.00000, 0.20579)
(500.00000, 0.22261)
(510.00000, 0.21443)
(520.00000, 0.24224)
(530.00000, 0.20293)
(540.00000, 0.20193)
(550.00000, 0.25101)
(560.00000, 0.23577)
(570.00000, 0.25158)
(580.00000, 0.24977)
(590.00000, 0.25410)
(600.00000, 0.28784)
(610.00000, 0.26960)
(620.00000, 0.28996)
(630.00000, 0.27818)
(640.00000, 0.25683)
(650.00000, 0.25646)
(660.00000, 0.27151)
(670.00000, 0.29301)
(680.00000, 0.27895)
(690.00000, 0.28660)
(700.00000, 0.27624)
(710.00000, 0.27460)
(720.00000, 0.26140)
(730.00000, 0.25669)
(740.00000, 0.26826)
(750.00000, 0.28798)
(760.00000, 0.28119)
(770.00000, 0.29009)
(780.00000, 0.29080)
(790.00000, 0.22148)
(800.00000, 0.21964)
(810.00000, 0.24585)
(820.00000, 0.23802)
(830.00000, 0.21614)
(840.00000, 0.19490)
(850.00000, 0.21155)
(860.00000, 0.19392)
(870.00000, 0.17026)
(880.00000, 0.17105)
(890.00000, 0.17038)
(900.00000, 0.14863)
(910.00000, 0.12896)
(920.00000, 0.12664)
(930.00000, 0.10244)
(940.00000, 0.12608)
(950.00000, 0.10896)
(960.00000, 0.12210)
(970.00000, 0.10031)
(980.00000, 0.12321)
(990.00000, 0.12895)
(1000.00000, 0.14402)
(1010.00000, 0.11850)
(1020.00000, 0.11979)
(1030.00000, 0.11190)
(1040.00000, 0.10047)
(1050.00000, 0.12548)
(1060.00000, 0.11248)
(1070.00000, 0.13235)
(1080.00000, 0.13889)
(1090.00000, 0.13452)
(1100.00000, 0.14208)
(1110.00000, 0.13333)
(1120.00000, 0.16984)
(1130.00000, 0.14599)
(1140.00000, 0.13114)
(1150.00000, 0.12502)
(1160.00000, 0.12492)
(1170.00000, 0.15613)
(1180.00000, 0.16656)
(1190.00000, 0.14744)
(1200.00000, 0.16774)
(1210.00000, 0.16005)
(1220.00000, 0.16983)
(1230.00000, 0.19192)
(1240.00000, 0.18503)
(1250.00000, 0.17744)
(1260.00000, 0.16908)
(1270.00000, 0.18864)
(1280.00000, 0.17223)
(1290.00000, 0.19802)
(1300.00000, 0.18919)
(1310.00000, 0.16469)
(1320.00000, 0.17387)
(1330.00000, 0.18342)
(1340.00000, 0.17457)
(1350.00000, 0.17771)
(1360.00000, 0.17627)
(1370.00000, 0.16964)
(1380.00000, 0.17027)
(1390.00000, 0.16144)
(1400.00000, 0.17545)
(1410.00000, 0.17489)
(1420.00000, 0.17204)
(1430.00000, 0.17499)
(1440.00000, 0.18714)
(1450.00000, 0.16911)
(1460.00000, 0.19332)
(1470.00000, 0.18354)
(1480.00000, 0.18980)
(1490.00000, 0.19291)
(1500.00000, 0.18837)
(1510.00000, 0.17977)
(1520.00000, 0.18767)
(1530.00000, 0.19647)
(1540.00000, 0.16834)
(1550.00000, 0.16222)
(1560.00000, 0.18500)
(1570.00000, 0.18246)
(1580.00000, 0.17845)
(1590.00000, 0.17023)
(1600.00000, 0.16273)
(1610.00000, 0.18019)
(1620.00000, 0.18036)
(1630.00000, 0.17203)
(1640.00000, 0.17712)
(1650.00000, 0.17944)
(1660.00000, 0.17247)
(1670.00000, 0.16562)
(1680.00000, 0.18371)
(1690.00000, 0.17833)
(1700.00000, 0.16992)
(1710.00000, 0.15381)
(1720.00000, 0.16651)
(1730.00000, 0.18186)
(1740.00000, 0.13488)
(1750.00000, 0.17126)
(1760.00000, 0.15250)
(1770.00000, 0.15063)
(1780.00000, 0.14302)
(1790.00000, 0.14324)
(1800.00000, 0.16105)
(1810.00000, 0.15568)
(1820.00000, 0.15282)
(1830.00000, 0.13923)
(1840.00000, 0.15967)
(1850.00000, 0.14992)
(1860.00000, 0.14535)
(1870.00000, 0.14200)
(1880.00000, 0.12794)
(1890.00000, 0.12683)
(1900.00000, 0.12870)
(1910.00000, 0.12867)
(1920.00000, 0.14430)
(1930.00000, 0.12395)
(1940.00000, 0.13480)
(1950.00000, 0.13899)
(1960.00000, 0.12501)
(1970.00000, 0.10710)
(1980.00000, 0.09853)
(1990.00000, 0.11610)
(2000.00000, 0.12068)
(2010.00000, 0.11603)
(2020.00000, 0.09844)
(2030.00000, 0.11645)
(2040.00000, 0.12818)
(2050.00000, 0.11693)
(2060.00000, 0.09676)
(2070.00000, 0.09337)
(2080.00000, 0.11130)
(2090.00000, 0.10620)
(2100.00000, 0.08931)
(2110.00000, 0.10650)
(2120.00000, 0.10519)
(2130.00000, 0.09026)
(2140.00000, 0.10569)
(2150.00000, 0.10149)
(2160.00000, 0.09885)
(2170.00000, 0.10972)
(2180.00000, 0.09688)
(2190.00000, 0.10998)
(2200.00000, 0.10658)
(2210.00000, 0.09252)
(2220.00000, 0.09388)
(2230.00000, 0.11272)
(2240.00000, 0.10274)
(2250.00000, 0.10383)
(2260.00000, 0.10738)
(2270.00000, 0.11100)
(2280.00000, 0.10031)
(2290.00000, 0.12616)
(2300.00000, 0.11255)
(2310.00000, 0.11426)
(2320.00000, 0.10558)
(2330.00000, 0.10990)
(2340.00000, 0.12953)
(2350.00000, 0.11328)
(2360.00000, 0.11635)
(2370.00000, 0.11184)
(2380.00000, 0.11001)
(2390.00000, 0.11796)
(2400.00000, 0.09631)
(2410.00000, 0.11466)
(2420.00000, 0.11173)
(2430.00000, 0.12412)
(2440.00000, 0.09955)
(2450.00000, 0.10890)
(2460.00000, 0.12983)
(2470.00000, 0.11250)
(2480.00000, 0.12040)
(2490.00000, 0.11435)
(2500.00000, 0.12180)
(2510.00000, 0.10857)
(2520.00000, 0.11622)
(2530.00000, 0.11625)
(2540.00000, 0.10210)
(2550.00000, 0.11997)
(2560.00000, 0.11431)
(2570.00000, 0.12229)
(2580.00000, 0.10832)
(2590.00000, 0.11563)
(2600.00000, 0.08651)
(2610.00000, 0.10073)
(2620.00000, 0.10476)
(2630.00000, 0.09595)
(2640.00000, 0.10661)
(2650.00000, 0.10454)
(2660.00000, 0.12305)
(2670.00000, 0.10898)
(2680.00000, 0.09453)
(2690.00000, 0.10362)
(2700.00000, 0.11159)
(2710.00000, 0.10129)
(2720.00000, 0.10326)
(2730.00000, 0.10100)
(2740.00000, 0.08516)
(2750.00000, 0.10186)
(2760.00000, 0.09328)
(2770.00000, 0.09226)
(2780.00000, 0.09640)
(2790.00000, 0.09314)
(2800.00000, 0.08924)
(2810.00000, 0.10188)
(2820.00000, 0.10052)
(2830.00000, 0.09582)
(2840.00000, 0.09084)
(2850.00000, 0.10277)
(2860.00000, 0.08750)
(2870.00000, 0.07083)
(2880.00000, 0.07918)
(2890.00000, 0.07676)
(2900.00000, 0.07238)
(2910.00000, 0.07277)
(2920.00000, 0.08400)
(2930.00000, 0.08485)
(2940.00000, 0.07265)
(2950.00000, 0.08555)
(2960.00000, 0.08012)
(2970.00000, 0.06951)
(2980.00000, 0.08151)
(2990.00000, 0.06817)
(3000.00000, 0.08817)
(3010.00000, 0.09068)
(3020.00000, 0.07732)
(3030.00000, 0.07892)
(3040.00000, 0.07467)
(3050.00000, 0.07096)
(3060.00000, 0.07791)
(3070.00000, 0.07506)
(3080.00000, 0.08024)
(3090.00000, 0.07355)
(3100.00000, 0.07821)
(3110.00000, 0.07728)
(3120.00000, 0.06607)
(3130.00000, 0.08397)
(3140.00000, 0.07136)
(3150.00000, 0.09183)
(3160.00000, 0.07429)
(3170.00000, 0.07189)
(3180.00000, 0.08007)
(3190.00000, 0.08653)
(3200.00000, 0.07356)
(3210.00000, 0.07600)
(3220.00000, 0.08454)
(3230.00000, 0.06784)
(3240.00000, 0.09181)
(3250.00000, 0.07430)
(3260.00000, 0.08661)
(3270.00000, 0.08285)
(3280.00000, 0.08203)
(3290.00000, 0.07693)
(3300.00000, 0.08088)
(3310.00000, 0.08738)
(3320.00000, 0.06627)
(3330.00000, 0.07159)
(3340.00000, 0.08236)
(3350.00000, 0.07987)
(3360.00000, 0.07868)
(3370.00000, 0.07238)
(3380.00000, 0.07646)
(3390.00000, 0.07976)
(3400.00000, 0.07476)
(3410.00000, 0.08221)
(3420.00000, 0.08729)
(3430.00000, 0.08303)
(3440.00000, 0.09422)
(3450.00000, 0.08896)
(3460.00000, 0.08256)
(3470.00000, 0.08258)
(3480.00000, 0.07838)
(3490.00000, 0.08744)
(3500.00000, 0.07270)
(3510.00000, 0.07593)
(3520.00000, 0.07789)
(3530.00000, 0.09001)
(3540.00000, 0.07122)
(3550.00000, 0.08001)
(3560.00000, 0.07738)
(3570.00000, 0.07259)
(3580.00000, 0.07723)
(3590.00000, 0.07601)
(3600.00000, 0.07555)
(3610.00000, 0.07078)
(3620.00000, 0.05401)
(3630.00000, 0.08003)
(3640.00000, 0.07519)
(3650.00000, 0.07515)
(3660.00000, 0.07206)
(3670.00000, 0.07512)
(3680.00000, 0.07121)
(3690.00000, 0.07933)
(3700.00000, 0.07365)
(3710.00000, 0.08210)
(3720.00000, 0.07729)
(3730.00000, 0.07673)
(3740.00000, 0.08481)
(3750.00000, 0.07331)
(3760.00000, 0.07905)
(3770.00000, 0.07456)
(3780.00000, 0.07883)
(3790.00000, 0.06683)
(3800.00000, 0.08618)
(3810.00000, 0.08068)
(3820.00000, 0.07445)
(3830.00000, 0.08113)
(3840.00000, 0.06931)
(3850.00000, 0.07415)
(3860.00000, 0.07008)
(3870.00000, 0.06785)
(3880.00000, 0.08499)
(3890.00000, 0.08299)
(3900.00000, 0.06469)
(3910.00000, 0.08243)
(3920.00000, 0.08388)
(3930.00000, 0.07601)
(3940.00000, 0.08090)
(3950.00000, 0.07213)
(3960.00000, 0.07438)
(3970.00000, 0.07462)
(3980.00000, 0.07942)
(3990.00000, 0.08354)
(4000.00000, 0.07951)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,Cyan1] plot coordinates {
(100.00000, 0.56571)
(110.00000, 0.72941)
(120.00000, 0.33976)
(130.00000, 0.30888)
(140.00000, 0.36870)
(150.00000, 0.28646)
(160.00000, 0.25443)
(170.00000, 0.27941)
(180.00000, 0.28818)
(190.00000, 0.27184)
(200.00000, 0.28859)
(210.00000, 0.27044)
(220.00000, 0.33437)
(230.00000, 0.28264)
(240.00000, 0.22732)
(250.00000, 0.24650)
(260.00000, 0.21499)
(270.00000, 0.26219)
(280.00000, 0.26242)
(290.00000, 0.24382)
(300.00000, 0.23877)
(310.00000, 0.22778)
(320.00000, 0.19326)
(330.00000, 0.22168)
(340.00000, 0.21933)
(350.00000, 0.19330)
(360.00000, 0.22252)
(370.00000, 0.21439)
(380.00000, 0.21638)
(390.00000, 0.23045)
(400.00000, 0.22123)
(410.00000, 0.19367)
(420.00000, 0.20683)
(430.00000, 0.20782)
(440.00000, 0.21179)
(450.00000, 0.17706)
(460.00000, 0.16234)
(470.00000, 0.19933)
(480.00000, 0.22799)
(490.00000, 0.18983)
(500.00000, 0.20610)
(510.00000, 0.18167)
(520.00000, 0.19370)
(530.00000, 0.16723)
(540.00000, 0.17601)
(550.00000, 0.17155)
(560.00000, 0.15930)
(570.00000, 0.18633)
(580.00000, 0.18183)
(590.00000, 0.14561)
(600.00000, 0.16320)
(610.00000, 0.18024)
(620.00000, 0.15428)
(630.00000, 0.14104)
(640.00000, 0.14386)
(650.00000, 0.14427)
(660.00000, 0.15186)
(670.00000, 0.14296)
(680.00000, 0.16812)
(690.00000, 0.13699)
(700.00000, 0.16239)
(710.00000, 0.16575)
(720.00000, 0.16444)
(730.00000, 0.15848)
(740.00000, 0.18563)
(750.00000, 0.17149)
(760.00000, 0.20262)
(770.00000, 0.15313)
(780.00000, 0.14943)
(790.00000, 0.19009)
(800.00000, 0.18111)
(810.00000, 0.23656)
(820.00000, 0.19596)
(830.00000, 0.21485)
(840.00000, 0.23289)
(850.00000, 0.22800)
(860.00000, 0.24844)
(870.00000, 0.23446)
(880.00000, 0.26273)
(890.00000, 0.24824)
(900.00000, 0.29488)
(910.00000, 0.25107)
(920.00000, 0.25522)
(930.00000, 0.27671)
(940.00000, 0.26392)
(950.00000, 0.27619)
(960.00000, 0.27914)
(970.00000, 0.27503)
(980.00000, 0.23517)
(990.00000, 0.26817)
(1000.00000, 0.25978)
(1010.00000, 0.26783)
(1020.00000, 0.25539)
(1030.00000, 0.27257)
(1040.00000, 0.24662)
(1050.00000, 0.25214)
(1060.00000, 0.24016)
(1070.00000, 0.22545)
(1080.00000, 0.22592)
(1090.00000, 0.24699)
(1100.00000, 0.22867)
(1110.00000, 0.24026)
(1120.00000, 0.23651)
(1130.00000, 0.21248)
(1140.00000, 0.18068)
(1150.00000, 0.19929)
(1160.00000, 0.18994)
(1170.00000, 0.19229)
(1180.00000, 0.18931)
(1190.00000, 0.15879)
(1200.00000, 0.16697)
(1210.00000, 0.15815)
(1220.00000, 0.16113)
(1230.00000, 0.17891)
(1240.00000, 0.16166)
(1250.00000, 0.15199)
(1260.00000, 0.13286)
(1270.00000, 0.14457)
(1280.00000, 0.13386)
(1290.00000, 0.14232)
(1300.00000, 0.13563)
(1310.00000, 0.12320)
(1320.00000, 0.12202)
(1330.00000, 0.13267)
(1340.00000, 0.14575)
(1350.00000, 0.14128)
(1360.00000, 0.12997)
(1370.00000, 0.12497)
(1380.00000, 0.11408)
(1390.00000, 0.12490)
(1400.00000, 0.12886)
(1410.00000, 0.13608)
(1420.00000, 0.12698)
(1430.00000, 0.12040)
(1440.00000, 0.11962)
(1450.00000, 0.11759)
(1460.00000, 0.12182)
(1470.00000, 0.12192)
(1480.00000, 0.11891)
(1490.00000, 0.10825)
(1500.00000, 0.11377)
(1510.00000, 0.11424)
(1520.00000, 0.11458)
(1530.00000, 0.10908)
(1540.00000, 0.11356)
(1550.00000, 0.09381)
(1560.00000, 0.11660)
(1570.00000, 0.10797)
(1580.00000, 0.10890)
(1590.00000, 0.08985)
(1600.00000, 0.10063)
(1610.00000, 0.09745)
(1620.00000, 0.09566)
(1630.00000, 0.09688)
(1640.00000, 0.10049)
(1650.00000, 0.10919)
(1660.00000, 0.11641)
(1670.00000, 0.09464)
(1680.00000, 0.10437)
(1690.00000, 0.10644)
(1700.00000, 0.10799)
(1710.00000, 0.09545)
(1720.00000, 0.10376)
(1730.00000, 0.11326)
(1740.00000, 0.08987)
(1750.00000, 0.09645)
(1760.00000, 0.09686)
(1770.00000, 0.10141)
(1780.00000, 0.10862)
(1790.00000, 0.09042)
(1800.00000, 0.08410)
(1810.00000, 0.09356)
(1820.00000, 0.09490)
(1830.00000, 0.08768)
(1840.00000, 0.10060)
(1850.00000, 0.08431)
(1860.00000, 0.08507)
(1870.00000, 0.08383)
(1880.00000, 0.09197)
(1890.00000, 0.09657)
(1900.00000, 0.08844)
(1910.00000, 0.08376)
(1920.00000, 0.09874)
(1930.00000, 0.09733)
(1940.00000, 0.09097)
(1950.00000, 0.09194)
(1960.00000, 0.06954)
(1970.00000, 0.10006)
(1980.00000, 0.08880)
(1990.00000, 0.08397)
(2000.00000, 0.08786)
(2010.00000, 0.07404)
(2020.00000, 0.09861)
(2030.00000, 0.09526)
(2040.00000, 0.08404)
(2050.00000, 0.08272)
(2060.00000, 0.07309)
(2070.00000, 0.08613)
(2080.00000, 0.07876)
(2090.00000, 0.07904)
(2100.00000, 0.07782)
(2110.00000, 0.08958)
(2120.00000, 0.07922)
(2130.00000, 0.08940)
(2140.00000, 0.08629)
(2150.00000, 0.08597)
(2160.00000, 0.09207)
(2170.00000, 0.08532)
(2180.00000, 0.09870)
(2190.00000, 0.09188)
(2200.00000, 0.08655)
(2210.00000, 0.08789)
(2220.00000, 0.09610)
(2230.00000, 0.08603)
(2240.00000, 0.08899)
(2250.00000, 0.09339)
(2260.00000, 0.08294)
(2270.00000, 0.08108)
(2280.00000, 0.07937)
(2290.00000, 0.07719)
(2300.00000, 0.08143)
(2310.00000, 0.09279)
(2320.00000, 0.07622)
(2330.00000, 0.08841)
(2340.00000, 0.08296)
(2350.00000, 0.06869)
(2360.00000, 0.09255)
(2370.00000, 0.08801)
(2380.00000, 0.07252)
(2390.00000, 0.08299)
(2400.00000, 0.06855)
(2410.00000, 0.07949)
(2420.00000, 0.07724)
(2430.00000, 0.07208)
(2440.00000, 0.07906)
(2450.00000, 0.08452)
(2460.00000, 0.08355)
(2470.00000, 0.08211)
(2480.00000, 0.08434)
(2490.00000, 0.06782)
(2500.00000, 0.07445)
(2510.00000, 0.06927)
(2520.00000, 0.09206)
(2530.00000, 0.07596)
(2540.00000, 0.07337)
(2550.00000, 0.09036)
(2560.00000, 0.07990)
(2570.00000, 0.06281)
(2580.00000, 0.07481)
(2590.00000, 0.07237)
(2600.00000, 0.07375)
(2610.00000, 0.07075)
(2620.00000, 0.06545)
(2630.00000, 0.06828)
(2640.00000, 0.06641)
(2650.00000, 0.08002)
(2660.00000, 0.07213)
(2670.00000, 0.06187)
(2680.00000, 0.07987)
(2690.00000, 0.06563)
(2700.00000, 0.06112)
(2710.00000, 0.06411)
(2720.00000, 0.07113)
(2730.00000, 0.06731)
(2740.00000, 0.06152)
(2750.00000, 0.07274)
(2760.00000, 0.06168)
(2770.00000, 0.06510)
(2780.00000, 0.06677)
(2790.00000, 0.06249)
(2800.00000, 0.07569)
(2810.00000, 0.08071)
(2820.00000, 0.06891)
(2830.00000, 0.06783)
(2840.00000, 0.06176)
(2850.00000, 0.07580)
(2860.00000, 0.06548)
(2870.00000, 0.06419)
(2880.00000, 0.07669)
(2890.00000, 0.07376)
(2900.00000, 0.06801)
(2910.00000, 0.07008)
(2920.00000, 0.07244)
(2930.00000, 0.06967)
(2940.00000, 0.06432)
(2950.00000, 0.06388)
(2960.00000, 0.07876)
(2970.00000, 0.06676)
(2980.00000, 0.05530)
(2990.00000, 0.07019)
(3000.00000, 0.06794)
(3010.00000, 0.06326)
(3020.00000, 0.06443)
(3030.00000, 0.07116)
(3040.00000, 0.06778)
(3050.00000, 0.07508)
(3060.00000, 0.06429)
(3070.00000, 0.05928)
(3080.00000, 0.05998)
(3090.00000, 0.06110)
(3100.00000, 0.06753)
(3110.00000, 0.06561)
(3120.00000, 0.07170)
(3130.00000, 0.06954)
(3140.00000, 0.06488)
(3150.00000, 0.05032)
(3160.00000, 0.06060)
(3170.00000, 0.07306)
(3180.00000, 0.06548)
(3190.00000, 0.06020)
(3200.00000, 0.06642)
(3210.00000, 0.06317)
(3220.00000, 0.06790)
(3230.00000, 0.06183)
(3240.00000, 0.06378)
(3250.00000, 0.07005)
(3260.00000, 0.05691)
(3270.00000, 0.07022)
(3280.00000, 0.06059)
(3290.00000, 0.05317)
(3300.00000, 0.05630)
(3310.00000, 0.06441)
(3320.00000, 0.05606)
(3330.00000, 0.05871)
(3340.00000, 0.05839)
(3350.00000, 0.04327)
(3360.00000, 0.05682)
(3370.00000, 0.05621)
(3380.00000, 0.05725)
(3390.00000, 0.06256)
(3400.00000, 0.05451)
(3410.00000, 0.05315)
(3420.00000, 0.06238)
(3430.00000, 0.05529)
(3440.00000, 0.05914)
(3450.00000, 0.06019)
(3460.00000, 0.05454)
(3470.00000, 0.04886)
(3480.00000, 0.04983)
(3490.00000, 0.06713)
(3500.00000, 0.05391)
(3510.00000, 0.05648)
(3520.00000, 0.05671)
(3530.00000, 0.06036)
(3540.00000, 0.05103)
(3550.00000, 0.04718)
(3560.00000, 0.05834)
(3570.00000, 0.05516)
(3580.00000, 0.05314)
(3590.00000, 0.05344)
(3600.00000, 0.05308)
(3610.00000, 0.05206)
(3620.00000, 0.05802)
(3630.00000, 0.06282)
(3640.00000, 0.05431)
(3650.00000, 0.05182)
(3660.00000, 0.06435)
(3670.00000, 0.06422)
(3680.00000, 0.05597)
(3690.00000, 0.05933)
(3700.00000, 0.05093)
(3710.00000, 0.05922)
(3720.00000, 0.04558)
(3730.00000, 0.05870)
(3740.00000, 0.05512)
(3750.00000, 0.05178)
(3760.00000, 0.04761)
(3770.00000, 0.04785)
(3780.00000, 0.04380)
(3790.00000, 0.04875)
(3800.00000, 0.05831)
(3810.00000, 0.05472)
(3820.00000, 0.05641)
(3830.00000, 0.04839)
(3840.00000, 0.05122)
(3850.00000, 0.06218)
(3860.00000, 0.04898)
(3870.00000, 0.05711)
(3880.00000, 0.04679)
(3890.00000, 0.04711)
(3900.00000, 0.04585)
(3910.00000, 0.05034)
(3920.00000, 0.05178)
(3930.00000, 0.05527)
(3940.00000, 0.05394)
(3950.00000, 0.05625)
(3960.00000, 0.04766)
(3970.00000, 0.05493)
(3980.00000, 0.05503)
(3990.00000, 0.06009)
(4000.00000, 0.05128)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,Cyan3] plot coordinates {
(100.00000, 2.29562)
(110.00000, 1.63607)
(120.00000, 1.36342)
(130.00000, 0.74247)
(140.00000, 0.64751)
(150.00000, 1.00201)
(160.00000, 0.66058)
(170.00000, 0.99215)
(180.00000, 0.62297)
(190.00000, 0.56915)
(200.00000, 0.62328)
(210.00000, 0.56997)
(220.00000, 0.52162)
(230.00000, 0.43728)
(240.00000, 0.42854)
(250.00000, 0.37956)
(260.00000, 0.37112)
(270.00000, 0.30177)
(280.00000, 0.26804)
(290.00000, 0.28350)
(300.00000, 0.30525)
(310.00000, 0.27874)
(320.00000, 0.24987)
(330.00000, 0.22754)
(340.00000, 0.24918)
(350.00000, 0.21397)
(360.00000, 0.19271)
(370.00000, 0.20047)
(380.00000, 0.19795)
(390.00000, 0.22182)
(400.00000, 0.15093)
(410.00000, 0.18389)
(420.00000, 0.19988)
(430.00000, 0.15785)
(440.00000, 0.15974)
(450.00000, 0.18389)
(460.00000, 0.18320)
(470.00000, 0.16657)
(480.00000, 0.13716)
(490.00000, 0.17770)
(500.00000, 0.14669)
(510.00000, 0.13385)
(520.00000, 0.14958)
(530.00000, 0.15097)
(540.00000, 0.13915)
(550.00000, 0.16471)
(560.00000, 0.15250)
(570.00000, 0.18496)
(580.00000, 0.14186)
(590.00000, 0.14851)
(600.00000, 0.15263)
(610.00000, 0.15735)
(620.00000, 0.14042)
(630.00000, 0.13765)
(640.00000, 0.16083)
(650.00000, 0.15869)
(660.00000, 0.17273)
(670.00000, 0.15921)
(680.00000, 0.16478)
(690.00000, 0.15988)
(700.00000, 0.17011)
(710.00000, 0.16539)
(720.00000, 0.13678)
(730.00000, 0.16385)
(740.00000, 0.18178)
(750.00000, 0.13095)
(760.00000, 0.15012)
(770.00000, 0.14790)
(780.00000, 0.12166)
(790.00000, 0.14567)
(800.00000, 0.11926)
(810.00000, 0.13640)
(820.00000, 0.11545)
(830.00000, 0.12719)
(840.00000, 0.10669)
(850.00000, 0.09750)
(860.00000, 0.10001)
(870.00000, 0.10932)
(880.00000, 0.11292)
(890.00000, 0.11663)
(900.00000, 0.10267)
(910.00000, 0.10005)
(920.00000, 0.08595)
(930.00000, 0.10060)
(940.00000, 0.09999)
(950.00000, 0.09671)
(960.00000, 0.09323)
(970.00000, 0.10044)
(980.00000, 0.08816)
(990.00000, 0.08916)
(1000.00000, 0.10678)
(1010.00000, 0.11005)
(1020.00000, 0.10751)
(1030.00000, 0.08944)
(1040.00000, 0.11012)
(1050.00000, 0.12159)
(1060.00000, 0.11171)
(1070.00000, 0.10038)
(1080.00000, 0.09584)
(1090.00000, 0.10358)
(1100.00000, 0.09178)
(1110.00000, 0.10735)
(1120.00000, 0.09495)
(1130.00000, 0.08374)
(1140.00000, 0.09692)
(1150.00000, 0.08228)
(1160.00000, 0.11989)
(1170.00000, 0.08949)
(1180.00000, 0.09492)
(1190.00000, 0.07766)
(1200.00000, 0.10273)
(1210.00000, 0.08311)
(1220.00000, 0.08617)
(1230.00000, 0.09256)
(1240.00000, 0.09228)
(1250.00000, 0.09340)
(1260.00000, 0.08900)
(1270.00000, 0.08411)
(1280.00000, 0.08884)
(1290.00000, 0.08161)
(1300.00000, 0.08475)
(1310.00000, 0.08261)
(1320.00000, 0.08587)
(1330.00000, 0.09923)
(1340.00000, 0.07918)
(1350.00000, 0.08235)
(1360.00000, 0.08249)
(1370.00000, 0.08890)
(1380.00000, 0.08168)
(1390.00000, 0.09511)
(1400.00000, 0.07973)
(1410.00000, 0.08295)
(1420.00000, 0.07606)
(1430.00000, 0.09027)
(1440.00000, 0.08483)
(1450.00000, 0.07996)
(1460.00000, 0.06666)
(1470.00000, 0.06686)
(1480.00000, 0.10031)
(1490.00000, 0.08904)
(1500.00000, 0.08164)
(1510.00000, 0.07729)
(1520.00000, 0.07925)
(1530.00000, 0.08525)
(1540.00000, 0.09030)
(1550.00000, 0.09330)
(1560.00000, 0.07784)
(1570.00000, 0.09233)
(1580.00000, 0.08965)
(1590.00000, 0.08550)
(1600.00000, 0.07611)
(1610.00000, 0.07110)
(1620.00000, 0.07728)
(1630.00000, 0.07388)
(1640.00000, 0.08091)
(1650.00000, 0.09247)
(1660.00000, 0.07546)
(1670.00000, 0.07009)
(1680.00000, 0.09888)
(1690.00000, 0.08337)
(1700.00000, 0.08260)
(1710.00000, 0.08521)
(1720.00000, 0.07381)
(1730.00000, 0.08454)
(1740.00000, 0.07708)
(1750.00000, 0.07038)
(1760.00000, 0.08133)
(1770.00000, 0.09384)
(1780.00000, 0.07876)
(1790.00000, 0.08179)
(1800.00000, 0.08877)
(1810.00000, 0.09722)
(1820.00000, 0.07620)
(1830.00000, 0.08152)
(1840.00000, 0.10167)
(1850.00000, 0.07914)
(1860.00000, 0.08839)
(1870.00000, 0.08252)
(1880.00000, 0.09127)
(1890.00000, 0.07538)
(1900.00000, 0.08482)
(1910.00000, 0.07350)
(1920.00000, 0.07979)
(1930.00000, 0.07244)
(1940.00000, 0.07762)
(1950.00000, 0.07489)
(1960.00000, 0.07704)
(1970.00000, 0.07620)
(1980.00000, 0.07500)
(1990.00000, 0.08844)
(2000.00000, 0.08557)
(2010.00000, 0.07355)
(2020.00000, 0.07260)
(2030.00000, 0.09070)
(2040.00000, 0.07753)
(2050.00000, 0.09583)
(2060.00000, 0.07212)
(2070.00000, 0.06971)
(2080.00000, 0.09187)
(2090.00000, 0.09058)
(2100.00000, 0.07179)
(2110.00000, 0.06807)
(2120.00000, 0.07046)
(2130.00000, 0.07469)
(2140.00000, 0.07674)
(2150.00000, 0.06608)
(2160.00000, 0.08499)
(2170.00000, 0.07228)
(2180.00000, 0.07105)
(2190.00000, 0.06410)
(2200.00000, 0.08538)
(2210.00000, 0.06186)
(2220.00000, 0.05959)
(2230.00000, 0.08786)
(2240.00000, 0.07170)
(2250.00000, 0.07420)
(2260.00000, 0.07259)
(2270.00000, 0.07037)
(2280.00000, 0.06522)
(2290.00000, 0.06763)
(2300.00000, 0.06685)
(2310.00000, 0.06339)
(2320.00000, 0.07516)
(2330.00000, 0.06313)
(2340.00000, 0.07373)
(2350.00000, 0.06670)
(2360.00000, 0.06299)
(2370.00000, 0.07344)
(2380.00000, 0.06314)
(2390.00000, 0.07471)
(2400.00000, 0.07001)
(2410.00000, 0.07297)
(2420.00000, 0.05552)
(2430.00000, 0.07813)
(2440.00000, 0.06117)
(2450.00000, 0.06195)
(2460.00000, 0.06573)
(2470.00000, 0.05524)
(2480.00000, 0.06021)
(2490.00000, 0.07374)
(2500.00000, 0.07658)
(2510.00000, 0.06068)
(2520.00000, 0.06207)
(2530.00000, 0.07270)
(2540.00000, 0.07840)
(2550.00000, 0.07011)
(2560.00000, 0.07828)
(2570.00000, 0.07356)
(2580.00000, 0.06310)
(2590.00000, 0.06819)
(2600.00000, 0.06092)
(2610.00000, 0.07706)
(2620.00000, 0.06435)
(2630.00000, 0.06474)
(2640.00000, 0.06959)
(2650.00000, 0.06876)
(2660.00000, 0.06667)
(2670.00000, 0.06646)
(2680.00000, 0.07092)
(2690.00000, 0.07253)
(2700.00000, 0.05746)
(2710.00000, 0.06912)
(2720.00000, 0.08043)
(2730.00000, 0.06093)
(2740.00000, 0.07477)
(2750.00000, 0.07013)
(2760.00000, 0.07331)
(2770.00000, 0.06116)
(2780.00000, 0.07160)
(2790.00000, 0.06690)
(2800.00000, 0.06038)
(2810.00000, 0.06434)
(2820.00000, 0.06492)
(2830.00000, 0.06789)
(2840.00000, 0.06212)
(2850.00000, 0.05673)
(2860.00000, 0.07329)
(2870.00000, 0.06404)
(2880.00000, 0.06649)
(2890.00000, 0.07562)
(2900.00000, 0.07288)
(2910.00000, 0.05965)
(2920.00000, 0.06897)
(2930.00000, 0.06512)
(2940.00000, 0.05452)
(2950.00000, 0.05668)
(2960.00000, 0.06722)
(2970.00000, 0.06805)
(2980.00000, 0.06641)
(2990.00000, 0.05391)
(3000.00000, 0.07193)
(3010.00000, 0.06574)
(3020.00000, 0.05938)
(3030.00000, 0.06289)
(3040.00000, 0.07131)
(3050.00000, 0.06542)
(3060.00000, 0.04813)
(3070.00000, 0.06780)
(3080.00000, 0.06663)
(3090.00000, 0.04889)
(3100.00000, 0.06383)
(3110.00000, 0.06082)
(3120.00000, 0.06522)
(3130.00000, 0.06557)
(3140.00000, 0.06668)
(3150.00000, 0.06411)
(3160.00000, 0.06652)
(3170.00000, 0.05315)
(3180.00000, 0.05952)
(3190.00000, 0.05965)
(3200.00000, 0.05528)
(3210.00000, 0.06434)
(3220.00000, 0.05822)
(3230.00000, 0.05724)
(3240.00000, 0.06009)
(3250.00000, 0.05148)
(3260.00000, 0.05111)
(3270.00000, 0.04918)
(3280.00000, 0.05451)
(3290.00000, 0.05472)
(3300.00000, 0.06006)
(3310.00000, 0.05855)
(3320.00000, 0.06425)
(3330.00000, 0.06036)
(3340.00000, 0.04552)
(3350.00000, 0.05098)
(3360.00000, 0.05901)
(3370.00000, 0.05349)
(3380.00000, 0.05811)
(3390.00000, 0.05095)
(3400.00000, 0.05571)
(3410.00000, 0.05627)
(3420.00000, 0.05236)
(3430.00000, 0.05183)
(3440.00000, 0.05811)
(3450.00000, 0.05249)
(3460.00000, 0.05531)
(3470.00000, 0.05055)
(3480.00000, 0.04906)
(3490.00000, 0.05299)
(3500.00000, 0.05697)
(3510.00000, 0.04959)
(3520.00000, 0.05697)
(3530.00000, 0.05466)
(3540.00000, 0.06139)
(3550.00000, 0.04938)
(3560.00000, 0.04347)
(3570.00000, 0.04765)
(3580.00000, 0.05633)
(3590.00000, 0.04542)
(3600.00000, 0.04872)
(3610.00000, 0.05165)
(3620.00000, 0.05459)
(3630.00000, 0.05516)
(3640.00000, 0.04598)
(3650.00000, 0.05489)
(3660.00000, 0.04609)
(3670.00000, 0.05151)
(3680.00000, 0.04944)
(3690.00000, 0.06101)
(3700.00000, 0.05367)
(3710.00000, 0.04390)
(3720.00000, 0.05017)
(3730.00000, 0.04459)
(3740.00000, 0.05777)
(3750.00000, 0.05771)
(3760.00000, 0.04903)
(3770.00000, 0.05168)
(3780.00000, 0.05377)
(3790.00000, 0.05024)
(3800.00000, 0.04845)
(3810.00000, 0.05024)
(3820.00000, 0.04463)
(3830.00000, 0.04835)
(3840.00000, 0.04942)
(3850.00000, 0.03939)
(3860.00000, 0.05015)
(3870.00000, 0.04847)
(3880.00000, 0.05372)
(3890.00000, 0.04888)
(3900.00000, 0.05353)
(3910.00000, 0.05317)
(3920.00000, 0.05102)
(3930.00000, 0.04669)
(3940.00000, 0.04282)
(3950.00000, 0.06124)
(3960.00000, 0.04854)
(3970.00000, 0.04284)
(3980.00000, 0.04760)
(3990.00000, 0.04797)
(4000.00000, 0.05618)
};


==> Figures/convheart.tex <==
\addplot[thin,only marks, mark options={opacity=0.9},mark=*,mark size=.5pt,Red1] plot coordinates {
(1000.00000, 0.01632)
(1500.00000, 0.02989)
(2000.00000, 0.13745)
(2500.00000, 0.07515)
(3000.00000, 0.04353)
(3500.00000, 0.03501)
(4000.00000, 0.05008)
(4500.00000, 0.03524)
(5000.00000, 0.01586)
(5500.00000, 0.03279)
(6000.00000, 0.00905)
(6500.00000, 0.00976)
(7000.00000, 0.04005)
(7500.00000, 0.01448)
(8000.00000, 0.06353)
(8500.00000, 0.04885)
(9000.00000, 0.05446)
(9500.00000, 0.05251)
(10000.00000, 0.03595)
(10500.00000, 0.04508)
(11000.00000, 0.03786)
(11500.00000, 0.00985)
(12000.00000, 0.03683)
(12500.00000, 0.02144)
(13000.00000, 0.00643)
(13500.00000, 0.02055)
(14000.00000, 0.01065)
(14500.00000, 0.00934)
(15000.00000, 0.00971)
(15500.00000, 0.00667)
(16000.00000, 0.00828)
(16500.00000, 0.02100)
(17000.00000, 0.00705)
(17500.00000, 0.00709)
(18000.00000, 0.02441)
(18500.00000, 0.03951)
(19000.00000, 0.02465)
(19500.00000, 0.01443)
(20000.00000, 0.03989)
(20500.00000, 0.05202)
(21000.00000, 0.03912)
(21500.00000, 0.02604)
(22000.00000, 0.02909)
(22500.00000, 0.03722)
(23000.00000, 0.04031)
(23500.00000, 0.03028)
(24000.00000, 0.03054)
(24500.00000, 0.02590)
(25000.00000, 0.02608)
(25500.00000, 0.03418)
(26000.00000, 0.02508)
(26500.00000, 0.03778)
(27000.00000, 0.02802)
(27500.00000, 0.02004)
(28000.00000, 0.01286)
(28500.00000, 0.01509)
(29000.00000, 0.01834)
(29500.00000, 0.01710)
(30000.00000, 0.02003)
(30500.00000, 0.02438)
(31000.00000, 0.01424)
(31500.00000, 0.01034)
(32000.00000, 0.00579)
(32500.00000, 0.00379)
(33000.00000, 0.00414)
(33500.00000, 0.00398)
(34000.00000, 0.00448)
(34500.00000, 0.00987)
(35000.00000, 0.00435)
(35500.00000, 0.00445)
(36000.00000, 0.00663)
(36500.00000, 0.00326)
(37000.00000, 0.00425)
(37500.00000, 0.00342)
(38000.00000, 0.00485)
(38500.00000, 0.00763)
(39000.00000, 0.00323)
(39500.00000, 0.00293)
(40000.00000, 0.00327)
(40500.00000, 0.00425)
(41000.00000, 0.00336)
(41500.00000, 0.00575)
(42000.00000, 0.00336)
(42500.00000, 0.00299)
(43000.00000, 0.00671)
(43500.00000, 0.00555)
(44000.00000, 0.00618)
(44500.00000, 0.00710)
(45000.00000, 0.00992)
(45500.00000, 0.01054)
(46000.00000, 0.01115)
(46500.00000, 0.01575)
(47000.00000, 0.00480)
(47500.00000, 0.00618)
(48000.00000, 0.00990)
(48500.00000, 0.01260)
(49000.00000, 0.00999)
(49500.00000, 0.01186)
(50000.00000, 0.00953)
(50500.00000, 0.00859)
(51000.00000, 0.01232)
(51500.00000, 0.00670)
(52000.00000, 0.00299)
(52500.00000, 0.00650)
(53000.00000, 0.00998)
(53500.00000, 0.00882)
(54000.00000, 0.00459)
(54500.00000, 0.00274)
(55000.00000, 0.00276)
(55500.00000, 0.00436)
(56000.00000, 0.00349)
(56500.00000, 0.00262)
(57000.00000, 0.00257)
(57500.00000, 0.00277)
(58000.00000, 0.00294)
(58500.00000, 0.00332)
(59000.00000, 0.00376)
(59500.00000, 0.00258)
(60000.00000, 0.00300)
(60500.00000, 0.00698)
(61000.00000, 0.00284)
(61500.00000, 0.00527)
(62000.00000, 0.00331)
(62500.00000, 0.00696)
(63000.00000, 0.00720)
(63500.00000, 0.00507)
(64000.00000, 0.00494)
(64500.00000, 0.00541)
(65000.00000, 0.00761)
(65500.00000, 0.00631)
(66000.00000, 0.00606)
(66500.00000, 0.00682)
(67000.00000, 0.00554)
(67500.00000, 0.00537)
(68000.00000, 0.00465)
(68500.00000, 0.00333)
(69000.00000, 0.00242)
(69500.00000, 0.00260)
(70000.00000, 0.00388)
(70500.00000, 0.00343)
(71000.00000, 0.00350)
(71500.00000, 0.00435)
(72000.00000, 0.00372)
(72500.00000, 0.00261)
(73000.00000, 0.00338)
(73500.00000, 0.00237)
(74000.00000, 0.00301)
(74500.00000, 0.00227)
(75000.00000, 0.00254)
(75500.00000, 0.00246)
(76000.00000, 0.00438)
(76500.00000, 0.00312)
(77000.00000, 0.00663)
(77500.00000, 0.00726)
(78000.00000, 0.00371)
(78500.00000, 0.00735)
(79000.00000, 0.00433)
(79500.00000, 0.00292)
(80000.00000, 0.00603)
(80500.00000, 0.00848)
(81000.00000, 0.00607)
(81500.00000, 0.01162)
(82000.00000, 0.01073)
(82500.00000, 0.01342)
(83000.00000, 0.00702)
(83500.00000, 0.00846)
(84000.00000, 0.00813)
(84500.00000, 0.00600)
(85000.00000, 0.00892)
(85500.00000, 0.00811)
(86000.00000, 0.00512)
(86500.00000, 0.00531)
(87000.00000, 0.00591)
(87500.00000, 0.00480)
(88000.00000, 0.00464)
(88500.00000, 0.00229)
(89000.00000, 0.00327)
(89500.00000, 0.00426)
(90000.00000, 0.00304)
(90500.00000, 0.00357)
(91000.00000, 0.00301)
(91500.00000, 0.00245)
(92000.00000, 0.00276)
(92500.00000, 0.00568)
(93000.00000, 0.00542)
(93500.00000, 0.00326)
(94000.00000, 0.00279)
(94500.00000, 0.00333)
(95000.00000, 0.00413)
(95500.00000, 0.00574)
(96000.00000, 0.00276)
(96500.00000, 0.00401)
(97000.00000, 0.00271)
(97500.00000, 0.00203)
(98000.00000, 0.00174)
(98500.00000, 0.00311)
(99000.00000, 0.00472)
(99500.00000, 0.00348)
(100000.00000, 0.00195)
(100500.00000, 0.00240)
(101000.00000, 0.00191)
(101500.00000, 0.00223)
(102000.00000, 0.00244)
(102500.00000, 0.00259)
(103000.00000, 0.00192)
(103500.00000, 0.00245)
(104000.00000, 0.00354)
(104500.00000, 0.00196)
(105000.00000, 0.00190)
(105500.00000, 0.00296)
(106000.00000, 0.00334)
(106500.00000, 0.00255)
(107000.00000, 0.00221)
(107500.00000, 0.00197)
(108000.00000, 0.00364)
(108500.00000, 0.00269)
(109000.00000, 0.00289)
(109500.00000, 0.00355)
(110000.00000, 0.00266)
(110500.00000, 0.00343)
(111000.00000, 0.00363)
(111500.00000, 0.00417)
(112000.00000, 0.00508)
(112500.00000, 0.00548)
(113000.00000, 0.00435)
(113500.00000, 0.00588)
(114000.00000, 0.00527)
(114500.00000, 0.00545)
(115000.00000, 0.00577)
(115500.00000, 0.00645)
(116000.00000, 0.00865)
(116500.00000, 0.00934)
(117000.00000, 0.00759)
(117500.00000, 0.01125)
(118000.00000, 0.00877)
(118500.00000, 0.01263)
(119000.00000, 0.00939)
(119500.00000, 0.00822)
(120000.00000, 0.00975)
(120500.00000, 0.01154)
(121000.00000, 0.01064)
(121500.00000, 0.01016)
(122000.00000, 0.00993)
(122500.00000, 0.00917)
(123000.00000, 0.01005)
(123500.00000, 0.00941)
(124000.00000, 0.00683)
(124500.00000, 0.00680)
(125000.00000, 0.00886)
(125500.00000, 0.00885)
(126000.00000, 0.00789)
(126500.00000, 0.00804)
(127000.00000, 0.00577)
(127500.00000, 0.00472)
(128000.00000, 0.00469)
(128500.00000, 0.00389)
(129000.00000, 0.00454)
(129500.00000, 0.00438)
(130000.00000, 0.00508)
(130500.00000, 0.00530)
(131000.00000, 0.00493)
(131500.00000, 0.00382)
(132000.00000, 0.00613)
(132500.00000, 0.00306)
(133000.00000, 0.00523)
(133500.00000, 0.00379)
(134000.00000, 0.00296)
(134500.00000, 0.00309)
(135000.00000, 0.00236)
(135500.00000, 0.00224)
(136000.00000, 0.00185)
(136500.00000, 0.00171)
(137000.00000, 0.00191)
(137500.00000, 0.00135)
(138000.00000, 0.00221)
(138500.00000, 0.00182)
(139000.00000, 0.00209)
(139500.00000, 0.00339)
(140000.00000, 0.00179)
(140500.00000, 0.00269)
(141000.00000, 0.00364)
(141500.00000, 0.00314)
(142000.00000, 0.00331)
(142500.00000, 0.00378)
(143000.00000, 0.00535)
(143500.00000, 0.00473)
(144000.00000, 0.00499)
(144500.00000, 0.00404)
(145000.00000, 0.00604)
(145500.00000, 0.00557)
(146000.00000, 0.00427)
(146500.00000, 0.00466)
(147000.00000, 0.00470)
(147500.00000, 0.00613)
(148000.00000, 0.00482)
(148500.00000, 0.00539)
(149000.00000, 0.00613)
(149500.00000, 0.00562)
(150000.00000, 0.00527)
(150500.00000, 0.00577)
(151000.00000, 0.00674)
(151500.00000, 0.00631)
(152000.00000, 0.00461)
(152500.00000, 0.00336)
(153000.00000, 0.00404)
(153500.00000, 0.00474)
(154000.00000, 0.00406)
(154500.00000, 0.00534)
(155000.00000, 0.00464)
(155500.00000, 0.00309)
(156000.00000, 0.00433)
(156500.00000, 0.00373)
(157000.00000, 0.00338)
(157500.00000, 0.00370)
(158000.00000, 0.00357)
(158500.00000, 0.00337)
(159000.00000, 0.00323)
(159500.00000, 0.00277)
(160000.00000, 0.00164)
(160500.00000, 0.00160)
(161000.00000, 0.00158)
(161500.00000, 0.00142)
(162000.00000, 0.00218)
(162500.00000, 0.00312)
(163000.00000, 0.00496)
(163500.00000, 0.00329)
(164000.00000, 0.00394)
(164500.00000, 0.00533)
(165000.00000, 0.00615)
(165500.00000, 0.00582)
(166000.00000, 0.00430)
(166500.00000, 0.00427)
(167000.00000, 0.00518)
(167500.00000, 0.00518)
(168000.00000, 0.00392)
(168500.00000, 0.00395)
(169000.00000, 0.00319)
(169500.00000, 0.00248)
(170000.00000, 0.00392)
(170500.00000, 0.00296)
(171000.00000, 0.00420)
(171500.00000, 0.00364)
(172000.00000, 0.00236)
(172500.00000, 0.00218)
(173000.00000, 0.00184)
(173500.00000, 0.00184)
(174000.00000, 0.00305)
(174500.00000, 0.00260)
(175000.00000, 0.00205)
(175500.00000, 0.00246)
(176000.00000, 0.00200)
(176500.00000, 0.00165)
(177000.00000, 0.00170)
(177500.00000, 0.00160)
(178000.00000, 0.00175)
(178500.00000, 0.00135)
(179000.00000, 0.00154)
(179500.00000, 0.00133)
(180000.00000, 0.00135)
(180500.00000, 0.00161)
(181000.00000, 0.00151)
(181500.00000, 0.00233)
(182000.00000, 0.00182)
(182500.00000, 0.00297)
(183000.00000, 0.00226)
(183500.00000, 0.00275)
(184000.00000, 0.00320)
(184500.00000, 0.00387)
(185000.00000, 0.00526)
(185500.00000, 0.00524)
(186000.00000, 0.00519)
(186500.00000, 0.00508)
(187000.00000, 0.00557)
(187500.00000, 0.00589)
(188000.00000, 0.00525)
(188500.00000, 0.00578)
(189000.00000, 0.00647)
(189500.00000, 0.00665)
(190000.00000, 0.00739)
(190500.00000, 0.00718)
(191000.00000, 0.00816)
(191500.00000, 0.00615)
(192000.00000, 0.00630)
(192500.00000, 0.00706)
(193000.00000, 0.00751)
(193500.00000, 0.00737)
(194000.00000, 0.00668)
(194500.00000, 0.00584)
(195000.00000, 0.00596)
(195500.00000, 0.00643)
(196000.00000, 0.00490)
(196500.00000, 0.00458)
(197000.00000, 0.00503)
(197500.00000, 0.00670)
(198000.00000, 0.00659)
(198500.00000, 0.00591)
(199000.00000, 0.00555)
(199500.00000, 0.00531)
(200000.00000, 0.00417)
(200500.00000, 0.00513)
(201000.00000, 0.00522)
(201500.00000, 0.00457)
(202000.00000, 0.00477)
(202500.00000, 0.00467)
(203000.00000, 0.00391)
(203500.00000, 0.00382)
(204000.00000, 0.00354)
(204500.00000, 0.00271)
(205000.00000, 0.00251)
(205500.00000, 0.00294)
(206000.00000, 0.00246)
(206500.00000, 0.00291)
(207000.00000, 0.00197)
(207500.00000, 0.00275)
(208000.00000, 0.00254)
(208500.00000, 0.00325)
(209000.00000, 0.00340)
(209500.00000, 0.00350)
(210000.00000, 0.00424)
(210500.00000, 0.00432)
(211000.00000, 0.00418)
(211500.00000, 0.00405)
(212000.00000, 0.00252)
(212500.00000, 0.00332)
(213000.00000, 0.00353)
(213500.00000, 0.00369)
(214000.00000, 0.00399)
(214500.00000, 0.00424)
(215000.00000, 0.00464)
(215500.00000, 0.00490)
(216000.00000, 0.00455)
(216500.00000, 0.00473)
(217000.00000, 0.00502)
(217500.00000, 0.00487)
(218000.00000, 0.00512)
(218500.00000, 0.00602)
(219000.00000, 0.00532)
(219500.00000, 0.00659)
(220000.00000, 0.00633)
(220500.00000, 0.00617)
(221000.00000, 0.00589)
(221500.00000, 0.00484)
(222000.00000, 0.00491)
(222500.00000, 0.00432)
(223000.00000, 0.00574)
(223500.00000, 0.00523)
(224000.00000, 0.00512)
(224500.00000, 0.00595)
(225000.00000, 0.00635)
(225500.00000, 0.00632)
(226000.00000, 0.00783)
(226500.00000, 0.00697)
(227000.00000, 0.00722)
(227500.00000, 0.00550)
(228000.00000, 0.00587)
(228500.00000, 0.00593)
(229000.00000, 0.00558)
(229500.00000, 0.00487)
(230000.00000, 0.00483)
(230500.00000, 0.00399)
(231000.00000, 0.00407)
(231500.00000, 0.00446)
(232000.00000, 0.00393)
(232500.00000, 0.00315)
(233000.00000, 0.00209)
(233500.00000, 0.00262)
(234000.00000, 0.00232)
(234500.00000, 0.00167)
(235000.00000, 0.00112)
(235500.00000, 0.00126)
(236000.00000, 0.00128)
(236500.00000, 0.00109)
(237000.00000, 0.00179)
(237500.00000, 0.00169)
(238000.00000, 0.00151)
(238500.00000, 0.00138)
(239000.00000, 0.00143)
(239500.00000, 0.00101)
(240000.00000, 0.00167)
(240500.00000, 0.00131)
(241000.00000, 0.00172)
(241500.00000, 0.00176)
(242000.00000, 0.00126)
(242500.00000, 0.00121)
(243000.00000, 0.00116)
(243500.00000, 0.00161)
(244000.00000, 0.00127)
(244500.00000, 0.00109)
(245000.00000, 0.00103)
(245500.00000, 0.00141)
(246000.00000, 0.00105)
(246500.00000, 0.00124)
(247000.00000, 0.00102)
(247500.00000, 0.00126)
(248000.00000, 0.00141)
(248500.00000, 0.00144)
(249000.00000, 0.00139)
(249500.00000, 0.00136)
(250000.00000, 0.00240)
(250500.00000, 0.00208)
(251000.00000, 0.00237)
(251500.00000, 0.00247)
(252000.00000, 0.00245)
(252500.00000, 0.00268)
(253000.00000, 0.00192)
(253500.00000, 0.00246)
(254000.00000, 0.00337)
};
\addplot[thin,only marks, mark options={opacity=0.9},mark=*,mark size=.5pt,Cyan2] plot coordinates {
(1000.00000, 0.03758)
(1500.00000, 0.01658)
(2000.00000, 0.14484)
(2500.00000, 0.13260)
(3000.00000, 0.05914)
(3500.00000, 0.08508)
(4000.00000, 0.06675)
(4500.00000, 0.05967)
(5000.00000, 0.07557)
(5500.00000, 0.01179)
(6000.00000, 0.01430)
(6500.00000, 0.03133)
(7000.00000, 0.05238)
(7500.00000, 0.02292)
(8000.00000, 0.02908)
(8500.00000, 0.01907)
(9000.00000, 0.01334)
(9500.00000, 0.01457)
(10000.00000, 0.05486)
(10500.00000, 0.05128)
(11000.00000, 0.02074)
(11500.00000, 0.03726)
(12000.00000, 0.06833)
(12500.00000, 0.07893)
(13000.00000, 0.07273)
(13500.00000, 0.05771)
(14000.00000, 0.05235)
(14500.00000, 0.03099)
(15000.00000, 0.02118)
(15500.00000, 0.03210)
(16000.00000, 0.03558)
(16500.00000, 0.04898)
(17000.00000, 0.05997)
(17500.00000, 0.03890)
(18000.00000, 0.04976)
(18500.00000, 0.02936)
(19000.00000, 0.01737)
(19500.00000, 0.01653)
(20000.00000, 0.02143)
(20500.00000, 0.02916)
(21000.00000, 0.02262)
(21500.00000, 0.01327)
(22000.00000, 0.01090)
(22500.00000, 0.00713)
(23000.00000, 0.01089)
(23500.00000, 0.01421)
(24000.00000, 0.00925)
(24500.00000, 0.00837)
(25000.00000, 0.00867)
(25500.00000, 0.01104)
(26000.00000, 0.01003)
(26500.00000, 0.01832)
(27000.00000, 0.01661)
(27500.00000, 0.03384)
(28000.00000, 0.03356)
(28500.00000, 0.03122)
(29000.00000, 0.03902)
(29500.00000, 0.03170)
(30000.00000, 0.03434)
(30500.00000, 0.03803)
(31000.00000, 0.03832)
(31500.00000, 0.04388)
(32000.00000, 0.03562)
(32500.00000, 0.03980)
(33000.00000, 0.03658)
(33500.00000, 0.04300)
(34000.00000, 0.04247)
(34500.00000, 0.04567)
(35000.00000, 0.03305)
(35500.00000, 0.04911)
(36000.00000, 0.05421)
(36500.00000, 0.03873)
(37000.00000, 0.03852)
(37500.00000, 0.04052)
(38000.00000, 0.04241)
(38500.00000, 0.04343)
(39000.00000, 0.03412)
(39500.00000, 0.03151)
(40000.00000, 0.03479)
(40500.00000, 0.03393)
(41000.00000, 0.03418)
(41500.00000, 0.03760)
(42000.00000, 0.03138)
(42500.00000, 0.02752)
(43000.00000, 0.02045)
(43500.00000, 0.02386)
(44000.00000, 0.02237)
(44500.00000, 0.02154)
(45000.00000, 0.02201)
(45500.00000, 0.01746)
(46000.00000, 0.01703)
(46500.00000, 0.02199)
(47000.00000, 0.01512)
(47500.00000, 0.01324)
(48000.00000, 0.01518)
(48500.00000, 0.00950)
(49000.00000, 0.01310)
(49500.00000, 0.00860)
(50000.00000, 0.00593)
(50500.00000, 0.00823)
(51000.00000, 0.00624)
(51500.00000, 0.00744)
(52000.00000, 0.00717)
(52500.00000, 0.00362)
(53000.00000, 0.00636)
(53500.00000, 0.00538)
(54000.00000, 0.00503)
(54500.00000, 0.00397)
(55000.00000, 0.00425)
(55500.00000, 0.00263)
(56000.00000, 0.00315)
(56500.00000, 0.00430)
(57000.00000, 0.00390)
(57500.00000, 0.00355)
(58000.00000, 0.00488)
(58500.00000, 0.00492)
(59000.00000, 0.00279)
(59500.00000, 0.00338)
(60000.00000, 0.00294)
(60500.00000, 0.00467)
(61000.00000, 0.00337)
(61500.00000, 0.00336)
(62000.00000, 0.00330)
(62500.00000, 0.00328)
(63000.00000, 0.00227)
(63500.00000, 0.00268)
(64000.00000, 0.00363)
(64500.00000, 0.00253)
(65000.00000, 0.00492)
(65500.00000, 0.00352)
(66000.00000, 0.00254)
(66500.00000, 0.00442)
(67000.00000, 0.00487)
(67500.00000, 0.00349)
(68000.00000, 0.00391)
(68500.00000, 0.00606)
(69000.00000, 0.00680)
(69500.00000, 0.00618)
(70000.00000, 0.00815)
(70500.00000, 0.01161)
(71000.00000, 0.01420)
(71500.00000, 0.01460)
(72000.00000, 0.01426)
(72500.00000, 0.01108)
(73000.00000, 0.00765)
(73500.00000, 0.00670)
(74000.00000, 0.00666)
(74500.00000, 0.00951)
(75000.00000, 0.01131)
(75500.00000, 0.01178)
(76000.00000, 0.01123)
(76500.00000, 0.01009)
(77000.00000, 0.00673)
(77500.00000, 0.00521)
(78000.00000, 0.00808)
(78500.00000, 0.00598)
(79000.00000, 0.00885)
(79500.00000, 0.00803)
(80000.00000, 0.00639)
(80500.00000, 0.00388)
(81000.00000, 0.00218)
(81500.00000, 0.00281)
(82000.00000, 0.00222)
(82500.00000, 0.00262)
(83000.00000, 0.00252)
(83500.00000, 0.00361)
(84000.00000, 0.00300)
(84500.00000, 0.00215)
(85000.00000, 0.00301)
(85500.00000, 0.00328)
(86000.00000, 0.00313)
(86500.00000, 0.00557)
(87000.00000, 0.00437)
(87500.00000, 0.00358)
(88000.00000, 0.00611)
(88500.00000, 0.00634)
(89000.00000, 0.00831)
(89500.00000, 0.01013)
(90000.00000, 0.00729)
(90500.00000, 0.01028)
(91000.00000, 0.00728)
(91500.00000, 0.00645)
(92000.00000, 0.00834)
(92500.00000, 0.00849)
(93000.00000, 0.00853)
(93500.00000, 0.00574)
(94000.00000, 0.00765)
(94500.00000, 0.01094)
(95000.00000, 0.00949)
(95500.00000, 0.00683)
(96000.00000, 0.00746)
(96500.00000, 0.00862)
(97000.00000, 0.00962)
(97500.00000, 0.00764)
(98000.00000, 0.00651)
(98500.00000, 0.00770)
(99000.00000, 0.00770)
(99500.00000, 0.00599)
(100000.00000, 0.00787)
(100500.00000, 0.00839)
(101000.00000, 0.00458)
(101500.00000, 0.00555)
(102000.00000, 0.00421)
(102500.00000, 0.00327)
(103000.00000, 0.00353)
(103500.00000, 0.00315)
(104000.00000, 0.00307)
(104500.00000, 0.00311)
(105000.00000, 0.00266)
(105500.00000, 0.00538)
(106000.00000, 0.00252)
(106500.00000, 0.00451)
(107000.00000, 0.00444)
(107500.00000, 0.00297)
(108000.00000, 0.00429)
(108500.00000, 0.00284)
(109000.00000, 0.00344)
(109500.00000, 0.00279)
(110000.00000, 0.00337)
(110500.00000, 0.00196)
(111000.00000, 0.00180)
(111500.00000, 0.00174)
(112000.00000, 0.00211)
(112500.00000, 0.00194)
(113000.00000, 0.00161)
(113500.00000, 0.00322)
(114000.00000, 0.00384)
(114500.00000, 0.00247)
(115000.00000, 0.00321)
(115500.00000, 0.00327)
(116000.00000, 0.00183)
(116500.00000, 0.00227)
(117000.00000, 0.00282)
(117500.00000, 0.00272)
(118000.00000, 0.00227)
(118500.00000, 0.00235)
(119000.00000, 0.00408)
(119500.00000, 0.00271)
(120000.00000, 0.00361)
(120500.00000, 0.00363)
(121000.00000, 0.00442)
(121500.00000, 0.00193)
(122000.00000, 0.00418)
(122500.00000, 0.00215)
(123000.00000, 0.00263)
(123500.00000, 0.00204)
(124000.00000, 0.00181)
(124500.00000, 0.00191)
(125000.00000, 0.00418)
(125500.00000, 0.00556)
(126000.00000, 0.00428)
(126500.00000, 0.00428)
(127000.00000, 0.00559)
(127500.00000, 0.00620)
(128000.00000, 0.00656)
(128500.00000, 0.00645)
(129000.00000, 0.00804)
(129500.00000, 0.00947)
(130000.00000, 0.00915)
(130500.00000, 0.00948)
(131000.00000, 0.00846)
(131500.00000, 0.00729)
(132000.00000, 0.00604)
(132500.00000, 0.00609)
(133000.00000, 0.00865)
(133500.00000, 0.00868)
(134000.00000, 0.00972)
(134500.00000, 0.01019)
(135000.00000, 0.00857)
(135500.00000, 0.00904)
(136000.00000, 0.00707)
(136500.00000, 0.00745)
(137000.00000, 0.00567)
(137500.00000, 0.00738)
(138000.00000, 0.00643)
(138500.00000, 0.00704)
(139000.00000, 0.00542)
(139500.00000, 0.00324)
(140000.00000, 0.00245)
(140500.00000, 0.00220)
(141000.00000, 0.00183)
(141500.00000, 0.00171)
(142000.00000, 0.00155)
(142500.00000, 0.00198)
(143000.00000, 0.00199)
(143500.00000, 0.00182)
(144000.00000, 0.00215)
(144500.00000, 0.00243)
(145000.00000, 0.00361)
(145500.00000, 0.00271)
(146000.00000, 0.00300)
(146500.00000, 0.00294)
(147000.00000, 0.00246)
(147500.00000, 0.00453)
(148000.00000, 0.00362)
(148500.00000, 0.00484)
(149000.00000, 0.00519)
(149500.00000, 0.00375)
(150000.00000, 0.00436)
(150500.00000, 0.00316)
(151000.00000, 0.00494)
(151500.00000, 0.00573)
(152000.00000, 0.00582)
(152500.00000, 0.00388)
(153000.00000, 0.00626)
(153500.00000, 0.00576)
(154000.00000, 0.00397)
(154500.00000, 0.00398)
(155000.00000, 0.00535)
(155500.00000, 0.00515)
(156000.00000, 0.00530)
(156500.00000, 0.00340)
(157000.00000, 0.00347)
(157500.00000, 0.00452)
(158000.00000, 0.00438)
(158500.00000, 0.00406)
(159000.00000, 0.00388)
(159500.00000, 0.00316)
(160000.00000, 0.00218)
(160500.00000, 0.00183)
(161000.00000, 0.00214)
(161500.00000, 0.00143)
(162000.00000, 0.00166)
(162500.00000, 0.00144)
(163000.00000, 0.00166)
(163500.00000, 0.00174)
(164000.00000, 0.00173)
(164500.00000, 0.00181)
(165000.00000, 0.00310)
(165500.00000, 0.00194)
(166000.00000, 0.00292)
(166500.00000, 0.00198)
(167000.00000, 0.00258)
(167500.00000, 0.00252)
(168000.00000, 0.00324)
(168500.00000, 0.00365)
(169000.00000, 0.00297)
(169500.00000, 0.00264)
(170000.00000, 0.00252)
(170500.00000, 0.00239)
(171000.00000, 0.00293)
(171500.00000, 0.00302)
(172000.00000, 0.00226)
(172500.00000, 0.00356)
(173000.00000, 0.00426)
(173500.00000, 0.00357)
(174000.00000, 0.00390)
(174500.00000, 0.00369)
(175000.00000, 0.00355)
(175500.00000, 0.00420)
(176000.00000, 0.00508)
(176500.00000, 0.00608)
(177000.00000, 0.00632)
(177500.00000, 0.00591)
(178000.00000, 0.00524)
(178500.00000, 0.00590)
(179000.00000, 0.00579)
(179500.00000, 0.00655)
(180000.00000, 0.00488)
(180500.00000, 0.00603)
(181000.00000, 0.00560)
(181500.00000, 0.00493)
(182000.00000, 0.00455)
(182500.00000, 0.00416)
(183000.00000, 0.00512)
(183500.00000, 0.00603)
(184000.00000, 0.00587)
(184500.00000, 0.00589)
(185000.00000, 0.00579)
(185500.00000, 0.00638)
(186000.00000, 0.00732)
(186500.00000, 0.00729)
(187000.00000, 0.00779)
(187500.00000, 0.00751)
(188000.00000, 0.00882)
(188500.00000, 0.00871)
(189000.00000, 0.00873)
(189500.00000, 0.00882)
(190000.00000, 0.00771)
(190500.00000, 0.00652)
(191000.00000, 0.00623)
(191500.00000, 0.00690)
(192000.00000, 0.00811)
(192500.00000, 0.00820)
(193000.00000, 0.00934)
(193500.00000, 0.00686)
(194000.00000, 0.00749)
(194500.00000, 0.00595)
(195000.00000, 0.00556)
(195500.00000, 0.00600)
(196000.00000, 0.00540)
(196500.00000, 0.00638)
(197000.00000, 0.00641)
(197500.00000, 0.00541)
(198000.00000, 0.00566)
(198500.00000, 0.00482)
(199000.00000, 0.00468)
(199500.00000, 0.00490)
(200000.00000, 0.00452)
(200500.00000, 0.00568)
(201000.00000, 0.00531)
(201500.00000, 0.00534)
(202000.00000, 0.00501)
(202500.00000, 0.00430)
(203000.00000, 0.00366)
(203500.00000, 0.00331)
(204000.00000, 0.00288)
(204500.00000, 0.00262)
(205000.00000, 0.00352)
(205500.00000, 0.00270)
(206000.00000, 0.00182)
(206500.00000, 0.00220)
(207000.00000, 0.00191)
(207500.00000, 0.00206)
(208000.00000, 0.00163)
(208500.00000, 0.00135)
(209000.00000, 0.00152)
(209500.00000, 0.00161)
(210000.00000, 0.00131)
(210500.00000, 0.00204)
(211000.00000, 0.00144)
(211500.00000, 0.00163)
(212000.00000, 0.00149)
(212500.00000, 0.00147)
(213000.00000, 0.00160)
(213500.00000, 0.00152)
(214000.00000, 0.00098)
(214500.00000, 0.00153)
(215000.00000, 0.00237)
(215500.00000, 0.00208)
(216000.00000, 0.00143)
(216500.00000, 0.00158)
(217000.00000, 0.00147)
(217500.00000, 0.00148)
(218000.00000, 0.00238)
(218500.00000, 0.00232)
(219000.00000, 0.00215)
(219500.00000, 0.00243)
(220000.00000, 0.00242)
(220500.00000, 0.00200)
(221000.00000, 0.00211)
(221500.00000, 0.00130)
(222000.00000, 0.00122)
(222500.00000, 0.00147)
(223000.00000, 0.00159)
(223500.00000, 0.00204)
(224000.00000, 0.00192)
(224500.00000, 0.00196)
(225000.00000, 0.00137)
(225500.00000, 0.00136)
(226000.00000, 0.00168)
(226500.00000, 0.00131)
(227000.00000, 0.00123)
(227500.00000, 0.00177)
(228000.00000, 0.00166)
(228500.00000, 0.00136)
(229000.00000, 0.00149)
(229500.00000, 0.00194)
(230000.00000, 0.00161)
(230500.00000, 0.00149)
(231000.00000, 0.00188)
(231500.00000, 0.00142)
(232000.00000, 0.00176)
(232500.00000, 0.00162)
(233000.00000, 0.00136)
(233500.00000, 0.00137)
(234000.00000, 0.00131)
(234500.00000, 0.00127)
(235000.00000, 0.00129)
(235500.00000, 0.00124)
(236000.00000, 0.00130)
(236500.00000, 0.00121)
(237000.00000, 0.00134)
(237500.00000, 0.00130)
(238000.00000, 0.00191)
(238500.00000, 0.00128)
(239000.00000, 0.00162)
(239500.00000, 0.00170)
(240000.00000, 0.00210)
(240500.00000, 0.00136)
(241000.00000, 0.00201)
(241500.00000, 0.00174)
(242000.00000, 0.00167)
(242500.00000, 0.00150)
(243000.00000, 0.00140)
(243500.00000, 0.00125)
(244000.00000, 0.00126)
(244500.00000, 0.00185)
(245000.00000, 0.00199)
(245500.00000, 0.00170)
(246000.00000, 0.00239)
(246500.00000, 0.00294)
(247000.00000, 0.00317)
(247500.00000, 0.00360)
(248000.00000, 0.00335)
(248500.00000, 0.00347)
(249000.00000, 0.00299)
(249500.00000, 0.00205)
(250000.00000, 0.00227)
(250500.00000, 0.00290)
(251000.00000, 0.00335)
(251500.00000, 0.00374)
(252000.00000, 0.00333)
(252500.00000, 0.00368)
(253000.00000, 0.00259)
(253500.00000, 0.00224)
(254000.00000, 0.00241)
};
\addplot[thin,only marks, mark options={opacity=0.9},mark=*,mark size=.5pt,Green4] plot coordinates {
(1000.00000, 0.19880)
(1500.00000, 0.07006)
(2000.00000, 0.04134)
(2500.00000, 0.06135)
(3000.00000, 0.03781)
(3500.00000, 0.01895)
(4000.00000, 0.01217)
(4500.00000, 0.00830)
(5000.00000, 0.00772)
(5500.00000, 0.01049)
(6000.00000, 0.01240)
(6500.00000, 0.02257)
(7000.00000, 0.01899)
(7500.00000, 0.00796)
(8000.00000, 0.00739)
(8500.00000, 0.03990)
(9000.00000, 0.02040)
(9500.00000, 0.02145)
(10000.00000, 0.02473)
(10500.00000, 0.01529)
(11000.00000, 0.01019)
(11500.00000, 0.00833)
(12000.00000, 0.01920)
(12500.00000, 0.01950)
(13000.00000, 0.03539)
(13500.00000, 0.02133)
(14000.00000, 0.02002)
(14500.00000, 0.01424)
(15000.00000, 0.01006)
(15500.00000, 0.01198)
(16000.00000, 0.02052)
(16500.00000, 0.01825)
(17000.00000, 0.00942)
(17500.00000, 0.00584)
(18000.00000, 0.02261)
(18500.00000, 0.01876)
(19000.00000, 0.02328)
(19500.00000, 0.01281)
(20000.00000, 0.00887)
(20500.00000, 0.01294)
(21000.00000, 0.01049)
(21500.00000, 0.01613)
(22000.00000, 0.02131)
(22500.00000, 0.02335)
(23000.00000, 0.02594)
(23500.00000, 0.02040)
(24000.00000, 0.01788)
(24500.00000, 0.02553)
(25000.00000, 0.02765)
(25500.00000, 0.03691)
(26000.00000, 0.01545)
(26500.00000, 0.01792)
(27000.00000, 0.02926)
(27500.00000, 0.03038)
(28000.00000, 0.02154)
(28500.00000, 0.02278)
(29000.00000, 0.01860)
(29500.00000, 0.01873)
(30000.00000, 0.02460)
(30500.00000, 0.02144)
(31000.00000, 0.01040)
(31500.00000, 0.00509)
(32000.00000, 0.01397)
(32500.00000, 0.01912)
(33000.00000, 0.01150)
(33500.00000, 0.01329)
(34000.00000, 0.00629)
(34500.00000, 0.00523)
(35000.00000, 0.00903)
(35500.00000, 0.00580)
(36000.00000, 0.00441)
(36500.00000, 0.01038)
(37000.00000, 0.01327)
(37500.00000, 0.00349)
(38000.00000, 0.00471)
(38500.00000, 0.00439)
(39000.00000, 0.00516)
(39500.00000, 0.00461)
(40000.00000, 0.00409)
(40500.00000, 0.00367)
(41000.00000, 0.00359)
(41500.00000, 0.00482)
(42000.00000, 0.00330)
(42500.00000, 0.00325)
(43000.00000, 0.00392)
(43500.00000, 0.00553)
(44000.00000, 0.00439)
(44500.00000, 0.00557)
(45000.00000, 0.00403)
(45500.00000, 0.00299)
(46000.00000, 0.00374)
(46500.00000, 0.00335)
(47000.00000, 0.00551)
(47500.00000, 0.00479)
(48000.00000, 0.00532)
(48500.00000, 0.00742)
(49000.00000, 0.01106)
(49500.00000, 0.00735)
(50000.00000, 0.00483)
(50500.00000, 0.00523)
(51000.00000, 0.01524)
(51500.00000, 0.01452)
(52000.00000, 0.00717)
(52500.00000, 0.00703)
(53000.00000, 0.00567)
(53500.00000, 0.00852)
(54000.00000, 0.00417)
(54500.00000, 0.00453)
(55000.00000, 0.00459)
(55500.00000, 0.00309)
(56000.00000, 0.00357)
(56500.00000, 0.00258)
(57000.00000, 0.00274)
(57500.00000, 0.00433)
(58000.00000, 0.00298)
(58500.00000, 0.00308)
(59000.00000, 0.00319)
(59500.00000, 0.00248)
(60000.00000, 0.00237)
(60500.00000, 0.00410)
(61000.00000, 0.00515)
(61500.00000, 0.00466)
(62000.00000, 0.00334)
(62500.00000, 0.00301)
(63000.00000, 0.00222)
(63500.00000, 0.00207)
(64000.00000, 0.00199)
(64500.00000, 0.00329)
(65000.00000, 0.00409)
(65500.00000, 0.00446)
(66000.00000, 0.00378)
(66500.00000, 0.00298)
(67000.00000, 0.00252)
(67500.00000, 0.00216)
(68000.00000, 0.00166)
(68500.00000, 0.00360)
(69000.00000, 0.00249)
(69500.00000, 0.00222)
(70000.00000, 0.00210)
(70500.00000, 0.00213)
(71000.00000, 0.00319)
(71500.00000, 0.00278)
(72000.00000, 0.00324)
(72500.00000, 0.00218)
(73000.00000, 0.00252)
(73500.00000, 0.00356)
(74000.00000, 0.00253)
(74500.00000, 0.00277)
(75000.00000, 0.00476)
(75500.00000, 0.00309)
(76000.00000, 0.00287)
(76500.00000, 0.00606)
(77000.00000, 0.00825)
(77500.00000, 0.00984)
(78000.00000, 0.00496)
(78500.00000, 0.00434)
(79000.00000, 0.00756)
(79500.00000, 0.00786)
(80000.00000, 0.01066)
(80500.00000, 0.01039)
(81000.00000, 0.01064)
(81500.00000, 0.01173)
(82000.00000, 0.00987)
(82500.00000, 0.01044)
(83000.00000, 0.01139)
(83500.00000, 0.01284)
(84000.00000, 0.01293)
(84500.00000, 0.01181)
(85000.00000, 0.00782)
(85500.00000, 0.01343)
(86000.00000, 0.01374)
(86500.00000, 0.01230)
(87000.00000, 0.01197)
(87500.00000, 0.01117)
(88000.00000, 0.00860)
(88500.00000, 0.00975)
(89000.00000, 0.00949)
(89500.00000, 0.00687)
(90000.00000, 0.00624)
(90500.00000, 0.00522)
(91000.00000, 0.00658)
(91500.00000, 0.00715)
(92000.00000, 0.00554)
(92500.00000, 0.00269)
(93000.00000, 0.00209)
(93500.00000, 0.00227)
(94000.00000, 0.00281)
(94500.00000, 0.00178)
(95000.00000, 0.00312)
(95500.00000, 0.00372)
(96000.00000, 0.00247)
(96500.00000, 0.00682)
(97000.00000, 0.00464)
(97500.00000, 0.00282)
(98000.00000, 0.00458)
(98500.00000, 0.00335)
(99000.00000, 0.00229)
(99500.00000, 0.00297)
(100000.00000, 0.00354)
(100500.00000, 0.00302)
(101000.00000, 0.00298)
(101500.00000, 0.00288)
(102000.00000, 0.00266)
(102500.00000, 0.00362)
(103000.00000, 0.00377)
(103500.00000, 0.00473)
(104000.00000, 0.00259)
(104500.00000, 0.00304)
(105000.00000, 0.00388)
(105500.00000, 0.00359)
(106000.00000, 0.00338)
(106500.00000, 0.00467)
(107000.00000, 0.00487)
(107500.00000, 0.00260)
(108000.00000, 0.00264)
(108500.00000, 0.00310)
(109000.00000, 0.00280)
(109500.00000, 0.00221)
(110000.00000, 0.00183)
(110500.00000, 0.00177)
(111000.00000, 0.00326)
(111500.00000, 0.00224)
(112000.00000, 0.00188)
(112500.00000, 0.00314)
(113000.00000, 0.00220)
(113500.00000, 0.00530)
(114000.00000, 0.00468)
(114500.00000, 0.00548)
(115000.00000, 0.00684)
(115500.00000, 0.00376)
(116000.00000, 0.00331)
(116500.00000, 0.00354)
(117000.00000, 0.00446)
(117500.00000, 0.00486)
(118000.00000, 0.00461)
(118500.00000, 0.00590)
(119000.00000, 0.00592)
(119500.00000, 0.00489)
(120000.00000, 0.00421)
(120500.00000, 0.00576)
(121000.00000, 0.00626)
(121500.00000, 0.00615)
(122000.00000, 0.00552)
(122500.00000, 0.00624)
(123000.00000, 0.00627)
(123500.00000, 0.00512)
(124000.00000, 0.00505)
(124500.00000, 0.00563)
(125000.00000, 0.00568)
(125500.00000, 0.00484)
(126000.00000, 0.00747)
(126500.00000, 0.00527)
(127000.00000, 0.00688)
(127500.00000, 0.00695)
(128000.00000, 0.00699)
(128500.00000, 0.00629)
(129000.00000, 0.00673)
(129500.00000, 0.00723)
(130000.00000, 0.00574)
(130500.00000, 0.00940)
(131000.00000, 0.00704)
(131500.00000, 0.00730)
(132000.00000, 0.00764)
(132500.00000, 0.00797)
(133000.00000, 0.00832)
(133500.00000, 0.00646)
(134000.00000, 0.00564)
(134500.00000, 0.00409)
(135000.00000, 0.00408)
(135500.00000, 0.00781)
(136000.00000, 0.00783)
(136500.00000, 0.00701)
(137000.00000, 0.00713)
(137500.00000, 0.00535)
(138000.00000, 0.00622)
(138500.00000, 0.00824)
(139000.00000, 0.00777)
(139500.00000, 0.00855)
(140000.00000, 0.00810)
(140500.00000, 0.00785)
(141000.00000, 0.00884)
(141500.00000, 0.00807)
(142000.00000, 0.00967)
(142500.00000, 0.00952)
(143000.00000, 0.01066)
(143500.00000, 0.00733)
(144000.00000, 0.00946)
(144500.00000, 0.01009)
(145000.00000, 0.00928)
(145500.00000, 0.00822)
(146000.00000, 0.00860)
(146500.00000, 0.00810)
(147000.00000, 0.00737)
(147500.00000, 0.00725)
(148000.00000, 0.00754)
(148500.00000, 0.00635)
(149000.00000, 0.00629)
(149500.00000, 0.00549)
(150000.00000, 0.00635)
(150500.00000, 0.00599)
(151000.00000, 0.00490)
(151500.00000, 0.00384)
(152000.00000, 0.00327)
(152500.00000, 0.00287)
(153000.00000, 0.00240)
(153500.00000, 0.00174)
(154000.00000, 0.00229)
(154500.00000, 0.00183)
(155000.00000, 0.00180)
(155500.00000, 0.00190)
(156000.00000, 0.00163)
(156500.00000, 0.00134)
(157000.00000, 0.00170)
(157500.00000, 0.00162)
(158000.00000, 0.00194)
(158500.00000, 0.00148)
(159000.00000, 0.00190)
(159500.00000, 0.00231)
(160000.00000, 0.00234)
(160500.00000, 0.00359)
(161000.00000, 0.00255)
(161500.00000, 0.00237)
(162000.00000, 0.00205)
(162500.00000, 0.00155)
(163000.00000, 0.00220)
(163500.00000, 0.00197)
(164000.00000, 0.00152)
(164500.00000, 0.00178)
(165000.00000, 0.00171)
(165500.00000, 0.00181)
(166000.00000, 0.00268)
(166500.00000, 0.00255)
(167000.00000, 0.00246)
(167500.00000, 0.00262)
(168000.00000, 0.00353)
(168500.00000, 0.00423)
(169000.00000, 0.00394)
(169500.00000, 0.00229)
(170000.00000, 0.00294)
(170500.00000, 0.00329)
(171000.00000, 0.00248)
(171500.00000, 0.00204)
(172000.00000, 0.00160)
(172500.00000, 0.00165)
(173000.00000, 0.00130)
(173500.00000, 0.00141)
(174000.00000, 0.00159)
(174500.00000, 0.00230)
(175000.00000, 0.00212)
(175500.00000, 0.00188)
(176000.00000, 0.00171)
(176500.00000, 0.00169)
(177000.00000, 0.00119)
(177500.00000, 0.00131)
(178000.00000, 0.00142)
(178500.00000, 0.00184)
(179000.00000, 0.00128)
(179500.00000, 0.00162)
(180000.00000, 0.00134)
(180500.00000, 0.00146)
(181000.00000, 0.00135)
(181500.00000, 0.00154)
(182000.00000, 0.00122)
(182500.00000, 0.00128)
(183000.00000, 0.00147)
(183500.00000, 0.00144)
(184000.00000, 0.00164)
(184500.00000, 0.00176)
(185000.00000, 0.00145)
(185500.00000, 0.00142)
(186000.00000, 0.00135)
(186500.00000, 0.00147)
(187000.00000, 0.00149)
(187500.00000, 0.00152)
(188000.00000, 0.00135)
(188500.00000, 0.00138)
(189000.00000, 0.00191)
(189500.00000, 0.00143)
(190000.00000, 0.00140)
(190500.00000, 0.00172)
(191000.00000, 0.00124)
(191500.00000, 0.00242)
(192000.00000, 0.00201)
(192500.00000, 0.00163)
(193000.00000, 0.00138)
(193500.00000, 0.00152)
(194000.00000, 0.00253)
(194500.00000, 0.00180)
(195000.00000, 0.00194)
(195500.00000, 0.00194)
(196000.00000, 0.00141)
(196500.00000, 0.00115)
(197000.00000, 0.00155)
(197500.00000, 0.00187)
(198000.00000, 0.00294)
(198500.00000, 0.00227)
(199000.00000, 0.00276)
(199500.00000, 0.00258)
(200000.00000, 0.00181)
(200500.00000, 0.00329)
(201000.00000, 0.00278)
(201500.00000, 0.00424)
(202000.00000, 0.00276)
(202500.00000, 0.00214)
(203000.00000, 0.00326)
(203500.00000, 0.00352)
(204000.00000, 0.00321)
(204500.00000, 0.00251)
(205000.00000, 0.00258)
(205500.00000, 0.00207)
(206000.00000, 0.00194)
(206500.00000, 0.00263)
(207000.00000, 0.00194)
(207500.00000, 0.00214)
(208000.00000, 0.00191)
(208500.00000, 0.00196)
(209000.00000, 0.00152)
(209500.00000, 0.00177)
(210000.00000, 0.00159)
(210500.00000, 0.00159)
(211000.00000, 0.00128)
(211500.00000, 0.00160)
(212000.00000, 0.00137)
(212500.00000, 0.00104)
(213000.00000, 0.00123)
(213500.00000, 0.00163)
(214000.00000, 0.00165)
(214500.00000, 0.00124)
(215000.00000, 0.00119)
(215500.00000, 0.00140)
(216000.00000, 0.00143)
(216500.00000, 0.00146)
(217000.00000, 0.00145)
(217500.00000, 0.00145)
(218000.00000, 0.00202)
(218500.00000, 0.00151)
(219000.00000, 0.00178)
(219500.00000, 0.00223)
(220000.00000, 0.00184)
(220500.00000, 0.00161)
(221000.00000, 0.00169)
(221500.00000, 0.00170)
(222000.00000, 0.00209)
(222500.00000, 0.00128)
(223000.00000, 0.00158)
(223500.00000, 0.00154)
(224000.00000, 0.00136)
(224500.00000, 0.00146)
(225000.00000, 0.00162)
(225500.00000, 0.00260)
(226000.00000, 0.00201)
(226500.00000, 0.00164)
(227000.00000, 0.00325)
(227500.00000, 0.00309)
(228000.00000, 0.00261)
(228500.00000, 0.00183)
(229000.00000, 0.00203)
(229500.00000, 0.00329)
(230000.00000, 0.00193)
(230500.00000, 0.00261)
(231000.00000, 0.00139)
(231500.00000, 0.00132)
(232000.00000, 0.00124)
(232500.00000, 0.00167)
(233000.00000, 0.00170)
(233500.00000, 0.00234)
(234000.00000, 0.00202)
(234500.00000, 0.00170)
(235000.00000, 0.00191)
(235500.00000, 0.00190)
(236000.00000, 0.00140)
(236500.00000, 0.00181)
(237000.00000, 0.00207)
(237500.00000, 0.00261)
(238000.00000, 0.00270)
(238500.00000, 0.00242)
(239000.00000, 0.00197)
(239500.00000, 0.00166)
(240000.00000, 0.00171)
(240500.00000, 0.00149)
(241000.00000, 0.00197)
(241500.00000, 0.00238)
(242000.00000, 0.00187)
(242500.00000, 0.00167)
(243000.00000, 0.00183)
(243500.00000, 0.00168)
(244000.00000, 0.00192)
(244500.00000, 0.00113)
(245000.00000, 0.00142)
(245500.00000, 0.00123)
(246000.00000, 0.00190)
(246500.00000, 0.00152)
(247000.00000, 0.00114)
(247500.00000, 0.00131)
(248000.00000, 0.00109)
(248500.00000, 0.00166)
(249000.00000, 0.00109)
(249500.00000, 0.00123)
(250000.00000, 0.00137)
(250500.00000, 0.00132)
(251000.00000, 0.00164)
(251500.00000, 0.00141)
(252000.00000, 0.00136)
(252500.00000, 0.00151)
(253000.00000, 0.00180)
(253500.00000, 0.00158)
(254000.00000, 0.00138)
};
\addplot[thin,only marks, mark options={opacity=0.9},mark=*,mark size=.5pt,blue] plot coordinates {
(1000.00000, 0.45578)
(1500.00000, 0.28009)
(2000.00000, 0.01322)
(2500.00000, 0.05442)
(3000.00000, 0.01230)
(3500.00000, 0.05460)
(4000.00000, 0.06340)
(4500.00000, 0.07742)
(5000.00000, 0.08342)
(5500.00000, 0.04346)
(6000.00000, 0.01169)
(6500.00000, 0.00754)
(7000.00000, 0.00857)
(7500.00000, 0.03031)
(8000.00000, 0.02801)
(8500.00000, 0.03032)
(9000.00000, 0.02043)
(9500.00000, 0.00914)
(10000.00000, 0.00594)
(10500.00000, 0.00454)
(11000.00000, 0.01029)
(11500.00000, 0.01322)
(12000.00000, 0.01269)
(12500.00000, 0.01226)
(13000.00000, 0.00789)
(13500.00000, 0.00547)
(14000.00000, 0.00639)
(14500.00000, 0.01992)
(15000.00000, 0.00692)
(15500.00000, 0.01308)
(16000.00000, 0.02256)
(16500.00000, 0.01315)
(17000.00000, 0.02537)
(17500.00000, 0.01202)
(18000.00000, 0.02229)
(18500.00000, 0.02707)
(19000.00000, 0.02576)
(19500.00000, 0.02287)
(20000.00000, 0.01887)
(20500.00000, 0.01880)
(21000.00000, 0.02042)
(21500.00000, 0.01585)
(22000.00000, 0.01261)
(22500.00000, 0.01340)
(23000.00000, 0.01547)
(23500.00000, 0.01512)
(24000.00000, 0.01392)
(24500.00000, 0.01576)
(25000.00000, 0.02053)
(25500.00000, 0.01924)
(26000.00000, 0.01881)
(26500.00000, 0.01299)
(27000.00000, 0.01816)
(27500.00000, 0.00975)
(28000.00000, 0.01819)
(28500.00000, 0.01518)
(29000.00000, 0.00512)
(29500.00000, 0.00387)
(30000.00000, 0.00819)
(30500.00000, 0.01714)
(31000.00000, 0.00996)
(31500.00000, 0.00887)
(32000.00000, 0.00470)
(32500.00000, 0.00723)
(33000.00000, 0.00825)
(33500.00000, 0.00499)
(34000.00000, 0.00552)
(34500.00000, 0.00482)
(35000.00000, 0.00825)
(35500.00000, 0.00487)
(36000.00000, 0.00338)
(36500.00000, 0.00666)
(37000.00000, 0.00676)
(37500.00000, 0.00795)
(38000.00000, 0.00649)
(38500.00000, 0.00310)
(39000.00000, 0.00422)
(39500.00000, 0.00368)
(40000.00000, 0.00414)
(40500.00000, 0.00278)
(41000.00000, 0.00301)
(41500.00000, 0.00290)
(42000.00000, 0.00326)
(42500.00000, 0.00462)
(43000.00000, 0.00573)
(43500.00000, 0.00399)
(44000.00000, 0.01045)
(44500.00000, 0.00900)
(45000.00000, 0.01053)
(45500.00000, 0.00930)
(46000.00000, 0.00780)
(46500.00000, 0.01005)
(47000.00000, 0.00988)
(47500.00000, 0.01057)
(48000.00000, 0.01536)
(48500.00000, 0.01509)
(49000.00000, 0.01230)
(49500.00000, 0.00830)
(50000.00000, 0.00816)
(50500.00000, 0.00866)
(51000.00000, 0.00780)
(51500.00000, 0.00730)
(52000.00000, 0.00928)
(52500.00000, 0.00968)
(53000.00000, 0.00881)
(53500.00000, 0.00832)
(54000.00000, 0.00872)
(54500.00000, 0.00632)
(55000.00000, 0.00697)
(55500.00000, 0.00644)
(56000.00000, 0.00805)
(56500.00000, 0.00816)
(57000.00000, 0.00781)
(57500.00000, 0.00765)
(58000.00000, 0.00767)
(58500.00000, 0.00822)
(59000.00000, 0.00865)
(59500.00000, 0.00805)
(60000.00000, 0.01098)
(60500.00000, 0.00933)
(61000.00000, 0.00882)
(61500.00000, 0.00941)
(62000.00000, 0.01099)
(62500.00000, 0.00552)
(63000.00000, 0.00862)
(63500.00000, 0.01144)
(64000.00000, 0.01045)
(64500.00000, 0.01187)
(65000.00000, 0.00973)
(65500.00000, 0.00942)
(66000.00000, 0.00916)
(66500.00000, 0.00909)
(67000.00000, 0.00731)
(67500.00000, 0.00848)
(68000.00000, 0.01009)
(68500.00000, 0.00888)
(69000.00000, 0.00783)
(69500.00000, 0.00872)
(70000.00000, 0.00771)
(70500.00000, 0.00762)
(71000.00000, 0.00823)
(71500.00000, 0.00812)
(72000.00000, 0.00739)
(72500.00000, 0.00830)
(73000.00000, 0.00709)
(73500.00000, 0.00580)
(74000.00000, 0.00636)
(74500.00000, 0.00608)
(75000.00000, 0.00656)
(75500.00000, 0.00403)
(76000.00000, 0.00533)
(76500.00000, 0.00598)
(77000.00000, 0.00424)
(77500.00000, 0.00607)
(78000.00000, 0.00650)
(78500.00000, 0.00487)
(79000.00000, 0.00598)
(79500.00000, 0.00436)
(80000.00000, 0.00402)
(80500.00000, 0.00490)
(81000.00000, 0.00392)
(81500.00000, 0.00434)
(82000.00000, 0.00631)
(82500.00000, 0.00459)
(83000.00000, 0.00472)
(83500.00000, 0.00270)
(84000.00000, 0.00351)
(84500.00000, 0.00447)
(85000.00000, 0.00231)
(85500.00000, 0.00340)
(86000.00000, 0.00417)
(86500.00000, 0.00274)
(87000.00000, 0.00587)
(87500.00000, 0.00522)
(88000.00000, 0.00245)
(88500.00000, 0.00254)
(89000.00000, 0.00434)
(89500.00000, 0.00517)
(90000.00000, 0.00279)
(90500.00000, 0.00289)
(91000.00000, 0.00288)
(91500.00000, 0.00436)
(92000.00000, 0.00372)
(92500.00000, 0.00227)
(93000.00000, 0.00188)
(93500.00000, 0.00393)
(94000.00000, 0.00402)
(94500.00000, 0.00484)
(95000.00000, 0.00508)
(95500.00000, 0.00454)
(96000.00000, 0.00304)
(96500.00000, 0.00209)
(97000.00000, 0.00215)
(97500.00000, 0.00321)
(98000.00000, 0.00337)
(98500.00000, 0.00290)
(99000.00000, 0.00304)
(99500.00000, 0.00226)
(100000.00000, 0.00202)
(100500.00000, 0.00218)
(101000.00000, 0.00201)
(101500.00000, 0.00247)
(102000.00000, 0.00277)
(102500.00000, 0.00287)
(103000.00000, 0.00314)
(103500.00000, 0.00426)
(104000.00000, 0.00418)
(104500.00000, 0.00258)
(105000.00000, 0.00445)
(105500.00000, 0.00258)
(106000.00000, 0.00368)
(106500.00000, 0.00407)
(107000.00000, 0.00616)
(107500.00000, 0.00523)
(108000.00000, 0.00393)
(108500.00000, 0.00563)
(109000.00000, 0.00652)
(109500.00000, 0.00690)
(110000.00000, 0.00539)
(110500.00000, 0.00603)
(111000.00000, 0.00706)
(111500.00000, 0.00646)
(112000.00000, 0.00488)
(112500.00000, 0.00503)
(113000.00000, 0.00573)
(113500.00000, 0.00629)
(114000.00000, 0.00616)
(114500.00000, 0.00641)
(115000.00000, 0.00580)
(115500.00000, 0.00534)
(116000.00000, 0.00529)
(116500.00000, 0.00491)
(117000.00000, 0.00428)
(117500.00000, 0.00425)
(118000.00000, 0.00346)
(118500.00000, 0.00528)
(119000.00000, 0.00383)
(119500.00000, 0.00304)
(120000.00000, 0.00409)
(120500.00000, 0.00479)
(121000.00000, 0.00439)
(121500.00000, 0.00373)
(122000.00000, 0.00321)
(122500.00000, 0.00353)
(123000.00000, 0.00329)
(123500.00000, 0.00366)
(124000.00000, 0.00266)
(124500.00000, 0.00224)
(125000.00000, 0.00326)
(125500.00000, 0.00505)
(126000.00000, 0.00359)
(126500.00000, 0.00353)
(127000.00000, 0.00210)
(127500.00000, 0.00175)
(128000.00000, 0.00242)
(128500.00000, 0.00189)
(129000.00000, 0.00255)
(129500.00000, 0.00328)
(130000.00000, 0.00395)
(130500.00000, 0.00408)
(131000.00000, 0.00379)
(131500.00000, 0.00241)
(132000.00000, 0.00327)
(132500.00000, 0.00219)
(133000.00000, 0.00366)
(133500.00000, 0.00537)
(134000.00000, 0.00443)
(134500.00000, 0.00690)
(135000.00000, 0.00510)
(135500.00000, 0.00691)
(136000.00000, 0.00491)
(136500.00000, 0.00536)
(137000.00000, 0.00589)
(137500.00000, 0.00539)
(138000.00000, 0.00587)
(138500.00000, 0.00633)
(139000.00000, 0.00713)
(139500.00000, 0.00536)
(140000.00000, 0.00535)
(140500.00000, 0.00627)
(141000.00000, 0.00617)
(141500.00000, 0.00500)
(142000.00000, 0.00582)
(142500.00000, 0.00567)
(143000.00000, 0.00603)
(143500.00000, 0.00562)
(144000.00000, 0.00506)
(144500.00000, 0.00544)
(145000.00000, 0.00533)
(145500.00000, 0.00524)
(146000.00000, 0.00561)
(146500.00000, 0.00512)
(147000.00000, 0.00531)
(147500.00000, 0.00504)
(148000.00000, 0.00535)
(148500.00000, 0.00520)
(149000.00000, 0.00618)
(149500.00000, 0.00515)
(150000.00000, 0.00820)
(150500.00000, 0.00704)
(151000.00000, 0.00738)
(151500.00000, 0.00756)
(152000.00000, 0.00728)
(152500.00000, 0.00873)
(153000.00000, 0.00658)
(153500.00000, 0.00750)
(154000.00000, 0.00803)
(154500.00000, 0.00803)
(155000.00000, 0.00743)
(155500.00000, 0.00771)
(156000.00000, 0.00770)
(156500.00000, 0.00784)
(157000.00000, 0.00719)
(157500.00000, 0.00635)
(158000.00000, 0.00679)
(158500.00000, 0.00694)
(159000.00000, 0.00657)
(159500.00000, 0.00647)
(160000.00000, 0.00643)
(160500.00000, 0.00701)
(161000.00000, 0.00638)
(161500.00000, 0.00628)
(162000.00000, 0.00572)
(162500.00000, 0.00577)
(163000.00000, 0.00520)
(163500.00000, 0.00525)
(164000.00000, 0.00482)
(164500.00000, 0.00424)
(165000.00000, 0.00463)
(165500.00000, 0.00471)
(166000.00000, 0.00418)
(166500.00000, 0.00501)
(167000.00000, 0.00513)
(167500.00000, 0.00453)
(168000.00000, 0.00406)
(168500.00000, 0.00458)
(169000.00000, 0.00398)
(169500.00000, 0.00393)
(170000.00000, 0.00473)
(170500.00000, 0.00423)
(171000.00000, 0.00402)
(171500.00000, 0.00446)
(172000.00000, 0.00350)
(172500.00000, 0.00412)
(173000.00000, 0.00330)
(173500.00000, 0.00392)
(174000.00000, 0.00416)
(174500.00000, 0.00292)
(175000.00000, 0.00381)
(175500.00000, 0.00326)
(176000.00000, 0.00294)
(176500.00000, 0.00280)
(177000.00000, 0.00190)
(177500.00000, 0.00327)
(178000.00000, 0.00297)
(178500.00000, 0.00175)
(179000.00000, 0.00184)
(179500.00000, 0.00291)
(180000.00000, 0.00190)
(180500.00000, 0.00147)
(181000.00000, 0.00149)
(181500.00000, 0.00178)
(182000.00000, 0.00196)
(182500.00000, 0.00172)
(183000.00000, 0.00139)
(183500.00000, 0.00149)
(184000.00000, 0.00173)
(184500.00000, 0.00147)
(185000.00000, 0.00172)
(185500.00000, 0.00205)
(186000.00000, 0.00195)
(186500.00000, 0.00154)
(187000.00000, 0.00139)
(187500.00000, 0.00181)
(188000.00000, 0.00144)
(188500.00000, 0.00160)
(189000.00000, 0.00164)
(189500.00000, 0.00158)
(190000.00000, 0.00176)
(190500.00000, 0.00146)
(191000.00000, 0.00169)
(191500.00000, 0.00176)
(192000.00000, 0.00176)
(192500.00000, 0.00157)
(193000.00000, 0.00175)
(193500.00000, 0.00161)
(194000.00000, 0.00207)
(194500.00000, 0.00173)
(195000.00000, 0.00205)
(195500.00000, 0.00173)
(196000.00000, 0.00201)
(196500.00000, 0.00253)
(197000.00000, 0.00208)
(197500.00000, 0.00387)
(198000.00000, 0.00233)
(198500.00000, 0.00296)
(199000.00000, 0.00354)
(199500.00000, 0.00330)
(200000.00000, 0.00306)
(200500.00000, 0.00272)
(201000.00000, 0.00306)
(201500.00000, 0.00308)
(202000.00000, 0.00332)
(202500.00000, 0.00273)
(203000.00000, 0.00263)
(203500.00000, 0.00289)
(204000.00000, 0.00277)
(204500.00000, 0.00276)
(205000.00000, 0.00256)
(205500.00000, 0.00257)
(206000.00000, 0.00243)
(206500.00000, 0.00211)
(207000.00000, 0.00231)
(207500.00000, 0.00183)
(208000.00000, 0.00201)
(208500.00000, 0.00216)
(209000.00000, 0.00198)
(209500.00000, 0.00166)
(210000.00000, 0.00160)
(210500.00000, 0.00163)
(211000.00000, 0.00168)
(211500.00000, 0.00185)
(212000.00000, 0.00137)
(212500.00000, 0.00166)
(213000.00000, 0.00195)
(213500.00000, 0.00153)
(214000.00000, 0.00160)
(214500.00000, 0.00124)
(215000.00000, 0.00140)
(215500.00000, 0.00179)
(216000.00000, 0.00143)
(216500.00000, 0.00158)
(217000.00000, 0.00134)
(217500.00000, 0.00133)
(218000.00000, 0.00143)
(218500.00000, 0.00139)
(219000.00000, 0.00115)
(219500.00000, 0.00135)
(220000.00000, 0.00122)
(220500.00000, 0.00119)
(221000.00000, 0.00114)
(221500.00000, 0.00127)
(222000.00000, 0.00149)
(222500.00000, 0.00159)
(223000.00000, 0.00123)
(223500.00000, 0.00123)
(224000.00000, 0.00125)
(224500.00000, 0.00150)
(225000.00000, 0.00150)
(225500.00000, 0.00185)
(226000.00000, 0.00170)
(226500.00000, 0.00162)
(227000.00000, 0.00196)
(227500.00000, 0.00156)
(228000.00000, 0.00155)
(228500.00000, 0.00173)
(229000.00000, 0.00173)
(229500.00000, 0.00197)
(230000.00000, 0.00200)
(230500.00000, 0.00178)
(231000.00000, 0.00218)
(231500.00000, 0.00168)
(232000.00000, 0.00152)
(232500.00000, 0.00200)
(233000.00000, 0.00185)
(233500.00000, 0.00195)
(234000.00000, 0.00184)
(234500.00000, 0.00184)
(235000.00000, 0.00176)
(235500.00000, 0.00177)
(236000.00000, 0.00199)
(236500.00000, 0.00214)
(237000.00000, 0.00205)
(237500.00000, 0.00192)
(238000.00000, 0.00173)
(238500.00000, 0.00202)
(239000.00000, 0.00176)
(239500.00000, 0.00198)
(240000.00000, 0.00172)
(240500.00000, 0.00222)
(241000.00000, 0.00184)
(241500.00000, 0.00169)
(242000.00000, 0.00191)
(242500.00000, 0.00246)
(243000.00000, 0.00178)
(243500.00000, 0.00171)
(244000.00000, 0.00226)
(244500.00000, 0.00233)
(245000.00000, 0.00258)
(245500.00000, 0.00226)
(246000.00000, 0.00223)
(246500.00000, 0.00199)
(247000.00000, 0.00205)
(247500.00000, 0.00147)
(248000.00000, 0.00217)
(248500.00000, 0.00219)
(249000.00000, 0.00206)
(249500.00000, 0.00168)
(250000.00000, 0.00196)
(250500.00000, 0.00218)
(251000.00000, 0.00209)
(251500.00000, 0.00206)
(252000.00000, 0.00131)
(252500.00000, 0.00170)
(253000.00000, 0.00142)
(253500.00000, 0.00150)
(254000.00000, 0.00134)
};
\addplot[thin,only marks, mark options={opacity=0.9},mark=*,mark size=.5pt,Green3] plot coordinates {
(1000.00000, 0.02958)
(1500.00000, 0.05158)
(2000.00000, 0.10691)
(2500.00000, 0.11006)
(3000.00000, 0.03091)
(3500.00000, 0.01879)
(4000.00000, 0.01146)
(4500.00000, 0.01598)
(5000.00000, 0.01191)
(5500.00000, 0.02981)
(6000.00000, 0.01572)
(6500.00000, 0.00887)
(7000.00000, 0.02054)
(7500.00000, 0.00628)
(8000.00000, 0.02671)
(8500.00000, 0.04169)
(9000.00000, 0.02595)
(9500.00000, 0.02015)
(10000.00000, 0.03342)
(10500.00000, 0.02483)
(11000.00000, 0.01291)
(11500.00000, 0.02634)
(12000.00000, 0.01322)
(12500.00000, 0.02792)
(13000.00000, 0.01786)
(13500.00000, 0.01158)
(14000.00000, 0.00773)
(14500.00000, 0.02902)
(15000.00000, 0.02486)
(15500.00000, 0.01889)
(16000.00000, 0.01243)
(16500.00000, 0.00536)
(17000.00000, 0.00956)
(17500.00000, 0.01134)
(18000.00000, 0.01174)
(18500.00000, 0.01188)
(19000.00000, 0.01210)
(19500.00000, 0.01592)
(20000.00000, 0.01318)
(20500.00000, 0.00941)
(21000.00000, 0.00871)
(21500.00000, 0.01646)
(22000.00000, 0.01064)
(22500.00000, 0.00761)
(23000.00000, 0.00532)
(23500.00000, 0.01604)
(24000.00000, 0.00800)
(24500.00000, 0.00700)
(25000.00000, 0.01558)
(25500.00000, 0.00432)
(26000.00000, 0.00480)
(26500.00000, 0.01071)
(27000.00000, 0.01253)
(27500.00000, 0.01370)
(28000.00000, 0.01093)
(28500.00000, 0.01866)
(29000.00000, 0.00944)
(29500.00000, 0.01781)
(30000.00000, 0.01661)
(30500.00000, 0.01848)
(31000.00000, 0.01698)
(31500.00000, 0.02123)
(32000.00000, 0.01288)
(32500.00000, 0.00781)
(33000.00000, 0.01870)
(33500.00000, 0.01017)
(34000.00000, 0.00987)
(34500.00000, 0.01008)
(35000.00000, 0.01091)
(35500.00000, 0.00785)
(36000.00000, 0.00904)
(36500.00000, 0.01240)
(37000.00000, 0.01170)
(37500.00000, 0.00993)
(38000.00000, 0.01209)
(38500.00000, 0.00833)
(39000.00000, 0.00773)
(39500.00000, 0.00885)
(40000.00000, 0.00507)
(40500.00000, 0.00496)
(41000.00000, 0.00905)
(41500.00000, 0.00554)
(42000.00000, 0.00753)
(42500.00000, 0.00673)
(43000.00000, 0.01243)
(43500.00000, 0.00400)
(44000.00000, 0.00757)
(44500.00000, 0.00934)
(45000.00000, 0.01010)
(45500.00000, 0.00572)
(46000.00000, 0.00919)
(46500.00000, 0.00862)
(47000.00000, 0.00338)
(47500.00000, 0.01067)
(48000.00000, 0.00391)
(48500.00000, 0.00309)
(49000.00000, 0.00532)
(49500.00000, 0.00459)
(50000.00000, 0.00291)
(50500.00000, 0.00363)
(51000.00000, 0.00289)
(51500.00000, 0.00287)
(52000.00000, 0.00376)
(52500.00000, 0.00305)
(53000.00000, 0.00410)
(53500.00000, 0.00326)
(54000.00000, 0.00343)
(54500.00000, 0.00325)
(55000.00000, 0.00413)
(55500.00000, 0.00307)
(56000.00000, 0.00423)
(56500.00000, 0.00802)
(57000.00000, 0.00772)
(57500.00000, 0.00344)
(58000.00000, 0.00315)
(58500.00000, 0.00809)
(59000.00000, 0.01298)
(59500.00000, 0.00733)
(60000.00000, 0.00504)
(60500.00000, 0.00791)
(61000.00000, 0.00756)
(61500.00000, 0.01114)
(62000.00000, 0.00851)
(62500.00000, 0.00749)
(63000.00000, 0.00670)
(63500.00000, 0.00318)
(64000.00000, 0.00702)
(64500.00000, 0.00298)
(65000.00000, 0.00444)
(65500.00000, 0.00280)
(66000.00000, 0.00456)
(66500.00000, 0.00255)
(67000.00000, 0.00274)
(67500.00000, 0.00448)
(68000.00000, 0.00281)
(68500.00000, 0.00256)
(69000.00000, 0.00370)
(69500.00000, 0.00193)
(70000.00000, 0.00179)
(70500.00000, 0.00305)
(71000.00000, 0.00487)
(71500.00000, 0.00561)
(72000.00000, 0.00352)
(72500.00000, 0.00318)
(73000.00000, 0.00348)
(73500.00000, 0.00235)
(74000.00000, 0.00223)
(74500.00000, 0.00242)
(75000.00000, 0.00257)
(75500.00000, 0.00332)
(76000.00000, 0.00321)
(76500.00000, 0.00231)
(77000.00000, 0.00241)
(77500.00000, 0.00346)
(78000.00000, 0.00373)
(78500.00000, 0.00282)
(79000.00000, 0.00683)
(79500.00000, 0.00377)
(80000.00000, 0.00421)
(80500.00000, 0.00509)
(81000.00000, 0.00625)
(81500.00000, 0.00572)
(82000.00000, 0.00584)
(82500.00000, 0.00561)
(83000.00000, 0.00324)
(83500.00000, 0.00652)
(84000.00000, 0.00305)
(84500.00000, 0.00424)
(85000.00000, 0.00595)
(85500.00000, 0.00269)
(86000.00000, 0.00241)
(86500.00000, 0.00354)
(87000.00000, 0.00591)
(87500.00000, 0.00635)
(88000.00000, 0.00339)
(88500.00000, 0.00332)
(89000.00000, 0.00330)
(89500.00000, 0.00320)
(90000.00000, 0.00274)
(90500.00000, 0.00336)
(91000.00000, 0.00379)
(91500.00000, 0.00478)
(92000.00000, 0.00269)
(92500.00000, 0.00335)
(93000.00000, 0.00363)
(93500.00000, 0.00361)
(94000.00000, 0.00526)
(94500.00000, 0.00360)
(95000.00000, 0.00349)
(95500.00000, 0.00542)
(96000.00000, 0.00482)
(96500.00000, 0.00650)
(97000.00000, 0.00694)
(97500.00000, 0.00244)
(98000.00000, 0.00419)
(98500.00000, 0.00487)
(99000.00000, 0.00646)
(99500.00000, 0.00498)
(100000.00000, 0.00454)
(100500.00000, 0.00672)
(101000.00000, 0.00437)
(101500.00000, 0.00589)
(102000.00000, 0.00551)
(102500.00000, 0.00437)
(103000.00000, 0.00701)
(103500.00000, 0.00806)
(104000.00000, 0.00672)
(104500.00000, 0.00842)
(105000.00000, 0.00777)
(105500.00000, 0.00828)
(106000.00000, 0.00618)
(106500.00000, 0.00515)
(107000.00000, 0.00637)
(107500.00000, 0.00660)
(108000.00000, 0.00661)
(108500.00000, 0.00685)
(109000.00000, 0.00733)
(109500.00000, 0.00713)
(110000.00000, 0.00753)
(110500.00000, 0.00656)
(111000.00000, 0.00588)
(111500.00000, 0.00656)
(112000.00000, 0.00610)
(112500.00000, 0.00556)
(113000.00000, 0.00652)
(113500.00000, 0.00558)
(114000.00000, 0.00463)
(114500.00000, 0.00497)
(115000.00000, 0.00569)
(115500.00000, 0.00483)
(116000.00000, 0.00496)
(116500.00000, 0.00636)
(117000.00000, 0.00479)
(117500.00000, 0.00414)
(118000.00000, 0.00442)
(118500.00000, 0.00367)
(119000.00000, 0.00298)
(119500.00000, 0.00563)
(120000.00000, 0.00360)
(120500.00000, 0.00483)
(121000.00000, 0.00717)
(121500.00000, 0.00769)
(122000.00000, 0.00572)
(122500.00000, 0.00536)
(123000.00000, 0.00559)
(123500.00000, 0.00528)
(124000.00000, 0.00441)
(124500.00000, 0.00393)
(125000.00000, 0.00365)
(125500.00000, 0.00304)
(126000.00000, 0.00346)
(126500.00000, 0.00226)
(127000.00000, 0.00228)
(127500.00000, 0.00317)
(128000.00000, 0.00324)
(128500.00000, 0.00208)
(129000.00000, 0.00280)
(129500.00000, 0.00171)
(130000.00000, 0.00208)
(130500.00000, 0.00227)
(131000.00000, 0.00234)
(131500.00000, 0.00258)
(132000.00000, 0.00275)
(132500.00000, 0.00226)
(133000.00000, 0.00331)
(133500.00000, 0.00244)
(134000.00000, 0.00261)
(134500.00000, 0.00429)
(135000.00000, 0.00336)
(135500.00000, 0.00295)
(136000.00000, 0.00228)
(136500.00000, 0.00221)
(137000.00000, 0.00195)
(137500.00000, 0.00201)
(138000.00000, 0.00182)
(138500.00000, 0.00165)
(139000.00000, 0.00177)
(139500.00000, 0.00149)
(140000.00000, 0.00147)
(140500.00000, 0.00248)
(141000.00000, 0.00281)
(141500.00000, 0.00212)
(142000.00000, 0.00170)
(142500.00000, 0.00204)
(143000.00000, 0.00311)
(143500.00000, 0.00324)
(144000.00000, 0.00281)
(144500.00000, 0.00314)
(145000.00000, 0.00319)
(145500.00000, 0.00234)
(146000.00000, 0.00219)
(146500.00000, 0.00165)
(147000.00000, 0.00223)
(147500.00000, 0.00257)
(148000.00000, 0.00304)
(148500.00000, 0.00266)
(149000.00000, 0.00334)
(149500.00000, 0.00269)
(150000.00000, 0.00234)
(150500.00000, 0.00276)
(151000.00000, 0.00271)
(151500.00000, 0.00268)
(152000.00000, 0.00252)
(152500.00000, 0.00346)
(153000.00000, 0.00407)
(153500.00000, 0.00397)
(154000.00000, 0.00336)
(154500.00000, 0.00345)
(155000.00000, 0.00323)
(155500.00000, 0.00335)
(156000.00000, 0.00279)
(156500.00000, 0.00218)
(157000.00000, 0.00477)
(157500.00000, 0.00354)
(158000.00000, 0.00198)
(158500.00000, 0.00301)
(159000.00000, 0.00420)
(159500.00000, 0.00458)
(160000.00000, 0.00468)
(160500.00000, 0.00338)
(161000.00000, 0.00198)
(161500.00000, 0.00165)
(162000.00000, 0.00278)
(162500.00000, 0.00433)
(163000.00000, 0.00381)
(163500.00000, 0.00321)
(164000.00000, 0.00289)
(164500.00000, 0.00339)
(165000.00000, 0.00461)
(165500.00000, 0.00489)
(166000.00000, 0.00439)
(166500.00000, 0.00416)
(167000.00000, 0.00364)
(167500.00000, 0.00351)
(168000.00000, 0.00534)
(168500.00000, 0.00534)
(169000.00000, 0.00576)
(169500.00000, 0.00499)
(170000.00000, 0.00406)
(170500.00000, 0.00489)
(171000.00000, 0.00502)
(171500.00000, 0.00548)
(172000.00000, 0.00625)
(172500.00000, 0.00637)
(173000.00000, 0.00641)
(173500.00000, 0.00604)
(174000.00000, 0.00707)
(174500.00000, 0.00679)
(175000.00000, 0.00629)
(175500.00000, 0.00590)
(176000.00000, 0.00657)
(176500.00000, 0.00668)
(177000.00000, 0.00703)
(177500.00000, 0.00717)
(178000.00000, 0.00604)
(178500.00000, 0.00533)
(179000.00000, 0.00629)
(179500.00000, 0.00545)
(180000.00000, 0.00564)
(180500.00000, 0.00563)
(181000.00000, 0.00641)
(181500.00000, 0.00618)
(182000.00000, 0.00620)
(182500.00000, 0.00564)
(183000.00000, 0.00526)
(183500.00000, 0.00474)
(184000.00000, 0.00547)
(184500.00000, 0.00524)
(185000.00000, 0.00486)
(185500.00000, 0.00484)
(186000.00000, 0.00398)
(186500.00000, 0.00419)
(187000.00000, 0.00447)
(187500.00000, 0.00401)
(188000.00000, 0.00321)
(188500.00000, 0.00438)
(189000.00000, 0.00467)
(189500.00000, 0.00359)
(190000.00000, 0.00337)
(190500.00000, 0.00355)
(191000.00000, 0.00334)
(191500.00000, 0.00298)
(192000.00000, 0.00443)
(192500.00000, 0.00410)
(193000.00000, 0.00406)
(193500.00000, 0.00441)
(194000.00000, 0.00437)
(194500.00000, 0.00472)
(195000.00000, 0.00547)
(195500.00000, 0.00546)
(196000.00000, 0.00577)
(196500.00000, 0.00519)
(197000.00000, 0.00496)
(197500.00000, 0.00503)
(198000.00000, 0.00513)
(198500.00000, 0.00459)
(199000.00000, 0.00395)
(199500.00000, 0.00389)
(200000.00000, 0.00397)
(200500.00000, 0.00377)
(201000.00000, 0.00261)
(201500.00000, 0.00264)
(202000.00000, 0.00301)
(202500.00000, 0.00263)
(203000.00000, 0.00202)
(203500.00000, 0.00223)
(204000.00000, 0.00278)
(204500.00000, 0.00316)
(205000.00000, 0.00270)
(205500.00000, 0.00225)
(206000.00000, 0.00200)
(206500.00000, 0.00189)
(207000.00000, 0.00190)
(207500.00000, 0.00223)
(208000.00000, 0.00239)
(208500.00000, 0.00132)
(209000.00000, 0.00179)
(209500.00000, 0.00130)
(210000.00000, 0.00208)
(210500.00000, 0.00173)
(211000.00000, 0.00193)
(211500.00000, 0.00148)
(212000.00000, 0.00223)
(212500.00000, 0.00252)
(213000.00000, 0.00257)
(213500.00000, 0.00300)
(214000.00000, 0.00234)
(214500.00000, 0.00325)
(215000.00000, 0.00278)
(215500.00000, 0.00342)
(216000.00000, 0.00290)
(216500.00000, 0.00291)
(217000.00000, 0.00304)
(217500.00000, 0.00317)
(218000.00000, 0.00273)
(218500.00000, 0.00215)
(219000.00000, 0.00248)
(219500.00000, 0.00321)
(220000.00000, 0.00336)
(220500.00000, 0.00324)
(221000.00000, 0.00325)
(221500.00000, 0.00266)
(222000.00000, 0.00291)
(222500.00000, 0.00258)
(223000.00000, 0.00205)
(223500.00000, 0.00351)
(224000.00000, 0.00232)
(224500.00000, 0.00293)
(225000.00000, 0.00375)
(225500.00000, 0.00378)
(226000.00000, 0.00360)
(226500.00000, 0.00365)
(227000.00000, 0.00381)
(227500.00000, 0.00276)
(228000.00000, 0.00417)
(228500.00000, 0.00326)
(229000.00000, 0.00329)
(229500.00000, 0.00358)
(230000.00000, 0.00337)
(230500.00000, 0.00298)
(231000.00000, 0.00404)
(231500.00000, 0.00476)
(232000.00000, 0.00422)
(232500.00000, 0.00422)
(233000.00000, 0.00361)
(233500.00000, 0.00339)
(234000.00000, 0.00405)
(234500.00000, 0.00415)
(235000.00000, 0.00386)
(235500.00000, 0.00427)
(236000.00000, 0.00381)
(236500.00000, 0.00354)
(237000.00000, 0.00349)
(237500.00000, 0.00362)
(238000.00000, 0.00417)
(238500.00000, 0.00324)
(239000.00000, 0.00342)
(239500.00000, 0.00400)
(240000.00000, 0.00384)
(240500.00000, 0.00389)
(241000.00000, 0.00403)
(241500.00000, 0.00348)
(242000.00000, 0.00263)
(242500.00000, 0.00247)
(243000.00000, 0.00248)
(243500.00000, 0.00339)
(244000.00000, 0.00287)
(244500.00000, 0.00267)
(245000.00000, 0.00436)
(245500.00000, 0.00336)
(246000.00000, 0.00452)
(246500.00000, 0.00350)
(247000.00000, 0.00329)
(247500.00000, 0.00413)
(248000.00000, 0.00378)
(248500.00000, 0.00338)
(249000.00000, 0.00409)
(249500.00000, 0.00433)
(250000.00000, 0.00410)
(250500.00000, 0.00340)
(251000.00000, 0.00356)
(251500.00000, 0.00380)
(252000.00000, 0.00374)
(252500.00000, 0.00356)
(253000.00000, 0.00385)
(253500.00000, 0.00374)
(254000.00000, 0.00359)
};
\addplot[thin,only marks, mark options={opacity=0.9},mark=*,mark size=.5pt,Yellow3] plot coordinates {
(1000.00000, 0.01792)
(1500.00000, 0.02223)
(2000.00000, 0.01841)
(2500.00000, 0.01666)
(3000.00000, 0.00970)
(3500.00000, 0.01115)
(4000.00000, 0.01116)
(4500.00000, 0.01057)
(5000.00000, 0.00789)
(5500.00000, 0.00655)
(6000.00000, 0.00874)
(6500.00000, 0.00762)
(7000.00000, 0.00852)
(7500.00000, 0.00737)
(8000.00000, 0.00800)
(8500.00000, 0.00682)
(9000.00000, 0.00583)
(9500.00000, 0.00664)
(10000.00000, 0.00683)
(10500.00000, 0.00590)
(11000.00000, 0.00497)
(11500.00000, 0.00669)
(12000.00000, 0.00528)
(12500.00000, 0.00613)
(13000.00000, 0.00571)
(13500.00000, 0.00527)
(14000.00000, 0.00588)
(14500.00000, 0.00622)
(15000.00000, 0.00441)
(15500.00000, 0.00455)
(16000.00000, 0.00489)
(16500.00000, 0.00463)
(17000.00000, 0.00402)
(17500.00000, 0.00564)
(18000.00000, 0.00445)
(18500.00000, 0.00364)
(19000.00000, 0.00297)
(19500.00000, 0.00401)
(20000.00000, 0.00387)
(20500.00000, 0.00424)
(21000.00000, 0.00563)
(21500.00000, 0.00472)
(22000.00000, 0.00410)
(22500.00000, 0.00511)
(23000.00000, 0.00435)
(23500.00000, 0.00506)
(24000.00000, 0.00537)
(24500.00000, 0.00618)
(25000.00000, 0.00576)
(25500.00000, 0.00452)
(26000.00000, 0.00516)
(26500.00000, 0.00510)
(27000.00000, 0.00454)
(27500.00000, 0.00488)
(28000.00000, 0.00428)
(28500.00000, 0.00435)
(29000.00000, 0.00381)
(29500.00000, 0.00474)
(30000.00000, 0.00561)
(30500.00000, 0.00431)
(31000.00000, 0.00521)
(31500.00000, 0.00670)
(32000.00000, 0.00680)
(32500.00000, 0.00562)
(33000.00000, 0.00612)
(33500.00000, 0.00564)
(34000.00000, 0.00465)
(34500.00000, 0.00477)
(35000.00000, 0.00453)
(35500.00000, 0.00560)
(36000.00000, 0.00480)
(36500.00000, 0.00329)
(37000.00000, 0.00515)
(37500.00000, 0.00474)
(38000.00000, 0.00380)
(38500.00000, 0.00450)
(39000.00000, 0.00567)
(39500.00000, 0.00460)
(40000.00000, 0.00419)
(40500.00000, 0.00554)
(41000.00000, 0.00427)
(41500.00000, 0.00403)
(42000.00000, 0.00399)
(42500.00000, 0.00403)
(43000.00000, 0.00320)
(43500.00000, 0.00354)
(44000.00000, 0.00291)
(44500.00000, 0.00296)
(45000.00000, 0.00292)
(45500.00000, 0.00240)
(46000.00000, 0.00249)
(46500.00000, 0.00275)
(47000.00000, 0.00298)
(47500.00000, 0.00252)
(48000.00000, 0.00276)
(48500.00000, 0.00289)
(49000.00000, 0.00303)
(49500.00000, 0.00243)
(50000.00000, 0.00288)
(50500.00000, 0.00300)
(51000.00000, 0.00303)
(51500.00000, 0.00297)
(52000.00000, 0.00242)
(52500.00000, 0.00271)
(53000.00000, 0.00242)
(53500.00000, 0.00261)
(54000.00000, 0.00250)
(54500.00000, 0.00372)
(55000.00000, 0.00268)
(55500.00000, 0.00207)
(56000.00000, 0.00233)
(56500.00000, 0.00235)
(57000.00000, 0.00272)
(57500.00000, 0.00276)
(58000.00000, 0.00175)
(58500.00000, 0.00214)
(59000.00000, 0.00203)
(59500.00000, 0.00229)
(60000.00000, 0.00242)
(60500.00000, 0.00228)
(61000.00000, 0.00225)
(61500.00000, 0.00245)
(62000.00000, 0.00262)
(62500.00000, 0.00244)
(63000.00000, 0.00229)
(63500.00000, 0.00220)
(64000.00000, 0.00226)
(64500.00000, 0.00203)
(65000.00000, 0.00243)
(65500.00000, 0.00301)
(66000.00000, 0.00240)
(66500.00000, 0.00218)
(67000.00000, 0.00291)
(67500.00000, 0.00285)
(68000.00000, 0.00241)
(68500.00000, 0.00284)
(69000.00000, 0.00237)
(69500.00000, 0.00244)
(70000.00000, 0.00201)
(70500.00000, 0.00246)
(71000.00000, 0.00217)
(71500.00000, 0.00255)
(72000.00000, 0.00293)
(72500.00000, 0.00250)
(73000.00000, 0.00221)
(73500.00000, 0.00247)
(74000.00000, 0.00258)
(74500.00000, 0.00243)
(75000.00000, 0.00220)
(75500.00000, 0.00254)
(76000.00000, 0.00225)
(76500.00000, 0.00242)
(77000.00000, 0.00179)
(77500.00000, 0.00227)
(78000.00000, 0.00207)
(78500.00000, 0.00210)
(79000.00000, 0.00190)
(79500.00000, 0.00194)
(80000.00000, 0.00212)
(80500.00000, 0.00199)
(81000.00000, 0.00212)
(81500.00000, 0.00227)
(82000.00000, 0.00192)
(82500.00000, 0.00206)
(83000.00000, 0.00233)
(83500.00000, 0.00228)
(84000.00000, 0.00262)
(84500.00000, 0.00239)
(85000.00000, 0.00259)
(85500.00000, 0.00229)
(86000.00000, 0.00241)
(86500.00000, 0.00202)
(87000.00000, 0.00219)
(87500.00000, 0.00242)
(88000.00000, 0.00251)
(88500.00000, 0.00254)
(89000.00000, 0.00202)
(89500.00000, 0.00201)
(90000.00000, 0.00276)
(90500.00000, 0.00214)
(91000.00000, 0.00212)
(91500.00000, 0.00223)
(92000.00000, 0.00225)
(92500.00000, 0.00216)
(93000.00000, 0.00238)
(93500.00000, 0.00246)
(94000.00000, 0.00209)
(94500.00000, 0.00192)
(95000.00000, 0.00170)
(95500.00000, 0.00190)
(96000.00000, 0.00215)
(96500.00000, 0.00208)
(97000.00000, 0.00212)
(97500.00000, 0.00239)
(98000.00000, 0.00216)
(98500.00000, 0.00210)
(99000.00000, 0.00189)
(99500.00000, 0.00191)
(100000.00000, 0.00174)
(100500.00000, 0.00244)
(101000.00000, 0.00213)
(101500.00000, 0.00227)
(102000.00000, 0.00256)
(102500.00000, 0.00226)
(103000.00000, 0.00230)
(103500.00000, 0.00187)
(104000.00000, 0.00236)
(104500.00000, 0.00209)
(105000.00000, 0.00198)
(105500.00000, 0.00228)
(106000.00000, 0.00217)
(106500.00000, 0.00185)
(107000.00000, 0.00183)
(107500.00000, 0.00211)
(108000.00000, 0.00197)
(108500.00000, 0.00155)
(109000.00000, 0.00163)
(109500.00000, 0.00208)
(110000.00000, 0.00219)
(110500.00000, 0.00207)
(111000.00000, 0.00161)
(111500.00000, 0.00171)
(112000.00000, 0.00131)
(112500.00000, 0.00198)
(113000.00000, 0.00163)
(113500.00000, 0.00167)
(114000.00000, 0.00177)
(114500.00000, 0.00168)
(115000.00000, 0.00170)
(115500.00000, 0.00201)
(116000.00000, 0.00176)
(116500.00000, 0.00188)
(117000.00000, 0.00147)
(117500.00000, 0.00168)
(118000.00000, 0.00169)
(118500.00000, 0.00144)
(119000.00000, 0.00182)
(119500.00000, 0.00164)
(120000.00000, 0.00157)
(120500.00000, 0.00145)
(121000.00000, 0.00151)
(121500.00000, 0.00173)
(122000.00000, 0.00173)
(122500.00000, 0.00162)
(123000.00000, 0.00192)
(123500.00000, 0.00162)
(124000.00000, 0.00172)
(124500.00000, 0.00173)
(125000.00000, 0.00157)
(125500.00000, 0.00143)
(126000.00000, 0.00161)
(126500.00000, 0.00185)
(127000.00000, 0.00169)
(127500.00000, 0.00186)
(128000.00000, 0.00150)
(128500.00000, 0.00179)
(129000.00000, 0.00184)
(129500.00000, 0.00163)
(130000.00000, 0.00184)
(130500.00000, 0.00138)
(131000.00000, 0.00170)
(131500.00000, 0.00170)
(132000.00000, 0.00167)
(132500.00000, 0.00207)
(133000.00000, 0.00167)
(133500.00000, 0.00154)
(134000.00000, 0.00147)
(134500.00000, 0.00138)
(135000.00000, 0.00125)
(135500.00000, 0.00117)
(136000.00000, 0.00135)
(136500.00000, 0.00152)
(137000.00000, 0.00144)
(137500.00000, 0.00172)
(138000.00000, 0.00142)
(138500.00000, 0.00156)
(139000.00000, 0.00158)
(139500.00000, 0.00167)
(140000.00000, 0.00148)
(140500.00000, 0.00152)
(141000.00000, 0.00154)
(141500.00000, 0.00160)
(142000.00000, 0.00175)
(142500.00000, 0.00162)
(143000.00000, 0.00165)
(143500.00000, 0.00159)
(144000.00000, 0.00162)
(144500.00000, 0.00162)
(145000.00000, 0.00167)
(145500.00000, 0.00177)
(146000.00000, 0.00152)
(146500.00000, 0.00171)
(147000.00000, 0.00161)
(147500.00000, 0.00152)
(148000.00000, 0.00161)
(148500.00000, 0.00210)
(149000.00000, 0.00162)
(149500.00000, 0.00176)
(150000.00000, 0.00145)
(150500.00000, 0.00150)
(151000.00000, 0.00158)
(151500.00000, 0.00191)
(152000.00000, 0.00131)
(152500.00000, 0.00136)
(153000.00000, 0.00160)
(153500.00000, 0.00174)
(154000.00000, 0.00138)
(154500.00000, 0.00149)
(155000.00000, 0.00128)
(155500.00000, 0.00135)
(156000.00000, 0.00149)
(156500.00000, 0.00152)
(157000.00000, 0.00123)
(157500.00000, 0.00117)
(158000.00000, 0.00115)
(158500.00000, 0.00139)
(159000.00000, 0.00168)
(159500.00000, 0.00127)
(160000.00000, 0.00156)
(160500.00000, 0.00142)
(161000.00000, 0.00153)
(161500.00000, 0.00140)
(162000.00000, 0.00150)
(162500.00000, 0.00138)
(163000.00000, 0.00118)
(163500.00000, 0.00117)
(164000.00000, 0.00147)
(164500.00000, 0.00166)
(165000.00000, 0.00153)
(165500.00000, 0.00151)
(166000.00000, 0.00116)
(166500.00000, 0.00138)
(167000.00000, 0.00141)
(167500.00000, 0.00121)
(168000.00000, 0.00128)
(168500.00000, 0.00122)
(169000.00000, 0.00168)
(169500.00000, 0.00155)
(170000.00000, 0.00141)
(170500.00000, 0.00131)
(171000.00000, 0.00138)
(171500.00000, 0.00122)
(172000.00000, 0.00137)
(172500.00000, 0.00137)
(173000.00000, 0.00135)
(173500.00000, 0.00127)
(174000.00000, 0.00157)
(174500.00000, 0.00135)
(175000.00000, 0.00135)
(175500.00000, 0.00130)
(176000.00000, 0.00144)
(176500.00000, 0.00139)
(177000.00000, 0.00138)
(177500.00000, 0.00121)
(178000.00000, 0.00114)
(178500.00000, 0.00119)
(179000.00000, 0.00159)
(179500.00000, 0.00125)
(180000.00000, 0.00158)
(180500.00000, 0.00110)
(181000.00000, 0.00145)
(181500.00000, 0.00155)
(182000.00000, 0.00127)
(182500.00000, 0.00134)
(183000.00000, 0.00140)
(183500.00000, 0.00134)
(184000.00000, 0.00118)
(184500.00000, 0.00141)
(185000.00000, 0.00151)
(185500.00000, 0.00143)
(186000.00000, 0.00134)
(186500.00000, 0.00123)
(187000.00000, 0.00146)
(187500.00000, 0.00160)
(188000.00000, 0.00124)
(188500.00000, 0.00134)
(189000.00000, 0.00133)
(189500.00000, 0.00135)
(190000.00000, 0.00143)
(190500.00000, 0.00138)
(191000.00000, 0.00147)
(191500.00000, 0.00149)
(192000.00000, 0.00144)
(192500.00000, 0.00155)
(193000.00000, 0.00161)
(193500.00000, 0.00127)
(194000.00000, 0.00133)
(194500.00000, 0.00160)
(195000.00000, 0.00168)
(195500.00000, 0.00160)
(196000.00000, 0.00152)
(196500.00000, 0.00175)
(197000.00000, 0.00169)
(197500.00000, 0.00138)
(198000.00000, 0.00151)
(198500.00000, 0.00133)
(199000.00000, 0.00172)
(199500.00000, 0.00155)
(200000.00000, 0.00171)
(200500.00000, 0.00159)
(201000.00000, 0.00158)
(201500.00000, 0.00140)
(202000.00000, 0.00150)
(202500.00000, 0.00126)
(203000.00000, 0.00154)
(203500.00000, 0.00133)
(204000.00000, 0.00114)
(204500.00000, 0.00145)
(205000.00000, 0.00160)
(205500.00000, 0.00161)
(206000.00000, 0.00142)
(206500.00000, 0.00133)
(207000.00000, 0.00120)
(207500.00000, 0.00124)
(208000.00000, 0.00119)
(208500.00000, 0.00127)
(209000.00000, 0.00115)
(209500.00000, 0.00101)
(210000.00000, 0.00140)
(210500.00000, 0.00137)
(211000.00000, 0.00123)
(211500.00000, 0.00135)
(212000.00000, 0.00135)
(212500.00000, 0.00132)
(213000.00000, 0.00132)
(213500.00000, 0.00129)
(214000.00000, 0.00119)
(214500.00000, 0.00133)
(215000.00000, 0.00130)
(215500.00000, 0.00142)
(216000.00000, 0.00103)
(216500.00000, 0.00139)
(217000.00000, 0.00138)
(217500.00000, 0.00121)
(218000.00000, 0.00114)
(218500.00000, 0.00118)
(219000.00000, 0.00139)
(219500.00000, 0.00130)
(220000.00000, 0.00131)
(220500.00000, 0.00115)
(221000.00000, 0.00123)
(221500.00000, 0.00135)
(222000.00000, 0.00107)
(222500.00000, 0.00134)
(223000.00000, 0.00132)
(223500.00000, 0.00133)
(224000.00000, 0.00121)
(224500.00000, 0.00154)
(225000.00000, 0.00153)
(225500.00000, 0.00144)
(226000.00000, 0.00128)
(226500.00000, 0.00128)
(227000.00000, 0.00140)
(227500.00000, 0.00138)
(228000.00000, 0.00120)
(228500.00000, 0.00146)
(229000.00000, 0.00142)
(229500.00000, 0.00116)
(230000.00000, 0.00104)
(230500.00000, 0.00136)
(231000.00000, 0.00136)
(231500.00000, 0.00115)
(232000.00000, 0.00106)
(232500.00000, 0.00112)
(233000.00000, 0.00143)
(233500.00000, 0.00147)
(234000.00000, 0.00119)
(234500.00000, 0.00118)
(235000.00000, 0.00131)
(235500.00000, 0.00155)
(236000.00000, 0.00129)
(236500.00000, 0.00134)
(237000.00000, 0.00127)
(237500.00000, 0.00130)
(238000.00000, 0.00140)
(238500.00000, 0.00117)
(239000.00000, 0.00143)
(239500.00000, 0.00125)
(240000.00000, 0.00107)
(240500.00000, 0.00117)
(241000.00000, 0.00146)
(241500.00000, 0.00139)
(242000.00000, 0.00119)
(242500.00000, 0.00140)
(243000.00000, 0.00130)
(243500.00000, 0.00138)
(244000.00000, 0.00130)
(244500.00000, 0.00118)
(245000.00000, 0.00144)
(245500.00000, 0.00129)
(246000.00000, 0.00133)
(246500.00000, 0.00110)
(247000.00000, 0.00126)
(247500.00000, 0.00114)
(248000.00000, 0.00122)
(248500.00000, 0.00137)
(249000.00000, 0.00143)
(249500.00000, 0.00155)
(250000.00000, 0.00137)
(250500.00000, 0.00190)
(251000.00000, 0.00139)
(251500.00000, 0.00125)
(252000.00000, 0.00155)
(252500.00000, 0.00124)
(253000.00000, 0.00133)
(253500.00000, 0.00146)
(254000.00000, 0.00125)
};
\addplot[thin,only marks, mark options={opacity=0.9},mark=*,mark size=.5pt,IndianRed2] plot coordinates {
(1000.00000, 0.08708)
(1500.00000, 0.03616)
(2000.00000, 0.01691)
(2500.00000, 0.02147)
(3000.00000, 0.02436)
(3500.00000, 0.02547)
(4000.00000, 0.01628)
(4500.00000, 0.01240)
(5000.00000, 0.02186)
(5500.00000, 0.00775)
(6000.00000, 0.00691)
(6500.00000, 0.00842)
(7000.00000, 0.01009)
(7500.00000, 0.00656)
(8000.00000, 0.00639)
(8500.00000, 0.00905)
(9000.00000, 0.00528)
(9500.00000, 0.00670)
(10000.00000, 0.01934)
(10500.00000, 0.00647)
(11000.00000, 0.00452)
(11500.00000, 0.00537)
(12000.00000, 0.00453)
(12500.00000, 0.00805)
(13000.00000, 0.01390)
(13500.00000, 0.00768)
(14000.00000, 0.00442)
(14500.00000, 0.00433)
(15000.00000, 0.00654)
(15500.00000, 0.00560)
(16000.00000, 0.00457)
(16500.00000, 0.00636)
(17000.00000, 0.00698)
(17500.00000, 0.00552)
(18000.00000, 0.00811)
(18500.00000, 0.00426)
(19000.00000, 0.00548)
(19500.00000, 0.00529)
(20000.00000, 0.00455)
(20500.00000, 0.00635)
(21000.00000, 0.00525)
(21500.00000, 0.00392)
(22000.00000, 0.00505)
(22500.00000, 0.00523)
(23000.00000, 0.00329)
(23500.00000, 0.00417)
(24000.00000, 0.00371)
(24500.00000, 0.00431)
(25000.00000, 0.00428)
(25500.00000, 0.00391)
(26000.00000, 0.00669)
(26500.00000, 0.00368)
(27000.00000, 0.00407)
(27500.00000, 0.00391)
(28000.00000, 0.00519)
(28500.00000, 0.00397)
(29000.00000, 0.00437)
(29500.00000, 0.00307)
(30000.00000, 0.00501)
(30500.00000, 0.00590)
(31000.00000, 0.00615)
(31500.00000, 0.00318)
(32000.00000, 0.00491)
(32500.00000, 0.00467)
(33000.00000, 0.00367)
(33500.00000, 0.00465)
(34000.00000, 0.00278)
(34500.00000, 0.00367)
(35000.00000, 0.00509)
(35500.00000, 0.00380)
(36000.00000, 0.00892)
(36500.00000, 0.00581)
(37000.00000, 0.00333)
(37500.00000, 0.00581)
(38000.00000, 0.00438)
(38500.00000, 0.00604)
(39000.00000, 0.00325)
(39500.00000, 0.00239)
(40000.00000, 0.00356)
(40500.00000, 0.00323)
(41000.00000, 0.00338)
(41500.00000, 0.00289)
(42000.00000, 0.00417)
(42500.00000, 0.00493)
(43000.00000, 0.00520)
(43500.00000, 0.00268)
(44000.00000, 0.00255)
(44500.00000, 0.00297)
(45000.00000, 0.00290)
(45500.00000, 0.00261)
(46000.00000, 0.00264)
(46500.00000, 0.00249)
(47000.00000, 0.00273)
(47500.00000, 0.00247)
(48000.00000, 0.00273)
(48500.00000, 0.00305)
(49000.00000, 0.00237)
(49500.00000, 0.00247)
(50000.00000, 0.00302)
(50500.00000, 0.00263)
(51000.00000, 0.00251)
(51500.00000, 0.00288)
(52000.00000, 0.00329)
(52500.00000, 0.00263)
(53000.00000, 0.00247)
(53500.00000, 0.00274)
(54000.00000, 0.00241)
(54500.00000, 0.00302)
(55000.00000, 0.00256)
(55500.00000, 0.00290)
(56000.00000, 0.00251)
(56500.00000, 0.00240)
(57000.00000, 0.00241)
(57500.00000, 0.00480)
(58000.00000, 0.00423)
(58500.00000, 0.00682)
(59000.00000, 0.00329)
(59500.00000, 0.00311)
(60000.00000, 0.00293)
(60500.00000, 0.00489)
(61000.00000, 0.00358)
(61500.00000, 0.00282)
(62000.00000, 0.00542)
(62500.00000, 0.00448)
(63000.00000, 0.00208)
(63500.00000, 0.00333)
(64000.00000, 0.00409)
(64500.00000, 0.00425)
(65000.00000, 0.00340)
(65500.00000, 0.00399)
(66000.00000, 0.00355)
(66500.00000, 0.00349)
(67000.00000, 0.00301)
(67500.00000, 0.00333)
(68000.00000, 0.00437)
(68500.00000, 0.00370)
(69000.00000, 0.00337)
(69500.00000, 0.00278)
(70000.00000, 0.00328)
(70500.00000, 0.00272)
(71000.00000, 0.00239)
(71500.00000, 0.00197)
(72000.00000, 0.00360)
(72500.00000, 0.00260)
(73000.00000, 0.00320)
(73500.00000, 0.00325)
(74000.00000, 0.00327)
(74500.00000, 0.00272)
(75000.00000, 0.00253)
(75500.00000, 0.00311)
(76000.00000, 0.00275)
(76500.00000, 0.00286)
(77000.00000, 0.00254)
(77500.00000, 0.00306)
(78000.00000, 0.00333)
(78500.00000, 0.00282)
(79000.00000, 0.00251)
(79500.00000, 0.00275)
(80000.00000, 0.00304)
(80500.00000, 0.00347)
(81000.00000, 0.00235)
(81500.00000, 0.00220)
(82000.00000, 0.00256)
(82500.00000, 0.00315)
(83000.00000, 0.00312)
(83500.00000, 0.00296)
(84000.00000, 0.00226)
(84500.00000, 0.00320)
(85000.00000, 0.00404)
(85500.00000, 0.00305)
(86000.00000, 0.00211)
(86500.00000, 0.00214)
(87000.00000, 0.00264)
(87500.00000, 0.00236)
(88000.00000, 0.00217)
(88500.00000, 0.00275)
(89000.00000, 0.00264)
(89500.00000, 0.00210)
(90000.00000, 0.00185)
(90500.00000, 0.00270)
(91000.00000, 0.00300)
(91500.00000, 0.00322)
(92000.00000, 0.00294)
(92500.00000, 0.00237)
(93000.00000, 0.00253)
(93500.00000, 0.00221)
(94000.00000, 0.00223)
(94500.00000, 0.00271)
(95000.00000, 0.00289)
(95500.00000, 0.00253)
(96000.00000, 0.00306)
(96500.00000, 0.00310)
(97000.00000, 0.00312)
(97500.00000, 0.00298)
(98000.00000, 0.00320)
(98500.00000, 0.00329)
(99000.00000, 0.00240)
(99500.00000, 0.00270)
(100000.00000, 0.00262)
(100500.00000, 0.00261)
(101000.00000, 0.00295)
(101500.00000, 0.00273)
(102000.00000, 0.00224)
(102500.00000, 0.00210)
(103000.00000, 0.00355)
(103500.00000, 0.00215)
(104000.00000, 0.00241)
(104500.00000, 0.00232)
(105000.00000, 0.00240)
(105500.00000, 0.00288)
(106000.00000, 0.00267)
(106500.00000, 0.00289)
(107000.00000, 0.00193)
(107500.00000, 0.00219)
(108000.00000, 0.00236)
(108500.00000, 0.00214)
(109000.00000, 0.00249)
(109500.00000, 0.00304)
(110000.00000, 0.00360)
(110500.00000, 0.00297)
(111000.00000, 0.00258)
(111500.00000, 0.00290)
(112000.00000, 0.00306)
(112500.00000, 0.00302)
(113000.00000, 0.00322)
(113500.00000, 0.00249)
(114000.00000, 0.00189)
(114500.00000, 0.00237)
(115000.00000, 0.00213)
(115500.00000, 0.00199)
(116000.00000, 0.00204)
(116500.00000, 0.00242)
(117000.00000, 0.00170)
(117500.00000, 0.00210)
(118000.00000, 0.00239)
(118500.00000, 0.00285)
(119000.00000, 0.00352)
(119500.00000, 0.00380)
(120000.00000, 0.00197)
(120500.00000, 0.00184)
(121000.00000, 0.00180)
(121500.00000, 0.00236)
(122000.00000, 0.00243)
(122500.00000, 0.00375)
(123000.00000, 0.00394)
(123500.00000, 0.00323)
(124000.00000, 0.00253)
(124500.00000, 0.00284)
(125000.00000, 0.00284)
(125500.00000, 0.00273)
(126000.00000, 0.00320)
(126500.00000, 0.00317)
(127000.00000, 0.00272)
(127500.00000, 0.00254)
(128000.00000, 0.00266)
(128500.00000, 0.00260)
(129000.00000, 0.00211)
(129500.00000, 0.00264)
(130000.00000, 0.00234)
(130500.00000, 0.00270)
(131000.00000, 0.00220)
(131500.00000, 0.00184)
(132000.00000, 0.00208)
(132500.00000, 0.00256)
(133000.00000, 0.00176)
(133500.00000, 0.00227)
(134000.00000, 0.00298)
(134500.00000, 0.00301)
(135000.00000, 0.00254)
(135500.00000, 0.00276)
(136000.00000, 0.00222)
(136500.00000, 0.00271)
(137000.00000, 0.00290)
(137500.00000, 0.00340)
(138000.00000, 0.00298)
(138500.00000, 0.00274)
(139000.00000, 0.00229)
(139500.00000, 0.00263)
(140000.00000, 0.00320)
(140500.00000, 0.00278)
(141000.00000, 0.00276)
(141500.00000, 0.00257)
(142000.00000, 0.00299)
(142500.00000, 0.00355)
(143000.00000, 0.00345)
(143500.00000, 0.00360)
(144000.00000, 0.00216)
(144500.00000, 0.00220)
(145000.00000, 0.00301)
(145500.00000, 0.00213)
(146000.00000, 0.00217)
(146500.00000, 0.00416)
(147000.00000, 0.00209)
(147500.00000, 0.00167)
(148000.00000, 0.00289)
(148500.00000, 0.00357)
(149000.00000, 0.00334)
(149500.00000, 0.00230)
(150000.00000, 0.00262)
(150500.00000, 0.00278)
(151000.00000, 0.00256)
(151500.00000, 0.00283)
(152000.00000, 0.00258)
(152500.00000, 0.00301)
(153000.00000, 0.00261)
(153500.00000, 0.00286)
(154000.00000, 0.00236)
(154500.00000, 0.00245)
(155000.00000, 0.00261)
(155500.00000, 0.00249)
(156000.00000, 0.00198)
(156500.00000, 0.00204)
(157000.00000, 0.00173)
(157500.00000, 0.00155)
(158000.00000, 0.00151)
(158500.00000, 0.00246)
(159000.00000, 0.00180)
(159500.00000, 0.00156)
(160000.00000, 0.00237)
(160500.00000, 0.00155)
(161000.00000, 0.00184)
(161500.00000, 0.00180)
(162000.00000, 0.00136)
(162500.00000, 0.00176)
(163000.00000, 0.00182)
(163500.00000, 0.00153)
(164000.00000, 0.00153)
(164500.00000, 0.00224)
(165000.00000, 0.00171)
(165500.00000, 0.00153)
(166000.00000, 0.00137)
(166500.00000, 0.00155)
(167000.00000, 0.00152)
(167500.00000, 0.00187)
(168000.00000, 0.00130)
(168500.00000, 0.00212)
(169000.00000, 0.00136)
(169500.00000, 0.00155)
(170000.00000, 0.00146)
(170500.00000, 0.00162)
(171000.00000, 0.00133)
(171500.00000, 0.00162)
(172000.00000, 0.00131)
(172500.00000, 0.00144)
(173000.00000, 0.00156)
(173500.00000, 0.00159)
(174000.00000, 0.00131)
(174500.00000, 0.00157)
(175000.00000, 0.00156)
(175500.00000, 0.00146)
(176000.00000, 0.00150)
(176500.00000, 0.00152)
(177000.00000, 0.00138)
(177500.00000, 0.00134)
(178000.00000, 0.00150)
(178500.00000, 0.00136)
(179000.00000, 0.00138)
(179500.00000, 0.00141)
(180000.00000, 0.00126)
(180500.00000, 0.00154)
(181000.00000, 0.00119)
(181500.00000, 0.00136)
(182000.00000, 0.00136)
(182500.00000, 0.00154)
(183000.00000, 0.00151)
(183500.00000, 0.00133)
(184000.00000, 0.00151)
(184500.00000, 0.00132)
(185000.00000, 0.00131)
(185500.00000, 0.00135)
(186000.00000, 0.00141)
(186500.00000, 0.00137)
(187000.00000, 0.00162)
(187500.00000, 0.00186)
(188000.00000, 0.00142)
(188500.00000, 0.00168)
(189000.00000, 0.00179)
(189500.00000, 0.00133)
(190000.00000, 0.00175)
(190500.00000, 0.00133)
(191000.00000, 0.00132)
(191500.00000, 0.00110)
(192000.00000, 0.00129)
(192500.00000, 0.00176)
(193000.00000, 0.00131)
(193500.00000, 0.00162)
(194000.00000, 0.00130)
(194500.00000, 0.00094)
(195000.00000, 0.00133)
(195500.00000, 0.00118)
(196000.00000, 0.00129)
(196500.00000, 0.00142)
(197000.00000, 0.00135)
(197500.00000, 0.00149)
(198000.00000, 0.00105)
(198500.00000, 0.00112)
(199000.00000, 0.00153)
(199500.00000, 0.00139)
(200000.00000, 0.00098)
(200500.00000, 0.00129)
(201000.00000, 0.00105)
(201500.00000, 0.00151)
(202000.00000, 0.00126)
(202500.00000, 0.00140)
(203000.00000, 0.00156)
(203500.00000, 0.00136)
(204000.00000, 0.00171)
(204500.00000, 0.00162)
(205000.00000, 0.00172)
(205500.00000, 0.00128)
(206000.00000, 0.00155)
(206500.00000, 0.00157)
(207000.00000, 0.00193)
(207500.00000, 0.00141)
(208000.00000, 0.00139)
(208500.00000, 0.00111)
(209000.00000, 0.00193)
(209500.00000, 0.00143)
(210000.00000, 0.00163)
(210500.00000, 0.00154)
(211000.00000, 0.00132)
(211500.00000, 0.00141)
(212000.00000, 0.00115)
(212500.00000, 0.00101)
(213000.00000, 0.00141)
(213500.00000, 0.00102)
(214000.00000, 0.00128)
(214500.00000, 0.00156)
(215000.00000, 0.00111)
(215500.00000, 0.00121)
(216000.00000, 0.00134)
(216500.00000, 0.00134)
(217000.00000, 0.00132)
(217500.00000, 0.00133)
(218000.00000, 0.00136)
(218500.00000, 0.00125)
(219000.00000, 0.00110)
(219500.00000, 0.00109)
(220000.00000, 0.00130)
(220500.00000, 0.00115)
(221000.00000, 0.00145)
(221500.00000, 0.00146)
(222000.00000, 0.00142)
(222500.00000, 0.00132)
(223000.00000, 0.00151)
(223500.00000, 0.00122)
(224000.00000, 0.00119)
(224500.00000, 0.00111)
(225000.00000, 0.00117)
(225500.00000, 0.00101)
(226000.00000, 0.00118)
(226500.00000, 0.00125)
(227000.00000, 0.00130)
(227500.00000, 0.00207)
(228000.00000, 0.00220)
(228500.00000, 0.00173)
(229000.00000, 0.00137)
(229500.00000, 0.00157)
(230000.00000, 0.00203)
(230500.00000, 0.00182)
(231000.00000, 0.00213)
(231500.00000, 0.00223)
(232000.00000, 0.00252)
(232500.00000, 0.00165)
(233000.00000, 0.00163)
(233500.00000, 0.00144)
(234000.00000, 0.00248)
(234500.00000, 0.00182)
(235000.00000, 0.00150)
(235500.00000, 0.00119)
(236000.00000, 0.00165)
(236500.00000, 0.00141)
(237000.00000, 0.00194)
(237500.00000, 0.00185)
(238000.00000, 0.00131)
(238500.00000, 0.00109)
(239000.00000, 0.00169)
(239500.00000, 0.00164)
(240000.00000, 0.00120)
(240500.00000, 0.00168)
(241000.00000, 0.00165)
(241500.00000, 0.00146)
(242000.00000, 0.00192)
(242500.00000, 0.00152)
(243000.00000, 0.00139)
(243500.00000, 0.00115)
(244000.00000, 0.00114)
(244500.00000, 0.00164)
(245000.00000, 0.00125)
(245500.00000, 0.00178)
(246000.00000, 0.00174)
(246500.00000, 0.00180)
(247000.00000, 0.00132)
(247500.00000, 0.00183)
(248000.00000, 0.00158)
(248500.00000, 0.00141)
(249000.00000, 0.00142)
(249500.00000, 0.00111)
(250000.00000, 0.00137)
(250500.00000, 0.00107)
(251000.00000, 0.00161)
(251500.00000, 0.00126)
(252000.00000, 0.00135)
(252500.00000, 0.00127)
(253000.00000, 0.00121)
(253500.00000, 0.00144)
(254000.00000, 0.00152)
};
\addplot[thin,only marks, mark options={opacity=0.9},mark=*,mark size=.5pt,gray] plot coordinates {
(1000.00000, 0.01726)
(1500.00000, 0.01462)
(2000.00000, 0.01460)
(2500.00000, 0.01238)
(3000.00000, 0.01095)
(3500.00000, 0.00925)
(4000.00000, 0.01089)
(4500.00000, 0.01009)
(5000.00000, 0.00805)
(5500.00000, 0.01025)
(6000.00000, 0.00777)
(6500.00000, 0.00782)
(7000.00000, 0.00680)
(7500.00000, 0.00655)
(8000.00000, 0.00535)
(8500.00000, 0.00669)
(9000.00000, 0.00647)
(9500.00000, 0.00658)
(10000.00000, 0.00625)
(10500.00000, 0.00606)
(11000.00000, 0.00497)
(11500.00000, 0.00599)
(12000.00000, 0.00473)
(12500.00000, 0.00551)
(13000.00000, 0.00655)
(13500.00000, 0.00591)
(14000.00000, 0.00519)
(14500.00000, 0.00468)
(15000.00000, 0.00477)
(15500.00000, 0.00409)
(16000.00000, 0.00375)
(16500.00000, 0.00502)
(17000.00000, 0.00394)
(17500.00000, 0.00422)
(18000.00000, 0.00384)
(18500.00000, 0.00414)
(19000.00000, 0.00342)
(19500.00000, 0.00398)
(20000.00000, 0.00382)
(20500.00000, 0.00366)
(21000.00000, 0.00432)
(21500.00000, 0.00356)
(22000.00000, 0.00376)
(22500.00000, 0.00391)
(23000.00000, 0.00386)
(23500.00000, 0.00458)
(24000.00000, 0.00419)
(24500.00000, 0.00271)
(25000.00000, 0.00367)
(25500.00000, 0.00428)
(26000.00000, 0.00269)
(26500.00000, 0.00360)
(27000.00000, 0.00326)
(27500.00000, 0.00312)
(28000.00000, 0.00278)
(28500.00000, 0.00391)
(29000.00000, 0.00320)
(29500.00000, 0.00383)
(30000.00000, 0.00289)
(30500.00000, 0.00358)
(31000.00000, 0.00294)
(31500.00000, 0.00355)
(32000.00000, 0.00281)
(32500.00000, 0.00365)
(33000.00000, 0.00297)
(33500.00000, 0.00337)
(34000.00000, 0.00265)
(34500.00000, 0.00410)
(35000.00000, 0.00389)
(35500.00000, 0.00361)
(36000.00000, 0.00417)
(36500.00000, 0.00356)
(37000.00000, 0.00348)
(37500.00000, 0.00317)
(38000.00000, 0.00368)
(38500.00000, 0.00328)
(39000.00000, 0.00298)
(39500.00000, 0.00326)
(40000.00000, 0.00379)
(40500.00000, 0.00377)
(41000.00000, 0.00363)
(41500.00000, 0.00370)
(42000.00000, 0.00371)
(42500.00000, 0.00388)
(43000.00000, 0.00359)
(43500.00000, 0.00424)
(44000.00000, 0.00344)
(44500.00000, 0.00378)
(45000.00000, 0.00387)
(45500.00000, 0.00324)
(46000.00000, 0.00381)
(46500.00000, 0.00311)
(47000.00000, 0.00269)
(47500.00000, 0.00367)
(48000.00000, 0.00293)
(48500.00000, 0.00324)
(49000.00000, 0.00310)
(49500.00000, 0.00274)
(50000.00000, 0.00263)
(50500.00000, 0.00295)
(51000.00000, 0.00291)
(51500.00000, 0.00272)
(52000.00000, 0.00261)
(52500.00000, 0.00250)
(53000.00000, 0.00364)
(53500.00000, 0.00268)
(54000.00000, 0.00272)
(54500.00000, 0.00262)
(55000.00000, 0.00257)
(55500.00000, 0.00290)
(56000.00000, 0.00237)
(56500.00000, 0.00224)
(57000.00000, 0.00229)
(57500.00000, 0.00288)
(58000.00000, 0.00244)
(58500.00000, 0.00239)
(59000.00000, 0.00226)
(59500.00000, 0.00232)
(60000.00000, 0.00251)
(60500.00000, 0.00260)
(61000.00000, 0.00289)
(61500.00000, 0.00263)
(62000.00000, 0.00298)
(62500.00000, 0.00237)
(63000.00000, 0.00307)
(63500.00000, 0.00308)
(64000.00000, 0.00240)
(64500.00000, 0.00264)
(65000.00000, 0.00313)
(65500.00000, 0.00303)
(66000.00000, 0.00245)
(66500.00000, 0.00326)
(67000.00000, 0.00278)
(67500.00000, 0.00251)
(68000.00000, 0.00231)
(68500.00000, 0.00249)
(69000.00000, 0.00217)
(69500.00000, 0.00231)
(70000.00000, 0.00197)
(70500.00000, 0.00253)
(71000.00000, 0.00243)
(71500.00000, 0.00269)
(72000.00000, 0.00207)
(72500.00000, 0.00214)
(73000.00000, 0.00222)
(73500.00000, 0.00204)
(74000.00000, 0.00207)
(74500.00000, 0.00202)
(75000.00000, 0.00215)
(75500.00000, 0.00154)
(76000.00000, 0.00170)
(76500.00000, 0.00198)
(77000.00000, 0.00208)
(77500.00000, 0.00218)
(78000.00000, 0.00243)
(78500.00000, 0.00203)
(79000.00000, 0.00160)
(79500.00000, 0.00222)
(80000.00000, 0.00236)
(80500.00000, 0.00207)
(81000.00000, 0.00180)
(81500.00000, 0.00206)
(82000.00000, 0.00221)
(82500.00000, 0.00203)
(83000.00000, 0.00212)
(83500.00000, 0.00178)
(84000.00000, 0.00207)
(84500.00000, 0.00236)
(85000.00000, 0.00208)
(85500.00000, 0.00222)
(86000.00000, 0.00175)
(86500.00000, 0.00202)
(87000.00000, 0.00228)
(87500.00000, 0.00197)
(88000.00000, 0.00206)
(88500.00000, 0.00178)
(89000.00000, 0.00200)
(89500.00000, 0.00173)
(90000.00000, 0.00187)
(90500.00000, 0.00207)
(91000.00000, 0.00166)
(91500.00000, 0.00189)
(92000.00000, 0.00161)
(92500.00000, 0.00182)
(93000.00000, 0.00167)
(93500.00000, 0.00216)
(94000.00000, 0.00175)
(94500.00000, 0.00169)
(95000.00000, 0.00185)
(95500.00000, 0.00235)
(96000.00000, 0.00210)
(96500.00000, 0.00160)
(97000.00000, 0.00189)
(97500.00000, 0.00190)
(98000.00000, 0.00158)
(98500.00000, 0.00189)
(99000.00000, 0.00124)
(99500.00000, 0.00195)
(100000.00000, 0.00173)
(100500.00000, 0.00161)
(101000.00000, 0.00190)
(101500.00000, 0.00157)
(102000.00000, 0.00162)
(102500.00000, 0.00178)
(103000.00000, 0.00176)
(103500.00000, 0.00152)
(104000.00000, 0.00202)
(104500.00000, 0.00188)
(105000.00000, 0.00183)
(105500.00000, 0.00162)
(106000.00000, 0.00191)
(106500.00000, 0.00166)
(107000.00000, 0.00181)
(107500.00000, 0.00142)
(108000.00000, 0.00180)
(108500.00000, 0.00165)
(109000.00000, 0.00178)
(109500.00000, 0.00231)
(110000.00000, 0.00156)
(110500.00000, 0.00166)
(111000.00000, 0.00185)
(111500.00000, 0.00150)
(112000.00000, 0.00165)
(112500.00000, 0.00172)
(113000.00000, 0.00146)
(113500.00000, 0.00185)
(114000.00000, 0.00213)
(114500.00000, 0.00181)
(115000.00000, 0.00171)
(115500.00000, 0.00197)
(116000.00000, 0.00164)
(116500.00000, 0.00156)
(117000.00000, 0.00190)
(117500.00000, 0.00195)
(118000.00000, 0.00172)
(118500.00000, 0.00171)
(119000.00000, 0.00193)
(119500.00000, 0.00152)
(120000.00000, 0.00156)
(120500.00000, 0.00178)
(121000.00000, 0.00160)
(121500.00000, 0.00167)
(122000.00000, 0.00173)
(122500.00000, 0.00173)
(123000.00000, 0.00149)
(123500.00000, 0.00153)
(124000.00000, 0.00192)
(124500.00000, 0.00133)
(125000.00000, 0.00179)
(125500.00000, 0.00136)
(126000.00000, 0.00150)
(126500.00000, 0.00127)
(127000.00000, 0.00194)
(127500.00000, 0.00136)
(128000.00000, 0.00174)
(128500.00000, 0.00139)
(129000.00000, 0.00160)
(129500.00000, 0.00164)
(130000.00000, 0.00157)
(130500.00000, 0.00176)
(131000.00000, 0.00175)
(131500.00000, 0.00177)
(132000.00000, 0.00156)
(132500.00000, 0.00151)
(133000.00000, 0.00143)
(133500.00000, 0.00167)
(134000.00000, 0.00153)
(134500.00000, 0.00188)
(135000.00000, 0.00143)
(135500.00000, 0.00137)
(136000.00000, 0.00161)
(136500.00000, 0.00134)
(137000.00000, 0.00143)
(137500.00000, 0.00183)
(138000.00000, 0.00159)
(138500.00000, 0.00154)
(139000.00000, 0.00177)
(139500.00000, 0.00163)
(140000.00000, 0.00161)
(140500.00000, 0.00162)
(141000.00000, 0.00166)
(141500.00000, 0.00164)
(142000.00000, 0.00178)
(142500.00000, 0.00192)
(143000.00000, 0.00142)
(143500.00000, 0.00182)
(144000.00000, 0.00163)
(144500.00000, 0.00167)
(145000.00000, 0.00163)
(145500.00000, 0.00159)
(146000.00000, 0.00190)
(146500.00000, 0.00211)
(147000.00000, 0.00179)
(147500.00000, 0.00162)
(148000.00000, 0.00164)
(148500.00000, 0.00153)
(149000.00000, 0.00179)
(149500.00000, 0.00175)
(150000.00000, 0.00155)
(150500.00000, 0.00158)
(151000.00000, 0.00192)
(151500.00000, 0.00147)
(152000.00000, 0.00156)
(152500.00000, 0.00173)
(153000.00000, 0.00154)
(153500.00000, 0.00139)
(154000.00000, 0.00167)
(154500.00000, 0.00136)
(155000.00000, 0.00191)
(155500.00000, 0.00164)
(156000.00000, 0.00170)
(156500.00000, 0.00197)
(157000.00000, 0.00194)
(157500.00000, 0.00166)
(158000.00000, 0.00167)
(158500.00000, 0.00141)
(159000.00000, 0.00178)
(159500.00000, 0.00179)
(160000.00000, 0.00182)
(160500.00000, 0.00191)
(161000.00000, 0.00141)
(161500.00000, 0.00165)
(162000.00000, 0.00148)
(162500.00000, 0.00172)
(163000.00000, 0.00150)
(163500.00000, 0.00146)
(164000.00000, 0.00155)
(164500.00000, 0.00142)
(165000.00000, 0.00188)
(165500.00000, 0.00137)
(166000.00000, 0.00152)
(166500.00000, 0.00157)
(167000.00000, 0.00188)
(167500.00000, 0.00159)
(168000.00000, 0.00124)
(168500.00000, 0.00142)
(169000.00000, 0.00166)
(169500.00000, 0.00160)
(170000.00000, 0.00162)
(170500.00000, 0.00170)
(171000.00000, 0.00149)
(171500.00000, 0.00165)
(172000.00000, 0.00184)
(172500.00000, 0.00206)
(173000.00000, 0.00208)
(173500.00000, 0.00180)
(174000.00000, 0.00217)
(174500.00000, 0.00204)
(175000.00000, 0.00231)
(175500.00000, 0.00222)
(176000.00000, 0.00223)
(176500.00000, 0.00198)
(177000.00000, 0.00220)
(177500.00000, 0.00248)
(178000.00000, 0.00206)
(178500.00000, 0.00227)
(179000.00000, 0.00257)
(179500.00000, 0.00216)
(180000.00000, 0.00250)
(180500.00000, 0.00195)
(181000.00000, 0.00163)
(181500.00000, 0.00212)
(182000.00000, 0.00235)
(182500.00000, 0.00225)
(183000.00000, 0.00218)
(183500.00000, 0.00198)
(184000.00000, 0.00244)
(184500.00000, 0.00243)
(185000.00000, 0.00226)
(185500.00000, 0.00220)
(186000.00000, 0.00267)
(186500.00000, 0.00257)
(187000.00000, 0.00260)
(187500.00000, 0.00272)
(188000.00000, 0.00268)
(188500.00000, 0.00290)
(189000.00000, 0.00240)
(189500.00000, 0.00230)
(190000.00000, 0.00243)
(190500.00000, 0.00248)
(191000.00000, 0.00256)
(191500.00000, 0.00269)
(192000.00000, 0.00250)
(192500.00000, 0.00247)
(193000.00000, 0.00253)
(193500.00000, 0.00269)
(194000.00000, 0.00282)
(194500.00000, 0.00249)
(195000.00000, 0.00265)
(195500.00000, 0.00319)
(196000.00000, 0.00299)
(196500.00000, 0.00335)
(197000.00000, 0.00269)
(197500.00000, 0.00310)
(198000.00000, 0.00307)
(198500.00000, 0.00307)
(199000.00000, 0.00300)
(199500.00000, 0.00298)
(200000.00000, 0.00300)
(200500.00000, 0.00271)
(201000.00000, 0.00283)
(201500.00000, 0.00247)
(202000.00000, 0.00313)
(202500.00000, 0.00282)
(203000.00000, 0.00300)
(203500.00000, 0.00287)
(204000.00000, 0.00248)
(204500.00000, 0.00300)
(205000.00000, 0.00307)
(205500.00000, 0.00282)
(206000.00000, 0.00328)
(206500.00000, 0.00283)
(207000.00000, 0.00278)
(207500.00000, 0.00317)
(208000.00000, 0.00301)
(208500.00000, 0.00297)
(209000.00000, 0.00297)
(209500.00000, 0.00295)
(210000.00000, 0.00268)
(210500.00000, 0.00257)
(211000.00000, 0.00320)
(211500.00000, 0.00288)
(212000.00000, 0.00295)
(212500.00000, 0.00303)
(213000.00000, 0.00272)
(213500.00000, 0.00291)
(214000.00000, 0.00306)
(214500.00000, 0.00315)
(215000.00000, 0.00285)
(215500.00000, 0.00314)
(216000.00000, 0.00293)
(216500.00000, 0.00272)
(217000.00000, 0.00309)
(217500.00000, 0.00268)
(218000.00000, 0.00290)
(218500.00000, 0.00280)
(219000.00000, 0.00265)
(219500.00000, 0.00247)
(220000.00000, 0.00252)
(220500.00000, 0.00238)
(221000.00000, 0.00227)
(221500.00000, 0.00250)
(222000.00000, 0.00251)
(222500.00000, 0.00266)
(223000.00000, 0.00232)
(223500.00000, 0.00222)
(224000.00000, 0.00219)
(224500.00000, 0.00234)
(225000.00000, 0.00230)
(225500.00000, 0.00207)
(226000.00000, 0.00249)
(226500.00000, 0.00231)
(227000.00000, 0.00225)
(227500.00000, 0.00209)
(228000.00000, 0.00258)
(228500.00000, 0.00223)
(229000.00000, 0.00220)
(229500.00000, 0.00222)
(230000.00000, 0.00234)
(230500.00000, 0.00234)
(231000.00000, 0.00227)
(231500.00000, 0.00204)
(232000.00000, 0.00201)
(232500.00000, 0.00212)
(233000.00000, 0.00204)
(233500.00000, 0.00220)
(234000.00000, 0.00188)
(234500.00000, 0.00194)
(235000.00000, 0.00207)
(235500.00000, 0.00196)
(236000.00000, 0.00195)
(236500.00000, 0.00189)
(237000.00000, 0.00200)
(237500.00000, 0.00224)
(238000.00000, 0.00202)
(238500.00000, 0.00184)
(239000.00000, 0.00192)
(239500.00000, 0.00212)
(240000.00000, 0.00235)
(240500.00000, 0.00153)
(241000.00000, 0.00216)
(241500.00000, 0.00215)
(242000.00000, 0.00204)
(242500.00000, 0.00197)
(243000.00000, 0.00195)
(243500.00000, 0.00192)
(244000.00000, 0.00182)
(244500.00000, 0.00202)
(245000.00000, 0.00188)
(245500.00000, 0.00191)
(246000.00000, 0.00192)
(246500.00000, 0.00220)
(247000.00000, 0.00186)
(247500.00000, 0.00201)
(248000.00000, 0.00216)
(248500.00000, 0.00212)
(249000.00000, 0.00209)
(249500.00000, 0.00181)
(250000.00000, 0.00185)
(250500.00000, 0.00199)
(251000.00000, 0.00151)
(251500.00000, 0.00209)
(252000.00000, 0.00176)
(252500.00000, 0.00146)
(253000.00000, 0.00152)
(253500.00000, 0.00158)
(254000.00000, 0.00173)
};
\addplot[thin,only marks, mark options={opacity=0.9},mark=*,mark size=.5pt,Cyan1] plot coordinates {
(1000.00000, 0.01972)
(1500.00000, 0.01731)
(2000.00000, 0.01352)
(2500.00000, 0.01167)
(3000.00000, 0.01109)
(3500.00000, 0.01020)
(4000.00000, 0.01140)
(4500.00000, 0.01148)
(5000.00000, 0.00931)
(5500.00000, 0.01036)
(6000.00000, 0.01013)
(6500.00000, 0.00830)
(7000.00000, 0.00768)
(7500.00000, 0.00833)
(8000.00000, 0.00774)
(8500.00000, 0.00622)
(9000.00000, 0.00555)
(9500.00000, 0.00692)
(10000.00000, 0.00541)
(10500.00000, 0.00629)
(11000.00000, 0.00479)
(11500.00000, 0.00509)
(12000.00000, 0.00634)
(12500.00000, 0.00465)
(13000.00000, 0.00474)
(13500.00000, 0.00474)
(14000.00000, 0.00430)
(14500.00000, 0.00485)
(15000.00000, 0.00542)
(15500.00000, 0.00424)
(16000.00000, 0.00438)
(16500.00000, 0.00792)
(17000.00000, 0.00572)
(17500.00000, 0.00439)
(18000.00000, 0.00422)
(18500.00000, 0.00564)
(19000.00000, 0.00535)
(19500.00000, 0.00520)
(20000.00000, 0.00485)
(20500.00000, 0.00588)
(21000.00000, 0.00648)
(21500.00000, 0.00349)
(22000.00000, 0.00499)
(22500.00000, 0.00430)
(23000.00000, 0.00562)
(23500.00000, 0.00514)
(24000.00000, 0.00500)
(24500.00000, 0.00477)
(25000.00000, 0.00436)
(25500.00000, 0.00451)
(26000.00000, 0.00417)
(26500.00000, 0.00377)
(27000.00000, 0.00433)
(27500.00000, 0.00381)
(28000.00000, 0.00371)
(28500.00000, 0.00387)
(29000.00000, 0.00339)
(29500.00000, 0.00452)
(30000.00000, 0.00354)
(30500.00000, 0.00350)
(31000.00000, 0.00319)
(31500.00000, 0.00335)
(32000.00000, 0.00300)
(32500.00000, 0.00351)
(33000.00000, 0.00372)
(33500.00000, 0.00356)
(34000.00000, 0.00321)
(34500.00000, 0.00305)
(35000.00000, 0.00321)
(35500.00000, 0.00337)
(36000.00000, 0.00336)
(36500.00000, 0.00283)
(37000.00000, 0.00324)
(37500.00000, 0.00301)
(38000.00000, 0.00343)
(38500.00000, 0.00317)
(39000.00000, 0.00326)
(39500.00000, 0.00379)
(40000.00000, 0.00290)
(40500.00000, 0.00329)
(41000.00000, 0.00257)
(41500.00000, 0.00297)
(42000.00000, 0.00286)
(42500.00000, 0.00291)
(43000.00000, 0.00275)
(43500.00000, 0.00275)
(44000.00000, 0.00232)
(44500.00000, 0.00299)
(45000.00000, 0.00235)
(45500.00000, 0.00262)
(46000.00000, 0.00222)
(46500.00000, 0.00284)
(47000.00000, 0.00250)
(47500.00000, 0.00285)
(48000.00000, 0.00338)
(48500.00000, 0.00283)
(49000.00000, 0.00329)
(49500.00000, 0.00258)
(50000.00000, 0.00236)
(50500.00000, 0.00211)
(51000.00000, 0.00239)
(51500.00000, 0.00213)
(52000.00000, 0.00259)
(52500.00000, 0.00248)
(53000.00000, 0.00238)
(53500.00000, 0.00322)
(54000.00000, 0.00278)
(54500.00000, 0.00267)
(55000.00000, 0.00251)
(55500.00000, 0.00251)
(56000.00000, 0.00245)
(56500.00000, 0.00194)
(57000.00000, 0.00238)
(57500.00000, 0.00270)
(58000.00000, 0.00178)
(58500.00000, 0.00248)
(59000.00000, 0.00219)
(59500.00000, 0.00219)
(60000.00000, 0.00225)
(60500.00000, 0.00196)
(61000.00000, 0.00205)
(61500.00000, 0.00198)
(62000.00000, 0.00208)
(62500.00000, 0.00229)
(63000.00000, 0.00271)
(63500.00000, 0.00192)
(64000.00000, 0.00200)
(64500.00000, 0.00217)
(65000.00000, 0.00213)
(65500.00000, 0.00218)
(66000.00000, 0.00289)
(66500.00000, 0.00276)
(67000.00000, 0.00239)
(67500.00000, 0.00292)
(68000.00000, 0.00359)
(68500.00000, 0.00402)
(69000.00000, 0.00343)
(69500.00000, 0.00340)
(70000.00000, 0.00345)
(70500.00000, 0.00445)
(71000.00000, 0.00401)
(71500.00000, 0.00373)
(72000.00000, 0.00394)
(72500.00000, 0.00412)
(73000.00000, 0.00343)
(73500.00000, 0.00401)
(74000.00000, 0.00307)
(74500.00000, 0.00377)
(75000.00000, 0.00340)
(75500.00000, 0.00388)
(76000.00000, 0.00339)
(76500.00000, 0.00378)
(77000.00000, 0.00406)
(77500.00000, 0.00329)
(78000.00000, 0.00359)
(78500.00000, 0.00384)
(79000.00000, 0.00330)
(79500.00000, 0.00336)
(80000.00000, 0.00329)
(80500.00000, 0.00334)
(81000.00000, 0.00324)
(81500.00000, 0.00405)
(82000.00000, 0.00294)
(82500.00000, 0.00346)
(83000.00000, 0.00288)
(83500.00000, 0.00354)
(84000.00000, 0.00341)
(84500.00000, 0.00339)
(85000.00000, 0.00276)
(85500.00000, 0.00244)
(86000.00000, 0.00284)
(86500.00000, 0.00273)
(87000.00000, 0.00273)
(87500.00000, 0.00236)
(88000.00000, 0.00270)
(88500.00000, 0.00252)
(89000.00000, 0.00238)
(89500.00000, 0.00258)
(90000.00000, 0.00279)
(90500.00000, 0.00242)
(91000.00000, 0.00250)
(91500.00000, 0.00260)
(92000.00000, 0.00235)
(92500.00000, 0.00282)
(93000.00000, 0.00276)
(93500.00000, 0.00271)
(94000.00000, 0.00290)
(94500.00000, 0.00227)
(95000.00000, 0.00256)
(95500.00000, 0.00257)
(96000.00000, 0.00251)
(96500.00000, 0.00270)
(97000.00000, 0.00229)
(97500.00000, 0.00242)
(98000.00000, 0.00243)
(98500.00000, 0.00196)
(99000.00000, 0.00233)
(99500.00000, 0.00220)
(100000.00000, 0.00231)
(100500.00000, 0.00208)
(101000.00000, 0.00257)
(101500.00000, 0.00292)
(102000.00000, 0.00220)
(102500.00000, 0.00213)
(103000.00000, 0.00183)
(103500.00000, 0.00247)
(104000.00000, 0.00194)
(104500.00000, 0.00189)
(105000.00000, 0.00197)
(105500.00000, 0.00168)
(106000.00000, 0.00198)
(106500.00000, 0.00165)
(107000.00000, 0.00190)
(107500.00000, 0.00224)
(108000.00000, 0.00161)
(108500.00000, 0.00212)
(109000.00000, 0.00206)
(109500.00000, 0.00180)
(110000.00000, 0.00231)
(110500.00000, 0.00222)
(111000.00000, 0.00182)
(111500.00000, 0.00183)
(112000.00000, 0.00162)
(112500.00000, 0.00200)
(113000.00000, 0.00176)
(113500.00000, 0.00183)
(114000.00000, 0.00170)
(114500.00000, 0.00170)
(115000.00000, 0.00140)
(115500.00000, 0.00215)
(116000.00000, 0.00168)
(116500.00000, 0.00157)
(117000.00000, 0.00167)
(117500.00000, 0.00164)
(118000.00000, 0.00235)
(118500.00000, 0.00206)
(119000.00000, 0.00196)
(119500.00000, 0.00202)
(120000.00000, 0.00192)
(120500.00000, 0.00152)
(121000.00000, 0.00193)
(121500.00000, 0.00171)
(122000.00000, 0.00183)
(122500.00000, 0.00199)
(123000.00000, 0.00204)
(123500.00000, 0.00169)
(124000.00000, 0.00227)
(124500.00000, 0.00189)
(125000.00000, 0.00211)
(125500.00000, 0.00204)
(126000.00000, 0.00224)
(126500.00000, 0.00175)
(127000.00000, 0.00180)
(127500.00000, 0.00194)
(128000.00000, 0.00220)
(128500.00000, 0.00174)
(129000.00000, 0.00161)
(129500.00000, 0.00184)
(130000.00000, 0.00188)
(130500.00000, 0.00157)
(131000.00000, 0.00151)
(131500.00000, 0.00136)
(132000.00000, 0.00162)
(132500.00000, 0.00174)
(133000.00000, 0.00166)
(133500.00000, 0.00128)
(134000.00000, 0.00174)
(134500.00000, 0.00130)
(135000.00000, 0.00163)
(135500.00000, 0.00163)
(136000.00000, 0.00189)
(136500.00000, 0.00185)
(137000.00000, 0.00161)
(137500.00000, 0.00141)
(138000.00000, 0.00145)
(138500.00000, 0.00181)
(139000.00000, 0.00134)
(139500.00000, 0.00157)
(140000.00000, 0.00190)
(140500.00000, 0.00146)
(141000.00000, 0.00173)
(141500.00000, 0.00160)
(142000.00000, 0.00154)
(142500.00000, 0.00177)
(143000.00000, 0.00184)
(143500.00000, 0.00142)
(144000.00000, 0.00176)
(144500.00000, 0.00126)
(145000.00000, 0.00145)
(145500.00000, 0.00132)
(146000.00000, 0.00178)
(146500.00000, 0.00143)
(147000.00000, 0.00153)
(147500.00000, 0.00151)
(148000.00000, 0.00176)
(148500.00000, 0.00144)
(149000.00000, 0.00147)
(149500.00000, 0.00150)
(150000.00000, 0.00157)
(150500.00000, 0.00185)
(151000.00000, 0.00163)
(151500.00000, 0.00135)
(152000.00000, 0.00161)
(152500.00000, 0.00146)
(153000.00000, 0.00174)
(153500.00000, 0.00175)
(154000.00000, 0.00163)
(154500.00000, 0.00160)
(155000.00000, 0.00174)
(155500.00000, 0.00167)
(156000.00000, 0.00175)
(156500.00000, 0.00144)
(157000.00000, 0.00187)
(157500.00000, 0.00168)
(158000.00000, 0.00169)
(158500.00000, 0.00194)
(159000.00000, 0.00176)
(159500.00000, 0.00149)
(160000.00000, 0.00172)
(160500.00000, 0.00156)
(161000.00000, 0.00144)
(161500.00000, 0.00147)
(162000.00000, 0.00174)
(162500.00000, 0.00155)
(163000.00000, 0.00178)
(163500.00000, 0.00151)
(164000.00000, 0.00141)
(164500.00000, 0.00155)
(165000.00000, 0.00157)
(165500.00000, 0.00154)
(166000.00000, 0.00138)
(166500.00000, 0.00139)
(167000.00000, 0.00149)
(167500.00000, 0.00127)
(168000.00000, 0.00143)
(168500.00000, 0.00138)
(169000.00000, 0.00155)
(169500.00000, 0.00178)
(170000.00000, 0.00130)
(170500.00000, 0.00126)
(171000.00000, 0.00152)
(171500.00000, 0.00127)
(172000.00000, 0.00145)
(172500.00000, 0.00117)
(173000.00000, 0.00120)
(173500.00000, 0.00119)
(174000.00000, 0.00134)
(174500.00000, 0.00131)
(175000.00000, 0.00115)
(175500.00000, 0.00126)
(176000.00000, 0.00138)
(176500.00000, 0.00160)
(177000.00000, 0.00143)
(177500.00000, 0.00129)
(178000.00000, 0.00127)
(178500.00000, 0.00135)
(179000.00000, 0.00116)
(179500.00000, 0.00160)
(180000.00000, 0.00119)
(180500.00000, 0.00147)
(181000.00000, 0.00136)
(181500.00000, 0.00152)
(182000.00000, 0.00141)
(182500.00000, 0.00109)
(183000.00000, 0.00137)
(183500.00000, 0.00121)
(184000.00000, 0.00138)
(184500.00000, 0.00147)
(185000.00000, 0.00164)
(185500.00000, 0.00122)
(186000.00000, 0.00140)
(186500.00000, 0.00143)
(187000.00000, 0.00144)
(187500.00000, 0.00133)
(188000.00000, 0.00140)
(188500.00000, 0.00131)
(189000.00000, 0.00133)
(189500.00000, 0.00103)
(190000.00000, 0.00126)
(190500.00000, 0.00137)
(191000.00000, 0.00137)
(191500.00000, 0.00126)
(192000.00000, 0.00124)
(192500.00000, 0.00122)
(193000.00000, 0.00120)
(193500.00000, 0.00125)
(194000.00000, 0.00141)
(194500.00000, 0.00113)
(195000.00000, 0.00118)
(195500.00000, 0.00098)
(196000.00000, 0.00114)
(196500.00000, 0.00149)
(197000.00000, 0.00117)
(197500.00000, 0.00117)
(198000.00000, 0.00103)
(198500.00000, 0.00118)
(199000.00000, 0.00136)
(199500.00000, 0.00120)
(200000.00000, 0.00123)
(200500.00000, 0.00104)
(201000.00000, 0.00135)
(201500.00000, 0.00143)
(202000.00000, 0.00111)
(202500.00000, 0.00130)
(203000.00000, 0.00142)
(203500.00000, 0.00110)
(204000.00000, 0.00134)
(204500.00000, 0.00126)
(205000.00000, 0.00132)
(205500.00000, 0.00102)
(206000.00000, 0.00115)
(206500.00000, 0.00147)
(207000.00000, 0.00106)
(207500.00000, 0.00118)
(208000.00000, 0.00119)
(208500.00000, 0.00115)
(209000.00000, 0.00118)
(209500.00000, 0.00102)
(210000.00000, 0.00133)
(210500.00000, 0.00108)
(211000.00000, 0.00120)
(211500.00000, 0.00135)
(212000.00000, 0.00125)
(212500.00000, 0.00125)
(213000.00000, 0.00135)
(213500.00000, 0.00128)
(214000.00000, 0.00149)
(214500.00000, 0.00114)
(215000.00000, 0.00129)
(215500.00000, 0.00132)
(216000.00000, 0.00105)
(216500.00000, 0.00141)
(217000.00000, 0.00105)
(217500.00000, 0.00107)
(218000.00000, 0.00120)
(218500.00000, 0.00123)
(219000.00000, 0.00131)
(219500.00000, 0.00127)
(220000.00000, 0.00114)
(220500.00000, 0.00120)
(221000.00000, 0.00126)
(221500.00000, 0.00136)
(222000.00000, 0.00116)
(222500.00000, 0.00106)
(223000.00000, 0.00116)
(223500.00000, 0.00093)
(224000.00000, 0.00121)
(224500.00000, 0.00103)
(225000.00000, 0.00106)
(225500.00000, 0.00122)
(226000.00000, 0.00145)
(226500.00000, 0.00134)
(227000.00000, 0.00092)
(227500.00000, 0.00122)
(228000.00000, 0.00137)
(228500.00000, 0.00118)
(229000.00000, 0.00101)
(229500.00000, 0.00103)
(230000.00000, 0.00133)
(230500.00000, 0.00129)
(231000.00000, 0.00129)
(231500.00000, 0.00115)
(232000.00000, 0.00118)
(232500.00000, 0.00131)
(233000.00000, 0.00118)
(233500.00000, 0.00101)
(234000.00000, 0.00107)
(234500.00000, 0.00108)
(235000.00000, 0.00114)
(235500.00000, 0.00117)
(236000.00000, 0.00107)
(236500.00000, 0.00121)
(237000.00000, 0.00143)
(237500.00000, 0.00098)
(238000.00000, 0.00113)
(238500.00000, 0.00123)
(239000.00000, 0.00108)
(239500.00000, 0.00114)
(240000.00000, 0.00121)
(240500.00000, 0.00122)
(241000.00000, 0.00119)
(241500.00000, 0.00103)
(242000.00000, 0.00131)
(242500.00000, 0.00112)
(243000.00000, 0.00098)
(243500.00000, 0.00129)
(244000.00000, 0.00145)
(244500.00000, 0.00103)
(245000.00000, 0.00122)
(245500.00000, 0.00131)
(246000.00000, 0.00119)
(246500.00000, 0.00114)
(247000.00000, 0.00112)
(247500.00000, 0.00105)
(248000.00000, 0.00124)
(248500.00000, 0.00123)
(249000.00000, 0.00109)
(249500.00000, 0.00134)
(250000.00000, 0.00100)
(250500.00000, 0.00113)
(251000.00000, 0.00112)
(251500.00000, 0.00137)
(252000.00000, 0.00106)
(252500.00000, 0.00123)
(253000.00000, 0.00096)
(253500.00000, 0.00121)
(254000.00000, 0.00104)
};
\addplot[thin,only marks, mark options={opacity=0.9},mark=*,mark size=.5pt,Cyan3] plot coordinates {
(1000.00000, 0.02931)
(1500.00000, 0.01914)
(2000.00000, 0.01417)
(2500.00000, 0.01240)
(3000.00000, 0.01051)
(3500.00000, 0.00942)
(4000.00000, 0.01064)
(4500.00000, 0.00835)
(5000.00000, 0.00610)
(5500.00000, 0.00807)
(6000.00000, 0.00934)
(6500.00000, 0.01056)
(7000.00000, 0.00967)
(7500.00000, 0.00716)
(8000.00000, 0.00648)
(8500.00000, 0.00694)
(9000.00000, 0.00638)
(9500.00000, 0.00631)
(10000.00000, 0.00671)
(10500.00000, 0.00595)
(11000.00000, 0.00588)
(11500.00000, 0.00575)
(12000.00000, 0.00673)
(12500.00000, 0.00552)
(13000.00000, 0.00415)
(13500.00000, 0.00490)
(14000.00000, 0.00507)
(14500.00000, 0.00452)
(15000.00000, 0.00614)
(15500.00000, 0.00589)
(16000.00000, 0.00499)
(16500.00000, 0.00442)
(17000.00000, 0.00510)
(17500.00000, 0.00447)
(18000.00000, 0.00472)
(18500.00000, 0.00512)
(19000.00000, 0.00389)
(19500.00000, 0.00411)
(20000.00000, 0.00461)
(20500.00000, 0.00408)
(21000.00000, 0.00414)
(21500.00000, 0.00361)
(22000.00000, 0.00384)
(22500.00000, 0.00431)
(23000.00000, 0.00396)
(23500.00000, 0.00387)
(24000.00000, 0.00366)
(24500.00000, 0.00415)
(25000.00000, 0.00463)
(25500.00000, 0.00456)
(26000.00000, 0.00433)
(26500.00000, 0.00464)
(27000.00000, 0.00464)
(27500.00000, 0.00509)
(28000.00000, 0.00419)
(28500.00000, 0.00321)
(29000.00000, 0.00411)
(29500.00000, 0.00342)
(30000.00000, 0.00276)
(30500.00000, 0.00368)
(31000.00000, 0.00318)
(31500.00000, 0.00315)
(32000.00000, 0.00342)
(32500.00000, 0.00323)
(33000.00000, 0.00354)
(33500.00000, 0.00347)
(34000.00000, 0.00283)
(34500.00000, 0.00290)
(35000.00000, 0.00311)
(35500.00000, 0.00340)
(36000.00000, 0.00322)
(36500.00000, 0.00402)
(37000.00000, 0.00396)
(37500.00000, 0.00367)
(38000.00000, 0.00312)
(38500.00000, 0.00335)
(39000.00000, 0.00352)
(39500.00000, 0.00259)
(40000.00000, 0.00303)
(40500.00000, 0.00335)
(41000.00000, 0.00228)
(41500.00000, 0.00284)
(42000.00000, 0.00270)
(42500.00000, 0.00307)
(43000.00000, 0.00267)
(43500.00000, 0.00309)
(44000.00000, 0.00310)
(44500.00000, 0.00242)
(45000.00000, 0.00295)
(45500.00000, 0.00278)
(46000.00000, 0.00327)
(46500.00000, 0.00285)
(47000.00000, 0.00275)
(47500.00000, 0.00367)
(48000.00000, 0.00284)
(48500.00000, 0.00271)
(49000.00000, 0.00329)
(49500.00000, 0.00289)
(50000.00000, 0.00284)
(50500.00000, 0.00324)
(51000.00000, 0.00312)
(51500.00000, 0.00339)
(52000.00000, 0.00305)
(52500.00000, 0.00319)
(53000.00000, 0.00372)
(53500.00000, 0.00287)
(54000.00000, 0.00283)
(54500.00000, 0.00266)
(55000.00000, 0.00245)
(55500.00000, 0.00249)
(56000.00000, 0.00242)
(56500.00000, 0.00280)
(57000.00000, 0.00287)
(57500.00000, 0.00218)
(58000.00000, 0.00275)
(58500.00000, 0.00225)
(59000.00000, 0.00287)
(59500.00000, 0.00232)
(60000.00000, 0.00234)
(60500.00000, 0.00260)
(61000.00000, 0.00287)
(61500.00000, 0.00283)
(62000.00000, 0.00249)
(62500.00000, 0.00272)
(63000.00000, 0.00272)
(63500.00000, 0.00315)
(64000.00000, 0.00272)
(64500.00000, 0.00285)
(65000.00000, 0.00259)
(65500.00000, 0.00247)
(66000.00000, 0.00265)
(66500.00000, 0.00282)
(67000.00000, 0.00247)
(67500.00000, 0.00193)
(68000.00000, 0.00292)
(68500.00000, 0.00232)
(69000.00000, 0.00299)
(69500.00000, 0.00261)
(70000.00000, 0.00220)
(70500.00000, 0.00288)
(71000.00000, 0.00254)
(71500.00000, 0.00298)
(72000.00000, 0.00207)
(72500.00000, 0.00256)
(73000.00000, 0.00255)
(73500.00000, 0.00297)
(74000.00000, 0.00270)
(74500.00000, 0.00294)
(75000.00000, 0.00328)
(75500.00000, 0.00264)
(76000.00000, 0.00335)
(76500.00000, 0.00348)
(77000.00000, 0.00329)
(77500.00000, 0.00289)
(78000.00000, 0.00349)
(78500.00000, 0.00279)
(79000.00000, 0.00251)
(79500.00000, 0.00280)
(80000.00000, 0.00290)
(80500.00000, 0.00272)
(81000.00000, 0.00270)
(81500.00000, 0.00252)
(82000.00000, 0.00292)
(82500.00000, 0.00245)
(83000.00000, 0.00280)
(83500.00000, 0.00211)
(84000.00000, 0.00282)
(84500.00000, 0.00233)
(85000.00000, 0.00228)
(85500.00000, 0.00226)
(86000.00000, 0.00222)
(86500.00000, 0.00196)
(87000.00000, 0.00251)
(87500.00000, 0.00198)
(88000.00000, 0.00193)
(88500.00000, 0.00208)
(89000.00000, 0.00246)
(89500.00000, 0.00205)
(90000.00000, 0.00210)
(90500.00000, 0.00206)
(91000.00000, 0.00188)
(91500.00000, 0.00195)
(92000.00000, 0.00197)
(92500.00000, 0.00190)
(93000.00000, 0.00193)
(93500.00000, 0.00177)
(94000.00000, 0.00158)
(94500.00000, 0.00144)
(95000.00000, 0.00189)
(95500.00000, 0.00187)
(96000.00000, 0.00154)
(96500.00000, 0.00170)
(97000.00000, 0.00200)
(97500.00000, 0.00130)
(98000.00000, 0.00212)
(98500.00000, 0.00143)
(99000.00000, 0.00182)
(99500.00000, 0.00164)
(100000.00000, 0.00164)
(100500.00000, 0.00210)
(101000.00000, 0.00160)
(101500.00000, 0.00160)
(102000.00000, 0.00163)
(102500.00000, 0.00194)
(103000.00000, 0.00159)
(103500.00000, 0.00175)
(104000.00000, 0.00184)
(104500.00000, 0.00185)
(105000.00000, 0.00206)
(105500.00000, 0.00163)
(106000.00000, 0.00183)
(106500.00000, 0.00207)
(107000.00000, 0.00183)
(107500.00000, 0.00179)
(108000.00000, 0.00172)
(108500.00000, 0.00169)
(109000.00000, 0.00167)
(109500.00000, 0.00174)
(110000.00000, 0.00153)
(110500.00000, 0.00174)
(111000.00000, 0.00203)
(111500.00000, 0.00174)
(112000.00000, 0.00232)
(112500.00000, 0.00170)
(113000.00000, 0.00189)
(113500.00000, 0.00175)
(114000.00000, 0.00174)
(114500.00000, 0.00168)
(115000.00000, 0.00200)
(115500.00000, 0.00125)
(116000.00000, 0.00199)
(116500.00000, 0.00202)
(117000.00000, 0.00144)
(117500.00000, 0.00185)
(118000.00000, 0.00161)
(118500.00000, 0.00203)
(119000.00000, 0.00139)
(119500.00000, 0.00161)
(120000.00000, 0.00191)
(120500.00000, 0.00173)
(121000.00000, 0.00162)
(121500.00000, 0.00174)
(122000.00000, 0.00139)
(122500.00000, 0.00170)
(123000.00000, 0.00179)
(123500.00000, 0.00142)
(124000.00000, 0.00159)
(124500.00000, 0.00145)
(125000.00000, 0.00180)
(125500.00000, 0.00144)
(126000.00000, 0.00161)
(126500.00000, 0.00193)
(127000.00000, 0.00149)
(127500.00000, 0.00144)
(128000.00000, 0.00173)
(128500.00000, 0.00164)
(129000.00000, 0.00159)
(129500.00000, 0.00143)
(130000.00000, 0.00162)
(130500.00000, 0.00141)
(131000.00000, 0.00161)
(131500.00000, 0.00156)
(132000.00000, 0.00149)
(132500.00000, 0.00169)
(133000.00000, 0.00129)
(133500.00000, 0.00167)
(134000.00000, 0.00163)
(134500.00000, 0.00167)
(135000.00000, 0.00142)
(135500.00000, 0.00169)
(136000.00000, 0.00152)
(136500.00000, 0.00130)
(137000.00000, 0.00145)
(137500.00000, 0.00157)
(138000.00000, 0.00137)
(138500.00000, 0.00145)
(139000.00000, 0.00150)
(139500.00000, 0.00153)
(140000.00000, 0.00126)
(140500.00000, 0.00147)
(141000.00000, 0.00147)
(141500.00000, 0.00155)
(142000.00000, 0.00139)
(142500.00000, 0.00162)
(143000.00000, 0.00139)
(143500.00000, 0.00141)
(144000.00000, 0.00134)
(144500.00000, 0.00148)
(145000.00000, 0.00167)
(145500.00000, 0.00186)
(146000.00000, 0.00152)
(146500.00000, 0.00156)
(147000.00000, 0.00174)
(147500.00000, 0.00169)
(148000.00000, 0.00152)
(148500.00000, 0.00168)
(149000.00000, 0.00173)
(149500.00000, 0.00166)
(150000.00000, 0.00151)
(150500.00000, 0.00177)
(151000.00000, 0.00176)
(151500.00000, 0.00129)
(152000.00000, 0.00140)
(152500.00000, 0.00178)
(153000.00000, 0.00157)
(153500.00000, 0.00136)
(154000.00000, 0.00162)
(154500.00000, 0.00142)
(155000.00000, 0.00171)
(155500.00000, 0.00150)
(156000.00000, 0.00146)
(156500.00000, 0.00165)
(157000.00000, 0.00147)
(157500.00000, 0.00149)
(158000.00000, 0.00153)
(158500.00000, 0.00141)
(159000.00000, 0.00169)
(159500.00000, 0.00155)
(160000.00000, 0.00170)
(160500.00000, 0.00133)
(161000.00000, 0.00158)
(161500.00000, 0.00171)
(162000.00000, 0.00191)
(162500.00000, 0.00132)
(163000.00000, 0.00162)
(163500.00000, 0.00144)
(164000.00000, 0.00168)
(164500.00000, 0.00153)
(165000.00000, 0.00157)
(165500.00000, 0.00180)
(166000.00000, 0.00142)
(166500.00000, 0.00160)
(167000.00000, 0.00162)
(167500.00000, 0.00158)
(168000.00000, 0.00130)
(168500.00000, 0.00134)
(169000.00000, 0.00126)
(169500.00000, 0.00145)
(170000.00000, 0.00158)
(170500.00000, 0.00186)
(171000.00000, 0.00152)
(171500.00000, 0.00140)
(172000.00000, 0.00161)
(172500.00000, 0.00134)
(173000.00000, 0.00130)
(173500.00000, 0.00130)
(174000.00000, 0.00126)
(174500.00000, 0.00162)
(175000.00000, 0.00157)
(175500.00000, 0.00156)
(176000.00000, 0.00157)
(176500.00000, 0.00160)
(177000.00000, 0.00129)
(177500.00000, 0.00162)
(178000.00000, 0.00166)
(178500.00000, 0.00124)
(179000.00000, 0.00144)
(179500.00000, 0.00138)
(180000.00000, 0.00134)
(180500.00000, 0.00156)
(181000.00000, 0.00135)
(181500.00000, 0.00145)
(182000.00000, 0.00142)
(182500.00000, 0.00146)
(183000.00000, 0.00147)
(183500.00000, 0.00153)
(184000.00000, 0.00159)
(184500.00000, 0.00127)
(185000.00000, 0.00160)
(185500.00000, 0.00137)
(186000.00000, 0.00165)
(186500.00000, 0.00148)
(187000.00000, 0.00130)
(187500.00000, 0.00120)
(188000.00000, 0.00104)
(188500.00000, 0.00103)
(189000.00000, 0.00138)
(189500.00000, 0.00134)
(190000.00000, 0.00122)
(190500.00000, 0.00154)
(191000.00000, 0.00137)
(191500.00000, 0.00143)
(192000.00000, 0.00107)
(192500.00000, 0.00131)
(193000.00000, 0.00127)
(193500.00000, 0.00154)
(194000.00000, 0.00131)
(194500.00000, 0.00145)
(195000.00000, 0.00145)
(195500.00000, 0.00136)
(196000.00000, 0.00124)
(196500.00000, 0.00123)
(197000.00000, 0.00128)
(197500.00000, 0.00110)
(198000.00000, 0.00130)
(198500.00000, 0.00145)
(199000.00000, 0.00139)
(199500.00000, 0.00109)
(200000.00000, 0.00122)
(200500.00000, 0.00151)
(201000.00000, 0.00131)
(201500.00000, 0.00144)
(202000.00000, 0.00115)
(202500.00000, 0.00112)
(203000.00000, 0.00109)
(203500.00000, 0.00113)
(204000.00000, 0.00160)
(204500.00000, 0.00129)
(205000.00000, 0.00127)
(205500.00000, 0.00135)
(206000.00000, 0.00117)
(206500.00000, 0.00119)
(207000.00000, 0.00106)
(207500.00000, 0.00116)
(208000.00000, 0.00142)
(208500.00000, 0.00114)
(209000.00000, 0.00141)
(209500.00000, 0.00128)
(210000.00000, 0.00134)
(210500.00000, 0.00114)
(211000.00000, 0.00128)
(211500.00000, 0.00134)
(212000.00000, 0.00134)
(212500.00000, 0.00156)
(213000.00000, 0.00132)
(213500.00000, 0.00155)
(214000.00000, 0.00125)
(214500.00000, 0.00139)
(215000.00000, 0.00123)
(215500.00000, 0.00128)
(216000.00000, 0.00146)
(216500.00000, 0.00147)
(217000.00000, 0.00148)
(217500.00000, 0.00130)
(218000.00000, 0.00142)
(218500.00000, 0.00149)
(219000.00000, 0.00113)
(219500.00000, 0.00129)
(220000.00000, 0.00143)
(220500.00000, 0.00106)
(221000.00000, 0.00118)
(221500.00000, 0.00136)
(222000.00000, 0.00156)
(222500.00000, 0.00133)
(223000.00000, 0.00117)
(223500.00000, 0.00141)
(224000.00000, 0.00123)
(224500.00000, 0.00132)
(225000.00000, 0.00149)
(225500.00000, 0.00119)
(226000.00000, 0.00136)
(226500.00000, 0.00163)
(227000.00000, 0.00124)
(227500.00000, 0.00133)
(228000.00000, 0.00127)
(228500.00000, 0.00115)
(229000.00000, 0.00127)
(229500.00000, 0.00132)
(230000.00000, 0.00140)
(230500.00000, 0.00143)
(231000.00000, 0.00118)
(231500.00000, 0.00144)
(232000.00000, 0.00110)
(232500.00000, 0.00130)
(233000.00000, 0.00123)
(233500.00000, 0.00112)
(234000.00000, 0.00127)
(234500.00000, 0.00127)
(235000.00000, 0.00125)
(235500.00000, 0.00136)
(236000.00000, 0.00116)
(236500.00000, 0.00117)
(237000.00000, 0.00116)
(237500.00000, 0.00128)
(238000.00000, 0.00118)
(238500.00000, 0.00172)
(239000.00000, 0.00171)
(239500.00000, 0.00133)
(240000.00000, 0.00143)
(240500.00000, 0.00119)
(241000.00000, 0.00120)
(241500.00000, 0.00157)
(242000.00000, 0.00106)
(242500.00000, 0.00133)
(243000.00000, 0.00128)
(243500.00000, 0.00098)
(244000.00000, 0.00115)
(244500.00000, 0.00119)
(245000.00000, 0.00123)
(245500.00000, 0.00139)
(246000.00000, 0.00138)
(246500.00000, 0.00133)
(247000.00000, 0.00140)
(247500.00000, 0.00147)
(248000.00000, 0.00132)
(248500.00000, 0.00112)
(249000.00000, 0.00132)
(249500.00000, 0.00141)
(250000.00000, 0.00102)
(250500.00000, 0.00105)
(251000.00000, 0.00112)
(251500.00000, 0.00117)
(252000.00000, 0.00123)
(252500.00000, 0.00106)
(253000.00000, 0.00112)
(253500.00000, 0.00135)
(254000.00000, 0.00101)
};


==> Figures/convogle.tex <==
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,Red1] plot coordinates {
(20.00000, 0.19240)
(21.00000, 0.20735)
(22.00000, 0.19671)
(23.00000, 0.20068)
(24.00000, 0.16495)
(25.00000, 0.18251)
(26.00000, 0.15468)
(27.00000, 0.36033)
(28.00000, 0.36417)
(29.00000, 0.14782)
(30.00000, 0.14508)
(31.00000, 0.32277)
(32.00000, 0.12507)
(33.00000, 0.15269)
(34.00000, 0.08320)
(35.00000, 0.12581)
(36.00000, 0.14613)
(37.00000, 0.13911)
(38.00000, 0.12741)
(39.00000, 0.15149)
(40.00000, 0.11827)
(41.00000, 0.14423)
(42.00000, 0.17930)
(43.00000, 0.13818)
(44.00000, 0.18024)
(45.00000, 0.19089)
(46.00000, 0.20596)
(47.00000, 0.23657)
(48.00000, 0.17027)
(49.00000, 0.19809)
(50.00000, 0.23076)
(51.00000, 0.25732)
(52.00000, 0.25361)
(53.00000, 0.27526)
(54.00000, 0.25751)
(55.00000, 0.26927)
(56.00000, 0.23502)
(57.00000, 0.23887)
(58.00000, 0.27914)
(59.00000, 0.30543)
(60.00000, 0.23725)
(61.00000, 0.25370)
(62.00000, 0.25345)
(63.00000, 0.22454)
(64.00000, 0.24249)
(65.00000, 0.20053)
(66.00000, 0.21988)
(67.00000, 0.20548)
(68.00000, 0.21308)
(69.00000, 0.22418)
(70.00000, 0.19278)
(71.00000, 0.20456)
(72.00000, 0.18391)
(73.00000, 0.17732)
(74.00000, 0.17018)
(75.00000, 0.15999)
(76.00000, 0.19182)
(77.00000, 0.15197)
(78.00000, 0.13908)
(79.00000, 0.14380)
(80.00000, 0.15053)
(81.00000, 0.13393)
(82.00000, 0.13138)
(83.00000, 0.10144)
(84.00000, 0.10236)
(85.00000, 0.12153)
(86.00000, 0.11363)
(87.00000, 0.12363)
(88.00000, 0.11361)
(89.00000, 0.13209)
(90.00000, 0.10023)
(91.00000, 0.12499)
(92.00000, 0.10385)
(93.00000, 0.10734)
(94.00000, 0.11480)
(95.00000, 0.09977)
(96.00000, 0.10148)
(97.00000, 0.10577)
(98.00000, 0.08854)
(99.00000, 0.08421)
(100.00000, 0.07102)
(101.00000, 0.09366)
(102.00000, 0.07627)
(103.00000, 0.08381)
(104.00000, 0.06784)
(105.00000, 0.08040)
(106.00000, 0.07122)
(107.00000, 0.06792)
(108.00000, 0.08306)
(109.00000, 0.07355)
(110.00000, 0.06987)
(111.00000, 0.08042)
(112.00000, 0.06288)
(113.00000, 0.06428)
(114.00000, 0.06132)
(115.00000, 0.06096)
(116.00000, 0.07514)
(117.00000, 0.06553)
(118.00000, 0.07381)
(119.00000, 0.05233)
(120.00000, 0.06963)
(121.00000, 0.07037)
(122.00000, 0.05038)
(123.00000, 0.06486)
(124.00000, 0.06044)
(125.00000, 0.06000)
(126.00000, 0.06172)
(127.00000, 0.05180)
(128.00000, 0.04165)
(129.00000, 0.04331)
(130.00000, 0.06748)
(131.00000, 0.04547)
(132.00000, 0.04753)
(133.00000, 0.04583)
(134.00000, 0.06050)
(135.00000, 0.04695)
(136.00000, 0.06065)
(137.00000, 0.05428)
(138.00000, 0.04955)
(139.00000, 0.05163)
(140.00000, 0.04865)
(141.00000, 0.05242)
(142.00000, 0.04992)
(143.00000, 0.05018)
(144.00000, 0.05796)
(145.00000, 0.04706)
(146.00000, 0.04535)
(147.00000, 0.04880)
(148.00000, 0.05289)
(149.00000, 0.05667)
(150.00000, 0.05475)
(151.00000, 0.05021)
(152.00000, 0.05752)
(153.00000, 0.05546)
(154.00000, 0.05348)
(155.00000, 0.05664)
(156.00000, 0.05046)
(157.00000, 0.05200)
(158.00000, 0.07275)
(159.00000, 0.05333)
(160.00000, 0.05054)
(161.00000, 0.05763)
(162.00000, 0.06004)
(163.00000, 0.04795)
(164.00000, 0.05579)
(165.00000, 0.06522)
(166.00000, 0.06900)
(167.00000, 0.06312)
(168.00000, 0.05766)
(169.00000, 0.05833)
(170.00000, 0.06924)
(171.00000, 0.06977)
(172.00000, 0.06851)
(173.00000, 0.05601)
(174.00000, 0.07312)
(175.00000, 0.05420)
(176.00000, 0.04810)
(177.00000, 0.06764)
(178.00000, 0.04719)
(179.00000, 0.05446)
(180.00000, 0.05473)
(181.00000, 0.05874)
(182.00000, 0.06456)
(183.00000, 0.05306)
(184.00000, 0.05599)
(185.00000, 0.06988)
(186.00000, 0.04654)
(187.00000, 0.03787)
(188.00000, 0.05550)
(189.00000, 0.06570)
(190.00000, 0.05975)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,Cyan2] plot coordinates {
(20.00000, 0.22623)
(21.00000, 0.15271)
(22.00000, 0.13235)
(23.00000, 0.13680)
(24.00000, 0.19589)
(25.00000, 0.12829)
(26.00000, 0.15303)
(27.00000, 0.17122)
(28.00000, 0.30696)
(29.00000, 0.13283)
(30.00000, 0.30405)
(31.00000, 0.09794)
(32.00000, 0.11611)
(33.00000, 0.12023)
(34.00000, 0.11348)
(35.00000, 0.10154)
(36.00000, 0.13464)
(37.00000, 0.13979)
(38.00000, 0.10334)
(39.00000, 0.12698)
(40.00000, 0.09748)
(41.00000, 0.09944)
(42.00000, 0.12589)
(43.00000, 0.09047)
(44.00000, 0.09012)
(45.00000, 0.09875)
(46.00000, 0.09756)
(47.00000, 0.08662)
(48.00000, 0.10701)
(49.00000, 0.09668)
(50.00000, 0.08795)
(51.00000, 0.09821)
(52.00000, 0.09089)
(53.00000, 0.08666)
(54.00000, 0.07478)
(55.00000, 0.10698)
(56.00000, 0.08198)
(57.00000, 0.12172)
(58.00000, 0.08231)
(59.00000, 0.08397)
(60.00000, 0.09450)
(61.00000, 0.08909)
(62.00000, 0.09945)
(63.00000, 0.07070)
(64.00000, 0.07166)
(65.00000, 0.08077)
(66.00000, 0.07286)
(67.00000, 0.07090)
(68.00000, 0.07262)
(69.00000, 0.07035)
(70.00000, 0.07086)
(71.00000, 0.06089)
(72.00000, 0.06186)
(73.00000, 0.06919)
(74.00000, 0.06938)
(75.00000, 0.06869)
(76.00000, 0.06981)
(77.00000, 0.08371)
(78.00000, 0.06073)
(79.00000, 0.07904)
(80.00000, 0.08188)
(81.00000, 0.07890)
(82.00000, 0.06871)
(83.00000, 0.06035)
(84.00000, 0.06812)
(85.00000, 0.06559)
(86.00000, 0.07111)
(87.00000, 0.06783)
(88.00000, 0.05960)
(89.00000, 0.06508)
(90.00000, 0.06047)
(91.00000, 0.06517)
(92.00000, 0.05947)
(93.00000, 0.06607)
(94.00000, 0.06441)
(95.00000, 0.05844)
(96.00000, 0.06282)
(97.00000, 0.06004)
(98.00000, 0.05502)
(99.00000, 0.07006)
(100.00000, 0.06161)
(101.00000, 0.06772)
(102.00000, 0.05891)
(103.00000, 0.05645)
(104.00000, 0.05513)
(105.00000, 0.06659)
(106.00000, 0.06554)
(107.00000, 0.05242)
(108.00000, 0.05739)
(109.00000, 0.05643)
(110.00000, 0.07600)
(111.00000, 0.07359)
(112.00000, 0.04654)
(113.00000, 0.06666)
(114.00000, 0.05839)
(115.00000, 0.06216)
(116.00000, 0.06144)
(117.00000, 0.05518)
(118.00000, 0.06890)
(119.00000, 0.05333)
(120.00000, 0.06642)
(121.00000, 0.05421)
(122.00000, 0.05324)
(123.00000, 0.05958)
(124.00000, 0.04610)
(125.00000, 0.04849)
(126.00000, 0.05870)
(127.00000, 0.04896)
(128.00000, 0.04611)
(129.00000, 0.05084)
(130.00000, 0.05352)
(131.00000, 0.04493)
(132.00000, 0.04796)
(133.00000, 0.05482)
(134.00000, 0.05652)
(135.00000, 0.05242)
(136.00000, 0.05455)
(137.00000, 0.04808)
(138.00000, 0.04453)
(139.00000, 0.05544)
(140.00000, 0.05379)
(141.00000, 0.03836)
(142.00000, 0.04041)
(143.00000, 0.04499)
(144.00000, 0.04423)
(145.00000, 0.04489)
(146.00000, 0.05025)
(147.00000, 0.04736)
(148.00000, 0.04513)
(149.00000, 0.04470)
(150.00000, 0.04157)
(151.00000, 0.04452)
(152.00000, 0.04466)
(153.00000, 0.04508)
(154.00000, 0.06225)
(155.00000, 0.04988)
(156.00000, 0.04672)
(157.00000, 0.04593)
(158.00000, 0.03975)
(159.00000, 0.05055)
(160.00000, 0.04418)
(161.00000, 0.04636)
(162.00000, 0.04518)
(163.00000, 0.05286)
(164.00000, 0.05179)
(165.00000, 0.04581)
(166.00000, 0.04413)
(167.00000, 0.04665)
(168.00000, 0.04281)
(169.00000, 0.04128)
(170.00000, 0.05556)
(171.00000, 0.05316)
(172.00000, 0.04658)
(173.00000, 0.04873)
(174.00000, 0.04060)
(175.00000, 0.05594)
(176.00000, 0.04375)
(177.00000, 0.05343)
(178.00000, 0.04447)
(179.00000, 0.06418)
(180.00000, 0.04634)
(181.00000, 0.05221)
(182.00000, 0.05660)
(183.00000, 0.05103)
(184.00000, 0.04886)
(185.00000, 0.04799)
(186.00000, 0.05739)
(187.00000, 0.05620)
(188.00000, 0.05287)
(189.00000, 0.06084)
(190.00000, 0.04645)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,Green4] plot coordinates {
(20.00000, 0.39247)
(21.00000, 0.15003)
(22.00000, 0.18995)
(23.00000, 0.16766)
(24.00000, 0.13728)
(25.00000, 0.16269)
(26.00000, 0.15470)
(27.00000, 0.15584)
(28.00000, 0.12077)
(29.00000, 0.15729)
(30.00000, 0.11656)
(31.00000, 0.10015)
(32.00000, 0.11355)
(33.00000, 0.12644)
(34.00000, 0.12826)
(35.00000, 0.11929)
(36.00000, 0.12509)
(37.00000, 0.10299)
(38.00000, 0.10334)
(39.00000, 0.08992)
(40.00000, 0.12807)
(41.00000, 0.07698)
(42.00000, 0.09999)
(43.00000, 0.09092)
(44.00000, 0.09254)
(45.00000, 0.11020)
(46.00000, 0.11319)
(47.00000, 0.07716)
(48.00000, 0.07735)
(49.00000, 0.09545)
(50.00000, 0.07648)
(51.00000, 0.09345)
(52.00000, 0.09398)
(53.00000, 0.06006)
(54.00000, 0.10421)
(55.00000, 0.07462)
(56.00000, 0.08888)
(57.00000, 0.07461)
(58.00000, 0.06955)
(59.00000, 0.09194)
(60.00000, 0.09036)
(61.00000, 0.08014)
(62.00000, 0.10494)
(63.00000, 0.08410)
(64.00000, 0.07448)
(65.00000, 0.07212)
(66.00000, 0.06939)
(67.00000, 0.08627)
(68.00000, 0.08458)
(69.00000, 0.05480)
(70.00000, 0.07926)
(71.00000, 0.06733)
(72.00000, 0.06875)
(73.00000, 0.07054)
(74.00000, 0.05622)
(75.00000, 0.06018)
(76.00000, 0.07667)
(77.00000, 0.06472)
(78.00000, 0.07809)
(79.00000, 0.05554)
(80.00000, 0.06238)
(81.00000, 0.06255)
(82.00000, 0.06224)
(83.00000, 0.07922)
(84.00000, 0.07287)
(85.00000, 0.07618)
(86.00000, 0.05775)
(87.00000, 0.05988)
(88.00000, 0.05581)
(89.00000, 0.05529)
(90.00000, 0.06458)
(91.00000, 0.05105)
(92.00000, 0.05427)
(93.00000, 0.07414)
(94.00000, 0.06741)
(95.00000, 0.06030)
(96.00000, 0.06738)
(97.00000, 0.06411)
(98.00000, 0.06094)
(99.00000, 0.07090)
(100.00000, 0.07999)
(101.00000, 0.07335)
(102.00000, 0.06631)
(103.00000, 0.06993)
(104.00000, 0.06535)
(105.00000, 0.08435)
(106.00000, 0.06067)
(107.00000, 0.08266)
(108.00000, 0.06603)
(109.00000, 0.07353)
(110.00000, 0.07227)
(111.00000, 0.07626)
(112.00000, 0.09895)
(113.00000, 0.08038)
(114.00000, 0.06626)
(115.00000, 0.06553)
(116.00000, 0.07769)
(117.00000, 0.07462)
(118.00000, 0.07407)
(119.00000, 0.07022)
(120.00000, 0.07593)
(121.00000, 0.07208)
(122.00000, 0.07904)
(123.00000, 0.05953)
(124.00000, 0.07272)
(125.00000, 0.06477)
(126.00000, 0.05893)
(127.00000, 0.05990)
(128.00000, 0.06477)
(129.00000, 0.04602)
(130.00000, 0.05559)
(131.00000, 0.05194)
(132.00000, 0.05038)
(133.00000, 0.05983)
(134.00000, 0.06040)
(135.00000, 0.04878)
(136.00000, 0.06118)
(137.00000, 0.06000)
(138.00000, 0.05664)
(139.00000, 0.06170)
(140.00000, 0.05137)
(141.00000, 0.05673)
(142.00000, 0.06269)
(143.00000, 0.04796)
(144.00000, 0.05405)
(145.00000, 0.05543)
(146.00000, 0.06189)
(147.00000, 0.05612)
(148.00000, 0.06326)
(149.00000, 0.04889)
(150.00000, 0.05867)
(151.00000, 0.05744)
(152.00000, 0.06408)
(153.00000, 0.06127)
(154.00000, 0.05704)
(155.00000, 0.06144)
(156.00000, 0.05323)
(157.00000, 0.05144)
(158.00000, 0.06605)
(159.00000, 0.06673)
(160.00000, 0.08384)
(161.00000, 0.05245)
(162.00000, 0.06648)
(163.00000, 0.05422)
(164.00000, 0.05762)
(165.00000, 0.04919)
(166.00000, 0.06328)
(167.00000, 0.05292)
(168.00000, 0.04513)
(169.00000, 0.04810)
(170.00000, 0.03878)
(171.00000, 0.04802)
(172.00000, 0.05043)
(173.00000, 0.04934)
(174.00000, 0.04424)
(175.00000, 0.04723)
(176.00000, 0.04983)
(177.00000, 0.04893)
(178.00000, 0.05703)
(179.00000, 0.05018)
(180.00000, 0.04868)
(181.00000, 0.04883)
(182.00000, 0.05298)
(183.00000, 0.05817)
(184.00000, 0.05078)
(185.00000, 0.05314)
(186.00000, 0.05080)
(187.00000, 0.05321)
(188.00000, 0.04816)
(189.00000, 0.05195)
(190.00000, 0.05299)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,blue] plot coordinates {
(20.00000, 0.30847)
(21.00000, 0.28169)
(22.00000, 0.20664)
(23.00000, 0.25889)
(24.00000, 0.22245)
(25.00000, 0.17265)
(26.00000, 0.17320)
(27.00000, 0.14141)
(28.00000, 0.14874)
(29.00000, 0.12525)
(30.00000, 0.12787)
(31.00000, 0.12956)
(32.00000, 0.13591)
(33.00000, 0.16132)
(34.00000, 0.12212)
(35.00000, 0.11125)
(36.00000, 0.09238)
(37.00000, 0.09756)
(38.00000, 0.10804)
(39.00000, 0.11495)
(40.00000, 0.11754)
(41.00000, 0.09978)
(42.00000, 0.09674)
(43.00000, 0.07741)
(44.00000, 0.09279)
(45.00000, 0.09214)
(46.00000, 0.08663)
(47.00000, 0.09503)
(48.00000, 0.08657)
(49.00000, 0.10276)
(50.00000, 0.08579)
(51.00000, 0.06404)
(52.00000, 0.09059)
(53.00000, 0.07168)
(54.00000, 0.08484)
(55.00000, 0.08423)
(56.00000, 0.07122)
(57.00000, 0.08773)
(58.00000, 0.09278)
(59.00000, 0.08802)
(60.00000, 0.11078)
(61.00000, 0.08707)
(62.00000, 0.07406)
(63.00000, 0.08286)
(64.00000, 0.08604)
(65.00000, 0.08561)
(66.00000, 0.09084)
(67.00000, 0.08197)
(68.00000, 0.09760)
(69.00000, 0.06862)
(70.00000, 0.06990)
(71.00000, 0.09205)
(72.00000, 0.08436)
(73.00000, 0.08588)
(74.00000, 0.08856)
(75.00000, 0.08128)
(76.00000, 0.08174)
(77.00000, 0.07417)
(78.00000, 0.06876)
(79.00000, 0.09340)
(80.00000, 0.08044)
(81.00000, 0.06948)
(82.00000, 0.06496)
(83.00000, 0.08024)
(84.00000, 0.07500)
(85.00000, 0.06628)
(86.00000, 0.06130)
(87.00000, 0.08111)
(88.00000, 0.06054)
(89.00000, 0.07204)
(90.00000, 0.06705)
(91.00000, 0.06789)
(92.00000, 0.06432)
(93.00000, 0.07485)
(94.00000, 0.05773)
(95.00000, 0.06663)
(96.00000, 0.06081)
(97.00000, 0.06346)
(98.00000, 0.06688)
(99.00000, 0.06101)
(100.00000, 0.06053)
(101.00000, 0.06670)
(102.00000, 0.06426)
(103.00000, 0.06834)
(104.00000, 0.07023)
(105.00000, 0.07144)
(106.00000, 0.06599)
(107.00000, 0.06373)
(108.00000, 0.05945)
(109.00000, 0.06417)
(110.00000, 0.06505)
(111.00000, 0.05965)
(112.00000, 0.07201)
(113.00000, 0.06115)
(114.00000, 0.05904)
(115.00000, 0.05360)
(116.00000, 0.06927)
(117.00000, 0.05775)
(118.00000, 0.06321)
(119.00000, 0.05254)
(120.00000, 0.07235)
(121.00000, 0.06232)
(122.00000, 0.07284)
(123.00000, 0.06716)
(124.00000, 0.06778)
(125.00000, 0.07381)
(126.00000, 0.07014)
(127.00000, 0.06341)
(128.00000, 0.06602)
(129.00000, 0.05873)
(130.00000, 0.05830)
(131.00000, 0.07110)
(132.00000, 0.07356)
(133.00000, 0.05740)
(134.00000, 0.07017)
(135.00000, 0.07205)
(136.00000, 0.06795)
(137.00000, 0.06804)
(138.00000, 0.06472)
(139.00000, 0.07540)
(140.00000, 0.05891)
(141.00000, 0.06690)
(142.00000, 0.06776)
(143.00000, 0.06941)
(144.00000, 0.06705)
(145.00000, 0.06152)
(146.00000, 0.06636)
(147.00000, 0.05943)
(148.00000, 0.07026)
(149.00000, 0.06618)
(150.00000, 0.06293)
(151.00000, 0.08226)
(152.00000, 0.08442)
(153.00000, 0.07389)
(154.00000, 0.05776)
(155.00000, 0.05383)
(156.00000, 0.06454)
(157.00000, 0.08489)
(158.00000, 0.06708)
(159.00000, 0.08617)
(160.00000, 0.05920)
(161.00000, 0.08491)
(162.00000, 0.07960)
(163.00000, 0.08435)
(164.00000, 0.06715)
(165.00000, 0.06816)
(166.00000, 0.07747)
(167.00000, 0.07083)
(168.00000, 0.08883)
(169.00000, 0.06329)
(170.00000, 0.07026)
(171.00000, 0.05666)
(172.00000, 0.06437)
(173.00000, 0.07636)
(174.00000, 0.07364)
(175.00000, 0.06819)
(176.00000, 0.06395)
(177.00000, 0.06210)
(178.00000, 0.05893)
(179.00000, 0.05397)
(180.00000, 0.04722)
(181.00000, 0.04964)
(182.00000, 0.05442)
(183.00000, 0.05269)
(184.00000, 0.05200)
(185.00000, 0.04073)
(186.00000, 0.05042)
(187.00000, 0.04238)
(188.00000, 0.05412)
(189.00000, 0.06274)
(190.00000, 0.04909)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,Green3] plot coordinates {
(20.00000, 0.20447)
(21.00000, 0.14459)
(22.00000, 0.35620)
(23.00000, 0.12453)
(24.00000, 0.14692)
(25.00000, 0.14499)
(26.00000, 0.14493)
(27.00000, 0.14863)
(28.00000, 0.15359)
(29.00000, 0.10047)
(30.00000, 0.11520)
(31.00000, 0.11029)
(32.00000, 0.12523)
(33.00000, 0.11450)
(34.00000, 0.12129)
(35.00000, 0.11230)
(36.00000, 0.09104)
(37.00000, 0.12083)
(38.00000, 0.08741)
(39.00000, 0.10469)
(40.00000, 0.09816)
(41.00000, 0.06743)
(42.00000, 0.10609)
(43.00000, 0.11469)
(44.00000, 0.11690)
(45.00000, 0.10323)
(46.00000, 0.09914)
(47.00000, 0.10279)
(48.00000, 0.09243)
(49.00000, 0.09400)
(50.00000, 0.08387)
(51.00000, 0.11151)
(52.00000, 0.10439)
(53.00000, 0.11064)
(54.00000, 0.10212)
(55.00000, 0.12529)
(56.00000, 0.10769)
(57.00000, 0.07992)
(58.00000, 0.09596)
(59.00000, 0.10074)
(60.00000, 0.09574)
(61.00000, 0.08627)
(62.00000, 0.07672)
(63.00000, 0.07865)
(64.00000, 0.08609)
(65.00000, 0.08777)
(66.00000, 0.06744)
(67.00000, 0.07204)
(68.00000, 0.08314)
(69.00000, 0.07282)
(70.00000, 0.05925)
(71.00000, 0.07490)
(72.00000, 0.06370)
(73.00000, 0.06703)
(74.00000, 0.06366)
(75.00000, 0.05814)
(76.00000, 0.06841)
(77.00000, 0.05679)
(78.00000, 0.05204)
(79.00000, 0.07564)
(80.00000, 0.06277)
(81.00000, 0.05888)
(82.00000, 0.07391)
(83.00000, 0.06561)
(84.00000, 0.06444)
(85.00000, 0.06806)
(86.00000, 0.08097)
(87.00000, 0.05638)
(88.00000, 0.07005)
(89.00000, 0.06676)
(90.00000, 0.06386)
(91.00000, 0.05987)
(92.00000, 0.05598)
(93.00000, 0.06552)
(94.00000, 0.07158)
(95.00000, 0.05493)
(96.00000, 0.06307)
(97.00000, 0.07325)
(98.00000, 0.07608)
(99.00000, 0.05966)
(100.00000, 0.04815)
(101.00000, 0.06401)
(102.00000, 0.06136)
(103.00000, 0.05006)
(104.00000, 0.05520)
(105.00000, 0.06858)
(106.00000, 0.06913)
(107.00000, 0.06106)
(108.00000, 0.05578)
(109.00000, 0.05049)
(110.00000, 0.05578)
(111.00000, 0.06529)
(112.00000, 0.06230)
(113.00000, 0.05976)
(114.00000, 0.06048)
(115.00000, 0.05042)
(116.00000, 0.05544)
(117.00000, 0.06063)
(118.00000, 0.05809)
(119.00000, 0.06480)
(120.00000, 0.05322)
(121.00000, 0.05808)
(122.00000, 0.05235)
(123.00000, 0.05692)
(124.00000, 0.05909)
(125.00000, 0.05922)
(126.00000, 0.06037)
(127.00000, 0.05774)
(128.00000, 0.04971)
(129.00000, 0.05703)
(130.00000, 0.04699)
(131.00000, 0.05114)
(132.00000, 0.05044)
(133.00000, 0.05270)
(134.00000, 0.04595)
(135.00000, 0.06586)
(136.00000, 0.06047)
(137.00000, 0.04193)
(138.00000, 0.05595)
(139.00000, 0.05002)
(140.00000, 0.06424)
(141.00000, 0.05448)
(142.00000, 0.05334)
(143.00000, 0.04883)
(144.00000, 0.05234)
(145.00000, 0.04902)
(146.00000, 0.05519)
(147.00000, 0.05031)
(148.00000, 0.05954)
(149.00000, 0.05546)
(150.00000, 0.05430)
(151.00000, 0.05892)
(152.00000, 0.06629)
(153.00000, 0.04904)
(154.00000, 0.05106)
(155.00000, 0.05747)
(156.00000, 0.05879)
(157.00000, 0.05558)
(158.00000, 0.06207)
(159.00000, 0.05020)
(160.00000, 0.05152)
(161.00000, 0.07093)
(162.00000, 0.05351)
(163.00000, 0.06157)
(164.00000, 0.04915)
(165.00000, 0.06130)
(166.00000, 0.05174)
(167.00000, 0.05945)
(168.00000, 0.05097)
(169.00000, 0.04937)
(170.00000, 0.04393)
(171.00000, 0.04982)
(172.00000, 0.04939)
(173.00000, 0.05017)
(174.00000, 0.06169)
(175.00000, 0.05479)
(176.00000, 0.05233)
(177.00000, 0.05305)
(178.00000, 0.05538)
(179.00000, 0.05026)
(180.00000, 0.04330)
(181.00000, 0.04751)
(182.00000, 0.04272)
(183.00000, 0.04089)
(184.00000, 0.04480)
(185.00000, 0.05515)
(186.00000, 0.04674)
(187.00000, 0.05615)
(188.00000, 0.04845)
(189.00000, 0.04969)
(190.00000, 0.03939)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,Yellow3] plot coordinates {
(20.00000, 0.14056)
(21.00000, 0.36502)
(22.00000, 0.36737)
(23.00000, 0.17998)
(24.00000, 0.32617)
(25.00000, 0.13909)
(26.00000, 0.34590)
(27.00000, 0.12746)
(28.00000, 0.16434)
(29.00000, 0.11264)
(30.00000, 0.11848)
(31.00000, 0.09638)
(32.00000, 0.12567)
(33.00000, 0.12190)
(34.00000, 0.14499)
(35.00000, 0.11583)
(36.00000, 0.14670)
(37.00000, 0.09047)
(38.00000, 0.09702)
(39.00000, 0.08967)
(40.00000, 0.08518)
(41.00000, 0.10657)
(42.00000, 0.12965)
(43.00000, 0.09438)
(44.00000, 0.08730)
(45.00000, 0.09850)
(46.00000, 0.07027)
(47.00000, 0.08916)
(48.00000, 0.09205)
(49.00000, 0.07940)
(50.00000, 0.09424)
(51.00000, 0.10259)
(52.00000, 0.07975)
(53.00000, 0.08882)
(54.00000, 0.08162)
(55.00000, 0.08219)
(56.00000, 0.07292)
(57.00000, 0.10685)
(58.00000, 0.08120)
(59.00000, 0.08973)
(60.00000, 0.08590)
(61.00000, 0.06494)
(62.00000, 0.09890)
(63.00000, 0.08766)
(64.00000, 0.09206)
(65.00000, 0.08447)
(66.00000, 0.06994)
(67.00000, 0.09838)
(68.00000, 0.09204)
(69.00000, 0.06376)
(70.00000, 0.07858)
(71.00000, 0.07291)
(72.00000, 0.07728)
(73.00000, 0.07423)
(74.00000, 0.07407)
(75.00000, 0.08274)
(76.00000, 0.08387)
(77.00000, 0.08836)
(78.00000, 0.07976)
(79.00000, 0.07935)
(80.00000, 0.08553)
(81.00000, 0.09840)
(82.00000, 0.08177)
(83.00000, 0.08390)
(84.00000, 0.09598)
(85.00000, 0.08598)
(86.00000, 0.10210)
(87.00000, 0.10755)
(88.00000, 0.12218)
(89.00000, 0.11536)
(90.00000, 0.11564)
(91.00000, 0.09718)
(92.00000, 0.10129)
(93.00000, 0.08738)
(94.00000, 0.10794)
(95.00000, 0.09592)
(96.00000, 0.10031)
(97.00000, 0.08245)
(98.00000, 0.09420)
(99.00000, 0.09172)
(100.00000, 0.09855)
(101.00000, 0.08093)
(102.00000, 0.09878)
(103.00000, 0.09727)
(104.00000, 0.10428)
(105.00000, 0.08301)
(106.00000, 0.08836)
(107.00000, 0.10380)
(108.00000, 0.09506)
(109.00000, 0.08421)
(110.00000, 0.09730)
(111.00000, 0.09800)
(112.00000, 0.08853)
(113.00000, 0.09142)
(114.00000, 0.08623)
(115.00000, 0.09025)
(116.00000, 0.08464)
(117.00000, 0.08804)
(118.00000, 0.08836)
(119.00000, 0.09578)
(120.00000, 0.08542)
(121.00000, 0.08727)
(122.00000, 0.08567)
(123.00000, 0.09075)
(124.00000, 0.06615)
(125.00000, 0.07588)
(126.00000, 0.07570)
(127.00000, 0.08454)
(128.00000, 0.08118)
(129.00000, 0.07020)
(130.00000, 0.07664)
(131.00000, 0.08066)
(132.00000, 0.07459)
(133.00000, 0.07924)
(134.00000, 0.07009)
(135.00000, 0.07528)
(136.00000, 0.09088)
(137.00000, 0.08310)
(138.00000, 0.09589)
(139.00000, 0.06415)
(140.00000, 0.05675)
(141.00000, 0.06879)
(142.00000, 0.06547)
(143.00000, 0.06166)
(144.00000, 0.06139)
(145.00000, 0.06299)
(146.00000, 0.06706)
(147.00000, 0.06721)
(148.00000, 0.07714)
(149.00000, 0.05806)
(150.00000, 0.06750)
(151.00000, 0.06820)
(152.00000, 0.07989)
(153.00000, 0.05817)
(154.00000, 0.07155)
(155.00000, 0.05410)
(156.00000, 0.04816)
(157.00000, 0.04811)
(158.00000, 0.06262)
(159.00000, 0.05289)
(160.00000, 0.05824)
(161.00000, 0.06062)
(162.00000, 0.05215)
(163.00000, 0.05391)
(164.00000, 0.06111)
(165.00000, 0.05686)
(166.00000, 0.03995)
(167.00000, 0.04007)
(168.00000, 0.04858)
(169.00000, 0.04660)
(170.00000, 0.04849)
(171.00000, 0.04858)
(172.00000, 0.06050)
(173.00000, 0.04848)
(174.00000, 0.04868)
(175.00000, 0.04680)
(176.00000, 0.04699)
(177.00000, 0.05078)
(178.00000, 0.04643)
(179.00000, 0.04896)
(180.00000, 0.04569)
(181.00000, 0.03765)
(182.00000, 0.04124)
(183.00000, 0.04650)
(184.00000, 0.03792)
(185.00000, 0.03466)
(186.00000, 0.04551)
(187.00000, 0.03746)
(188.00000, 0.03904)
(189.00000, 0.04123)
(190.00000, 0.03942)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,IndianRed2] plot coordinates {
(20.00000, 0.28596)
(21.00000, 0.47550)
(22.00000, 0.31089)
(23.00000, 0.35355)
(24.00000, 0.30123)
(25.00000, 0.34009)
(26.00000, 0.34487)
(27.00000, 0.28088)
(28.00000, 0.32144)
(29.00000, 0.31962)
(30.00000, 0.26727)
(31.00000, 0.33036)
(32.00000, 0.29463)
(33.00000, 0.34548)
(34.00000, 0.26832)
(35.00000, 0.32561)
(36.00000, 0.28303)
(37.00000, 0.28023)
(38.00000, 0.24657)
(39.00000, 0.28145)
(40.00000, 0.26095)
(41.00000, 0.31265)
(42.00000, 0.27290)
(43.00000, 0.29535)
(44.00000, 0.25229)
(45.00000, 0.25399)
(46.00000, 0.25567)
(47.00000, 0.22926)
(48.00000, 0.18480)
(49.00000, 0.19954)
(50.00000, 0.18610)
(51.00000, 0.23183)
(52.00000, 0.25353)
(53.00000, 0.20195)
(54.00000, 0.18665)
(55.00000, 0.22137)
(56.00000, 0.18075)
(57.00000, 0.21046)
(58.00000, 0.12689)
(59.00000, 0.17476)
(60.00000, 0.15611)
(61.00000, 0.14700)
(62.00000, 0.14965)
(63.00000, 0.15778)
(64.00000, 0.15014)
(65.00000, 0.16395)
(66.00000, 0.14659)
(67.00000, 0.12550)
(68.00000, 0.13779)
(69.00000, 0.14082)
(70.00000, 0.12620)
(71.00000, 0.11451)
(72.00000, 0.11989)
(73.00000, 0.09691)
(74.00000, 0.09113)
(75.00000, 0.09782)
(76.00000, 0.10189)
(77.00000, 0.10461)
(78.00000, 0.09586)
(79.00000, 0.08333)
(80.00000, 0.10866)
(81.00000, 0.10512)
(82.00000, 0.08812)
(83.00000, 0.11017)
(84.00000, 0.10499)
(85.00000, 0.08439)
(86.00000, 0.08843)
(87.00000, 0.09513)
(88.00000, 0.08477)
(89.00000, 0.08317)
(90.00000, 0.06921)
(91.00000, 0.07315)
(92.00000, 0.07854)
(93.00000, 0.09124)
(94.00000, 0.08626)
(95.00000, 0.07431)
(96.00000, 0.07460)
(97.00000, 0.07980)
(98.00000, 0.09045)
(99.00000, 0.06298)
(100.00000, 0.07004)
(101.00000, 0.06736)
(102.00000, 0.05584)
(103.00000, 0.06646)
(104.00000, 0.08659)
(105.00000, 0.08011)
(106.00000, 0.05802)
(107.00000, 0.06306)
(108.00000, 0.07115)
(109.00000, 0.07393)
(110.00000, 0.06677)
(111.00000, 0.05315)
(112.00000, 0.06838)
(113.00000, 0.05775)
(114.00000, 0.06083)
(115.00000, 0.06805)
(116.00000, 0.06084)
(117.00000, 0.06743)
(118.00000, 0.05520)
(119.00000, 0.04929)
(120.00000, 0.05837)
(121.00000, 0.05885)
(122.00000, 0.04876)
(123.00000, 0.05936)
(124.00000, 0.06194)
(125.00000, 0.06010)
(126.00000, 0.05871)
(127.00000, 0.06436)
(128.00000, 0.06988)
(129.00000, 0.05651)
(130.00000, 0.06089)
(131.00000, 0.05517)
(132.00000, 0.06062)
(133.00000, 0.04803)
(134.00000, 0.05116)
(135.00000, 0.04462)
(136.00000, 0.05421)
(137.00000, 0.06490)
(138.00000, 0.07021)
(139.00000, 0.04897)
(140.00000, 0.05496)
(141.00000, 0.04853)
(142.00000, 0.03758)
(143.00000, 0.05213)
(144.00000, 0.05511)
(145.00000, 0.05243)
(146.00000, 0.05778)
(147.00000, 0.05513)
(148.00000, 0.05749)
(149.00000, 0.04795)
(150.00000, 0.05414)
(151.00000, 0.05446)
(152.00000, 0.06103)
(153.00000, 0.05914)
(154.00000, 0.05464)
(155.00000, 0.06723)
(156.00000, 0.05987)
(157.00000, 0.05029)
(158.00000, 0.06880)
(159.00000, 0.06530)
(160.00000, 0.05923)
(161.00000, 0.06264)
(162.00000, 0.06125)
(163.00000, 0.05732)
(164.00000, 0.07820)
(165.00000, 0.05393)
(166.00000, 0.07303)
(167.00000, 0.05358)
(168.00000, 0.06456)
(169.00000, 0.05649)
(170.00000, 0.06842)
(171.00000, 0.06889)
(172.00000, 0.06154)
(173.00000, 0.06339)
(174.00000, 0.06120)
(175.00000, 0.06649)
(176.00000, 0.05969)
(177.00000, 0.05590)
(178.00000, 0.06500)
(179.00000, 0.05846)
(180.00000, 0.06246)
(181.00000, 0.06911)
(182.00000, 0.05145)
(183.00000, 0.05582)
(184.00000, 0.06031)
(185.00000, 0.06547)
(186.00000, 0.07122)
(187.00000, 0.06695)
(188.00000, 0.05678)
(189.00000, 0.06286)
(190.00000, 0.06839)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,gray] plot coordinates {
(20.00000, 0.21791)
(21.00000, 0.17214)
(22.00000, 0.34552)
(23.00000, 0.23270)
(24.00000, 0.18491)
(25.00000, 0.10873)
(26.00000, 0.15927)
(27.00000, 0.12376)
(28.00000, 0.12073)
(29.00000, 0.11830)
(30.00000, 0.12537)
(31.00000, 0.11040)
(32.00000, 0.11417)
(33.00000, 0.09983)
(34.00000, 0.11164)
(35.00000, 0.08800)
(36.00000, 0.11589)
(37.00000, 0.10221)
(38.00000, 0.11171)
(39.00000, 0.09857)
(40.00000, 0.12841)
(41.00000, 0.10383)
(42.00000, 0.09987)
(43.00000, 0.12904)
(44.00000, 0.09719)
(45.00000, 0.09226)
(46.00000, 0.10965)
(47.00000, 0.09375)
(48.00000, 0.09191)
(49.00000, 0.09660)
(50.00000, 0.07068)
(51.00000, 0.08109)
(52.00000, 0.06838)
(53.00000, 0.09139)
(54.00000, 0.08301)
(55.00000, 0.08190)
(56.00000, 0.05955)
(57.00000, 0.06858)
(58.00000, 0.08580)
(59.00000, 0.09421)
(60.00000, 0.08041)
(61.00000, 0.08523)
(62.00000, 0.06887)
(63.00000, 0.08260)
(64.00000, 0.06918)
(65.00000, 0.08689)
(66.00000, 0.08805)
(67.00000, 0.07573)
(68.00000, 0.06626)
(69.00000, 0.06651)
(70.00000, 0.05674)
(71.00000, 0.07292)
(72.00000, 0.07879)
(73.00000, 0.05979)
(74.00000, 0.06659)
(75.00000, 0.08119)
(76.00000, 0.07160)
(77.00000, 0.07066)
(78.00000, 0.06897)
(79.00000, 0.08351)
(80.00000, 0.08262)
(81.00000, 0.06833)
(82.00000, 0.07814)
(83.00000, 0.06707)
(84.00000, 0.06785)
(85.00000, 0.06927)
(86.00000, 0.06774)
(87.00000, 0.05938)
(88.00000, 0.08287)
(89.00000, 0.05295)
(90.00000, 0.05382)
(91.00000, 0.06413)
(92.00000, 0.05358)
(93.00000, 0.06578)
(94.00000, 0.06088)
(95.00000, 0.08160)
(96.00000, 0.06654)
(97.00000, 0.06339)
(98.00000, 0.06781)
(99.00000, 0.06241)
(100.00000, 0.07088)
(101.00000, 0.07633)
(102.00000, 0.05553)
(103.00000, 0.06523)
(104.00000, 0.06232)
(105.00000, 0.06462)
(106.00000, 0.06106)
(107.00000, 0.05866)
(108.00000, 0.07749)
(109.00000, 0.06652)
(110.00000, 0.05915)
(111.00000, 0.05842)
(112.00000, 0.05703)
(113.00000, 0.05733)
(114.00000, 0.06633)
(115.00000, 0.07834)
(116.00000, 0.07178)
(117.00000, 0.06424)
(118.00000, 0.06592)
(119.00000, 0.07223)
(120.00000, 0.06991)
(121.00000, 0.08165)
(122.00000, 0.06652)
(123.00000, 0.07860)
(124.00000, 0.09161)
(125.00000, 0.07120)
(126.00000, 0.07441)
(127.00000, 0.08028)
(128.00000, 0.08157)
(129.00000, 0.08208)
(130.00000, 0.08570)
(131.00000, 0.07671)
(132.00000, 0.08483)
(133.00000, 0.09294)
(134.00000, 0.09025)
(135.00000, 0.08866)
(136.00000, 0.09043)
(137.00000, 0.09565)
(138.00000, 0.09310)
(139.00000, 0.10861)
(140.00000, 0.11199)
(141.00000, 0.10724)
(142.00000, 0.10537)
(143.00000, 0.08894)
(144.00000, 0.09709)
(145.00000, 0.10156)
(146.00000, 0.08679)
(147.00000, 0.10587)
(148.00000, 0.10051)
(149.00000, 0.11610)
(150.00000, 0.11400)
(151.00000, 0.10246)
(152.00000, 0.10133)
(153.00000, 0.10394)
(154.00000, 0.09351)
(155.00000, 0.09952)
(156.00000, 0.09862)
(157.00000, 0.09600)
(158.00000, 0.08188)
(159.00000, 0.08896)
(160.00000, 0.09638)
(161.00000, 0.07539)
(162.00000, 0.08815)
(163.00000, 0.09632)
(164.00000, 0.09524)
(165.00000, 0.08721)
(166.00000, 0.07268)
(167.00000, 0.08807)
(168.00000, 0.08507)
(169.00000, 0.07788)
(170.00000, 0.08656)
(171.00000, 0.09459)
(172.00000, 0.07174)
(173.00000, 0.07931)
(174.00000, 0.09333)
(175.00000, 0.06592)
(176.00000, 0.08245)
(177.00000, 0.07051)
(178.00000, 0.06095)
(179.00000, 0.08102)
(180.00000, 0.08479)
(181.00000, 0.08511)
(182.00000, 0.08130)
(183.00000, 0.08106)
(184.00000, 0.06496)
(185.00000, 0.05992)
(186.00000, 0.07433)
(187.00000, 0.05680)
(188.00000, 0.07728)
(189.00000, 0.06470)
(190.00000, 0.07004)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,Cyan1] plot coordinates {
(20.00000, 0.19549)
(21.00000, 0.14969)
(22.00000, 0.14596)
(23.00000, 0.15093)
(24.00000, 0.38668)
(25.00000, 0.19334)
(26.00000, 0.15234)
(27.00000, 0.14758)
(28.00000, 0.12237)
(29.00000, 0.15897)
(30.00000, 0.16086)
(31.00000, 0.14732)
(32.00000, 0.15715)
(33.00000, 0.11130)
(34.00000, 0.13201)
(35.00000, 0.11897)
(36.00000, 0.12589)
(37.00000, 0.12425)
(38.00000, 0.12565)
(39.00000, 0.08614)
(40.00000, 0.09411)
(41.00000, 0.10709)
(42.00000, 0.10303)
(43.00000, 0.12299)
(44.00000, 0.11265)
(45.00000, 0.11826)
(46.00000, 0.10236)
(47.00000, 0.10479)
(48.00000, 0.09835)
(49.00000, 0.10723)
(50.00000, 0.08058)
(51.00000, 0.09421)
(52.00000, 0.07506)
(53.00000, 0.07853)
(54.00000, 0.10740)
(55.00000, 0.09009)
(56.00000, 0.10087)
(57.00000, 0.07919)
(58.00000, 0.07043)
(59.00000, 0.07395)
(60.00000, 0.08174)
(61.00000, 0.06945)
(62.00000, 0.08182)
(63.00000, 0.08475)
(64.00000, 0.08379)
(65.00000, 0.09519)
(66.00000, 0.08501)
(67.00000, 0.06425)
(68.00000, 0.07413)
(69.00000, 0.06393)
(70.00000, 0.07146)
(71.00000, 0.07685)
(72.00000, 0.06840)
(73.00000, 0.06765)
(74.00000, 0.07473)
(75.00000, 0.06991)
(76.00000, 0.06650)
(77.00000, 0.06058)
(78.00000, 0.05926)
(79.00000, 0.06449)
(80.00000, 0.05265)
(81.00000, 0.07319)
(82.00000, 0.07824)
(83.00000, 0.05932)
(84.00000, 0.06932)
(85.00000, 0.06575)
(86.00000, 0.07339)
(87.00000, 0.07109)
(88.00000, 0.06479)
(89.00000, 0.05926)
(90.00000, 0.07923)
(91.00000, 0.06611)
(92.00000, 0.07012)
(93.00000, 0.06745)
(94.00000, 0.06294)
(95.00000, 0.06251)
(96.00000, 0.06620)
(97.00000, 0.06999)
(98.00000, 0.06721)
(99.00000, 0.07527)
(100.00000, 0.07029)
(101.00000, 0.06371)
(102.00000, 0.06505)
(103.00000, 0.07282)
(104.00000, 0.07637)
(105.00000, 0.06811)
(106.00000, 0.08392)
(107.00000, 0.06480)
(108.00000, 0.06810)
(109.00000, 0.06383)
(110.00000, 0.07422)
(111.00000, 0.06613)
(112.00000, 0.06252)
(113.00000, 0.06520)
(114.00000, 0.05822)
(115.00000, 0.07028)
(116.00000, 0.05925)
(117.00000, 0.04615)
(118.00000, 0.05223)
(119.00000, 0.05812)
(120.00000, 0.05042)
(121.00000, 0.05436)
(122.00000, 0.06170)
(123.00000, 0.06435)
(124.00000, 0.06009)
(125.00000, 0.04177)
(126.00000, 0.05171)
(127.00000, 0.05268)
(128.00000, 0.05724)
(129.00000, 0.04501)
(130.00000, 0.05397)
(131.00000, 0.05081)
(132.00000, 0.04898)
(133.00000, 0.05572)
(134.00000, 0.05555)
(135.00000, 0.04551)
(136.00000, 0.05496)
(137.00000, 0.06638)
(138.00000, 0.04620)
(139.00000, 0.06471)
(140.00000, 0.06755)
(141.00000, 0.05505)
(142.00000, 0.06332)
(143.00000, 0.05425)
(144.00000, 0.05670)
(145.00000, 0.04892)
(146.00000, 0.05828)
(147.00000, 0.06177)
(148.00000, 0.06391)
(149.00000, 0.05937)
(150.00000, 0.05621)
(151.00000, 0.06838)
(152.00000, 0.05601)
(153.00000, 0.06177)
(154.00000, 0.05908)
(155.00000, 0.05350)
(156.00000, 0.06150)
(157.00000, 0.06533)
(158.00000, 0.04824)
(159.00000, 0.05533)
(160.00000, 0.06808)
(161.00000, 0.04992)
(162.00000, 0.05654)
(163.00000, 0.06101)
(164.00000, 0.06367)
(165.00000, 0.05573)
(166.00000, 0.06078)
(167.00000, 0.06432)
(168.00000, 0.06279)
(169.00000, 0.06281)
(170.00000, 0.05473)
(171.00000, 0.06504)
(172.00000, 0.05758)
(173.00000, 0.05634)
(174.00000, 0.07066)
(175.00000, 0.07179)
(176.00000, 0.07400)
(177.00000, 0.06873)
(178.00000, 0.07565)
(179.00000, 0.06107)
(180.00000, 0.06261)
(181.00000, 0.06421)
(182.00000, 0.05820)
(183.00000, 0.05714)
(184.00000, 0.06463)
(185.00000, 0.06127)
(186.00000, 0.05137)
(187.00000, 0.06236)
(188.00000, 0.06699)
(189.00000, 0.06868)
(190.00000, 0.05820)
};
\addplot[thin,only marks, mark options={opacity=0.8},mark=*,mark size=.5pt,Cyan3] plot coordinates {
(20.00000, 0.18930)
(21.00000, 0.19338)
(22.00000, 0.16532)
(23.00000, 0.15453)
(24.00000, 0.13879)
(25.00000, 0.14638)
(26.00000, 0.08151)
(27.00000, 0.13629)
(28.00000, 0.12988)
(29.00000, 0.12630)
(30.00000, 0.13121)
(31.00000, 0.11087)
(32.00000, 0.10975)
(33.00000, 0.11647)
(34.00000, 0.12402)
(35.00000, 0.11138)
(36.00000, 0.11360)
(37.00000, 0.15203)
(38.00000, 0.11599)
(39.00000, 0.12659)
(40.00000, 0.13297)
(41.00000, 0.12608)
(42.00000, 0.10076)
(43.00000, 0.13924)
(44.00000, 0.11899)
(45.00000, 0.08753)
(46.00000, 0.09659)
(47.00000, 0.10931)
(48.00000, 0.08362)
(49.00000, 0.08136)
(50.00000, 0.09299)
(51.00000, 0.09847)
(52.00000, 0.08860)
(53.00000, 0.07824)
(54.00000, 0.09203)
(55.00000, 0.09404)
(56.00000, 0.06521)
(57.00000, 0.07802)
(58.00000, 0.06827)
(59.00000, 0.06689)
(60.00000, 0.07523)
(61.00000, 0.08086)
(62.00000, 0.07970)
(63.00000, 0.07589)
(64.00000, 0.08670)
(65.00000, 0.06157)
(66.00000, 0.07422)
(67.00000, 0.07693)
(68.00000, 0.08338)
(69.00000, 0.07911)
(70.00000, 0.07408)
(71.00000, 0.08187)
(72.00000, 0.07094)
(73.00000, 0.08283)
(74.00000, 0.06683)
(75.00000, 0.08664)
(76.00000, 0.07517)
(77.00000, 0.06144)
(78.00000, 0.07711)
(79.00000, 0.06571)
(80.00000, 0.08151)
(81.00000, 0.06886)
(82.00000, 0.05458)
(83.00000, 0.06732)
(84.00000, 0.05707)
(85.00000, 0.05899)
(86.00000, 0.07849)
(87.00000, 0.07473)
(88.00000, 0.06520)
(89.00000, 0.06813)
(90.00000, 0.06920)
(91.00000, 0.06055)
(92.00000, 0.06924)
(93.00000, 0.05851)
(94.00000, 0.07002)
(95.00000, 0.05673)
(96.00000, 0.06198)
(97.00000, 0.05866)
(98.00000, 0.05586)
(99.00000, 0.06174)
(100.00000, 0.07222)
(101.00000, 0.07026)
(102.00000, 0.04351)
(103.00000, 0.07358)
(104.00000, 0.05934)
(105.00000, 0.05969)
(106.00000, 0.07123)
(107.00000, 0.06556)
(108.00000, 0.06363)
(109.00000, 0.05918)
(110.00000, 0.05579)
(111.00000, 0.06250)
(112.00000, 0.06631)
(113.00000, 0.05050)
(114.00000, 0.05178)
(115.00000, 0.05757)
(116.00000, 0.05986)
(117.00000, 0.05207)
(118.00000, 0.05246)
(119.00000, 0.05449)
(120.00000, 0.06259)
(121.00000, 0.05906)
(122.00000, 0.06503)
(123.00000, 0.06113)
(124.00000, 0.05066)
(125.00000, 0.05520)
(126.00000, 0.05708)
(127.00000, 0.05824)
(128.00000, 0.04905)
(129.00000, 0.05711)
(130.00000, 0.04921)
(131.00000, 0.05445)
(132.00000, 0.04890)
(133.00000, 0.05632)
(134.00000, 0.04265)
(135.00000, 0.05146)
(136.00000, 0.03956)
(137.00000, 0.05373)
(138.00000, 0.05601)
(139.00000, 0.05113)
(140.00000, 0.05023)
(141.00000, 0.04468)
(142.00000, 0.04938)
(143.00000, 0.04733)
(144.00000, 0.05770)
(145.00000, 0.03798)
(146.00000, 0.04857)
(147.00000, 0.05257)
(148.00000, 0.04535)
(149.00000, 0.04036)
(150.00000, 0.03485)
(151.00000, 0.04726)
(152.00000, 0.04816)
(153.00000, 0.04452)
(154.00000, 0.03152)
(155.00000, 0.04766)
(156.00000, 0.04823)
(157.00000, 0.04615)
(158.00000, 0.05289)
(159.00000, 0.04216)
(160.00000, 0.04734)
(161.00000, 0.04915)
(162.00000, 0.05209)
(163.00000, 0.04488)
(164.00000, 0.04258)
(165.00000, 0.04519)
(166.00000, 0.05152)
(167.00000, 0.04066)
(168.00000, 0.04184)
(169.00000, 0.04296)
(170.00000, 0.04504)
(171.00000, 0.04566)
(172.00000, 0.04507)
(173.00000, 0.04669)
(174.00000, 0.04304)
(175.00000, 0.04682)
(176.00000, 0.04552)
(177.00000, 0.04068)
(178.00000, 0.04707)
(179.00000, 0.04519)
(180.00000, 0.04180)
(181.00000, 0.03919)
(182.00000, 0.04752)
(183.00000, 0.04258)
(184.00000, 0.04349)
(185.00000, 0.04076)
(186.00000, 0.04846)
(187.00000, 0.04210)
(188.00000, 0.04351)
(189.00000, 0.04253)
(190.00000, 0.04429)
};


==> Figures/data1.tex <==
\addplot[ ultra thick,const plot,Red4] plot coordinates {
(1.00000, 0.50000)
(2.00000, 0.50000)
(3.00000, -0.50000)
(4.00000, -0.50000)
(5.00000, 0.50000)
(6.00000, 0.50000)
(7.00000, 0.50000)
(8.00000, 0.50000)
(9.00000, 0.50000)
(10.00000, 0.50000)
(11.00000, 0.50000)
(12.00000, 0.50000)
(13.00000, 0.50000)
(14.00000, -0.50000)
(15.00000, 0.50000)
(16.00000, 0.50000)
(17.00000, 0.50000)
(18.00000, 0.50000)
(19.00000, 0.50000)
(20.00000, 0.50000)
(21.00000, 0.50000)
(22.00000, 0.50000)
(23.00000, -0.50000)
(24.00000, 0.50000)
(25.00000, 0.50000)
(26.00000, -0.50000)
(27.00000, 0.50000)
(28.00000, 0.50000)
(29.00000, 0.50000)
(30.00000, 0.50000)
(31.00000, 0.50000)
(32.00000, 0.50000)
(33.00000, -0.50000)
(34.00000, 0.50000)
(35.00000, 0.50000)
(36.00000, 0.50000)
(37.00000, 0.50000)
(38.00000, 0.50000)
(39.00000, 0.50000)
(40.00000, 0.50000)
(41.00000, 0.50000)
(42.00000, 0.50000)
(43.00000, 0.50000)
(44.00000, 0.50000)
(45.00000, 0.50000)
(46.00000, 0.50000)
(47.00000, 0.50000)
(48.00000, 0.50000)
(49.00000, 0.50000)
(50.00000, 0.50000)
(51.00000, 0.50000)
(52.00000, 0.50000)
(53.00000, 0.50000)
(54.00000, 0.50000)
(55.00000, 0.50000)
(56.00000, 0.50000)
(57.00000, 0.50000)
(58.00000, 0.50000)
(59.00000, 0.50000)
(60.00000, 0.50000)
(61.00000, 0.50000)
(62.00000, 0.50000)
(63.00000, 0.50000)
(64.00000, 0.50000)
(65.00000, 0.50000)
(66.00000, 0.50000)
(67.00000, 0.50000)
(68.00000, 0.50000)
(69.00000, 0.50000)
(70.00000, 0.50000)
(71.00000, 0.50000)
(72.00000, -0.50000)
(73.00000, -0.50000)
(74.00000, 0.50000)
(75.00000, 0.50000)
(76.00000, 0.50000)
(77.00000, 0.50000)
(78.00000, 0.50000)
(79.00000, -0.50000)
(80.00000, 0.50000)
(81.00000, 0.50000)
(82.00000, 0.50000)
(83.00000, 0.50000)
(84.00000, 0.50000)
(85.00000, 0.50000)
(86.00000, 0.50000)
(87.00000, 0.50000)
(88.00000, 0.50000)
(89.00000, 0.50000)
(90.00000, -0.50000)
(91.00000, -0.50000)
(92.00000, 0.50000)
(93.00000, 0.50000)
(94.00000, 0.50000)
(95.00000, 0.50000)
(96.00000, 0.50000)
(97.00000, -0.50000)
(98.00000, -0.50000)
(99.00000, -0.50000)
(100.00000, -0.50000)
(101.00000, 0.50000)
(102.00000, 0.50000)
(103.00000, 0.50000)
(104.00000, 0.50000)
(105.00000, 0.50000)
(106.00000, 0.50000)
(107.00000, 0.50000)
(108.00000, 0.50000)
(109.00000, 0.50000)
(110.00000, 0.50000)
(111.00000, 0.50000)
(112.00000, 0.50000)
(113.00000, 0.50000)
(114.00000, 0.50000)
(115.00000, 0.50000)
(116.00000, 0.50000)
(117.00000, 0.50000)
(118.00000, 0.50000)
(119.00000, 0.50000)
(120.00000, 0.50000)
(121.00000, 0.50000)
(122.00000, 0.50000)
(123.00000, 0.50000)
(124.00000, 0.50000)
(125.00000, 0.50000)
(126.00000, 0.50000)
(127.00000, 0.50000)
(128.00000, 0.50000)
(129.00000, -0.50000)
(130.00000, 0.50000)
(131.00000, 0.50000)
(132.00000, 0.50000)
(133.00000, 0.50000)
(134.00000, 0.50000)
(135.00000, 0.50000)
(136.00000, 0.50000)
(137.00000, 0.50000)
(138.00000, 0.50000)
(139.00000, 0.50000)
(140.00000, 0.50000)
(141.00000, 0.50000)
(142.00000, 0.50000)
(143.00000, 0.50000)
(144.00000, -0.50000)
(145.00000, -0.50000)
(146.00000, 0.50000)
(147.00000, -0.50000)
(148.00000, 0.50000)
(149.00000, 0.50000)
(150.00000, 0.50000)
(151.00000, 0.50000)
(152.00000, 0.50000)
(153.00000, 0.50000)
(154.00000, 0.50000)
(155.00000, 0.50000)
(156.00000, 0.50000)
(157.00000, 0.50000)
(158.00000, 0.50000)
(159.00000, 0.50000)
(160.00000, 0.50000)
(161.00000, 0.50000)
(162.00000, 0.50000)
(163.00000, 0.50000)
(164.00000, 0.50000)
(165.00000, 0.50000)
(166.00000, 0.50000)
(167.00000, 0.50000)
(168.00000, 0.50000)
(169.00000, 0.50000)
(170.00000, 0.50000)
(171.00000, 0.50000)
(172.00000, 0.50000)
(173.00000, 0.50000)
(174.00000, 0.50000)
(175.00000, 0.50000)
(176.00000, 0.50000)
(177.00000, 0.50000)
(178.00000, 0.50000)
(179.00000, 0.50000)
(180.00000, 0.50000)
(181.00000, 0.50000)
(182.00000, -0.50000)
(183.00000, -0.50000)
(184.00000, 0.50000)
(185.00000, 0.50000)
(186.00000, 0.50000)
(187.00000, 0.50000)
(188.00000, 0.50000)
(189.00000, -0.50000)
(190.00000, 0.50000)
(191.00000, 0.50000)
(192.00000, 0.50000)
(193.00000, 0.50000)
(194.00000, 0.50000)
(195.00000, 0.50000)
(196.00000, 0.50000)
(197.00000, 0.50000)
(198.00000, 0.50000)
(199.00000, 0.50000)
(200.00000, 0.50000)
(201.00000, 0.50000)
(202.00000, 0.50000)
(203.00000, 0.50000)
(204.00000, 0.50000)
(205.00000, 0.50000)
(206.00000, -0.50000)
(207.00000, -0.50000)
(208.00000, 0.50000)
(209.00000, 0.50000)
(210.00000, 0.50000)
(211.00000, 0.50000)
(212.00000, 0.50000)
(213.00000, 0.50000)
(214.00000, -0.50000)
(215.00000, 0.50000)
(216.00000, 0.50000)
(217.00000, 0.50000)
(218.00000, 0.50000)
(219.00000, -0.50000)
(220.00000, 0.50000)
(221.00000, 0.50000)
(222.00000, -0.50000)
(223.00000, 0.50000)
(224.00000, -0.50000)
(225.00000, -0.50000)
(226.00000, 0.50000)
(227.00000, 0.50000)
(228.00000, 0.50000)
(229.00000, 0.50000)
(230.00000, 0.50000)
(231.00000, 0.50000)
(232.00000, 0.50000)
(233.00000, 0.50000)
(234.00000, 0.50000)
(235.00000, 0.50000)
(236.00000, 0.50000)
(237.00000, 0.50000)
(238.00000, 0.50000)
(239.00000, 0.50000)
(240.00000, 0.50000)
(241.00000, 0.50000)
(242.00000, -0.50000)
(243.00000, 0.50000)
(244.00000, 0.50000)
(245.00000, 0.50000)
(246.00000, 0.50000)
(247.00000, 0.50000)
(248.00000, 0.50000)
(249.00000, 0.50000)
(250.00000, 0.50000)
(251.00000, -0.50000)
(252.00000, -0.50000)
(253.00000, -0.50000)
(254.00000, -0.50000)
(255.00000, 0.50000)
(256.00000, 0.50000)
(257.00000, 0.50000)
(258.00000, -0.50000)
(259.00000, 0.50000)
(260.00000, 0.50000)
(261.00000, 0.50000)
(262.00000, 0.50000)
(263.00000, -0.50000)
(264.00000, -0.50000)
(265.00000, -0.50000)
(266.00000, 0.50000)
(267.00000, 0.50000)
(268.00000, -0.50000)
(269.00000, 0.50000)
(270.00000, 0.50000)
(271.00000, 0.50000)
(272.00000, -0.50000)
(273.00000, 0.50000)
(274.00000, -0.50000)
(275.00000, 0.50000)
(276.00000, 0.50000)
(277.00000, 0.50000)
(278.00000, 0.50000)
(279.00000, 0.50000)
(280.00000, 0.50000)
(281.00000, 0.50000)
(282.00000, 0.50000)
(283.00000, 0.50000)
(284.00000, 0.50000)
(285.00000, 0.50000)
(286.00000, -0.50000)
(287.00000, -0.50000)
(288.00000, -0.50000)
(289.00000, 0.50000)
(290.00000, 0.50000)
(291.00000, 0.50000)
(292.00000, 0.50000)
(293.00000, 0.50000)
(294.00000, 0.50000)
(295.00000, 0.50000)
(296.00000, 0.50000)
(297.00000, 0.50000)
(298.00000, 0.50000)
(299.00000, 0.50000)
(300.00000, 0.50000)
(301.00000, 0.50000)
(302.00000, -0.50000)
(303.00000, 0.50000)
(304.00000, 0.50000)
(305.00000, 0.50000)
(306.00000, 0.50000)
(307.00000, 0.50000)
(308.00000, -0.50000)
(309.00000, 0.50000)
(310.00000, 0.50000)
(311.00000, 0.50000)
(312.00000, 0.50000)
(313.00000, 0.50000)
(314.00000, 0.50000)
(315.00000, 0.50000)
(316.00000, 0.50000)
(317.00000, 0.50000)
(318.00000, 0.50000)
(319.00000, 0.50000)
(320.00000, 0.50000)
(321.00000, 0.50000)
(322.00000, 0.50000)
(323.00000, 0.50000)
(324.00000, 0.50000)
(325.00000, -0.50000)
(326.00000, 0.50000)
(327.00000, 0.50000)
(328.00000, 0.50000)
(329.00000, 0.50000)
(330.00000, -0.50000)
(331.00000, -0.50000)
(332.00000, -0.50000)
(333.00000, -0.50000)
(334.00000, -0.50000)
(335.00000, 0.50000)
(336.00000, 0.50000)
(337.00000, -0.50000)
(338.00000, 0.50000)
(339.00000, 0.50000)
(340.00000, 0.50000)
(341.00000, 0.50000)
(342.00000, 0.50000)
(343.00000, -0.50000)
(344.00000, -0.50000)
(345.00000, -0.50000)
(346.00000, 0.50000)
(347.00000, 0.50000)
(348.00000, 0.50000)
(349.00000, 0.50000)
(350.00000, -0.50000)
(351.00000, 0.50000)
(352.00000, 0.50000)
(353.00000, 0.50000)
(354.00000, 0.50000)
(355.00000, 0.50000)
(356.00000, 0.50000)
(357.00000, 0.50000)
(358.00000, 0.50000)
(359.00000, 0.50000)
(360.00000, -0.50000)
(361.00000, -0.50000)
(362.00000, 0.50000)
(363.00000, 0.50000)
(364.00000, 0.50000)
(365.00000, 0.50000)
(366.00000, 0.50000)
(367.00000, 0.50000)
(368.00000, -0.50000)
(369.00000, -0.50000)
(370.00000, 0.50000)
(371.00000, 0.50000)
(372.00000, 0.50000)
(373.00000, 0.50000)
(374.00000, 0.50000)
(375.00000, 0.50000)
(376.00000, 0.50000)
(377.00000, 0.50000)
(378.00000, 0.50000)
(379.00000, 0.50000)
(380.00000, -0.50000)
(381.00000, 0.50000)
(382.00000, 0.50000)
(383.00000, 0.50000)
(384.00000, 0.50000)
(385.00000, 0.50000)
(386.00000, 0.50000)
(387.00000, 0.50000)
(388.00000, 0.50000)
(389.00000, 0.50000)
(390.00000, 0.50000)
(391.00000, 0.50000)
(392.00000, 0.50000)
(393.00000, 0.50000)
(394.00000, 0.50000)
(395.00000, 0.50000)
(396.00000, 0.50000)
(397.00000, 0.50000)
(398.00000, 0.50000)
(399.00000, 0.50000)
(400.00000, 0.50000)
};


==> Figures/data2.tex <==
\addplot[ ultra thick,const plot,DodgerBlue4] plot coordinates {
(1.00000, -0.50000)
(2.00000, -0.50000)
(3.00000, 0.50000)
(4.00000, -0.50000)
(5.00000, -0.50000)
(6.00000, -0.50000)
(7.00000, 0.50000)
(8.00000, -0.50000)
(9.00000, 0.50000)
(10.00000, -0.50000)
(11.00000, -0.50000)
(12.00000, -0.50000)
(13.00000, -0.50000)
(14.00000, 0.50000)
(15.00000, -0.50000)
(16.00000, -0.50000)
(17.00000, -0.50000)
(18.00000, -0.50000)
(19.00000, -0.50000)
(20.00000, -0.50000)
(21.00000, -0.50000)
(22.00000, -0.50000)
(23.00000, -0.50000)
(24.00000, -0.50000)
(25.00000, -0.50000)
(26.00000, -0.50000)
(27.00000, -0.50000)
(28.00000, -0.50000)
(29.00000, 0.50000)
(30.00000, -0.50000)
(31.00000, 0.50000)
(32.00000, 0.50000)
(33.00000, -0.50000)
(34.00000, 0.50000)
(35.00000, -0.50000)
(36.00000, -0.50000)
(37.00000, 0.50000)
(38.00000, 0.50000)
(39.00000, -0.50000)
(40.00000, -0.50000)
(41.00000, -0.50000)
(42.00000, 0.50000)
(43.00000, -0.50000)
(44.00000, -0.50000)
(45.00000, 0.50000)
(46.00000, -0.50000)
(47.00000, -0.50000)
(48.00000, -0.50000)
(49.00000, -0.50000)
(50.00000, -0.50000)
(51.00000, 0.50000)
(52.00000, -0.50000)
(53.00000, -0.50000)
(54.00000, -0.50000)
(55.00000, -0.50000)
(56.00000, 0.50000)
(57.00000, -0.50000)
(58.00000, -0.50000)
(59.00000, -0.50000)
(60.00000, -0.50000)
(61.00000, 0.50000)
(62.00000, -0.50000)
(63.00000, -0.50000)
(64.00000, -0.50000)
(65.00000, -0.50000)
(66.00000, -0.50000)
(67.00000, -0.50000)
(68.00000, -0.50000)
(69.00000, -0.50000)
(70.00000, -0.50000)
(71.00000, -0.50000)
(72.00000, -0.50000)
(73.00000, -0.50000)
(74.00000, -0.50000)
(75.00000, 0.50000)
(76.00000, -0.50000)
(77.00000, -0.50000)
(78.00000, -0.50000)
(79.00000, -0.50000)
(80.00000, 0.50000)
(81.00000, -0.50000)
(82.00000, -0.50000)
(83.00000, -0.50000)
(84.00000, -0.50000)
(85.00000, -0.50000)
(86.00000, -0.50000)
(87.00000, -0.50000)
(88.00000, -0.50000)
(89.00000, 0.50000)
(90.00000, -0.50000)
(91.00000, 0.50000)
(92.00000, -0.50000)
(93.00000, -0.50000)
(94.00000, -0.50000)
(95.00000, -0.50000)
(96.00000, 0.50000)
(97.00000, 0.50000)
(98.00000, -0.50000)
(99.00000, 0.50000)
(100.00000, -0.50000)
(101.00000, -0.50000)
(102.00000, -0.50000)
(103.00000, 0.50000)
(104.00000, -0.50000)
(105.00000, -0.50000)
(106.00000, -0.50000)
(107.00000, -0.50000)
(108.00000, -0.50000)
(109.00000, -0.50000)
(110.00000, -0.50000)
(111.00000, -0.50000)
(112.00000, -0.50000)
(113.00000, -0.50000)
(114.00000, -0.50000)
(115.00000, -0.50000)
(116.00000, 0.50000)
(117.00000, -0.50000)
(118.00000, -0.50000)
(119.00000, -0.50000)
(120.00000, -0.50000)
(121.00000, -0.50000)
(122.00000, -0.50000)
(123.00000, -0.50000)
(124.00000, -0.50000)
(125.00000, 0.50000)
(126.00000, -0.50000)
(127.00000, -0.50000)
(128.00000, -0.50000)
(129.00000, 0.50000)
(130.00000, 0.50000)
(131.00000, -0.50000)
(132.00000, 0.50000)
(133.00000, -0.50000)
(134.00000, 0.50000)
(135.00000, -0.50000)
(136.00000, -0.50000)
(137.00000, -0.50000)
(138.00000, -0.50000)
(139.00000, -0.50000)
(140.00000, -0.50000)
(141.00000, -0.50000)
(142.00000, -0.50000)
(143.00000, -0.50000)
(144.00000, 0.50000)
(145.00000, -0.50000)
(146.00000, -0.50000)
(147.00000, -0.50000)
(148.00000, -0.50000)
(149.00000, -0.50000)
(150.00000, -0.50000)
(151.00000, -0.50000)
(152.00000, -0.50000)
(153.00000, -0.50000)
(154.00000, -0.50000)
(155.00000, -0.50000)
(156.00000, -0.50000)
(157.00000, -0.50000)
(158.00000, 0.50000)
(159.00000, 0.50000)
(160.00000, -0.50000)
(161.00000, -0.50000)
(162.00000, 0.50000)
(163.00000, -0.50000)
(164.00000, -0.50000)
(165.00000, -0.50000)
(166.00000, -0.50000)
(167.00000, -0.50000)
(168.00000, 0.50000)
(169.00000, -0.50000)
(170.00000, 0.50000)
(171.00000, -0.50000)
(172.00000, -0.50000)
(173.00000, -0.50000)
(174.00000, 0.50000)
(175.00000, -0.50000)
(176.00000, 0.50000)
(177.00000, -0.50000)
(178.00000, -0.50000)
(179.00000, -0.50000)
(180.00000, -0.50000)
(181.00000, -0.50000)
(182.00000, -0.50000)
(183.00000, -0.50000)
(184.00000, -0.50000)
(185.00000, -0.50000)
(186.00000, -0.50000)
(187.00000, -0.50000)
(188.00000, -0.50000)
(189.00000, -0.50000)
(190.00000, 0.50000)
(191.00000, -0.50000)
(192.00000, -0.50000)
(193.00000, -0.50000)
(194.00000, -0.50000)
(195.00000, -0.50000)
(196.00000, -0.50000)
(197.00000, 0.50000)
(198.00000, -0.50000)
(199.00000, -0.50000)
(200.00000, -0.50000)
(201.00000, -0.50000)
(202.00000, -0.50000)
(203.00000, -0.50000)
(204.00000, -0.50000)
(205.00000, -0.50000)
(206.00000, -0.50000)
(207.00000, -0.50000)
(208.00000, -0.50000)
(209.00000, 0.50000)
(210.00000, -0.50000)
(211.00000, -0.50000)
(212.00000, 0.50000)
(213.00000, -0.50000)
(214.00000, -0.50000)
(215.00000, -0.50000)
(216.00000, -0.50000)
(217.00000, -0.50000)
(218.00000, -0.50000)
(219.00000, -0.50000)
(220.00000, -0.50000)
(221.00000, -0.50000)
(222.00000, 0.50000)
(223.00000, -0.50000)
(224.00000, -0.50000)
(225.00000, -0.50000)
(226.00000, -0.50000)
(227.00000, 0.50000)
(228.00000, -0.50000)
(229.00000, 0.50000)
(230.00000, -0.50000)
(231.00000, -0.50000)
(232.00000, 0.50000)
(233.00000, -0.50000)
(234.00000, -0.50000)
(235.00000, -0.50000)
(236.00000, -0.50000)
(237.00000, -0.50000)
(238.00000, -0.50000)
(239.00000, 0.50000)
(240.00000, -0.50000)
(241.00000, -0.50000)
(242.00000, -0.50000)
(243.00000, -0.50000)
(244.00000, 0.50000)
(245.00000, -0.50000)
(246.00000, -0.50000)
(247.00000, 0.50000)
(248.00000, -0.50000)
(249.00000, -0.50000)
(250.00000, -0.50000)
(251.00000, 0.50000)
(252.00000, -0.50000)
(253.00000, 0.50000)
(254.00000, -0.50000)
(255.00000, -0.50000)
(256.00000, 0.50000)
(257.00000, -0.50000)
(258.00000, 0.50000)
(259.00000, -0.50000)
(260.00000, -0.50000)
(261.00000, 0.50000)
(262.00000, -0.50000)
(263.00000, -0.50000)
(264.00000, -0.50000)
(265.00000, 0.50000)
(266.00000, -0.50000)
(267.00000, -0.50000)
(268.00000, -0.50000)
(269.00000, -0.50000)
(270.00000, -0.50000)
(271.00000, -0.50000)
(272.00000, -0.50000)
(273.00000, 0.50000)
(274.00000, -0.50000)
(275.00000, 0.50000)
(276.00000, -0.50000)
(277.00000, -0.50000)
(278.00000, -0.50000)
(279.00000, -0.50000)
(280.00000, 0.50000)
(281.00000, -0.50000)
(282.00000, 0.50000)
(283.00000, -0.50000)
(284.00000, 0.50000)
(285.00000, -0.50000)
(286.00000, 0.50000)
(287.00000, -0.50000)
(288.00000, -0.50000)
(289.00000, -0.50000)
(290.00000, -0.50000)
(291.00000, -0.50000)
(292.00000, 0.50000)
(293.00000, 0.50000)
(294.00000, -0.50000)
(295.00000, -0.50000)
(296.00000, -0.50000)
(297.00000, -0.50000)
(298.00000, 0.50000)
(299.00000, -0.50000)
(300.00000, -0.50000)
(301.00000, -0.50000)
(302.00000, 0.50000)
(303.00000, -0.50000)
(304.00000, -0.50000)
(305.00000, -0.50000)
(306.00000, 0.50000)
(307.00000, -0.50000)
(308.00000, -0.50000)
(309.00000, -0.50000)
(310.00000, -0.50000)
(311.00000, -0.50000)
(312.00000, -0.50000)
(313.00000, -0.50000)
(314.00000, -0.50000)
(315.00000, 0.50000)
(316.00000, -0.50000)
(317.00000, -0.50000)
(318.00000, -0.50000)
(319.00000, -0.50000)
(320.00000, -0.50000)
(321.00000, -0.50000)
(322.00000, -0.50000)
(323.00000, -0.50000)
(324.00000, -0.50000)
(325.00000, 0.50000)
(326.00000, 0.50000)
(327.00000, -0.50000)
(328.00000, 0.50000)
(329.00000, -0.50000)
(330.00000, -0.50000)
(331.00000, -0.50000)
(332.00000, -0.50000)
(333.00000, -0.50000)
(334.00000, -0.50000)
(335.00000, -0.50000)
(336.00000, -0.50000)
(337.00000, 0.50000)
(338.00000, -0.50000)
(339.00000, -0.50000)
(340.00000, -0.50000)
(341.00000, -0.50000)
(342.00000, -0.50000)
(343.00000, -0.50000)
(344.00000, -0.50000)
(345.00000, -0.50000)
(346.00000, -0.50000)
(347.00000, -0.50000)
(348.00000, 0.50000)
(349.00000, -0.50000)
(350.00000, -0.50000)
(351.00000, -0.50000)
(352.00000, 0.50000)
(353.00000, -0.50000)
(354.00000, -0.50000)
(355.00000, -0.50000)
(356.00000, -0.50000)
(357.00000, 0.50000)
(358.00000, -0.50000)
(359.00000, -0.50000)
(360.00000, -0.50000)
(361.00000, -0.50000)
(362.00000, -0.50000)
(363.00000, 0.50000)
(364.00000, -0.50000)
(365.00000, -0.50000)
(366.00000, 0.50000)
(367.00000, -0.50000)
(368.00000, -0.50000)
(369.00000, -0.50000)
(370.00000, 0.50000)
(371.00000, -0.50000)
(372.00000, 0.50000)
(373.00000, -0.50000)
(374.00000, 0.50000)
(375.00000, 0.50000)
(376.00000, -0.50000)
(377.00000, -0.50000)
(378.00000, -0.50000)
(379.00000, -0.50000)
(380.00000, -0.50000)
(381.00000, -0.50000)
(382.00000, -0.50000)
(383.00000, -0.50000)
(384.00000, -0.50000)
(385.00000, -0.50000)
(386.00000, -0.50000)
(387.00000, -0.50000)
(388.00000, -0.50000)
(389.00000, -0.50000)
(390.00000, 0.50000)
(391.00000, 0.50000)
(392.00000, -0.50000)
(393.00000, -0.50000)
(394.00000, 0.50000)
(395.00000, -0.50000)
(396.00000, -0.50000)
(397.00000, -0.50000)
(398.00000, -0.50000)
(399.00000, -0.50000)
(400.00000, 0.50000)
};


==> Figures/data3.tex <==
\addplot[ thick,const plot,black] plot coordinates {
(1.00000, -0.50000)
(2.00000, 0.50000)
(3.00000, 0.50000)
(4.00000, -0.50000)
(5.00000, -0.50000)
(6.00000, 0.50000)
(7.00000, -0.50000)
(8.00000, 0.50000)
(9.00000, -0.50000)
(10.00000, 0.50000)
(11.00000, 0.50000)
(12.00000, 0.50000)
(13.00000, 0.50000)
(14.00000, -0.50000)
(15.00000, 0.50000)
(16.00000, 0.50000)
(17.00000, 0.50000)
(18.00000, -0.50000)
(19.00000, 0.50000)
(20.00000, 0.50000)
(21.00000, 0.50000)
(22.00000, 0.50000)
(23.00000, -0.50000)
(24.00000, -0.50000)
(25.00000, -0.50000)
(26.00000, -0.50000)
(27.00000, 0.50000)
(28.00000, 0.50000)
(29.00000, -0.50000)
(30.00000, 0.50000)
(31.00000, 0.50000)
(32.00000, -0.50000)
(33.00000, 0.50000)
(34.00000, 0.50000)
(35.00000, 0.50000)
(36.00000, -0.50000)
(37.00000, 0.50000)
(38.00000, -0.50000)
(39.00000, -0.50000)
(40.00000, -0.50000)
(41.00000, -0.50000)
(42.00000, -0.50000)
(43.00000, -0.50000)
(44.00000, -0.50000)
(45.00000, -0.50000)
(46.00000, 0.50000)
(47.00000, -0.50000)
(48.00000, -0.50000)
(49.00000, -0.50000)
(50.00000, -0.50000)
(51.00000, 0.50000)
(52.00000, -0.50000)
(53.00000, 0.50000)
(54.00000, 0.50000)
(55.00000, 0.50000)
(56.00000, -0.50000)
(57.00000, 0.50000)
(58.00000, 0.50000)
(59.00000, -0.50000)
(60.00000, -0.50000)
(61.00000, -0.50000)
(62.00000, 0.50000)
(63.00000, -0.50000)
(64.00000, 0.50000)
(65.00000, -0.50000)
(66.00000, 0.50000)
(67.00000, 0.50000)
(68.00000, -0.50000)
(69.00000, 0.50000)
(70.00000, 0.50000)
(71.00000, -0.50000)
(72.00000, 0.50000)
(73.00000, 0.50000)
(74.00000, -0.50000)
(75.00000, 0.50000)
(76.00000, -0.50000)
(77.00000, -0.50000)
(78.00000, -0.50000)
(79.00000, -0.50000)
(80.00000, -0.50000)
(81.00000, -0.50000)
(82.00000, -0.50000)
(83.00000, 0.50000)
(84.00000, -0.50000)
(85.00000, -0.50000)
(86.00000, 0.50000)
(87.00000, -0.50000)
(88.00000, -0.50000)
(89.00000, 0.50000)
(90.00000, -0.50000)
(91.00000, -0.50000)
(92.00000, 0.50000)
(93.00000, -0.50000)
(94.00000, -0.50000)
(95.00000, 0.50000)
(96.00000, 0.50000)
(97.00000, -0.50000)
(98.00000, -0.50000)
(99.00000, -0.50000)
(100.00000, 0.50000)
(101.00000, -0.50000)
(102.00000, -0.50000)
(103.00000, 0.50000)
(104.00000, -0.50000)
(105.00000, -0.50000)
(106.00000, 0.50000)
(107.00000, -0.50000)
(108.00000, -0.50000)
(109.00000, 0.50000)
(110.00000, -0.50000)
(111.00000, 0.50000)
(112.00000, 0.50000)
(113.00000, -0.50000)
(114.00000, -0.50000)
(115.00000, -0.50000)
(116.00000, -0.50000)
(117.00000, -0.50000)
(118.00000, 0.50000)
(119.00000, 0.50000)
(120.00000, -0.50000)
(121.00000, 0.50000)
(122.00000, 0.50000)
(123.00000, -0.50000)
(124.00000, -0.50000)
(125.00000, 0.50000)
(126.00000, -0.50000)
(127.00000, -0.50000)
(128.00000, 0.50000)
(129.00000, -0.50000)
(130.00000, 0.50000)
(131.00000, 0.50000)
(132.00000, 0.50000)
(133.00000, -0.50000)
(134.00000, -0.50000)
(135.00000, -0.50000)
(136.00000, -0.50000)
(137.00000, -0.50000)
(138.00000, -0.50000)
(139.00000, -0.50000)
(140.00000, -0.50000)
(141.00000, 0.50000)
(142.00000, -0.50000)
(143.00000, 0.50000)
(144.00000, 0.50000)
(145.00000, 0.50000)
(146.00000, -0.50000)
(147.00000, -0.50000)
(148.00000, -0.50000)
(149.00000, 0.50000)
(150.00000, -0.50000)
(151.00000, 0.50000)
(152.00000, -0.50000)
(153.00000, -0.50000)
(154.00000, 0.50000)
(155.00000, -0.50000)
(156.00000, -0.50000)
(157.00000, 0.50000)
(158.00000, 0.50000)
(159.00000, -0.50000)
(160.00000, -0.50000)
(161.00000, 0.50000)
(162.00000, -0.50000)
(163.00000, 0.50000)
(164.00000, -0.50000)
(165.00000, 0.50000)
(166.00000, -0.50000)
(167.00000, -0.50000)
(168.00000, 0.50000)
(169.00000, 0.50000)
(170.00000, -0.50000)
(171.00000, -0.50000)
(172.00000, -0.50000)
(173.00000, -0.50000)
(174.00000, 0.50000)
(175.00000, 0.50000)
(176.00000, -0.50000)
(177.00000, 0.50000)
(178.00000, 0.50000)
(179.00000, -0.50000)
(180.00000, -0.50000)
(181.00000, 0.50000)
(182.00000, 0.50000)
(183.00000, 0.50000)
(184.00000, 0.50000)
(185.00000, -0.50000)
(186.00000, 0.50000)
(187.00000, -0.50000)
(188.00000, 0.50000)
(189.00000, -0.50000)
(190.00000, -0.50000)
(191.00000, -0.50000)
(192.00000, 0.50000)
(193.00000, -0.50000)
(194.00000, 0.50000)
(195.00000, 0.50000)
(196.00000, 0.50000)
(197.00000, -0.50000)
(198.00000, -0.50000)
(199.00000, -0.50000)
(200.00000, 0.50000)
(201.00000, -0.50000)
(202.00000, -0.50000)
(203.00000, -0.50000)
(204.00000, 0.50000)
(205.00000, -0.50000)
(206.00000, -0.50000)
(207.00000, -0.50000)
(208.00000, 0.50000)
(209.00000, 0.50000)
(210.00000, -0.50000)
(211.00000, -0.50000)
(212.00000, 0.50000)
(213.00000, -0.50000)
(214.00000, 0.50000)
(215.00000, 0.50000)
(216.00000, -0.50000)
(217.00000, 0.50000)
(218.00000, 0.50000)
(219.00000, -0.50000)
(220.00000, -0.50000)
(221.00000, -0.50000)
(222.00000, 0.50000)
(223.00000, -0.50000)
(224.00000, -0.50000)
(225.00000, -0.50000)
(226.00000, 0.50000)
(227.00000, 0.50000)
(228.00000, 0.50000)
(229.00000, -0.50000)
(230.00000, 0.50000)
(231.00000, -0.50000)
(232.00000, -0.50000)
(233.00000, 0.50000)
(234.00000, 0.50000)
(235.00000, 0.50000)
(236.00000, 0.50000)
(237.00000, 0.50000)
(238.00000, 0.50000)
(239.00000, 0.50000)
(240.00000, -0.50000)
(241.00000, 0.50000)
(242.00000, -0.50000)
(243.00000, 0.50000)
(244.00000, -0.50000)
(245.00000, 0.50000)
(246.00000, -0.50000)
(247.00000, -0.50000)
(248.00000, 0.50000)
(249.00000, 0.50000)
(250.00000, 0.50000)
(251.00000, 0.50000)
(252.00000, -0.50000)
(253.00000, -0.50000)
(254.00000, -0.50000)
(255.00000, -0.50000)
(256.00000, 0.50000)
(257.00000, 0.50000)
(258.00000, 0.50000)
(259.00000, 0.50000)
(260.00000, -0.50000)
(261.00000, -0.50000)
(262.00000, 0.50000)
(263.00000, 0.50000)
(264.00000, -0.50000)
(265.00000, 0.50000)
(266.00000, -0.50000)
(267.00000, -0.50000)
(268.00000, 0.50000)
(269.00000, 0.50000)
(270.00000, 0.50000)
(271.00000, -0.50000)
(272.00000, 0.50000)
(273.00000, 0.50000)
(274.00000, 0.50000)
(275.00000, -0.50000)
(276.00000, -0.50000)
(277.00000, 0.50000)
(278.00000, 0.50000)
(279.00000, -0.50000)
(280.00000, 0.50000)
(281.00000, -0.50000)
(282.00000, 0.50000)
(283.00000, -0.50000)
(284.00000, 0.50000)
(285.00000, -0.50000)
(286.00000, -0.50000)
(287.00000, 0.50000)
(288.00000, -0.50000)
(289.00000, 0.50000)
(290.00000, 0.50000)
(291.00000, -0.50000)
(292.00000, -0.50000)
(293.00000, 0.50000)
(294.00000, 0.50000)
(295.00000, -0.50000)
(296.00000, -0.50000)
(297.00000, -0.50000)
(298.00000, 0.50000)
(299.00000, -0.50000)
(300.00000, -0.50000)
(301.00000, 0.50000)
(302.00000, 0.50000)
(303.00000, 0.50000)
(304.00000, -0.50000)
(305.00000, 0.50000)
(306.00000, -0.50000)
(307.00000, 0.50000)
(308.00000, 0.50000)
(309.00000, -0.50000)
(310.00000, -0.50000)
(311.00000, -0.50000)
(312.00000, -0.50000)
(313.00000, -0.50000)
(314.00000, 0.50000)
(315.00000, 0.50000)
(316.00000, -0.50000)
(317.00000, 0.50000)
(318.00000, -0.50000)
(319.00000, 0.50000)
(320.00000, -0.50000)
(321.00000, -0.50000)
(322.00000, 0.50000)
(323.00000, 0.50000)
(324.00000, -0.50000)
(325.00000, -0.50000)
(326.00000, -0.50000)
(327.00000, 0.50000)
(328.00000, -0.50000)
(329.00000, -0.50000)
(330.00000, -0.50000)
(331.00000, 0.50000)
(332.00000, 0.50000)
(333.00000, 0.50000)
(334.00000, 0.50000)
(335.00000, -0.50000)
(336.00000, 0.50000)
(337.00000, -0.50000)
(338.00000, 0.50000)
(339.00000, -0.50000)
(340.00000, -0.50000)
(341.00000, 0.50000)
(342.00000, 0.50000)
(343.00000, 0.50000)
(344.00000, 0.50000)
(345.00000, -0.50000)
(346.00000, -0.50000)
(347.00000, 0.50000)
(348.00000, 0.50000)
(349.00000, -0.50000)
(350.00000, -0.50000)
(351.00000, -0.50000)
(352.00000, 0.50000)
(353.00000, 0.50000)
(354.00000, 0.50000)
(355.00000, -0.50000)
(356.00000, -0.50000)
(357.00000, -0.50000)
(358.00000, 0.50000)
(359.00000, 0.50000)
(360.00000, -0.50000)
(361.00000, -0.50000)
(362.00000, 0.50000)
(363.00000, 0.50000)
(364.00000, -0.50000)
(365.00000, -0.50000)
(366.00000, -0.50000)
(367.00000, 0.50000)
(368.00000, -0.50000)
(369.00000, 0.50000)
(370.00000, -0.50000)
(371.00000, 0.50000)
(372.00000, 0.50000)
(373.00000, -0.50000)
(374.00000, 0.50000)
(375.00000, 0.50000)
(376.00000, -0.50000)
(377.00000, 0.50000)
(378.00000, 0.50000)
(379.00000, -0.50000)
(380.00000, 0.50000)
(381.00000, -0.50000)
(382.00000, 0.50000)
(383.00000, 0.50000)
(384.00000, -0.50000)
(385.00000, -0.50000)
(386.00000, -0.50000)
(387.00000, -0.50000)
(388.00000, -0.50000)
(389.00000, -0.50000)
(390.00000, 0.50000)
(391.00000, 0.50000)
(392.00000, -0.50000)
(393.00000, 0.50000)
(394.00000, -0.50000)
(395.00000, -0.50000)
(396.00000, -0.50000)
(397.00000, -0.50000)
(398.00000, -0.50000)
(399.00000, 0.50000)
(400.00000, -0.50000)
};


==> Figures/dataS1.tex <==
\addplot[ ultra thick,smooth,Red4] plot coordinates {
(1.00000, 0.50054)
(2.00000, 0.16677)
(3.00000, -0.11477)
(4.00000, -0.14245)
(5.00000, 0.17558)
(6.00000, 0.56324)
(7.00000, 0.58133)
(8.00000, 0.50018)
(9.00000, 0.57879)
(10.00000, 0.53952)
(11.00000, 0.56973)
(12.00000, 0.50825)
(13.00000, 0.19752)
(14.00000, 0.19247)
(15.00000, 0.18603)
(16.00000, 0.58279)
(17.00000, 0.53261)
(18.00000, 0.50289)
(19.00000, 0.52222)
(20.00000, 0.58404)
(21.00000, 0.58363)
(22.00000, 0.23439)
(23.00000, 0.20047)
(24.00000, 0.16791)
(25.00000, 0.23559)
(26.00000, 0.19534)
(27.00000, 0.22829)
(28.00000, 0.56383)
(29.00000, 0.59603)
(30.00000, 0.59279)
(31.00000, 0.52595)
(32.00000, 0.20911)
(33.00000, 0.26496)
(34.00000, 0.18586)
(35.00000, 0.57340)
(36.00000, 0.50186)
(37.00000, 0.50383)
(38.00000, 0.55928)
(39.00000, 0.51177)
(40.00000, 0.51677)
(41.00000, 0.57627)
(42.00000, 0.58101)
(43.00000, 0.53013)
(44.00000, 0.53817)
(45.00000, 0.56095)
(46.00000, 0.57095)
(47.00000, 0.54644)
(48.00000, 0.53639)
(49.00000, 0.59955)
(50.00000, 0.53336)
(51.00000, 0.54128)
(52.00000, 0.55162)
(53.00000, 0.53066)
(54.00000, 0.56372)
(55.00000, 0.57058)
(56.00000, 0.58436)
(57.00000, 0.59491)
(58.00000, 0.53452)
(59.00000, 0.54344)
(60.00000, 0.57581)
(61.00000, 0.58775)
(62.00000, 0.57930)
(63.00000, 0.59402)
(64.00000, 0.53499)
(65.00000, 0.53653)
(66.00000, 0.56148)
(67.00000, 0.59715)
(68.00000, 0.56993)
(69.00000, 0.50996)
(70.00000, 0.57462)
(71.00000, 0.19391)
(72.00000, -0.12608)
(73.00000, -0.13460)
(74.00000, 0.19718)
(75.00000, 0.53552)
(76.00000, 0.53615)
(77.00000, 0.58865)
(78.00000, 0.22892)
(79.00000, 0.18671)
(80.00000, 0.23374)
(81.00000, 0.50567)
(82.00000, 0.58289)
(83.00000, 0.59254)
(84.00000, 0.59086)
(85.00000, 0.56559)
(86.00000, 0.52775)
(87.00000, 0.58499)
(88.00000, 0.52345)
(89.00000, 0.25791)
(90.00000, -0.12667)
(91.00000, -0.14296)
(92.00000, 0.18591)
(93.00000, 0.52702)
(94.00000, 0.59133)
(95.00000, 0.56994)
(96.00000, 0.25651)
(97.00000, -0.12865)
(98.00000, -0.48789)
(99.00000, -0.45194)
(100.00000, -0.15324)
(101.00000, 0.20541)
(102.00000, 0.54261)
(103.00000, 0.59978)
(104.00000, 0.51020)
(105.00000, 0.50472)
(106.00000, 0.59654)
(107.00000, 0.52109)
(108.00000, 0.50368)
(109.00000, 0.54731)
(110.00000, 0.52510)
(111.00000, 0.51843)
(112.00000, 0.50463)
(113.00000, 0.56115)
(114.00000, 0.52876)
(115.00000, 0.50483)
(116.00000, 0.51358)
(117.00000, 0.55985)
(118.00000, 0.54584)
(119.00000, 0.57794)
(120.00000, 0.57410)
(121.00000, 0.57819)
(122.00000, 0.51401)
(123.00000, 0.56562)
(124.00000, 0.59518)
(125.00000, 0.56110)
(126.00000, 0.55729)
(127.00000, 0.59684)
(128.00000, 0.22885)
(129.00000, 0.19211)
(130.00000, 0.20991)
(131.00000, 0.59874)
(132.00000, 0.59150)
(133.00000, 0.58737)
(134.00000, 0.51050)
(135.00000, 0.53232)
(136.00000, 0.59481)
(137.00000, 0.50537)
(138.00000, 0.59666)
(139.00000, 0.54495)
(140.00000, 0.57274)
(141.00000, 0.55957)
(142.00000, 0.52740)
(143.00000, 0.21270)
(144.00000, -0.15978)
(145.00000, -0.14557)
(146.00000, -0.08706)
(147.00000, 0.22409)
(148.00000, 0.19364)
(149.00000, 0.57959)
(150.00000, 0.53352)
(151.00000, 0.50236)
(152.00000, 0.50055)
(153.00000, 0.51465)
(154.00000, 0.57301)
(155.00000, 0.51906)
(156.00000, 0.58925)
(157.00000, 0.50397)
(158.00000, 0.53358)
(159.00000, 0.53192)
(160.00000, 0.51101)
(161.00000, 0.51084)
(162.00000, 0.57564)
(163.00000, 0.57632)
(164.00000, 0.54122)
(165.00000, 0.55754)
(166.00000, 0.57146)
(167.00000, 0.53138)
(168.00000, 0.56702)
(169.00000, 0.56910)
(170.00000, 0.50017)
(171.00000, 0.58717)
(172.00000, 0.54399)
(173.00000, 0.54661)
(174.00000, 0.54333)
(175.00000, 0.59540)
(176.00000, 0.55852)
(177.00000, 0.56725)
(178.00000, 0.56467)
(179.00000, 0.56900)
(180.00000, 0.56656)
(181.00000, 0.18761)
(182.00000, -0.11489)
(183.00000, -0.10909)
(184.00000, 0.24457)
(185.00000, 0.56348)
(186.00000, 0.59725)
(187.00000, 0.54786)
(188.00000, 0.19179)
(189.00000, 0.24370)
(190.00000, 0.19954)
(191.00000, 0.53368)
(192.00000, 0.58907)
(193.00000, 0.50284)
(194.00000, 0.56935)
(195.00000, 0.54031)
(196.00000, 0.54881)
(197.00000, 0.53487)
(198.00000, 0.55071)
(199.00000, 0.59040)
(200.00000, 0.56475)
(201.00000, 0.53432)
(202.00000, 0.59238)
(203.00000, 0.58888)
(204.00000, 0.50117)
(205.00000, 0.25323)
(206.00000, -0.13029)
(207.00000, -0.07457)
(208.00000, 0.22469)
(209.00000, 0.57413)
(210.00000, 0.59936)
(211.00000, 0.54935)
(212.00000, 0.50769)
(213.00000, 0.18903)
(214.00000, 0.24125)
(215.00000, 0.17086)
(216.00000, 0.56331)
(217.00000, 0.58803)
(218.00000, 0.18239)
(219.00000, 0.24132)
(220.00000, 0.24125)
(221.00000, 0.25592)
(222.00000, 0.23368)
(223.00000, -0.09798)
(224.00000, -0.16061)
(225.00000, -0.14080)
(226.00000, 0.22695)
(227.00000, 0.50622)
(228.00000, 0.56020)
(229.00000, 0.52547)
(230.00000, 0.58904)
(231.00000, 0.51849)
(232.00000, 0.52513)
(233.00000, 0.54580)
(234.00000, 0.52087)
(235.00000, 0.54740)
(236.00000, 0.58385)
(237.00000, 0.50703)
(238.00000, 0.51175)
(239.00000, 0.55912)
(240.00000, 0.53282)
(241.00000, 0.18765)
(242.00000, 0.17918)
(243.00000, 0.24867)
(244.00000, 0.59822)
(245.00000, 0.57253)
(246.00000, 0.54492)
(247.00000, 0.56536)
(248.00000, 0.50469)
(249.00000, 0.51699)
(250.00000, 0.19759)
(251.00000, -0.09498)
(252.00000, -0.42949)
(253.00000, -0.49933)
(254.00000, -0.09045)
(255.00000, 0.24866)
(256.00000, 0.55310)
(257.00000, 0.22047)
(258.00000, 0.25415)
(259.00000, 0.22260)
(260.00000, 0.50033)
(261.00000, 0.55922)
(262.00000, 0.19198)
(263.00000, -0.09770)
(264.00000, -0.40200)
(265.00000, -0.13060)
(266.00000, 0.18826)
(267.00000, 0.25539)
(268.00000, 0.21475)
(269.00000, 0.20677)
(270.00000, 0.57313)
(271.00000, 0.22551)
(272.00000, 0.23312)
(273.00000, -0.10700)
(274.00000, 0.23833)
(275.00000, 0.25641)
(276.00000, 0.52907)
(277.00000, 0.55123)
(278.00000, 0.58573)
(279.00000, 0.55164)
(280.00000, 0.59983)
(281.00000, 0.58305)
(282.00000, 0.56445)
(283.00000, 0.55354)
(284.00000, 0.59812)
(285.00000, 0.24309)
(286.00000, -0.12197)
(287.00000, -0.47270)
(288.00000, -0.15871)
(289.00000, 0.25224)
(290.00000, 0.51123)
(291.00000, 0.51599)
(292.00000, 0.57714)
(293.00000, 0.53396)
(294.00000, 0.56473)
(295.00000, 0.59746)
(296.00000, 0.57607)
(297.00000, 0.52894)
(298.00000, 0.55228)
(299.00000, 0.53961)
(300.00000, 0.54601)
(301.00000, 0.25038)
(302.00000, 0.23248)
(303.00000, 0.20675)
(304.00000, 0.53701)
(305.00000, 0.55324)
(306.00000, 0.57887)
(307.00000, 0.20798)
(308.00000, 0.26301)
(309.00000, 0.26144)
(310.00000, 0.52283)
(311.00000, 0.51805)
(312.00000, 0.50465)
(313.00000, 0.55162)
(314.00000, 0.51133)
(315.00000, 0.54255)
(316.00000, 0.52264)
(317.00000, 0.58125)
(318.00000, 0.53895)
(319.00000, 0.51687)
(320.00000, 0.52536)
(321.00000, 0.54205)
(322.00000, 0.57458)
(323.00000, 0.52441)
(324.00000, 0.25045)
(325.00000, 0.24977)
(326.00000, 0.21205)
(327.00000, 0.52176)
(328.00000, 0.58718)
(329.00000, 0.21685)
(330.00000, -0.15031)
(331.00000, -0.42226)
(332.00000, -0.42710)
(333.00000, -0.49880)
(334.00000, -0.10471)
(335.00000, 0.17421)
(336.00000, 0.22709)
(337.00000, 0.18066)
(338.00000, 0.20324)
(339.00000, 0.51330)
(340.00000, 0.59451)
(341.00000, 0.52978)
(342.00000, 0.20633)
(343.00000, -0.16501)
(344.00000, -0.44332)
(345.00000, -0.11515)
(346.00000, 0.25650)
(347.00000, 0.59259)
(348.00000, 0.55365)
(349.00000, 0.23697)
(350.00000, 0.25076)
(351.00000, 0.17516)
(352.00000, 0.54660)
(353.00000, 0.58577)
(354.00000, 0.54176)
(355.00000, 0.52801)
(356.00000, 0.58042)
(357.00000, 0.51973)
(358.00000, 0.58050)
(359.00000, 0.25231)
(360.00000, -0.11737)
(361.00000, -0.11999)
(362.00000, 0.21171)
(363.00000, 0.52558)
(364.00000, 0.58546)
(365.00000, 0.55405)
(366.00000, 0.56216)
(367.00000, 0.21511)
(368.00000, -0.12834)
(369.00000, -0.13526)
(370.00000, 0.24089)
(371.00000, 0.59256)
(372.00000, 0.53332)
(373.00000, 0.54077)
(374.00000, 0.53406)
(375.00000, 0.53101)
(376.00000, 0.58385)
(377.00000, 0.50483)
(378.00000, 0.54943)
(379.00000, 0.17102)
(380.00000, 0.20518)
(381.00000, 0.26492)
(382.00000, 0.56327)
(383.00000, 0.54631)
(384.00000, 0.57821)
(385.00000, 0.53470)
(386.00000, 0.55483)
(387.00000, 0.51636)
(388.00000, 0.53170)
(389.00000, 0.58636)
(390.00000, 0.50281)
(391.00000, 0.51903)
(392.00000, 0.56401)
(393.00000, 0.56036)
(394.00000, 0.52739)
(395.00000, 0.58505)
(396.00000, 0.55572)
(397.00000, 0.52001)
(398.00000, 0.54607)
(399.00000, 0.52404)
(400.00000, 0.57133)
};


==> Figures/dataS2.tex <==
\addplot[ ultra thick,smooth,DodgerBlue4] plot coordinates {
(1.00000, -0.11183)
(2.00000, -0.08749)
(3.00000, -0.15654)
(4.00000, -0.14711)
(5.00000, -0.40307)
(6.00000, -0.07176)
(7.00000, -0.07013)
(8.00000, 0.23409)
(9.00000, -0.12984)
(10.00000, -0.11341)
(11.00000, -0.45823)
(12.00000, -0.42396)
(13.00000, -0.14172)
(14.00000, -0.13896)
(15.00000, -0.12960)
(16.00000, -0.47289)
(17.00000, -0.40019)
(18.00000, -0.46878)
(19.00000, -0.42498)
(20.00000, -0.48083)
(21.00000, -0.47572)
(22.00000, -0.44905)
(23.00000, -0.40178)
(24.00000, -0.42693)
(25.00000, -0.45873)
(26.00000, -0.44192)
(27.00000, -0.42463)
(28.00000, -0.15485)
(29.00000, -0.11871)
(30.00000, 0.19426)
(31.00000, 0.18737)
(32.00000, 0.24924)
(33.00000, 0.20695)
(34.00000, -0.13575)
(35.00000, -0.11315)
(36.00000, -0.11086)
(37.00000, 0.19873)
(38.00000, 0.17808)
(39.00000, -0.13130)
(40.00000, -0.45780)
(41.00000, -0.11375)
(42.00000, -0.10818)
(43.00000, -0.07606)
(44.00000, -0.11343)
(45.00000, -0.15296)
(46.00000, -0.07304)
(47.00000, -0.47387)
(48.00000, -0.46368)
(49.00000, -0.43969)
(50.00000, -0.09446)
(51.00000, -0.12112)
(52.00000, -0.08708)
(53.00000, -0.40730)
(54.00000, -0.46003)
(55.00000, -0.13813)
(56.00000, -0.13199)
(57.00000, -0.15343)
(58.00000, -0.40545)
(59.00000, -0.49075)
(60.00000, -0.13064)
(61.00000, -0.12317)
(62.00000, -0.06866)
(63.00000, -0.45159)
(64.00000, -0.49404)
(65.00000, -0.40048)
(66.00000, -0.43071)
(67.00000, -0.46528)
(68.00000, -0.46731)
(69.00000, -0.47441)
(70.00000, -0.41845)
(71.00000, -0.44752)
(72.00000, -0.49917)
(73.00000, -0.42406)
(74.00000, -0.09255)
(75.00000, -0.10673)
(76.00000, -0.08399)
(77.00000, -0.46499)
(78.00000, -0.40060)
(79.00000, -0.15111)
(80.00000, -0.07684)
(81.00000, -0.12473)
(82.00000, -0.42220)
(83.00000, -0.48357)
(84.00000, -0.42503)
(85.00000, -0.42907)
(86.00000, -0.47781)
(87.00000, -0.47878)
(88.00000, -0.08409)
(89.00000, -0.09359)
(90.00000, 0.23057)
(91.00000, -0.14025)
(92.00000, -0.08993)
(93.00000, -0.41650)
(94.00000, -0.40822)
(95.00000, -0.15706)
(96.00000, 0.18440)
(97.00000, 0.24603)
(98.00000, 0.24156)
(99.00000, -0.16120)
(100.00000, -0.10065)
(101.00000, -0.42408)
(102.00000, -0.09581)
(103.00000, -0.07999)
(104.00000, -0.08430)
(105.00000, -0.42782)
(106.00000, -0.44405)
(107.00000, -0.40119)
(108.00000, -0.40901)
(109.00000, -0.40607)
(110.00000, -0.45972)
(111.00000, -0.49783)
(112.00000, -0.44083)
(113.00000, -0.46121)
(114.00000, -0.41251)
(115.00000, -0.08842)
(116.00000, -0.13220)
(117.00000, -0.14747)
(118.00000, -0.46222)
(119.00000, -0.47371)
(120.00000, -0.41669)
(121.00000, -0.43654)
(122.00000, -0.45725)
(123.00000, -0.45270)
(124.00000, -0.12379)
(125.00000, -0.08790)
(126.00000, -0.09466)
(127.00000, -0.44294)
(128.00000, -0.09697)
(129.00000, 0.26255)
(130.00000, 0.16916)
(131.00000, 0.17110)
(132.00000, -0.14843)
(133.00000, 0.26029)
(134.00000, -0.14185)
(135.00000, -0.13090)
(136.00000, -0.44784)
(137.00000, -0.47033)
(138.00000, -0.42490)
(139.00000, -0.40975)
(140.00000, -0.47226)
(141.00000, -0.43110)
(142.00000, -0.45690)
(143.00000, -0.11852)
(144.00000, -0.12736)
(145.00000, -0.10580)
(146.00000, -0.41274)
(147.00000, -0.41485)
(148.00000, -0.41063)
(149.00000, -0.46378)
(150.00000, -0.46717)
(151.00000, -0.44481)
(152.00000, -0.41526)
(153.00000, -0.49833)
(154.00000, -0.41218)
(155.00000, -0.45892)
(156.00000, -0.43402)
(157.00000, -0.10719)
(158.00000, 0.23769)
(159.00000, 0.25065)
(160.00000, -0.07157)
(161.00000, -0.14706)
(162.00000, -0.14754)
(163.00000, -0.08863)
(164.00000, -0.42190)
(165.00000, -0.42419)
(166.00000, -0.46296)
(167.00000, -0.16514)
(168.00000, -0.08591)
(169.00000, 0.25186)
(170.00000, -0.07885)
(171.00000, -0.12519)
(172.00000, -0.45661)
(173.00000, -0.10530)
(174.00000, -0.12163)
(175.00000, 0.19111)
(176.00000, -0.12662)
(177.00000, -0.07418)
(178.00000, -0.48166)
(179.00000, -0.48456)
(180.00000, -0.40274)
(181.00000, -0.46600)
(182.00000, -0.42770)
(183.00000, -0.40769)
(184.00000, -0.45015)
(185.00000, -0.44896)
(186.00000, -0.44424)
(187.00000, -0.46212)
(188.00000, -0.41840)
(189.00000, -0.12486)
(190.00000, -0.09671)
(191.00000, -0.15331)
(192.00000, -0.49626)
(193.00000, -0.41806)
(194.00000, -0.43136)
(195.00000, -0.44591)
(196.00000, -0.11736)
(197.00000, -0.13948)
(198.00000, -0.10916)
(199.00000, -0.49889)
(200.00000, -0.42886)
(201.00000, -0.42187)
(202.00000, -0.42631)
(203.00000, -0.45579)
(204.00000, -0.47215)
(205.00000, -0.42767)
(206.00000, -0.48296)
(207.00000, -0.44438)
(208.00000, -0.06858)
(209.00000, -0.15621)
(210.00000, -0.14894)
(211.00000, -0.16423)
(212.00000, -0.16060)
(213.00000, -0.10171)
(214.00000, -0.48174)
(215.00000, -0.48299)
(216.00000, -0.45583)
(217.00000, -0.49372)
(218.00000, -0.47876)
(219.00000, -0.41261)
(220.00000, -0.43816)
(221.00000, -0.09029)
(222.00000, -0.13272)
(223.00000, -0.12304)
(224.00000, -0.43728)
(225.00000, -0.46191)
(226.00000, -0.08641)
(227.00000, -0.07236)
(228.00000, 0.18806)
(229.00000, -0.11021)
(230.00000, -0.07845)
(231.00000, -0.08421)
(232.00000, -0.15505)
(233.00000, -0.13333)
(234.00000, -0.42200)
(235.00000, -0.45453)
(236.00000, -0.47265)
(237.00000, -0.46518)
(238.00000, -0.10961)
(239.00000, -0.13810)
(240.00000, -0.09793)
(241.00000, -0.40283)
(242.00000, -0.49793)
(243.00000, -0.07422)
(244.00000, -0.11640)
(245.00000, -0.15788)
(246.00000, -0.14507)
(247.00000, -0.07901)
(248.00000, -0.08805)
(249.00000, -0.49509)
(250.00000, -0.13294)
(251.00000, -0.15808)
(252.00000, 0.16806)
(253.00000, -0.16499)
(254.00000, -0.12777)
(255.00000, -0.09852)
(256.00000, -0.07876)
(257.00000, 0.26454)
(258.00000, -0.08723)
(259.00000, -0.09106)
(260.00000, -0.14055)
(261.00000, -0.11770)
(262.00000, -0.09389)
(263.00000, -0.42604)
(264.00000, -0.07384)
(265.00000, -0.14491)
(266.00000, -0.12993)
(267.00000, -0.48347)
(268.00000, -0.44176)
(269.00000, -0.42831)
(270.00000, -0.43591)
(271.00000, -0.47241)
(272.00000, -0.15889)
(273.00000, -0.10232)
(274.00000, 0.19686)
(275.00000, -0.08582)
(276.00000, -0.12711)
(277.00000, -0.48952)
(278.00000, -0.47583)
(279.00000, -0.08377)
(280.00000, -0.15448)
(281.00000, 0.23264)
(282.00000, -0.12589)
(283.00000, 0.25246)
(284.00000, -0.16468)
(285.00000, 0.18164)
(286.00000, -0.13511)
(287.00000, -0.12716)
(288.00000, -0.41092)
(289.00000, -0.48990)
(290.00000, -0.48076)
(291.00000, -0.13121)
(292.00000, 0.19118)
(293.00000, 0.22022)
(294.00000, -0.13886)
(295.00000, -0.45645)
(296.00000, -0.42342)
(297.00000, -0.13302)
(298.00000, -0.09642)
(299.00000, -0.08955)
(300.00000, -0.44692)
(301.00000, -0.07083)
(302.00000, -0.09869)
(303.00000, -0.15757)
(304.00000, -0.48162)
(305.00000, -0.13896)
(306.00000, -0.12574)
(307.00000, -0.15277)
(308.00000, -0.40947)
(309.00000, -0.41821)
(310.00000, -0.44709)
(311.00000, -0.43590)
(312.00000, -0.48227)
(313.00000, -0.46890)
(314.00000, -0.16020)
(315.00000, -0.10802)
(316.00000, -0.13877)
(317.00000, -0.40259)
(318.00000, -0.40043)
(319.00000, -0.47777)
(320.00000, -0.42267)
(321.00000, -0.42009)
(322.00000, -0.43140)
(323.00000, -0.41546)
(324.00000, -0.14909)
(325.00000, 0.23763)
(326.00000, 0.17861)
(327.00000, 0.22012)
(328.00000, -0.10229)
(329.00000, -0.14699)
(330.00000, -0.48308)
(331.00000, -0.41196)
(332.00000, -0.41404)
(333.00000, -0.41896)
(334.00000, -0.44104)
(335.00000, -0.46442)
(336.00000, -0.15147)
(337.00000, -0.13620)
(338.00000, -0.16447)
(339.00000, -0.41518)
(340.00000, -0.41190)
(341.00000, -0.42564)
(342.00000, -0.47374)
(343.00000, -0.40689)
(344.00000, -0.42385)
(345.00000, -0.42258)
(346.00000, -0.48846)
(347.00000, -0.12313)
(348.00000, -0.16659)
(349.00000, -0.15832)
(350.00000, -0.45045)
(351.00000, -0.10765)
(352.00000, -0.16199)
(353.00000, -0.16042)
(354.00000, -0.47675)
(355.00000, -0.41145)
(356.00000, -0.16479)
(357.00000, -0.13507)
(358.00000, -0.07838)
(359.00000, -0.48041)
(360.00000, -0.40876)
(361.00000, -0.49085)
(362.00000, -0.16527)
(363.00000, -0.11140)
(364.00000, -0.08500)
(365.00000, -0.07011)
(366.00000, -0.14858)
(367.00000, -0.13126)
(368.00000, -0.44941)
(369.00000, -0.08291)
(370.00000, -0.11343)
(371.00000, 0.24410)
(372.00000, -0.12191)
(373.00000, 0.22723)
(374.00000, 0.17138)
(375.00000, 0.25353)
(376.00000, -0.08638)
(377.00000, -0.45245)
(378.00000, -0.46562)
(379.00000, -0.49091)
(380.00000, -0.46028)
(381.00000, -0.45327)
(382.00000, -0.41787)
(383.00000, -0.49792)
(384.00000, -0.46318)
(385.00000, -0.41217)
(386.00000, -0.44296)
(387.00000, -0.48045)
(388.00000, -0.48829)
(389.00000, -0.07451)
(390.00000, 0.23452)
(391.00000, 0.18887)
(392.00000, -0.07428)
(393.00000, -0.09492)
(394.00000, -0.12906)
(395.00000, -0.14106)
(396.00000, -0.46477)
(397.00000, -0.42975)
(398.00000, -0.43451)
(399.00000, -0.07646)
(400.00000, -0.12740)
};


==> Figures/heart_surf.tex <==
00000 2.55000e-02 2.51092e-02
00000 3.05000e-02 2.46112e-02
00000 3.55000e-02 2.41753e-02
00000 4.05000e-02 2.25232e-02
00000 4.55000e-02 2.00718e-02
00000 5.05000e-02 1.71275e-02
00000 5.55000e-02 1.39025e-02
00000 6.05000e-02 1.05409e-02
00000 6.55000e-02 7.13431e-03

1.00000e-02 2.55000e-02 2.75636e-02
1.00000e-02 3.05000e-02 2.58517e-02
1.00000e-02 3.55000e-02 2.39497e-02
1.00000e-02 4.05000e-02 2.14986e-02
1.00000e-02 4.55000e-02 1.85907e-02
1.00000e-02 5.05000e-02 1.53464e-02
1.00000e-02 5.55000e-02 1.18852e-02
1.00000e-02 6.05000e-02 8.30852e-03
1.00000e-02 6.55000e-02 4.69091e-03

2.00000e-02 2.55000e-02 2.99190e-02
2.00000e-02 3.05000e-02 2.67578e-02
2.00000e-02 3.55000e-02 2.37739e-02
2.00000e-02 4.05000e-02 2.05847e-02
2.00000e-02 4.55000e-02 1.72034e-02
2.00000e-02 5.05000e-02 1.36335e-02
2.00000e-02 5.55000e-02 9.92044e-03
2.00000e-02 6.05000e-02 6.12263e-03
2.00000e-02 6.55000e-02 2.29254e-03

3.00000e-02 2.55000e-02 3.22663e-02
3.00000e-02 3.05000e-02 2.74109e-02
3.00000e-02 3.55000e-02 2.36203e-02
3.00000e-02 4.05000e-02 1.98641e-02
3.00000e-02 4.55000e-02 1.60049e-02
3.00000e-02 5.05000e-02 1.20752e-02
3.00000e-02 5.55000e-02 8.08783e-03
3.00000e-02 6.05000e-02 4.06326e-03
3.00000e-02 6.55000e-02 2.51852e-05

4.00000e-02 2.55000e-02 3.32526e-02
4.00000e-02 3.05000e-02 2.85402e-02
4.00000e-02 3.55000e-02 2.39831e-02
4.00000e-02 4.05000e-02 1.94288e-02
4.00000e-02 4.55000e-02 1.50483e-02
4.00000e-02 5.05000e-02 1.07446e-02
4.00000e-02 5.55000e-02 6.47279e-03
4.00000e-02 6.05000e-02 2.23063e-03
4.00000e-02 6.55000e-02 -1.99289e-03

5.00000e-02 2.55000e-02 3.35604e-02
5.00000e-02 3.05000e-02 2.86345e-02
5.00000e-02 3.55000e-02 2.39579e-02
5.00000e-02 4.05000e-02 1.92015e-02
5.00000e-02 4.55000e-02 1.44061e-02
5.00000e-02 5.05000e-02 9.70753e-03
5.00000e-02 5.55000e-02 5.15754e-03
5.00000e-02 6.05000e-02 7.35180e-04
5.00000e-02 6.55000e-02 -3.62992e-03

6.00000e-02 2.55000e-02 3.37165e-02
6.00000e-02 3.05000e-02 2.88454e-02
6.00000e-02 3.55000e-02 2.42022e-02
6.00000e-02 4.05000e-02 1.93727e-02
6.00000e-02 4.55000e-02 1.40992e-02
6.00000e-02 5.05000e-02 8.98656e-03
6.00000e-02 5.55000e-02 4.23318e-03
6.00000e-02 6.05000e-02 -3.05065e-04
6.00000e-02 6.55000e-02 -4.77276e-03

7.00000e-02 2.55000e-02 3.39986e-02
7.00000e-02 3.05000e-02 2.93599e-02
7.00000e-02 3.55000e-02 2.48706e-02
7.00000e-02 4.05000e-02 2.00385e-02
7.00000e-02 4.55000e-02 1.42323e-02
7.00000e-02 5.05000e-02 8.67703e-03
7.00000e-02 5.55000e-02 3.84030e-03
7.00000e-02 6.05000e-02 -7.85187e-04
7.00000e-02 6.55000e-02 -5.36556e-03

8.00000e-02 2.55000e-02 3.44564e-02
8.00000e-02 3.05000e-02 2.97557e-02
8.00000e-02 3.55000e-02 2.52084e-02
8.00000e-02 4.05000e-02 2.05074e-02
8.00000e-02 4.55000e-02 1.48982e-02
8.00000e-02 5.05000e-02 9.21665e-03
8.00000e-02 5.55000e-02 4.11996e-03
8.00000e-02 6.05000e-02 -6.74306e-04
8.00000e-02 6.55000e-02 -5.42297e-03

9.00000e-02 2.55000e-02 3.49905e-02
9.00000e-02 3.05000e-02 3.03064e-02
9.00000e-02 3.55000e-02 2.55914e-02
9.00000e-02 4.05000e-02 2.05777e-02
9.00000e-02 4.55000e-02 1.55130e-02
9.00000e-02 5.05000e-02 9.78403e-03
9.00000e-02 5.55000e-02 4.87203e-03
9.00000e-02 6.05000e-02 -6.25436e-05
9.00000e-02 6.55000e-02 -5.00481e-03

1.00000e-01 2.55000e-02 3.53477e-02
1.00000e-01 3.05000e-02 3.05476e-02
1.00000e-01 3.55000e-02 2.56590e-02
1.00000e-01 4.05000e-02 2.04817e-02
1.00000e-01 4.55000e-02 1.56718e-02
1.00000e-01 5.05000e-02 1.04973e-02
1.00000e-01 5.55000e-02 5.87084e-03
1.00000e-01 6.05000e-02 7.48738e-04
1.00000e-01 6.55000e-02 -4.21645e-03

1.10000e-01 2.55000e-02 3.53059e-02
1.10000e-01 3.05000e-02 3.03065e-02
1.10000e-01 3.55000e-02 2.50196e-02
1.10000e-01 4.05000e-02 1.95287e-02
1.10000e-01 4.55000e-02 1.45791e-02
1.10000e-01 5.05000e-02 1.00397e-02
1.10000e-01 5.55000e-02 5.90385e-03
1.10000e-01 6.05000e-02 1.45302e-03
1.10000e-01 6.55000e-02 -3.15559e-03

1.20000e-01 2.55000e-02 3.47318e-02
1.20000e-01 3.05000e-02 2.96415e-02
1.20000e-01 3.55000e-02 2.44727e-02
1.20000e-01 4.05000e-02 1.93270e-02
1.20000e-01 4.55000e-02 1.44032e-02
1.20000e-01 5.05000e-02 9.65645e-03
1.20000e-01 5.55000e-02 5.74560e-03
1.20000e-01 6.05000e-02 1.93611e-03
1.20000e-01 6.55000e-02 -2.15820e-03

1.30000e-01 2.55000e-02 3.37794e-02
1.30000e-01 3.05000e-02 2.88457e-02
1.30000e-01 3.55000e-02 2.39985e-02
1.30000e-01 4.05000e-02 1.93354e-02
1.30000e-01 4.55000e-02 1.46790e-02
1.30000e-01 5.05000e-02 1.02233e-02
1.30000e-01 5.55000e-02 6.15526e-03
1.30000e-01 6.05000e-02 2.39059e-03
1.30000e-01 6.55000e-02 -1.40243e-03

1.40000e-01 2.55000e-02 3.26811e-02
1.40000e-01 3.05000e-02 2.79900e-02
1.40000e-01 3.55000e-02 2.34448e-02
1.40000e-01 4.05000e-02 1.91479e-02
1.40000e-01 4.55000e-02 1.49149e-02
1.40000e-01 5.05000e-02 1.07569e-02
1.40000e-01 5.55000e-02 6.72519e-03
1.40000e-01 6.05000e-02 2.90427e-03
1.40000e-01 6.55000e-02 -7.81659e-04



==> Figures/quant1.tex <==
\addplot[semithick, opacity=.5,mark options={opacity=0.8},mark=*,mark size=1.5pt,Red4] plot coordinates {
(2, 0.000493271)
(3, 0.002062508)
(4, 0.005353180)
(5, 0.018200521)
(6, 0.125870301)
(7, 0.229157736)
(8, 0.391857615)
(9, 0.424359764)
(10, 0.454545455)
};\addplot[semithick, opacity=.5,mark options={opacity=0.8},mark=*,mark size=1.5pt,DodgerBlue4] plot coordinates {
(2, 0.002029866)
(3, 0.014219724)
(4, 0.019372434)
(5, 0.030907580)
(6, 0.223376896)
(7, 0.452088614)
(8, 0.771451507)
(9, 0.845580338)
(10, 0.899908173)
};

==> Figures/quant2.tex <==
\addplot[semithick,opacity=.6, mark options={opacity=0.5},mark=*,mark size=1.5pt,black] plot coordinates {
(2, 0.243006508)
(3, 0.145045591)
(4, 0.276329761)
(5, 0.588869161)
(6, 0.563488448)
(7, 0.506886766)
(8, 0.507948473)
(9, 0.501856234)
(10, 0.505102041)
};

==> sc_tab.tex <==
\definecolor{blcol}{RGB}{150,150,250}
\definecolor{murcol}{RGB}{255,150,150}
\definecolor{healcol}{RGB}{150,235,150}
\definecolor{colzeta}{RGB}{250,250,200}
\definecolor{leftpcol}{RGB}{200,255,200}
\definecolor{rightpcol}{RGB}{200,200,255}
\definecolor{boxcol}{RGB}{210,200,200}
\definecolor{linecol}{RGB}{200,180,180}
\definecolor{colplus}{RGB}{235,220,220}
\definecolor{colinv}{RGB}{200,220,255}
\definecolor{cof}{RGB}{219,144,71}
\definecolor{pur}{RGB}{200,200,200}
\definecolor{greeo}{RGB}{91,173,69}
\definecolor{greet}{RGB}{52,111,72}
 \definecolor{nodecol}{RGB}{180,180,220}
 \definecolor{nodeedge}{RGB}{240,248,255}
  \definecolor{nodecolb}{RGB}{220,180,180}
  \definecolor{nodecolc}{RGB}{180,220,180}
  \definecolor{nodecolcD}{RGB}{100,160,100} 
  \definecolor{nodecolW}{RGB}{190,190,190}
  \definecolor{edgecol}{RGB}{160,160,180}   
 \definecolor{nodecolD}{RGB}{140,140,180}
  \definecolor{nodecolbD}{RGB}{180,140,140}% ##########################################################
\tikzset{oplus/.style={path picture={% 
      \draw[black]
       (path picture bounding box.south) -- (path picture bounding box.north) 
       (path picture bounding box.west) -- (path picture bounding box.east);
      }}} 
% ##########################################################
% ##########################################################
\tikzset{%
  highlight/.style={draw=Red4,rectangle,rounded corners=1pt, opacity=1,fill=gray!10,thick,inner sep=-1.25pt,on background layer,fill opacity=.3}
}
\tikzset{%
  highlightg/.style={draw=DodgerBlue4,rectangle,rounded corners=1pt, opacity=1,fill=gray!10,thick,inner sep=-1.25pt,on background layer,fill opacity=.3}
}
% 
\tikzset{%
fshadow/.style={      preaction={
         fill=black,opacity=.1,
         path fading=circle with fuzzy edge 20 percent,
         transform canvas={xshift=1mm,yshift=-1mm}
       }}
}
% ##########################################################
\def\ITEMSEP{.5pt}  \small \sffamily 
% ##########################################################
\newcommand{\tikzmark}[2]{\tikz[overlay,remember picture,baseline=(#1.base)] \node (#1) {#2};}
%
\newcommand{\Highlight}[3][submatrix]{%
    \tikz[overlay,remember picture]{
    \node[highlight,fit=(#2.north west) (#3.south east)] (#1) {};}
}
\newcommand{\HighlightG}[3][submatrix]{%
    \tikz[overlay,remember picture]{
    \node[highlightg,fit=(#2.north west) (#3.south east)] (#1) {};}
}\newcommand{\scpy}{\begin{tikzpicture}[very thick,scale=10] 
\node at (0.05,0.05) [fill=green!10,draw,rectangle, drop shadow] (n2){$\mathcal{C}$};
 \node at (-0.065,0.1) {$s$};
 \node at (0.165,0.055) {$s'$};
\draw (-0.05,0.1) -- (0.15,0.1);
\draw (-0.02,0.05) -- (0.03,0.05);
\draw (-0.02,0.1) -- (-0.02,0.05);
\draw  (0.07,0.05) -- (0.15,0.05);
\end{tikzpicture}
}
\newcommand{\sinv}{\begin{tikzpicture}[very thick,scale=10] 
\node at (0.05,0.05) [fill=colinv,draw,diamond, drop shadow,inner sep=0.5pt,minimum size=10pt] (n2){$\mathds{-1}$};
 \node at (-0.065,0.05) {$s$};
 \node at (0.165,0.055) {$s'$};
\draw (-0.05,0.05) -- (0.015,0.05);
\draw  (0.085,0.05) -- (0.15,0.05);
\end{tikzpicture}
}
\newcommand{\ssum}{\begin{tikzpicture}[very thick,scale=10] 
\node at (0.05,0.05) [fill=colplus,draw,oplus, circle,drop shadow,inner sep=0.5pt,minimum size=15pt, very thick] (n2){};
 \node at (-0.065,0.1) {$s_1$};
 \node at (-0.065,0) {$s_2$};
 \node at (0.165,0.055) {$s'$};
\draw (-0.05,0.1) -- (0.05,0.1);
\draw (0.05,0.1) -- (0.05,0.075);
\draw (-0.05,-0.0) -- (0.05,-0.0);
\draw (0.05,0) -- (0.05,0.025);
\draw  (0.08,0.05) -- (0.15,0.05);
\end{tikzpicture}
}
% ##########################################################
% ##########################################################
\newcommand{\mest}{\begin{tikzpicture}[very thick,scale=10] 
\node at (0.05,0.0) [fill=colzeta,draw,rectangle, drop shadow] (n2){$\hat{\zeta}$};
\draw (-0.05,0.0) -- (0.025,0.0);
 \node at (-0.065,0.0) {$s$};
 \node at (0.225,0.0) {\mnp{1in}{\fontsize{7}{7}\selectfont \sffamily \mnp{.35in}{Real Number \\ output\\
in $[0,1]$}}};
\end{tikzpicture}
}
%  ##################################
\newcommand{\VSP}{\rule{0pt}{2ex}}
\begin{tabular}{m{2.85in} m{3.75in}}\hline
\VSP\bf Stream Operation & \VSP \bf Algorithmic Procedure (Pseudocode) \\\hline
% --------------------------

\mnp{2.75in}{\bf $\blacksquare$ Independent
Stream Copy$^\dag$\\}

\mnp{1in}{
\scpy
}\hfill
\mnp{1.5in}{
\raggedright\bf \sffamily \small Generate an independent sample path from the same hidden stochastic source. }
 &

% 
\begin{list}{\labelitemi}{\leftmargin=0.75em} \setlength{\itemsep}{\ITEMSEP}% 
\item[1] Generate stream $\omega_0$ from FWN
 \item[2] Read current symbol $\sigma_1$ from $s_1$, and $\sigma_2$ from
$\omega_0$
\item[3] If $\sigma_1= \sigma_2$, then write $\sigma_1$  to output $s'$
\item[4] Move read positions one step to right, and go to step 1
\end{list}
% 
{\itshape This operation is required internally in  stream inversion.}
% 
 \\\hline
%--------------------------

\mnp{2.75in}{
\bf $\blacksquare$ Stream 
%x
Inversion$^\dag$\\}

\mnp{1in}{%\vspace{-8pt}
\sinv}
\hfill
\mnp{1.5in}{
\raggedright \bf \sffamily   \small
Generate sample path from  inverse model of  hidden  source. }
 &
 
 
\begin{list}{\labelitemi}{\leftmargin=0.75em} \setlength{\itemsep}{\ITEMSEP}% 
\item[1] Generate $\vert \Sigma \vert-1$ independent copies of $s_1$: $s_1,\cdots, s_{\vert\Sigma\vert -1}$
 \item[2] Read current symbols $\sigma_i$ from $s_i$ ($i=1,\cdots,\vert\Sigma\vert-1$)
\item[3] If $\sigma_i\neq  \sigma_j$ for all distinct  $i,j$, then write 
$\Sigma \setminus \bigcup_{i=1}^{\vert \Sigma \vert-1}\sigma_i$
to output $s'$
\item[4] Move read positions one step to right, and go to step 1
\vspace{-5pt}
\end{list}
% 
 \\\hline
% 
\mnp{2.75in}{
\vspace{5pt}

\bf$\blacksquare$  Stream Summation$^\dag$\\}


\mnp{1in}{\ssum}
\hfill
\mnp{1.5in}{\raggedright\bf \sffamily  \small
Generating sample path from  sum of hidden sources.}
 &
 
 
% 
\begin{list}{\labelitemi}{\leftmargin=0.75em}  \setlength{\itemsep}{\ITEMSEP}% 
 \item[1] Read current symbols $\sigma_i$ from $s_i$ ($i=1,2$)
\item[2] If $\sigma_1 =  \sigma_2$, then write 
to output $s'$
\item[3] Move read positions one step to right, and go to step 1
\end{list}
\\\hline
% 
\mnp{2.75in}{
\bf$\blacksquare$  Deviation
from FWN$^\ddag$\\}

\mnp{1.2in}{\mest}
\hfill
\mnp{1.5in}{\raggedright\bf \sffamily  \small
Estimating the deviation of a symbolic stream from FWN. 
}
\vspace{2pt}

(Symbolic derivatives (Definition~\ref{defsymderivative}) in  Section~\ref{sec-pfsa} formalizes $\phi^s(\cdot)$. If $s$ is generated by a FWN process, then $\phi^s(x) \rightarrow \mathcal{U}_\Sigma$ for any $x \in \Sigma^\star$, and hence $\hat{\zeta}(s,\ell) \rightarrow 0$.)
 &\cgatherd[-3pt][-5pt]{
\hat{\zeta}(s,\ell)=
\frac{\vert \Sigma \vert -1}{\vert \Sigma\vert}\sum_{x: \vert x \vert \leqq \ell} \frac{\vert \vert \phi^s(x) - \mathcal{U}_\Sigma \vert \vert_\infty}{\vert \Sigma \vert^{2\vert x \vert}} 
 ,\ \textrm{where}}
\begin{itemize} \setlength{\itemsep}{\ITEMSEP}% 
 \item $\vert \Sigma \vert$ is the alphabet size, $\vert x\vert$ is the length of the string $x$
\item $\ell$ is the maximum length of strings upto which the sum is evaluated. For a given  $\epsilon^\star$, we choose $\ell = \ln(1/\epsilon^\star)/\ln (\vert \Sigma \vert)$ (See Proposition~\ref{prophiddenmodeltwo})
\item $\mathcal{U}_\Sigma$ is the uniform probability vector of length $\vert\Sigma\vert$
\item For $\sigma_i \in \Sigma$, $\phi^s(x) \big \vert_i = \frac{\txt{\# of occurrences of  $x\sigma_i$ in string $s$}}{\txt{\# of occurrences of  $x$ in string $s$}}$ 
\end{itemize}
% 
 \\\hline
% 
\end{tabular}

